Mapping the Skies of Ultracool Worlds: Detecting Storms and Spots with Extremely Large Telescopes

Extremely large telescopes (ELTs) present an unparalleled opportunity to study the magnetism, atmospheric dynamics, and chemistry of very low mass stars (VLMs), brown dwarfs, and exoplanets. Instruments such as the Giant Magellan Telescope - Consortium Large Earth Finder (GMT/GCLEF), the Thirty Meter Telescope's Multi-Objective Diffraction-limited High-Resolution Infrared Spectrograph (TMT/MODHIS), and the European Southern Observatory's Mid-Infrared ELT Imager and Spectrograph (ELT/METIS) provide the spectral resolution and signal-to-noise (S/N) necessary to Doppler image ultracool targets' surfaces based on temporal spectral variations due to surface inhomogeneities. Using our publicly-available code, $Imber$, developed and validated in Plummer & Wang (2022), we evaluate these instruments' abilities to discern magnetic star spots and cloud systems on a VLM star (TRAPPIST-1); two L/T transition ultracool dwarfs (VHS J1256$-$1257 b and SIMP J0136+0933); and three exoplanets (Beta Pic b and HR 8799 d and e). We find that TMT/MODHIS and ELT/METIS are suitable for Doppler imaging the ultracool dwarfs and Beta Pic b over a single rotation. Uncertainties for longitude and radius are typically $\lesssim 10^{\circ}$, and latitude uncertainties range from $\sim 10^{\circ} \ \rm{to} \ 30^{\circ}$. TRAPPIST-1's edge-on inclination and low $\upsilon \sin i$ provide a challenge for all three instruments while GMT/GCLEF and the HR 8799 planets may require observations over multiple rotations. We compare the spectroscopic technique, photometry-only inference, and the combination of the two. We find combining spectroscopic and photometric observations can lead to improved Bayesian inference of surface inhomogeneities and offers insight into whether ultracool atmospheres are dominated by spotted or banded features.

==> Mapping the Skies of Ultracool Worlds (Arxiv)/references.tex <==
@ARTICLE{Schweitzer1996,
       author = {{Schweitzer}, Andreas and {Hauschildt}, Peter H. and {Allard}, France and {Basri}, G.},
        title = "{Analysis of Keck high-resolution spectra of VB 10}",
      journal = {\mnras},
     keywords = {ATOMIC PROCESSES, LINE: PROFILES, STARS: ATMOSPHERES, STARS: FUNDAMENTAL PARAMETERS, STARS: INDIVIDUAL: VB10, STARS: LOW-MASS, BROWN DWARFS, Astrophysics},
         year = 1996,
        month = dec,
       volume = {283},
       number = {3},
        pages = {821-829},
          doi = {10.1093/mnras/283.3.821},
archivePrefix = {arXiv},
       eprint = {astro-ph/9606150},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996MNRAS.283..821S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Miles-Paez2021,
       author = {{Miles-P{\'a}ez}, P.~A.},
        title = "{Detection of photometric variability in the very low-mass binary VHS J1256-1257AB using TESS and Spitzer}",
      journal = {\aap},
     keywords = {brown dwarfs, stars: rotation, stars: late-type, stars: low-mass, stars: atmospheres, stars: individual: VHS J1256-1257, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jul,
       volume = {651},
          eid = {L7},
        pages = {L7},
          doi = {10.1051/0004-6361/202141203},
archivePrefix = {arXiv},
       eprint = {2107.00220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...651L...7M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Miles-Paez2023,
       author = {{Miles-P{\'a}ez}, Paulo A. and {Metchev}, Stanimir A. and {George}, Benjamin},
        title = "{The photometric periods of rapidly rotating field ultra-cool dwarfs}",
      journal = {\mnras},
     keywords = {stars: activity, stars: low-mass, stars: rotation, stars: late-type, (stars:) brown dwarfs, surveys, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Physics - Space Physics},
         year = 2023,
        month = may,
       volume = {521},
       number = {1},
        pages = {952-968},
          doi = {10.1093/mnras/stad273},
archivePrefix = {arXiv},
       eprint = {2301.09932},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.521..952M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INCOLLECTION{Kochukhov2016,
       author = {{Kochukhov}, Oleg},
        title = "{Doppler and Zeeman Doppler Imaging of Stars}",
     keywords = {Physics},
    booktitle = {Lecture Notes in Physics, Berlin Springer Verlag},
         year = 2016,
       editor = {{Rozelot}, Jean-Pierre and {Neiner}, Coralie},
       volume = {914},
        pages = {177},
          doi = {10.1007/978-3-319-24151-7_9},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016LNP...914..177K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hebrard2016,
       author = {{H{\'e}brard}, {\'E}. M. and {Donati}, J. -F. and {Delfosse}, X. and {Morin}, J. and {Moutou}, C. and {Boisse}, I.},
        title = "{Modelling the RV jitter of early-M dwarfs using tomographic imaging}",
      journal = {\mnras},
     keywords = {line: profiles, techniques: polarimetric, techniques: radial velocities, magnetic fields, starspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = sep,
       volume = {461},
       number = {2},
        pages = {1465-1497},
          doi = {10.1093/mnras/stw1346},
archivePrefix = {arXiv},
       eprint = {1606.01775},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.461.1465H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Petit2008,
       author = {{Petit}, P. and {Dintrans}, B. and {Solanki}, S.~K. and {Donati}, J. -F. and {Auri{\`e}re}, M. and {Ligni{\`e}res}, F. and {Morin}, J. and {Paletou}, F. and {Ramirez Velez}, J. and {Catala}, C. and {Fares}, R.},
        title = "{Toroidal versus poloidal magnetic fields in Sun-like stars: a rotation threshold}",
      journal = {\mnras},
     keywords = {stars: individual: HD 73350, stars: individual: HD 76151, stars: individual: HD 146233, stars: individual: HD 190771, stars: magnetic fields, stars: rotation, Astrophysics},
         year = 2008,
        month = jul,
       volume = {388},
       number = {1},
        pages = {80-88},
          doi = {10.1111/j.1365-2966.2008.13411.x},
archivePrefix = {arXiv},
       eprint = {0804.1290},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.388...80P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hauschildt1996,
       author = {{Hauschildt}, Peter H. and {Baron}, E. and {Starrfield}, Sumner and {Allard}, France},
        title = "{The Effects of Fe II Non-LTE on Nova Atmospheres and Spectra}",
      journal = {\apj},
     keywords = {STARS: NOVAE, CATACLYSMIC VARIABLES, RADIATIVE TRANSFER, STARS: ATMOSPHERES, Astrophysics},
         year = 1996,
        month = may,
       volume = {462},
        pages = {386},
          doi = {10.1086/177160},
archivePrefix = {arXiv},
       eprint = {astro-ph/9601149},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...462..386H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baron1996,
       author = {{Baron}, E. and {Hauschildt}, P.~H. and {Branch}, D. and {Kirshner}, R.~P. and {Filippenko}, A.~V.},
        title = "{Preliminary spectral analysis of SN 1994I}",
      journal = {\mnras},
     keywords = {STARS: EVOLUTION, SUPERNOVAE: GENERAL, SUPERNOVAE: INDIVIDUAL: SN 1994I, Astrophysics},
         year = 1996,
        month = apr,
       volume = {279},
       number = {3},
        pages = {799-803},
          doi = {10.1093/mnras/279.3.799},
archivePrefix = {arXiv},
       eprint = {astro-ph/9510070},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996MNRAS.279..799B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Allard&Hauschildt1995,
       author = {{Allard}, France and {Hauschildt}, Peter H.},
        title = "{Model Atmospheres for M (Sub)Dwarf Stars. I. The Base Model Grid}",
      journal = {\apj},
     keywords = {Abundance, Infrared Signatures, Molecular Spectra, Stellar Atmospheres, Stellar Luminosity, Stellar Spectra, Subdwarf Stars, Hydrodynamics, Line Spectra, Metallicity, Opacity, Optical Thickness, Stellar Models, Astrophysics, ATOMIC DATA, MOLECULAR DATA, STARS: ATMOSPHERES, STARS: LATE-TYPE, STARS: SUBDWARFS, Astrophysics},
         year = 1995,
        month = may,
       volume = {445},
        pages = {433},
          doi = {10.1086/175708},
archivePrefix = {arXiv},
       eprint = {astro-ph/9601150},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...445..433A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hauschildt&Baron1995,
       author = {{Hauschildt}, P.~H. and {Baron}, E.},
        title = "{Non-LTE treatment of Fe II in astrophysical plasmas.}",
      journal = {\jqsrt},
     keywords = {Radiative Transfer: Plasma, Radiative Transfer: Iron Lines, Radiative Transfer: Novae, Radiative Transfer: Supernovae, Astrophysics},
         year = 1995,
        month = dec,
       volume = {54},
       number = {6},
        pages = {987-999},
          doi = {10.1016/0022-4073(95)00118-5},
archivePrefix = {arXiv},
       eprint = {astro-ph/9601148},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995JQSRT..54..987H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt1995,
       author = {{Hauschildt}, Peter H. and {Starrfield}, Sumner and {Shore}, Steven N. and {Allard}, France and {Baron}, E.},
        title = "{The Physics of Early Nova Spectra}",
      journal = {\apj},
     keywords = {STARS: NOVAE, CATACLYSMIC VARIABLES, RADIATIVE TRANSFER, STARS: ATMOSPHERES},
         year = 1995,
        month = jul,
       volume = {447},
        pages = {829},
          doi = {10.1086/175921},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...447..829H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Hauschildt1993,
       author = {{Hauschildt}, P.~H.},
        title = "{Multi-level non-LTE radiative transfer in expanding shells.}",
      journal = {\jqsrt},
         year = 1993,
        month = sep,
       volume = {50},
       number = {3},
        pages = {301-318},
          doi = {10.1016/0022-4073(93)90080-2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993JQSRT..50..301H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hauschildt1992,
       author = {{Hauschildt}, P.~H.},
        title = "{A fast operator perturbation method for the solution of the special relativistic equation of radiative transfer in spherical symmetry.}",
      journal = {\jqsrt},
     keywords = {Iterative Solution, Novae, Perturbation Theory, Radiative Transfer, Relativistic Theory, Run Time (Computers), Convergence, Method Of Characteristics, Radiation Distribution, Supernovae, Wolf-Rayet Stars, Astrophysics},
         year = 1992,
        month = jun,
       volume = {47},
       number = {6},
        pages = {433-453},
          doi = {10.1016/0022-4073(92)90105-D},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992JQSRT..47..433H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Hauschildt1999,
       author = {{Hauschildt}, Peter H. and {Allard}, France and {Baron}, E.},
        title = "{The NextGen Model Atmosphere Grid for 3000<=T$_{eff}$<=10,000 K}",
      journal = {\apj},
     keywords = {RADIATIVE TRANSFER, STARS: ATMOSPHERES, STARS: LATE-TYPE, Radiative Transfer, Stars: Atmospheres, Stars: Late-Type, Astrophysics},
         year = 1999,
        month = feb,
       volume = {512},
       number = {1},
        pages = {377-385},
          doi = {10.1086/306745},
archivePrefix = {arXiv},
       eprint = {astro-ph/9807286},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...512..377H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt1997,
       author = {{Hauschildt}, Peter H. and {Baron}, E. and {Allard}, France},
        title = "{Parallel Implementation of the PHOENIX Generalized Stellar Atmosphere Program}",
      journal = {\apj},
     keywords = {Methods: Numerical, Radiative Transfer, Stars: Atmospheres, Astrophysics},
         year = 1997,
        month = jul,
       volume = {483},
       number = {1},
        pages = {390-398},
          doi = {10.1086/304233},
archivePrefix = {arXiv},
       eprint = {astro-ph/9607087},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...483..390H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Froning2006,
       author = {{Froning}, Cynthia and {Osterman}, Steven and {Beasley}, Matthew and {Green}, James and {Beland}, Stephane},
        title = "{Conceptual design for the High Resolution Optical Spectrograph on the Thirty-Meter Telescope: a new concept for a ground-based high-resolution optical spectrograph}",
    booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
         year = 2006,
       editor = {{McLean}, Ian S. and {Iye}, Masanori},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {6269},
        month = jun,
          eid = {62691V},
        pages = {62691V},
          doi = {10.1117/12.669358},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006SPIE.6269E..1VF},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Fitzgerald2019,
       author = {{Fitzgerald}, Michael and {Bailey}, Vanessa and {Baranec}, Christoph and {Batalha}, Natasha and {Benneke}, Bj{\"o}rn and {Beichman}, Charles and {Brandt}, Timothy and {Chilcote}, Jeffrey and {Chun}, Mark and {Crossfield}, Ian and {Currie}, Thayne and {Davis}, Kristina and {Dekany}, Richard and {Delorme}, Jacques-Robert and {Dong}, Ruobing and {Doyon}, Rene and {Dressing}, Courtney and {Echeverri}, Daniel and {Fortney}, Jonathan and {Frazin}, Richard A. and {Guyon}, Olivier and {Hashimoto}, Jun and {Hillenbrand}, Lynne and {Hinz}, Philip and {Howard}, Andrew and {Jensen-Clem}, Rebecca and {Jovanovic}, Nemanja and {Kawahara}, Hajime and {Knutson}, Heather and {Konopacky}, Quinn and {Kotani}, Takayuki and {Lafreni{\`e}re}, David and {Liu}, Michael and {Lozi}, Julien and {Lu}, Jessica R. and {Males}, Jared and {Marley}, Mark and {Marois}, Christian and {Mawet}, Dimitri and {Mazin}, Benjamin and {Millar-Blanchaer}, Maxwell and {Mondal}, Soumen and {Murakami}, Naoshi and {Murray-Clay}, Ruth and {Narita}, Norio and {Pezzato}, Jacklyn and {Pyo}, Tae-Soo and {Roberts}, Lewis and {Ruane}, Garreth and {Sallum}, Steph and {Serabyn}, Gene and {Shields}, Aomawa and {Simard}, Luc and {Skemer}, Andy and {Stelter}, R. Deno and {Tamura}, Motohide and {Troy}, Mitchell and {Vasisht}, Gautam and {Wallace}, J. Kent and {Wang}, Jason and {Wang}, Ji and {Wright}, Shelley A.},
        title = "{The Planetary Systems Imager for TMT}",
    booktitle = {Bulletin of the American Astronomical Society},
         year = 2019,
       volume = {51},
        month = sep,
          eid = {251},
        pages = {251},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019BAAS...51g.251F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Packham2014,
       author = {{Packham}, Chris and {Honda}, M. and {Okamoto}, Y.~K. and {Richter}, M. and {Chun}, M. and {Kataza}, H. and {Onaka}, T. and {Sakon}, I. and {MICHI Team}},
        title = "{MICHI: A MIR Instrument for the TMT}",
    booktitle = {Thirty Meter Telescope Science Forum},
         year = 2014,
       editor = {{Dickinson}, Mark and {Inami}, Hanae},
        month = jul,
          eid = {20},
        pages = {20},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014tmt..confE..20P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Jaffe2016,
       author = {{Jaffe}, Daniel T. and {Barnes}, Stuart and {Brooks}, Cynthia and {Lee}, Hanshin and {Mace}, Gregory and {Pak}, Soojong and {Park}, Byeong-Gon and {Park}, Chan},
        title = "{GMTNIRS: progress toward the Giant Magellan Telescope near-infrared spectrograph}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy VI},
         year = 2016,
       editor = {{Evans}, Christopher J. and {Simard}, Luc and {Takami}, Hideki},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9908},
        month = aug,
          eid = {990821},
        pages = {990821},
          doi = {10.1117/12.2232994},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9908E..21J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Marconi2022,
       author = {{Marconi}, A. and {Abreu}, M. and {Adibekyan}, V. and {Alberti}, V. and {Albrecht}, S. and {Alcaniz}, J. and {Aliverti}, M. and {Allende Prieto}, C. and {Alvarado G{\'o}mez}, J.~D. and {Amado}, P.~J. and {Amate}, M. and {Andersen}, M.~I. and {Artigau}, E. and {Baker}, C. and {Baldini}, V. and {Balestra}, A. and {Barnes}, S.~A. and {Baron}, F. and {Barros}, S.~C.~C. and {Bauer}, S.~M. and {Beaulieu}, M. and {Bellido-Tirado}, O. and {Benneke}, B. and {Bensby}, T. and {Bergin}, E.~A. and {Biazzo}, K. and {Bik}, A. and {Birkby}, J.~L. and {Blind}, N. and {Boisse}, I. and {Bolmont}, E. and {Bonaglia}, M. and {Bonfils}, X. and {Borsa}, F. and {Brandeker}, A. and {Brandner}, W. and {Broeg}, C.~H. and {Brogi}, M. and {Brousseau}, D. and {Brucalassi}, A. and {Brynnel}, J. and {Buchhave}, L.~A. and {Buscher}, D.~F. and {Cabral}, A. and {Calderone}, G. and {Calvo-Ortega}, R. and {Canto Martins}, B.~L. and {Cantalloube}, F. and {Carbonaro}, L. and {Chauvin}, G. and {Chazelas}, B. and {Cheffot}, A. -L. and {Cheng}, Y.~S. and {Chiavassa}, A. and {Christensen}, L. and {Cirami}, R. and {Cook}, N.~J. and {Cooke}, R.~J. and {Coretti}, I. and {Covino}, S. and {Cowan}, N. and {Cresci}, G. and {Cristiani}, S. and {Cunha Parro}, V. and {Cupani}, G. and {D'Odorico}, V. and {de Castro Le{\~a}o}, I. and {De Cia}, A. and {De Medeiros}, J.~R. and {Debras}, F. and {Debus}, M. and {Demangeon}, O. and {Dessauges-Zavadsky}, M. and {Di Marcantonio}, P. and {Dionies}, F. and {Doyon}, R. and {Dunn}, J. and {Ehrenreich}, D. and {Faria}, J.~P. and {Feruglio}, C. and {Fisher}, M. and {Fontana}, A. and {Fumagalli}, M. and {Fusco}, T. and {Fynbo}, J. and {Gabella}, O. and {Gaessler}, W. and {Gallo}, E. and {Gao}, X. and {Genolet}, L. and {Genoni}, M. and {Giacobbe}, P. and {Giro}, E. and {Gon{\c{c}}alves}, R.~S. and {Gonzalez}, O. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Gracia T{\'e}mich}, F. and {Haehnelt}, M.~G. and {Haniff}, C. and {Hatzes}, A. and {Helled}, R. and {Hoeijmakers}, H.~J. and {Huke}, P. and {J{\"a}rvinen}, S. and {J{\"a}rvinen}, A. and {Kaminski}, A. and {Korn}, A. and {Kouach}, D. and {Kowzan}, G. and {Kreidberg}, L. and {Landoni}, M. and {Lanotte}, A. and {Lavail}, A. and {Li}, J. and {Liske}, J. and {Lovis}, C. and {Lucatello}, S. and {Lunney}, D. and {MacIntosh}, M. and {Madhusudhan}, N. and {Magrini}, L. and {Maiolino}, R. and {Malo}, L. and {Man}, A. and {Marquart}, T. and {Marques}, E.~L. and {Martins}, A.~M. and {Martins}, C.~J.~A.~P. and {Maslowski}, P. and {Mason}, C. and {Mason}, E. and {McCracken}, R.~A. and {Mergo}, P. and {Micela}, G. and {Mitchell}, T. and {Molli{\`e}re}, P. and {Monteiro}, M. and {Montgomery}, D. and {Mordasini}, C. and {Morin}, J. and {Mucciarelli}, A. and {Murphy}, M.~T. and {N'Diaye}, M. and {Neichel}, B. and {Niedzielski}, A.~T. and {Niemczura}, E. and {Nortmann}, L. and {Noterdaeme}, P. and {Nunes}, N. and {Oggioni}, L. and {Oliva}, E. and {{\"O}nel}, H. and {Origlia}, L. and {{\"O}stlin}, G. and {Palle}, E. and {Papaderos}, P. and {Pariani}, G. and {Pe{\~n}ate Castro}, J. and {Pepe}, F. and {Perreault Levasseur}, L. and {Petit}, P. and {Pino}, L. and {Piqueras}, J. and {Pollo}, A. and {Poppenhaeger}, K. and {Quirrenbach}, A. and {Rauscher}, E. and {Rebolo}, R. and {Redaelli}, E.~M.~A. and {Reffert}, S. and {Reid}, D.~T. and {Reiners}, A. and {Richter}, P. and {Riva}, M. and {Rivoire}, S. and {Rodr{\'\i}guez-L{\'o}pez}, C. and {Roederer}, I.~U. and {Romano}, D. and {Rousseau}, S. and {Rowe}, J. and {Salvadori}, S. and {Santos}, N. and {Santos Diaz}, P. and {Sanz-Forcada}, J. and {Sarajlic}, M. and {Sauvage}, J. -F. and {Sch{\"a}fer}, S. and {Schiavon}, R.~P. and {Schmidt}, T.~M. and {Selmi}, C. and {Sivanandam}, S. and {Sordet}, M. and {Sordo}, R. and {Sortino}, F. and {Sosnowska}, D. and {Sousa}, S.~G. and {Stempels}, E. and {Strassmeier}, K.~G. and {Su{\'a}rez Mascare{\~n}o}, A. and {Sulich}, A. and {Sun}, X. and {Tanvir}, N.~R. and {Tenegi-Sangin{\'e}s}, F. and {Thibault}, S. and {Thompson}, S.~J. and {Tozzi}, A. and {Turbet}, M. and {Vall{\'e}e}, P. and {Varas}, R. and {Venn}, K. and {V{\'e}ran}, J. -P. and {Verma}, A. and {Viel}, M. and {Wade}, G. and {Waring}, C. and {Weber}, M. and {Weder}, J. and {Wehbe}, B. and {Weingrill}, J. and {Woche}, M. and {Xompero}, M. and {Zackrisson}, E. and {Zanutta}, A. and {Zapatero Osorio}, M.~R. and {Zechmeister}, M. and {Zimara}, J.},
        title = "{ANDES, the high resolution spectrograph for the ELT: science case, baseline design and path to construction}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy IX},
         year = 2022,
       editor = {{Evans}, Christopher J. and {Bryant}, Julia J. and {Motohara}, Kentaro},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {12184},
        month = aug,
          eid = {1218424},
        pages = {1218424},
          doi = {10.1117/12.2628689},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022SPIE12184E..24M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{Decadal2021,
       author = {{National Academies of Sciences} and Medicine},
        title = "{Pathways to Discovery in Astronomy and Astrophysics for the 2020s}",
         year = 2021,
          doi = {10.17226/26141},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021pdaa.book.....N}
}

@ARTICLE{Martin2023,
       author = {{Martin}, David V. and {Sethi}, Ritika and {Armitage}, Tayt and {Gilbert}, Gregory J. and {Rodr{\'\i}guez Mart{\'\i}nez}, Romy and {Gilbert}, Emily A.},
        title = "{The Benchmark M Dwarf Eclipsing Binary CM Draconis With TESS: Spots, Flares and Ultra-Precise Parameters}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2023,
        month = jan,
          eid = {arXiv:2301.10858},
        pages = {arXiv:2301.10858},
archivePrefix = {arXiv},
       eprint = {2301.10858},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv230110858M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{McCarthy2016,
       author = {{McCarthy}, Patrick J. and {Fanson}, James and {Bernstein}, Rebecca and {Ashby}, David and {Bigelow}, Bruce and {Boyadjian}, Nune and {Bouchez}, Antonin and {Chauvin}, Eric and {Donoso}, Eduardo and {Filgueira}, Jose and {Goodrich}, Robert and {Groark}, Frank and {Jacoby}, George and {Pearce}, Eric},
        title = "{Overview and status of the Giant Magellan Telescope Project}",
    booktitle = {Ground-based and Airborne Telescopes VI},
         year = 2016,
       editor = {{Hall}, Helen J. and {Gilmozzi}, Roberto and {Marshall}, Heather K.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9906},
        month = aug,
          eid = {990612},
        pages = {990612},
          doi = {10.1117/12.2234505},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9906E..12M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{JJWang2018,
       author = {{Wang}, Jason J. and {Graham}, James R. and {Dawson}, Rebekah and {Fabrycky}, Daniel and {De Rosa}, Robert J. and {Pueyo}, Laurent and {Konopacky}, Quinn and {Macintosh}, Bruce and {Marois}, Christian and {Chiang}, Eugene and {Ammons}, S. Mark and {Arriaga}, Pauline and {Bailey}, Vanessa P. and {Barman}, Travis and {Bulger}, Joanna and {Chilcote}, Jeffrey and {Cotten}, Tara and {Doyon}, Rene and {Duch{\^e}ne}, Gaspard and {Esposito}, Thomas M. and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Gerard}, Benjamin L. and {Goodsell}, Stephen J. and {Greenbaum}, Alexandra Z. and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Kalas}, Paul and {Larkin}, James E. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marley}, Mark S. and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Nielsen}, Eric L. and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall and {Poyneer}, Lisa and {Rajan}, Abhijith and {Rameau}, Julien and {Rantakyr{\"o}}, Fredrik T. and {Ruffio}, Jean-Baptiste and {Savransky}, Dmitry and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Ward-Duong}, Kimberly and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{Dynamical Constraints on the HR 8799 Planets with GPI}",
      journal = {\aj},
     keywords = {astrometry, planet{\textendash}disk interactions, planets and satellites: dynamical evolution and stability, planets and satellites: gaseous planets, stars: individual: HR 8799, techniques: high angular resolution, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = nov,
       volume = {156},
       number = {5},
          eid = {192},
        pages = {192},
          doi = {10.3847/1538-3881/aae15010.48550/arXiv.1809.04107},
archivePrefix = {arXiv},
       eprint = {1809.04107},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..192W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Vos2017,
       author = {{Vos}, Johanna M. and {Allers}, Katelyn N. and {Biller}, Beth A.},
        title = "{The Viewing Geometry of Brown Dwarfs Influences Their Observed Colors and Variability Amplitudes}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: rotation, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jun,
       volume = {842},
       number = {2},
          eid = {78},
        pages = {78},
          doi = {10.3847/1538-4357/aa73cf},
archivePrefix = {arXiv},
       eprint = {1705.06045},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...842...78V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bryan2020a,
       author = {{Bryan}, Marta L. and {Chiang}, Eugene and {Bowler}, Brendan P. and {Morley}, Caroline V. and {Millholland}, Sarah and {Blunt}, Sarah and {Ashok}, Katelyn B. and {Nielsen}, Eric and {Ngo}, Henry and {Mawet}, Dimitri and {Knutson}, Heather A.},
        title = "{Obliquity Constraints on an Extrasolar Planetary-mass Companion}",
      journal = {\aj},
     keywords = {Exoplanet systems, High resolution spectroscopy, Direct imaging, Photometry, 484, 2096, 387, 1234, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = apr,
       volume = {159},
       number = {4},
          eid = {181},
        pages = {181},
          doi = {10.3847/1538-3881/ab76c610.48550/arXiv.2002.11131},
archivePrefix = {arXiv},
       eprint = {2002.11131},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159..181B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Zhou2016,
       author = {{Zhou}, Yifan and {Apai}, D{\'a}niel and {Schneider}, Glenn H. and {Marley}, Mark S. and {Showman}, Adam P.},
        title = "{Discovery of Rotational Modulations in the Planetary-mass Companion 2M1207b: Intermediate Rotation Period and Heterogeneous Clouds in a Low Gravity Atmosphere}",
      journal = {\apj},
     keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: individual: 2M1207b, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = feb,
       volume = {818},
       number = {2},
          eid = {176},
        pages = {176},
          doi = {10.3847/0004-637X/818/2/176},
archivePrefix = {arXiv},
       eprint = {1512.02706},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...818..176Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhou2019,
       author = {{Zhou}, Yifan and {Apai}, D{\'a}niel and {Lew}, Ben W.~P. and {Schneider}, Glenn and {Manjavacas}, Elena and {Bedin}, Luigi R. and {Cowan}, Nicolas B. and {Marley}, Mark S. and {Radigan}, Jacqueline and {Karalidi}, Theodora and {Lowrance}, Patrick J. and {Miles-P{\'a}ez}, Paulo A. and {Metchev}, Stanimir and {Burgasser}, Adam J.},
        title = "{Cloud Atlas: High-contrast Time-resolved Observations of Planetary-mass Companions}",
      journal = {\aj},
     keywords = {methods: observational, planetary systems, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {157},
       number = {3},
          eid = {128},
        pages = {128},
          doi = {10.3847/1538-3881/ab037f},
archivePrefix = {arXiv},
       eprint = {1902.00085},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..128Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Biller2015,
       author = {{Biller}, Beth A. and {Vos}, Johanna and {Bonavita}, Mariangela and {Buenzli}, Esther and {Baxter}, Claire and {Crossfield}, Ian J.~M. and {Allers}, Katelyn and {Liu}, Michael C. and {Bonnefoy}, Micka{\"e}l and {Deacon}, Niall and {Brandner}, Wolfgang and {Schlieder}, Joshua E. and {Dupuy}, Trent and {Kopytova}, Taisiya and {Manjavacas}, Elena and {Allard}, France and {Homeier}, Derek and {Henning}, Thomas},
        title = "{Variability in a Young, L/T Transition Planetary-mass Object}",
      journal = {\apjl},
     keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = nov,
       volume = {813},
       number = {2},
          eid = {L23},
        pages = {L23},
          doi = {10.1088/2041-8205/813/2/L23},
archivePrefix = {arXiv},
       eprint = {1510.07625},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...813L..23B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lew2016,
       author = {{Lew}, Ben W.~P. and {Apai}, Daniel and {Zhou}, Yifan and {Schneider}, Glenn and {Burgasser}, Adam J. and {Karalidi}, Theodora and {Yang}, Hao and {Marley}, Mark S. and {Cowan}, Nicolas B. and {Bedin}, Luigi R. and {Metchev}, Stanimir A. and {Radigan}, Jacqueline and {Lowrance}, Patrick J.},
        title = "{Cloud Atlas: Discovery of Patchy Clouds and High-amplitude Rotational Modulations in a Young, Extremely Red L-type Brown Dwarf}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: atmospheres, stars: individual: WISEP J004701.06+680352.1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {829},
       number = {2},
          eid = {L32},
        pages = {L32},
          doi = {10.3847/2041-8205/829/2/L32},
archivePrefix = {arXiv},
       eprint = {1609.04804},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...829L..32L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Vos2022,
       author = {{Vos}, Johanna M. and {Faherty}, Jacqueline K. and {Gagn{\'e}}, Jonathan and {Marley}, Mark and {Metchev}, Stanimir and {Gizis}, John and {Rice}, Emily L. and {Cruz}, Kelle},
        title = "{Let the Great World Spin: Revealing the Stormy, Turbulent Nature of Young Giant Exoplanet Analogs with the Spitzer Space Telescope}",
      journal = {\apj},
     keywords = {185, 1679, 894, 549, 2119, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jan,
       volume = {924},
       number = {2},
          eid = {68},
        pages = {68},
          doi = {10.3847/1538-4357/ac4502},
archivePrefix = {arXiv},
       eprint = {2201.04711},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...924...68V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Vos2019,
       author = {{Vos}, Johanna M. and {Biller}, Beth A. and {Bonavita}, Mariangela and {Eriksson}, Simon and {Liu}, Michael C. and {Best}, William M.~J. and {Metchev}, Stanimir and {Radigan}, Jacqueline and {Allers}, Katelyn N. and {Janson}, Markus and {Buenzli}, Esther and {Dupuy}, Trent J. and {Bonnefoy}, Micka{\"e}l and {Manjavacas}, Elena and {Brandner}, Wolfgang and {Crossfield}, Ian and {Deacon}, Niall and {Henning}, Thomas and {Homeier}, Derek and {Kopytova}, Taisiya and {Schlieder}, Joshua},
        title = "{A search for variability in exoplanet analogues and low-gravity brown dwarfs}",
      journal = {\mnras},
     keywords = {brown dwarfs, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = feb,
       volume = {483},
       number = {1},
        pages = {480-502},
          doi = {10.1093/mnras/sty3123},
archivePrefix = {arXiv},
       eprint = {1811.08370},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483..480V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Schmidt2015,
       author = {{Schmidt}, Sarah J. and {Hawley}, Suzanne L. and {West}, Andrew A. and {Bochanski}, John J. and {Davenport}, James R.~A. and {Ge}, Jian and {Schneider}, Donald P.},
        title = "{BOSS Ultracool Dwarfs. I. Colors and Magnetic Activity of M and L Dwarfs}",
      journal = {\aj},
     keywords = {astronomical databases: miscellaneous, brown dwarfs, stars: chromospheres, stars: late-type, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = may,
       volume = {149},
       number = {5},
          eid = {158},
        pages = {158},
          doi = {10.1088/0004-6256/149/5/158},
archivePrefix = {arXiv},
       eprint = {1410.0014},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AJ....149..158S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oppenheimer1995,
       author = {{Oppenheimer}, B.~R. and {Kulkarni}, S.~R. and {Matthews}, K. and {Nakajima}, T.},
        title = "{Infrared Spectrum of the Cool Brown Dwarf Gl 229B}",
      journal = {Science},
         year = 1995,
        month = dec,
       volume = {270},
       number = {5241},
        pages = {1478-1479},
          doi = {10.1126/science.270.5241.1478},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995Sci...270.1478O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Dulaimi2023,
       author = {{Dulaimi}, S. and {Golden}, A. and {Boyle}, R.~P. and {Butler}, R.~F.},
        title = "{Optical variabiphase dispersion minimizationlity, rotation period, and inclination angle of the M9.5 dwarf BRI 0021-0214}",
      journal = {\mnras},
     keywords = {auroral activity, dust clouds, inclination angle, optical variability, rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2023,
        month = jan,
       volume = {518},
       number = {3},
        pages = {4428-4437},
          doi = {10.1093/mnras/stac2894},
archivePrefix = {arXiv},
       eprint = {2211.00809},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.518.4428D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lane2007,
       author = {{Lane}, C. and {Hallinan}, G. and {Zavala}, R.~T. and {Butler}, R.~F. and {Boyle}, R.~P. and {Bourke}, S. and {Antonova}, A. and {Doyle}, J.~G. and {Vrba}, F.~J. and {Golden}, A.},
        title = "{Rotational Modulation of M/L Dwarfs due to Magnetic Spots}",
      journal = {\apjl},
     keywords = {Methods: Data Analysis, Stars: Low-Mass, Brown Dwarfs, Stars: Rotation, Stars: Spots, Stars: Variables: Other, Techniques: Photometric, Astrophysics},
         year = 2007,
        month = oct,
       volume = {668},
       number = {2},
        pages = {L163-L166},
          doi = {10.1086/523041},
archivePrefix = {arXiv},
       eprint = {0709.1045},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...668L.163L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Tsuji1996a,
       author = {{Tsuji}, T. and {Ohnaka}, K. and {Aoki}, W.},
        title = "{Dust formation in stellar photospheres: a case of very low mass stars and a possible resolution on the effective temperature scale of M dwarfs.}",
      journal = {\aap},
         year = 1996,
        month = jan,
       volume = {305},
        pages = {L1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...305L...1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Helling2008,
       author = {{Helling}, Ch. and {Ackerman}, A. and {Allard}, F. and {Dehn}, M. and {Hauschildt}, P. and {Homeier}, D. and {Lodders}, K. and {Marley}, M. and {Rietmeijer}, F. and {Tsuji}, T. and {Woitke}, P.},
        title = "{A comparison of chemistry and dust cloud formation in ultracool dwarf model atmospheres}",
      journal = {\mnras},
     keywords = {stars: atmospheres, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = dec,
       volume = {391},
       number = {4},
        pages = {1854-1873},
          doi = {10.1111/j.1365-2966.2008.13991.x},
archivePrefix = {arXiv},
       eprint = {0809.3657},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.391.1854H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Witte2011,
       author = {{Witte}, S. and {Helling}, Ch. and {Barman}, T. and {Heidrich}, N. and {Hauschildt}, P.~H.},
        title = "{Dust in brown dwarfs and extra-solar planets. III. Testing synthetic spectra on observations}",
      journal = {\aap},
     keywords = {astrochemistry, methods: numerical, stars: atmospheres, stars: low-mass, brown dwarfs},
         year = 2011,
        month = may,
       volume = {529},
          eid = {A44},
        pages = {A44},
          doi = {10.1051/0004-6361/201014105},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...529A..44W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Heinze2013,
       author = {{Heinze}, Aren N. and {Metchev}, Stanimir and {Apai}, Daniel and {Flateau}, Davin and {Kurtev}, Radostin and {Marley}, Mark and {Radigan}, Jacqueline and {Burgasser}, Adam J. and {Artigau}, {\'E}tienne and {Plavchan}, Peter},
        title = "{Weather on Other Worlds. I. Detection of Periodic Variability in the L3 Dwarf DENIS-P J1058.7-1548 with Precise Multi-wavelength Photometry}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: DENIS-P J1058.7-1548, stars: low-mass, stars: rotation, starspots, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = apr,
       volume = {767},
       number = {2},
          eid = {173},
        pages = {173},
          doi = {10.1088/0004-637X/767/2/173},
archivePrefix = {arXiv},
       eprint = {1303.2948},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767..173H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Millar-Blanchaer2020,
       author = {{Millar-Blanchaer}, Maxwell A. and {Girard}, Julien H. and {Karalidi}, Theodora and {Marley}, Mark S. and {van Holstein}, Rob G. and {Sengupta}, Sujan and {Mawet}, Dimitri and {Kataria}, Tiffany and {Snik}, Frans and {de Boer}, Jos and {Jensen-Clem}, Rebecca and {Vigan}, Arthur and {Hinkley}, Sasha},
        title = "{Detection of Polarization due to Cloud Bands in the Nearby Luhman 16 Brown Dwarf Binary}",
      journal = {\apj},
     keywords = {Near infrared astronomy, Very Large Telescope, Polarimetry, 1093, 1767, 1278},
         year = 2020,
        month = may,
       volume = {894},
       number = {1},
          eid = {42},
        pages = {42},
          doi = {10.3847/1538-4357/ab6ef2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...894...42M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Brady2022,
       author = {{Brady}, Madison and {Bean}, Jacob and {Seifahrt}, Andreas and {Kasper}, David and {Luque}, Rafael and {Reiners}, Ansgar and {Benneke}, Bj{\"o}rn and {Stef{\'a}nsson}, Gu{\dh}mundur and {St{\"u}rmer}, Julian},
        title = "{Measuring the Obliquities of the TRAPPIST-1 Planets with MAROON-X}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = nov,
          eid = {arXiv:2211.11841},
        pages = {arXiv:2211.11841},
archivePrefix = {arXiv},
       eprint = {2211.11841},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv221111841B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{WISE2010,
       author = {{Wright}, Edward L. and {Eisenhardt}, Peter R.~M. and {Mainzer}, Amy K. and {Ressler}, Michael E. and {Cutri}, Roc M. and {Jarrett}, Thomas and {Kirkpatrick}, J. Davy and {Padgett}, Deborah and {McMillan}, Robert S. and {Skrutskie}, Michael and {Stanford}, S.~A. and {Cohen}, Martin and {Walker}, Russell G. and {Mather}, John C. and {Leisawitz}, David and {Gautier}, Thomas N., III and {McLean}, Ian and {Benford}, Dominic and {Lonsdale}, Carol J. and {Blain}, Andrew and {Mendez}, Bryan and {Irace}, William R. and {Duval}, Valerie and {Liu}, Fengchuan and {Royer}, Don and {Heinrichsen}, Ingolf and {Howard}, Joan and {Shannon}, Mark and {Kendall}, Martha and {Walsh}, Amy L. and {Larsen}, Mark and {Cardon}, Joel G. and {Schick}, Scott and {Schwalm}, Mark and {Abid}, Mohamed and {Fabinsky}, Beth and {Naes}, Larry and {Tsai}, Chao-Wei},
        title = "{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}",
      journal = {\aj},
     keywords = {infrared: general, space vehicles, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = dec,
       volume = {140},
       number = {6},
        pages = {1868-1881},
          doi = {10.1088/0004-6256/140/6/1868},
archivePrefix = {arXiv},
       eprint = {1008.0031},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....140.1868W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{McPherson2012,
       author = {{McPherson}, Alistair and {Spyromilio}, Jason and {Kissler-Patig}, Markus and {Ramsay}, Suzanne and {Brunetto}, Enzo and {Dierickx}, Philippe and {Cassali}, Mark},
        title = "{E-ELT update of project and effect of change to 39m design}",
    booktitle = {Ground-based and Airborne Telescopes IV},
         year = 2012,
       editor = {{Stepp}, Larry M. and {Gilmozzi}, Roberto and {Hall}, Helen J.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {8444},
        month = sep,
          eid = {84441F},
        pages = {84441F},
          doi = {10.1117/12.927787},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SPIE.8444E..1FM},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allard2012,
       author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B.},
        title = "{Models of very-low-mass stars, brown dwarfs and exoplanets}",
      journal = {Philosophical Transactions of the Royal Society of London Series A},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jun,
       volume = {370},
       number = {1968},
        pages = {2765-2777},
          doi = {10.1098/rsta.2011.0269},
archivePrefix = {arXiv},
       eprint = {1112.3591},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012RSPTA.370.2765A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Maihara1993,
       author = {{Maihara}, Toshinori and {Iwamuro}, Fumihide and {Yamashita}, Takuya and {Hall}, Donald N.~B. and {Cowie}, Lennox L. and {Tokunaga}, Alan T. and {Pickles}, Andrew},
        title = "{Observations of the OH Airglow Emission}",
      journal = {\pasp},
     keywords = {Airglow, Background Radiation, Hydroxyl Radicals, Spectral Bands, Spectral Emission, Infrared Astronomy, Line Spectra, Near Infrared Radiation, Geophysics, ATMOSPHERIC EFFECTS, LINE: IDENTIFICATION, TECHNIQUES: PHOTOMETRIC},
         year = 1993,
        month = sep,
       volume = {105},
        pages = {940},
          doi = {10.1086/133259},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993PASP..105..940M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Lord1992,
       author = {{Lord}, Steven D.},
        title = "{A new software tool for computing Earth's atmospheric transmission of near- and far-infrared radiation}",
     keywords = {Atmospheric Models, Earth Atmosphere, Far Infrared Radiation, Infrared Spectra, Radiative Transfer, Software Tools, Transmittance, Calibrating, Data Reduction, Ozone, Water Vapor, Geophysics},
 howpublished = {NASA Technical Memorandum 103957},
         year = 1992,
        month = dec,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992nstc.rept.....L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Skidmore2015,
       author = {{Skidmore}, Warren and {TMT International Science Development Teams} and {Science Advisory Committee}, TMT},
        title = "{Thirty Meter Telescope Detailed Science Case: 2015}",
      journal = {Research in Astronomy and Astrophysics},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = dec,
       volume = {15},
       number = {12},
          eid = {1945},
        pages = {1945},
          doi = {10.1088/1674-4527/15/12/001},
archivePrefix = {arXiv},
       eprint = {1505.01195},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015RAA....15.1945S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Noll2012,
       author = {{Noll}, S. and {Kausch}, W. and {Barden}, M. and {Jones}, A.~M. and {Szyszka}, C. and {Kimeswenger}, S.},
        title = "{An atmospheric radiation model for the Very Large Telescope at Cerro Paranal in Chile}",
    booktitle = {EGU General Assembly Conference Abstracts},
         year = 2012,
       series = {EGU General Assembly Conference Abstracts},
        month = apr,
        pages = {9813},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012EGUGA..14.9813N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jones2013,
       author = {{Jones}, A. and {Noll}, S. and {Kausch}, W. and {Szyszka}, C. and {Kimeswenger}, S.},
        title = "{An advanced scattered moonlight model for Cerro Paranal}",
      journal = {\aap},
     keywords = {Moon, atmospheric effects, radiative transfer, scattering, methods: data analysis, techniques: spectroscopic, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2013,
        month = dec,
       volume = {560},
          eid = {A91},
        pages = {A91},
          doi = {10.1051/0004-6361/201322433},
archivePrefix = {arXiv},
       eprint = {1310.7030},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...560A..91J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Zhou2022,
       author = {{Zhou}, Yifan and {Bowler}, Brendan P. and {Apai}, D{\'a}niel and {Kataria}, Tiffany and {Morley}, Caroline V. and {Bryan}, Marta L. and {Skemer}, Andrew J. and {Benneke}, Bj{\"o}rn},
        title = "{Roaring Storms in the Planetary-Mass Companion VHS 1256-1257 b: Hubble Space Telescope Multi-epoch Monitoring Reveals Vigorous Evolution in an Ultra-cool Atmosphere}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = oct,
          eid = {arXiv:2210.02464},
        pages = {arXiv:2210.02464},
archivePrefix = {arXiv},
       eprint = {2210.02464},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv221002464Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wang2022,
       author = {{Wang}, Ji and {Kolecki}, Jared R. and {Ruffio}, Jean-Baptiste and {Wang}, Jason J. and {Mawet}, Dimitri and {Baker}, Ashley and {Bartos}, Randall and {Blake}, Geoffrey A. and {Bond}, Charlotte Z. and {Calvin}, Benjamin and {Cetre}, Sylvain and {Delorme}, Jacques-Robert and {Doppmann}, Greg and {Echeverri}, Daniel and {Finnerty}, Luke and {Fitzgerald}, Michael P. and {Jovanovic}, Nemanja and {Liu}, Michael C. and {Lopez}, Ronald and {Morris}, Evan and {Pai Asnodkar}, Anusha and {Pezzato}, Jacklyn and {Ragland}, Sam and {Roy}, Arpita and {Ruane}, Garreth and {Sappey}, Ben and {Schofield}, Tobias and {Skemer}, Andrew and {Venenciano}, Taylor and {Kent Wallace}, J. and {Wallack}, Nicole L. and {Wizinowich}, Peter and {Xuan}, Jerry W.},
        title = "{Retrieving the C and O Abundances of HR 7672 AB: A Solar-type Primary Star with a Benchmark Brown Dwarf}",
      journal = {\aj},
     keywords = {Exoplanet atmospheric composition, Brown dwarfs, Chemical abundances, 2021, 185, 224, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = apr,
       volume = {163},
       number = {4},
          eid = {189},
        pages = {189},
          doi = {10.3847/1538-3881/ac56e2},
archivePrefix = {arXiv},
       eprint = {2202.02477},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....163..189W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@INPROCEEDINGS{Thomas-Osip2008,
       author = {{Thomas-Osip}, Joanna E. and {Prieto}, Gabriel and {Johns}, Matt and {Phillips}, Mark M.},
        title = "{Giant Magellan Telescope site evaluation and characterization at Las Campanas Observatory}",
    booktitle = {Ground-based and Airborne Telescopes II},
         year = 2008,
       editor = {{Stepp}, Larry M. and {Gilmozzi}, Roberto},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7012},
        month = jul,
          eid = {70121U},
        pages = {70121U},
          doi = {10.1117/12.789863},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7012E..1UT},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chabrier&Baraffe2000,
       author = {{Chabrier}, Gilles and {Baraffe}, Isabelle},
        title = "{Theory of Low-Mass Stars and Substellar Objects}",
      journal = {\araa},
     keywords = {STARS: FUNDAMENTAL PARAMETERS, STARS: LOW MASS, BROWN DWARFS, STARS: CATACLYSMIC VARIABLES, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, STARS: PLANETARY SYSTEMS, GALAXY: STELLAR CONTENT, Astrophysics},
         year = 2000,
        month = jan,
       volume = {38},
        pages = {337-377},
          doi = {10.1146/annurev.astro.38.1.337},
archivePrefix = {arXiv},
       eprint = {astro-ph/0006383},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ARA&A..38..337C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@INPROCEEDINGS{Johns2008,
       author = {{Johns}, Matt},
        title = "{Progress on the GMT}",
    booktitle = {Ground-based and Airborne Telescopes II},
         year = 2008,
       editor = {{Stepp}, Larry M. and {Gilmozzi}, Roberto},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7012},
        month = jul,
          eid = {70121B},
        pages = {70121B},
          doi = {10.1117/12.788063},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7012E..1BJ},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Johns2006,
       author = {{Johns}, Matt},
        title = "{The Giant Magellan Telescope (GMT)}",
    booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
         year = 2006,
       editor = {{Stepp}, Larry M.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {6267},
        month = jun,
          eid = {626729},
        pages = {626729},
          doi = {10.1117/12.670839},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006SPIE.6267E..29J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Grigel2018,
       author = {{Grigel}, Eric and {Bigelow}, Bruce C. and {Burgett}, William S. and {Arriagada}, Gustavo and {Turner}, Robert and {Talison}, Bahram and {Madden}, Christopher and {Figueroa}, Francisco and {Teran}, Jose and {Manuel}, Eric},
        title = "{GMT site, enclosure, and facilities: design and construction update}",
    booktitle = {Ground-based and Airborne Telescopes VII},
         year = 2018,
       editor = {{Marshall}, Heather K. and {Spyromilio}, Jason},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {10700},
        month = jul,
          eid = {107000A},
        pages = {107000A},
          doi = {10.1117/12.2314554},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018SPIE10700E..0AG},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Fanson2018,
       author = {{Fanson}, James and {McCarthy}, Patrick J. and {Bernstein}, Rebecca and {Angeli}, George and {Ashby}, David and {Bigelow}, Bruce and {Bouchez}, Antonin and {Burgett}, William and {Chauvin}, Eric and {Contos}, Adam and {Figueroa}, Francisco and {Gray}, Peter and {Groark}, Frank and {Laskin}, Robert and {Millan-Gabet}, Rafael and {Rakich}, Andrew and {Sandoval}, Rodrigo and {Pi}, Marti and {Wheeler}, Nune},
        title = "{Overview and status of the Giant Magellan Telescope project}",
    booktitle = {Ground-based and Airborne Telescopes VII},
         year = 2018,
       editor = {{Marshall}, Heather K. and {Spyromilio}, Jason},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {10700},
        month = jul,
          eid = {1070012},
        pages = {1070012},
          doi = {10.1117/12.2313340},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018SPIE10700E..12F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@INPROCEEDINGS{Fanson2020,
       author = {{Fanson}, James and {Bernstein}, Rebecca and {Angeli}, George and {Ashby}, David and {Bigelow}, Bruce and {Brossus}, Glenn and {Bouchez}, Antonin and {Burgett}, William and {Contos}, Adam and {Demers}, Richard and {Figueroa}, Francisco and {Fischer}, Barbara and {Groark}, Frank and {Laskin}, Robert and {Millan-Gabet}, Rafael and {Pi}, Marti and {Wheeler}, Nune},
        title = "{Overview and status of the Giant Magellan Telescope project}",
    booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
         year = 2020,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {11445},
        month = dec,
          eid = {114451F},
        pages = {114451F},
          doi = {10.1117/12.2561852},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SPIE11445E..1FF},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Reiners&Basri2010,
       author = {{Reiners}, A. and {Basri}, G.},
        title = "{A Volume-Limited Sample of 63 M7-M9.5 Dwarfs. II. Activity, Magnetism, and the Fade of the Rotation-Dominated Dynamo}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: low-mass, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {2},
        pages = {924-935},
          doi = {10.1088/0004-637X/710/2/924},
archivePrefix = {arXiv},
       eprint = {0912.4259},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710..924R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Roettenbacher2017,
       author = {{Roettenbacher}, Rachael M. and {Kane}, Stephen R.},
        title = "{The Stellar Activity of TRAPPIST-1 and Consequences for the Planetary Atmospheres}",
      journal = {\apj},
     keywords = {stars: activity, stars: individual: TRAPPIST-1, stars: variables: general, starspots, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = dec,
       volume = {851},
       number = {2},
          eid = {77},
        pages = {77},
          doi = {10.3847/1538-4357/aa991e},
archivePrefix = {arXiv},
       eprint = {1711.02676},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...851...77R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Reiners2018,
       author = {{Reiners}, A. and {Zechmeister}, M. and {Caballero}, J.~A. and {Ribas}, I. and {Morales}, J.~C. and {Jeffers}, S.~V. and {Sch{\"o}fer}, P. and {Tal-Or}, L. and {Quirrenbach}, A. and {Amado}, P.~J. and {Kaminski}, A. and {Seifert}, W. and {Abril}, M. and {Aceituno}, J. and {Alonso-Floriano}, F.~J. and {Ammler-von Eiff}, M. and {Antona}, R. and {Anglada-Escud{\'e}}, G. and {Anwand-Heerwart}, H. and {Arroyo-Torres}, B. and {Azzaro}, M. and {Baroch}, D. and {Barrado}, D. and {Bauer}, F.~F. and {Becerril}, S. and {B{\'e}jar}, V.~J.~S. and {Ben{\'\i}tez}, D. and {Berdinas}, Z.~M. and {Bergond}, G. and {Bl{\"u}mcke}, M. and {Brinkm{\"o}ller}, M. and {del Burgo}, C. and {Cano}, J. and {C{\'a}rdenas V{\'a}zquez}, M.~C. and {Casal}, E. and {Cifuentes}, C. and {Claret}, A. and {Colom{\'e}}, J. and {Cort{\'e}s-Contreras}, M. and {Czesla}, S. and {D{\'\i}ez-Alonso}, E. and {Dreizler}, S. and {Feiz}, C. and {Fern{\'a}ndez}, M. and {Ferro}, I.~M. and {Fuhrmeister}, B. and {Galad{\'\i}-Enr{\'\i}quez}, D. and {Garcia-Piquer}, A. and {Garc{\'\i}a Vargas}, M.~L. and {Gesa}, L. and {G{\'o}mez Galera}, V. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Gonz{\'a}lez-Peinado}, R. and {Gr{\"o}zinger}, U. and {Grohnert}, S. and {Gu{\`a}rdia}, J. and {Guenther}, E.~W. and {Guijarro}, A. and {de Guindos}, E. and {Guti{\'e}rrez-Soto}, J. and {Hagen}, H. -J. and {Hatzes}, A.~P. and {Hauschildt}, P.~H. and {Hedrosa}, R.~P. and {Helmling}, J. and {Henning}, Th. and {Hermelo}, I. and {Hern{\'a}ndez Arab{\'\i}}, R. and {Hern{\'a}ndez Casta{\~n}o}, L. and {Hern{\'a}ndez Hernando}, F. and {Herrero}, E. and {Huber}, A. and {Huke}, P. and {Johnson}, E.~N. and {de Juan}, E. and {Kim}, M. and {Klein}, R. and {Kl{\"u}ter}, J. and {Klutsch}, A. and {K{\"u}rster}, M. and {Lafarga}, M. and {Lamert}, A. and {Lamp{\'o}n}, M. and {Lara}, L.~M. and {Laun}, W. and {Lemke}, U. and {Lenzen}, R. and {Launhardt}, R. and {L{\'o}pez del Fresno}, M. and {L{\'o}pez-Gonz{\'a}lez}, J. and {L{\'o}pez-Puertas}, M. and {L{\'o}pez Salas}, J.~F. and {L{\'o}pez-Santiago}, J. and {Luque}, R. and {Mag{\'a}n Madinabeitia}, H. and {Mall}, U. and {Mancini}, L. and {Mandel}, H. and {Marfil}, E. and {Mar{\'\i}n Molina}, J.~A. and {Maroto Fern{\'a}ndez}, D. and {Mart{\'\i}n}, E.~L. and {Mart{\'\i}n-Ruiz}, S. and {Marvin}, C.~J. and {Mathar}, R.~J. and {Mirabet}, E. and {Montes}, D. and {Moreno-Raya}, M.~E. and {Moya}, A. and {Mundt}, R. and {Nagel}, E. and {Naranjo}, V. and {Nortmann}, L. and {Nowak}, G. and {Ofir}, A. and {Oreiro}, R. and {Pall{\'e}}, E. and {Panduro}, J. and {Pascual}, J. and {Passegger}, V.~M. and {Pavlov}, A. and {Pedraz}, S. and {P{\'e}rez-Calpena}, A. and {P{\'e}rez Medialdea}, D. and {Perger}, M. and {Perryman}, M.~A.~C. and {Pluto}, M. and {Rabaza}, O. and {Ram{\'o}n}, A. and {Rebolo}, R. and {Redondo}, P. and {Reffert}, S. and {Reinhart}, S. and {Rhode}, P. and {Rix}, H. -W. and {Rodler}, F. and {Rodr{\'\i}guez}, E. and {Rodr{\'\i}guez-L{\'o}pez}, C. and {Rodr{\'\i}guez Trinidad}, A. and {Rohloff}, R. -R. and {Rosich}, A. and {Sadegi}, S. and {S{\'a}nchez-Blanco}, E. and {S{\'a}nchez Carrasco}, M.~A. and {S{\'a}nchez-L{\'o}pez}, A. and {Sanz-Forcada}, J. and {Sarkis}, P. and {Sarmiento}, L.~F. and {Sch{\"a}fer}, S. and {Schmitt}, J.~H.~M.~M. and {Schiller}, J. and {Schweitzer}, A. and {Solano}, E. and {Stahl}, O. and {Strachan}, J.~B.~P. and {St{\"u}rmer}, J. and {Su{\'a}rez}, J.~C. and {Tabernero}, H.~M. and {Tala}, M. and {Trifonov}, T. and {Tulloch}, S.~M. and {Ulbrich}, R.~G. and {Veredas}, G. and {Vico Linares}, J.~I. and {Vilardell}, F. and {Wagner}, K. and {Winkler}, J. and {Wolthoff}, V. and {Xu}, W. and {Yan}, F. and {Zapatero Osorio}, M.~R.},
        title = "{The CARMENES search for exoplanets around M dwarfs. High-resolution optical and near-infrared spectroscopy of 324 survey stars}",
      journal = {\aap},
     keywords = {atlases, catalogs, stars: rotation, stars: late-type, stars: low-mass, infrared: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = apr,
       volume = {612},
          eid = {A49},
        pages = {A49},
          doi = {10.1051/0004-6361/201732054},
archivePrefix = {arXiv},
       eprint = {1711.06576},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...612A..49R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Vida2017,
       author = {{Vida}, K. and {K{\H{o}}v{\'a}ri}, Zs. and {P{\'a}l}, A. and {Ol{\'a}h}, K. and {Kriskovics}, L.},
        title = "{Frequent Flaring in the TRAPPIST-1 System{\textemdash}Unsuited for Life?}",
      journal = {\apj},
     keywords = {stars: activity, stars: chromospheres, stars: flare, stars: late-type, stars: low-mass, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jun,
       volume = {841},
       number = {2},
          eid = {124},
        pages = {124},
          doi = {10.3847/1538-4357/aa6f05},
archivePrefix = {arXiv},
       eprint = {1703.10130},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...841..124V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Luger2017,
       author = {{Luger}, Rodrigo and {Sestovic}, Marko and {Kruse}, Ethan and {Grimm}, Simon L. and {Demory}, Brice-Olivier and {Agol}, Eric and {Bolmont}, Emeline and {Fabrycky}, Daniel and {Fernandes}, Catarina S. and {Van Grootel}, Val{\'e}rie and {Burgasser}, Adam and {Gillon}, Micha{\"e}l and {Ingalls}, James G. and {Jehin}, Emmanu{\"e}l and {Raymond}, Sean N. and {Selsis}, Franck and {Triaud}, Amaury H.~M.~J. and {Barclay}, Thomas and {Barentsen}, Geert and {Howell}, Steve B. and {Delrez}, Laetitia and {de Wit}, Julien and {Foreman-Mackey}, Daniel and {Holdsworth}, Daniel L. and {Leconte}, J{\'e}r{\'e}my and {Lederer}, Susan and {Turbet}, Martin and {Almleaky}, Yaseen and {Benkhaldoun}, Zouhair and {Magain}, Pierre and {Morris}, Brett M. and {Heng}, Kevin and {Queloz}, Didier},
        title = "{A seven-planet resonant chain in TRAPPIST-1}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jun,
       volume = {1},
          eid = {0129},
        pages = {0129},
          doi = {10.1038/s41550-017-0129},
archivePrefix = {arXiv},
       eprint = {1703.04166},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017NatAs...1E.129L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Morris2018,
       author = {{Morris}, Brett M. and {Agol}, Eric and {Davenport}, James R.~A. and {Hawley}, Suzanne L.},
        title = "{Possible Bright Starspots on TRAPPIST-1}",
      journal = {\apj},
     keywords = {stars: activity, stars: atmospheres, stars: flare, stars: individual: TRAPPIST-1, stars: low-mass, starspots, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = apr,
       volume = {857},
       number = {1},
          eid = {39},
        pages = {39},
          doi = {10.3847/1538-4357/aab6a5},
archivePrefix = {arXiv},
       eprint = {1803.04543},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...857...39M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Wheatley2017,
       author = {{Wheatley}, Peter J. and {Louden}, Tom and {Bourrier}, Vincent and {Ehrenreich}, David and {Gillon}, Micha{\"e}l},
        title = "{Strong XUV irradiation of the Earth-sized exoplanets orbiting the ultracool dwarf TRAPPIST-1}",
      journal = {\mnras},
     keywords = {planets and satellites: atmospheres, planets and satellites: terrestrial planets, planet-star interactions, stars: individual: TRAPPIST-1, stars: late-type, X-rays: stars, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = feb,
       volume = {465},
       number = {1},
        pages = {L74-L78},
          doi = {10.1093/mnrasl/slw192},
archivePrefix = {arXiv},
       eprint = {1605.01564},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465L..74W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gonzales2019,
       author = {{Gonzales}, Eileen C. and {Faherty}, Jacqueline K. and {Gagn{\'e}}, Jonathan and {Teske}, Johanna and {McWilliam}, Andrew and {Cruz}, Kelle},
        title = "{A Reanalysis of the Fundamental Parameters and Age of TRAPPIST-1}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: fundamental parameters, stars: individual: 2MASSJ23062928-0502285, TRAPPIST-1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {886},
       number = {2},
          eid = {131},
        pages = {131},
          doi = {10.3847/1538-4357/ab48fc},
archivePrefix = {arXiv},
       eprint = {1909.13859},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886..131G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Burgasser&Mamajek2017,
       author = {{Burgasser}, Adam J. and {Mamajek}, Eric E.},
        title = "{On the Age of the TRAPPIST-1 System}",
      journal = {\apj},
     keywords = {stars: activity, stars: atmospheres, stars: individual: 2MASS J23062928-0502285, TRAPPIST-1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = aug,
       volume = {845},
       number = {2},
          eid = {110},
        pages = {110},
          doi = {10.3847/1538-4357/aa7fea},
archivePrefix = {arXiv},
       eprint = {1706.02018},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...845..110B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wilson2021,
       author = {{Wilson}, David J. and {Froning}, Cynthia S. and {Duvvuri}, Girish M. and {France}, Kevin and {Youngblood}, Allison and {Schneider}, P. Christian and {Berta-Thompson}, Zachory and {Brown}, Alexander and {Buccino}, Andrea P. and {Hawley}, Suzanne and {Irwin}, Jonathan and {Kaltenegger}, Lisa and {Kowalski}, Adam and {Linsky}, Jeffrey and {Parke Loyd}, R.~O. and {Miguel}, Yamila and {Pineda}, J. Sebastian and {Redfield}, Seth and {Roberge}, Aki and {Rugheimer}, Sarah and {Tian}, Feng and {Vieytes}, Mariela},
        title = "{The Mega-MUSCLES Spectral Energy Distribution of TRAPPIST-1}",
      journal = {\apj},
     keywords = {M dwarf stars, Exoplanet astronomy, Exoplanet atmospheres, Ultraviolet astronomy, X-ray astronomy, Spectral energy distribution, Spectroscopy, Stellar atmospheres, 982, 486, 487, 1736, 1810, 2129, 1558, 1584, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
       volume = {911},
       number = {1},
          eid = {18},
        pages = {18},
          doi = {10.3847/1538-4357/abe771},
archivePrefix = {arXiv},
       eprint = {2102.11415},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911...18W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{O'Malley-James2017,
       author = {{O'Malley-James}, Jack T. and {Kaltenegger}, L.},
        title = "{UV surface habitability of the TRAPPIST-1 system}",
      journal = {\mnras},
     keywords = {planets and satellites: individual: TRAPPIST-1, stars: activity, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jul,
       volume = {469},
       number = {1},
        pages = {L26-L30},
          doi = {10.1093/mnrasl/slx047},
archivePrefix = {arXiv},
       eprint = {1702.06936},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.469L..26O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gillon2017,
       author = {{Gillon}, Micha{\"e}l and {Triaud}, Amaury H.~M.~J. and {Demory}, Brice-Olivier and {Jehin}, Emmanu{\"e}l and {Agol}, Eric and {Deck}, Katherine M. and {Lederer}, Susan M. and {de Wit}, Julien and {Burdanov}, Artem and {Ingalls}, James G. and {Bolmont}, Emeline and {Leconte}, Jeremy and {Raymond}, Sean N. and {Selsis}, Franck and {Turbet}, Martin and {Barkaoui}, Khalid and {Burgasser}, Adam and {Burleigh}, Matthew R. and {Carey}, Sean J. and {Chaushev}, Aleksander and {Copperwheat}, Chris M. and {Delrez}, Laetitia and {Fernandes}, Catarina S. and {Holdsworth}, Daniel L. and {Kotze}, Enrico J. and {Van Grootel}, Val{\'e}rie and {Almleaky}, Yaseen and {Benkhaldoun}, Zouhair and {Magain}, Pierre and {Queloz}, Didier},
        title = "{Seven temperate terrestrial planets around the nearby ultracool dwarf star TRAPPIST-1}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = feb,
       volume = {542},
       number = {7642},
        pages = {456-460},
          doi = {10.1038/nature21360},
archivePrefix = {arXiv},
       eprint = {1703.01424},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Natur.542..456G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gillon2016,
       author = {{Gillon}, Micha{\"e}l and {Jehin}, Emmanu{\"e}l and {Lederer}, Susan M. and {Delrez}, Laetitia and {de Wit}, Julien and {Burdanov}, Artem and {Van Grootel}, Val{\'e}rie and {Burgasser}, Adam J. and {Triaud}, Amaury H.~M.~J. and {Opitom}, Cyrielle and {Demory}, Brice-Olivier and {Sahu}, Devendra K. and {Bardalez Gagliuffi}, Daniella and {Magain}, Pierre and {Queloz}, Didier},
        title = "{Temperate Earth-sized planets transiting a nearby ultracool dwarf star}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = may,
       volume = {533},
       number = {7602},
        pages = {221-224},
          doi = {10.1038/nature17448},
archivePrefix = {arXiv},
       eprint = {1605.07211},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016Natur.533..221G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Molliere2019,
       author = {{Molli{\`e}re}, P. and {Wardenier}, J.~P. and {van Boekel}, R. and {Henning}, Th. and {Molaverdikhani}, K. and {Snellen}, I.~A.~G.},
        title = "{petitRADTRANS. A Python radiative transfer package for exoplanet characterization and retrieval}",
      journal = {\aap},
     keywords = {methods: numerical, planets and satellites: atmospheres, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/201935470},
archivePrefix = {arXiv},
       eprint = {1904.11504},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A..67M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zurlo2016,
       author = {{Zurlo}, A. and {Vigan}, A. and {Galicher}, R. and {Maire}, A. -L. and {Mesa}, D. and {Gratton}, R. and {Chauvin}, G. and {Kasper}, M. and {Moutou}, C. and {Bonnefoy}, M. and {Desidera}, S. and {Abe}, L. and {Apai}, D. and {Baruffolo}, A. and {Baudoz}, P. and {Baudrand}, J. and {Beuzit}, J. -L. and {Blancard}, P. and {Boccaletti}, A. and {Cantalloube}, F. and {Carle}, M. and {Cascone}, E. and {Charton}, J. and {Claudi}, R.~U. and {Costille}, A. and {de Caprio}, V. and {Dohlen}, K. and {Dominik}, C. and {Fantinel}, D. and {Feautrier}, P. and {Feldt}, M. and {Fusco}, T. and {Gigan}, P. and {Girard}, J.~H. and {Gisler}, D. and {Gluck}, L. and {Gry}, C. and {Henning}, T. and {Hugot}, E. and {Janson}, M. and {Jaquet}, M. and {Lagrange}, A. -M. and {Langlois}, M. and {Llored}, M. and {Madec}, F. and {Magnard}, Y. and {Martinez}, P. and {Maurel}, D. and {Mawet}, D. and {Meyer}, M.~R. and {Milli}, J. and {Moeller-Nilsson}, O. and {Mouillet}, D. and {Orign{\'e}}, A. and {Pavlov}, A. and {Petit}, C. and {Puget}, P. and {Quanz}, S.~P. and {Rabou}, P. and {Ramos}, J. and {Rousset}, G. and {Roux}, A. and {Salasnich}, B. and {Salter}, G. and {Sauvage}, J. -F. and {Schmid}, H.~M. and {Soenke}, C. and {Stadler}, E. and {Suarez}, M. and {Turatto}, M. and {Udry}, S. and {Vakili}, F. and {Wahhaj}, Z. and {Wildi}, F. and {Antichi}, J.},
        title = "{First light of the VLT planet finder SPHERE. III. New spectrophotometry and astrometry of the HR 8799 exoplanetary system}",
      journal = {\aap},
     keywords = {techniques: image processing, astrometry, techniques: high angular resolution, techniques: spectroscopic, methods: data analysis, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = mar,
       volume = {587},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201526835},
archivePrefix = {arXiv},
       eprint = {1511.04083},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...587A..57Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Greenbaum2018,
       author = {{Greenbaum}, Alexandra Z. and {Pueyo}, Laurent and {Ruffio}, Jean-Baptiste and {Wang}, Jason J. and {De Rosa}, Robert J. and {Aguilar}, Jonathan and {Rameau}, Julien and {Barman}, Travis and {Marois}, Christian and {Marley}, Mark S. and {Konopacky}, Quinn and {Rajan}, Abhijith and {Macintosh}, Bruce and {Ansdell}, Megan and {Arriaga}, Pauline and {Bailey}, Vanessa P. and {Bulger}, Joanna and {Burrows}, Adam S. and {Chilcote}, Jeffrey and {Cotten}, Tara and {Doyon}, Rene and {Duch{\^e}ne}, Gaspard and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Gerard}, Benjamin and {Goodsell}, Stephen J. and {Graham}, James R. and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Kalas}, Paul and {Larkin}, James E. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Nielsen}, Eric L. and {Norton}, Andrew and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall D. and {Poyneer}, Lisa and {Rantakyr{\"o}}, Fredrik T. and {Savransky}, Dmitry and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, R{\'e}mi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Ward-Duong}, Kimberly and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{GPI Spectra of HR 8799 c, d, and e from 1.5 to 2.4 {\ensuremath{\mu}}m with KLIP Forward Modeling}",
      journal = {\aj},
     keywords = {planets and satellites: gaseous planets, stars: individual: HR 8799, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = jun,
       volume = {155},
       number = {6},
          eid = {226},
        pages = {226},
          doi = {10.3847/1538-3881/aabcb8},
archivePrefix = {arXiv},
       eprint = {1804.07774},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....155..226G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{GravityCollab2019,
       author = {{GRAVITY Collaboration} and {Lacour}, S. and {Nowak}, M. and {Wang}, J. and {Pfuhl}, O. and {Eisenhauer}, F. and {Abuter}, R. and {Amorim}, A. and {Anugu}, N. and {Benisty}, M. and {Berger}, J.~P. and {Beust}, H. and {Blind}, N. and {Bonnefoy}, M. and {Bonnet}, H. and {Bourget}, P. and {Brandner}, W. and {Buron}, A. and {Collin}, C. and {Charnay}, B. and {Chapron}, F. and {Cl{\'e}net}, Y. and {Coud{\'e} Du Foresto}, V. and {de Zeeuw}, P.~T. and {Deen}, C. and {Dembet}, R. and {Dexter}, J. and {Duvert}, G. and {Eckart}, A. and {F{\"o}rster Schreiber}, N.~M. and {F{\'e}dou}, P. and {Garcia}, P. and {Garcia Lopez}, R. and {Gao}, F. and {Gendron}, E. and {Genzel}, R. and {Gillessen}, S. and {Gordo}, P. and {Greenbaum}, A. and {Habibi}, M. and {Haubois}, X. and {Hau{\ss}mann}, F. and {Henning}, Th. and {Hippler}, S. and {Horrobin}, M. and {Hubert}, Z. and {Jimenez Rosales}, A. and {Jocou}, L. and {Kendrew}, S. and {Kervella}, P. and {Kolb}, J. and {Lagrange}, A. -M. and {Lapeyr{\`e}re}, V. and {Le Bouquin}, J. -B. and {L{\'e}na}, P. and {Lippa}, M. and {Lenzen}, R. and {Maire}, A. -L. and {Molli{\`e}re}, P. and {Ott}, T. and {Paumard}, T. and {Perraut}, K. and {Perrin}, G. and {Pueyo}, L. and {Rabien}, S. and {Ram{\'\i}rez}, A. and {Rau}, C. and {Rodr{\'\i}guez-Coira}, G. and {Rousset}, G. and {Sanchez-Bermudez}, J. and {Scheithauer}, S. and {Schuhler}, N. and {Straub}, O. and {Straubmeier}, C. and {Sturm}, E. and {Tacconi}, L.~J. and {Vincent}, F. and {van Dishoeck}, E.~F. and {von Fellenberg}, S. and {Wank}, I. and {Waisberg}, I. and {Widmann}, F. and {Wieprecht}, E. and {Wiest}, M. and {Wiezorrek}, E. and {Woillez}, J. and {Yazici}, S. and {Ziegler}, D. and {Zins}, G.},
        title = "{First direct detection of an exoplanet by optical interferometry. Astrometry and K-band spectroscopy of HR 8799 e}",
      journal = {\aap},
     keywords = {stars: individual: HR 8799, planets and satellites: atmospheres, planet-star interactions, techniques: interferometric, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {L11},
        pages = {L11},
          doi = {10.1051/0004-6361/201935253},
archivePrefix = {arXiv},
       eprint = {1903.11903},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623L..11G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ruffio2021,
       author = {{Ruffio}, Jean-Baptiste and {Konopacky}, Quinn M. and {Barman}, Travis and {Macintosh}, Bruce and {Hoch}, Kielan K.~W. and {De Rosa}, Robert J. and {Wang}, Jason J. and {Czekala}, Ian and {Marois}, Christian},
        title = "{Deep Exploration of the Planets HR 8799 b, c, and d with Moderate-resolution Spectroscopy}",
      journal = {\aj},
     keywords = {509, 2021, 387, 492, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = dec,
       volume = {162},
       number = {6},
          eid = {290},
        pages = {290},
          doi = {10.3847/1538-3881/ac273a},
archivePrefix = {arXiv},
       eprint = {2109.07614},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....162..290R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{JJWang2021,
       author = {{Wang}, Jason J. and {Ruffio}, Jean-Baptiste and {Morris}, Evan and {Delorme}, Jacques-Robert and {Jovanovic}, Nemanja and {Pezzato}, Jacklyn and {Echeverri}, Daniel and {Finnerty}, Luke and {Hood}, Callie and {Zanazzi}, J.~J. and {Bryan}, Marta L. and {Bond}, Charlotte Z. and {Cetre}, Sylvain and {Martin}, Emily C. and {Mawet}, Dimitri and {Skemer}, Andy and {Baker}, Ashley and {Xuan}, Jerry W. and {Wallace}, J. Kent and {Wang}, Ji and {Bartos}, Randall and {Blake}, Geoffrey A. and {Boden}, Andy and {Buzard}, Cam and {Calvin}, Benjamin and {Chun}, Mark and {Doppmann}, Greg and {Dupuy}, Trent J. and {Duch{\^e}ne}, Gaspard and {Feng}, Y. Katherina and {Fitzgerald}, Michael P. and {Fortney}, Jonathan and {Freedman}, Richard S. and {Knutson}, Heather and {Konopacky}, Quinn and {Lilley}, Scott and {Liu}, Michael C. and {Lopez}, Ronald and {Lupu}, Roxana and {Marley}, Mark S. and {Meshkat}, Tiffany and {Miles}, Brittany and {Millar-Blanchaer}, Maxwell and {Ragland}, Sam and {Roy}, Arpita and {Ruane}, Garreth and {Sappey}, Ben and {Schofield}, Tobias and {Weiss}, Lauren and {Wetherell}, Edward and {Wizinowich}, Peter and {Ygouf}, Marie},
        title = "{Detection and Bulk Properties of the HR 8799 Planets with High-resolution Spectroscopy}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanet formation, High angular resolution, High resolution spectroscopy, 487, 492, 2167, 2096, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {162},
       number = {4},
          eid = {148},
        pages = {148},
          doi = {10.3847/1538-3881/ac1349},
archivePrefix = {arXiv},
       eprint = {2107.06949},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....162..148W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{JJWang2022,
       author = {{Wang}, Jason J. and {Gao}, Peter and {Chilcote}, Jeffrey and {Lozi}, Julien and {Guyon}, Olivier and {Marois}, Christian and {De Rosa}, Robert J. and {Sahoo}, Ananya and {Groff}, Tyler D. and {Vievard}, Sebastien and {Jovanovic}, Nemanja and {Greenbaum}, Alexandra Z. and {Macintosh}, Bruce},
        title = "{Atmospheric Monitoring and Precise Spectroscopy of the HR 8799 Planets with SCExAO/CHARIS}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanet atmospheric variability, Spectrophotometry, 487, 2020, 1556, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = oct,
       volume = {164},
       number = {4},
          eid = {143},
        pages = {143},
          doi = {10.3847/1538-3881/ac8984},
archivePrefix = {arXiv},
       eprint = {2208.05594},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....164..143W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Marley2012,
       author = {{Marley}, Mark S. and {Saumon}, Didier and {Cushing}, Michael and {Ackerman}, Andrew S. and {Fortney}, Jonathan J. and {Freedman}, Richard},
        title = "{Masses, Radii, and Cloud Properties of the HR 8799 Planets}",
      journal = {\apj},
     keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: individual: HR 8799, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = aug,
       volume = {754},
       number = {2},
          eid = {135},
        pages = {135},
          doi = {10.1088/0004-637X/754/2/135},
archivePrefix = {arXiv},
       eprint = {1205.6488},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...754..135M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Barman2011,
       author = {{Barman}, Travis S. and {Macintosh}, Bruce and {Konopacky}, Quinn M. and {Marois}, Christian},
        title = "{Clouds and Chemistry in the Atmosphere of Extrasolar Planet HR8799b}",
      journal = {\apj},
     keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = may,
       volume = {733},
       number = {1},
          eid = {65},
        pages = {65},
          doi = {10.1088/0004-637X/733/1/65},
archivePrefix = {arXiv},
       eprint = {1103.3895},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...733...65B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gaia2021,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties (Corrigendum)}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, errata, addenda},
         year = 2021,
        month = jun,
       volume = {650},
          eid = {C3},
        pages = {C3},
          doi = {10.1051/0004-6361/202039657e},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...650C...3G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bowler2010,
       author = {{Bowler}, Brendan P. and {Liu}, Michael C. and {Dupuy}, Trent J. and {Cushing}, Michael C.},
        title = "{Near-infrared Spectroscopy of the Extrasolar Planet HR 8799 b}",
      journal = {\apj},
     keywords = {planetary systems, stars: individual: HR 8799, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = nov,
       volume = {723},
       number = {1},
        pages = {850-868},
          doi = {10.1088/0004-637X/723/1/850},
archivePrefix = {arXiv},
       eprint = {1008.4582},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...723..850B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Janson2010,
       author = {{Janson}, M. and {Bergfors}, C. and {Goto}, M. and {Brandner}, W. and {Lafreni{\`e}re}, D.},
        title = "{Spatially Resolved Spectroscopy of the Exoplanet HR 8799 c}",
      journal = {\apjl},
     keywords = {planetary systems, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {1},
        pages = {L35-L38},
          doi = {10.1088/2041-8205/710/1/L35},
archivePrefix = {arXiv},
       eprint = {1001.2017},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710L..35J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hinz2010,
       author = {{Hinz}, Philip M. and {Rodigas}, Timothy J. and {Kenworthy}, Matthew A. and {Sivanandam}, Suresh and {Heinze}, Aren N. and {Mamajek}, Eric E. and {Meyer}, Michael R.},
        title = "{Thermal Infrared MMTAO Observations of the HR 8799 Planetary System}",
      journal = {\apj},
     keywords = {instrumentation: adaptive optics, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jun,
       volume = {716},
       number = {1},
        pages = {417-426},
          doi = {10.1088/0004-637X/716/1/417},
archivePrefix = {arXiv},
       eprint = {1003.4986},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...716..417H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Doyon2010,
       author = {{Doyon}, R. and {Lafreni{\`e}re}, D. and {Artigau}, E. and {Malo}, L. and {Marois}, C.},
        title = "{The age of HR8799}",
    booktitle = {In the Spirit of Lyot 2010},
         year = 2010,
       editor = {{Boccaletti}, A.},
        month = oct,
        pages = {E42},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010lyot.confE..42D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Zuckerman2011,
       author = {{Zuckerman}, B. and {Rhee}, Joseph H. and {Song}, Inseok and {Bessell}, M.~S.},
        title = "{The Tucana/Horologium, Columba, AB Doradus, and Argus Associations: New Members and Dusty Debris Disks}",
      journal = {\apj},
     keywords = {circumstellar matter, stars: evolution, stars: kinematics and dynamics, stars: pre-main sequence, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = may,
       volume = {732},
       number = {2},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/732/2/61},
archivePrefix = {arXiv},
       eprint = {1104.0284},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...732...61Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Su2009,
       author = {{Su}, K.~Y.~L. and {Rieke}, G.~H. and {Stapelfeldt}, K.~R. and {Malhotra}, R. and {Bryden}, G. and {Smith}, P.~S. and {Misselt}, K.~A. and {Moro-Martin}, A. and {Williams}, J.~P.},
        title = "{The Debris Disk Around HR 8799}",
      journal = {\apj},
     keywords = {circumstellar matter, infrared: stars, planetary systems, stars: individual: HR 8799, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = nov,
       volume = {705},
       number = {1},
        pages = {314-327},
          doi = {10.1088/0004-637X/705/1/314},
archivePrefix = {arXiv},
       eprint = {0909.2687},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...705..314S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Vandal2020,
       author = {{Vandal}, Thomas and {Rameau}, Julien and {Doyon}, Ren{\'e}},
        title = "{Dynamical Mass Estimates of the {\ensuremath{\beta}} Pictoris Planetary System through Gaussian Process Stellar Activity Modeling}",
      journal = {\aj},
     keywords = {Exoplanets, Radial velocity, Gaussian Processes regression, Astrometry, Orbit determination, Delta Scuti variable stars, 498, 1332, 1930, 80, 1175, 370, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
       volume = {160},
       number = {5},
          eid = {243},
        pages = {243},
          doi = {10.3847/1538-3881/abba30},
archivePrefix = {arXiv},
       eprint = {2009.09276},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160..243V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dupuy2019,
       author = {{Dupuy}, Trent J. and {Brandt}, Timothy D. and {Kratter}, Kaitlin M. and {Bowler}, Brendan P.},
        title = "{A Model-independent Mass and Moderate Eccentricity for {\ensuremath{\beta}} Pic b}",
      journal = {\apjl},
     keywords = {astrometry, planetary systems, stars: individual: bet Pic, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jan,
       volume = {871},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.3847/2041-8213/aafb31},
archivePrefix = {arXiv},
       eprint = {1812.11530},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...871L...4D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nielsen2020,
       author = {{Nielsen}, Eric L. and {De Rosa}, Robert J. and {Wang}, Jason J. and {Sahlmann}, Johannes and {Kalas}, Paul and {Duch{\^e}ne}, Gaspard and {Rameau}, Julien and {Marley}, Mark S. and {Saumon}, Didier and {Macintosh}, Bruce and {Millar-Blanchaer}, Maxwell A. and {Nguyen}, Meiji M. and {Ammons}, S. Mark and {Bailey}, Vanessa P. and {Barman}, Travis and {Bulger}, Joanna and {Chilcote}, Jeffrey and {Cotten}, Tara and {Doyon}, Rene and {Esposito}, Thomas M. and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Gerard}, Benjamin L. and {Goodsell}, Stephen J. and {Graham}, James R. and {Greenbaum}, Alexandra Z. and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Konopacky}, Quinn and {Larkin}, James E. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marois}, Christian and {Metchev}, Stanimir and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall and {Poyneer}, Lisa and {Pueyo}, Laurent and {Rajan}, Abhijith and {Rantakyr{\"o}}, Fredrik T. and {Ruffio}, Jean-Baptiste and {Savransky}, Dmitry and {Schneider}, Adam C. and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Ward-Duong}, Kimberly and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{The Gemini Planet Imager Exoplanet Survey: Dynamical Mass of the Exoplanet {\ensuremath{\beta}} Pictoris b from Combined Direct Imaging and Astrometry}",
      journal = {\aj},
     keywords = {Astrometry, Direct imaging, Exoplanets, Coronagraphic imaging, Orbit determination, 80, 387, 498, 313, 1175, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = feb,
       volume = {159},
       number = {2},
          eid = {71},
        pages = {71},
          doi = {10.3847/1538-3881/ab5b92},
archivePrefix = {arXiv},
       eprint = {1911.11273},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159...71N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kervella2019,
       author = {{Kervella}, Pierre and {Arenou}, Fr{\'e}d{\'e}ric and {Mignard}, Fran{\c{c}}ois and {Th{\'e}venin}, Fr{\'e}d{\'e}ric},
        title = "{Stellar and substellar companions of nearby stars from Gaia DR2. Binarity from proper motion anomaly}",
      journal = {\aap},
     keywords = {astrometry, proper motions, binaries: general, planetary systems, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {623},
          eid = {A72},
        pages = {A72},
          doi = {10.1051/0004-6361/201834371},
archivePrefix = {arXiv},
       eprint = {1811.08902},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623A..72K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lagrange2012,
       author = {{Lagrange}, A. -M. and {De Bondt}, K. and {Meunier}, N. and {Sterzik}, M. and {Beust}, H. and {Galland}, F.},
        title = "{Constraints on planets around {\ensuremath{\beta}} Pic with Harps radial velocity data}",
      journal = {\aap},
     keywords = {planets and satellites: detection, planets and satellites: individual:{\ensuremath{\beta}}Pic, techniques: radial velocities, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = jun,
       volume = {542},
          eid = {A18},
        pages = {A18},
          doi = {10.1051/0004-6361/201117985},
archivePrefix = {arXiv},
       eprint = {1202.2579},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...542A..18L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Brandt2021,
       author = {{Brandt}, G. Mirek and {Brandt}, Timothy D. and {Dupuy}, Trent J. and {Li}, Yiting and {Michalik}, Daniel},
        title = "{Precise Dynamical Masses and Orbital Fits for {\ensuremath{\beta}} Pic b and {\ensuremath{\beta}} Pic c}",
      journal = {\aj},
     keywords = {Exoplanet astronomy, Exoplanet dynamics, Exoplanet systems, Exoplanet formation, Radial velocity, Pulsating variable stars, Brown dwarfs, Exoplanet evolution, 486, 490, 484, 492, 1332, 1307, 185, 491, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = apr,
       volume = {161},
       number = {4},
          eid = {179},
        pages = {179},
          doi = {10.3847/1538-3881/abdc2e},
archivePrefix = {arXiv},
       eprint = {2011.06215},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..179B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{vanLeeuwen2007,
       author = {{van Leeuwen}, F.},
        title = "{Validation of the new Hipparcos reduction}",
      journal = {\aap},
     keywords = {space vehicles: instruments, methods: data analysis, catalogs, astrometry, instrumentation: miscellaneous, Astrophysics},
         year = 2007,
        month = nov,
       volume = {474},
       number = {2},
        pages = {653-664},
          doi = {10.1051/0004-6361:20078357},
archivePrefix = {arXiv},
       eprint = {0708.1752},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...474..653V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gray2006,
       author = {{Gray}, R.~O. and {Corbally}, C.~J. and {Garrison}, R.~F. and {McFadden}, M.~T. and {Bubar}, E.~J. and {McGahee}, C.~E. and {O'Donoghue}, A.~A. and {Knox}, E.~R.},
        title = "{Contributions to the Nearby Stars (NStars) Project: Spectroscopy of Stars Earlier than M0 within 40 pc-The Southern Sample}",
      journal = {\aj},
     keywords = {Galaxy: Solar Neighborhood, Stars: Abundances, Stars: Activity, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Statistics, Astrophysics},
         year = 2006,
        month = jul,
       volume = {132},
       number = {1},
        pages = {161-170},
          doi = {10.1086/504637},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603770},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....132..161G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bell2015,
       author = {{Bell}, Cameron P.~M. and {Mamajek}, Eric E. and {Naylor}, Tim},
        title = "{A self-consistent, absolute isochronal age scale for young moving groups in the solar neighbourhood}",
      journal = {\mnras},
     keywords = {techniques: photometric, stars: evolution, Hertzsprung-Russell and colour-magnitude diagrams, stars: pre-main-sequence, open clusters and associations: general, solar neighbourhood, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = nov,
       volume = {454},
       number = {1},
        pages = {593-614},
          doi = {10.1093/mnras/stv1981},
archivePrefix = {arXiv},
       eprint = {1508.05955},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.454..593B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lagrange2020,
       author = {{Lagrange}, A.~M. and {Rubini}, P. and {Nowak}, M. and {Lacour}, S. and {Grandjean}, A. and {Boccaletti}, A. and {Langlois}, M. and {Delorme}, P. and {Gratton}, R. and {Wang}, J. and {Flasseur}, O. and {Galicher}, R. and {Kral}, Q. and {Meunier}, N. and {Beust}, H. and {Babusiaux}, C. and {Le Coroller}, H. and {Thebault}, P. and {Kervella}, P. and {Zurlo}, A. and {Maire}, A. -L. and {Wahhaj}, Z. and {Amorim}, A. and {Asensio-Torres}, R. and {Benisty}, M. and {Berger}, J.~P. and {Bonnefoy}, M. and {Brandner}, W. and {Cantalloube}, F. and {Charnay}, B. and {Chauvin}, G. and {Choquet}, E. and {Cl{\'e}net}, Y. and {Christiaens}, V. and {Coud{\'e} Du Foresto}, V. and {de Zeeuw}, P.~T. and {Desidera}, S. and {Duvert}, G. and {Eckart}, A. and {Eisenhauer}, F. and {Galland}, F. and {Gao}, F. and {Garcia}, P. and {Garcia Lopez}, R. and {Gendron}, E. and {Genzel}, R. and {Gillessen}, S. and {Girard}, J. and {Hagelberg}, J. and {Haubois}, X. and {Henning}, T. and {Heissel}, G. and {Hippler}, S. and {Horrobin}, M. and {Janson}, M. and {Kammerer}, J. and {Kenworthy}, M. and {Keppler}, M. and {Kreidberg}, L. and {Lapeyr{\`e}re}, V. and {Le Bouquin}, J. -B. and {L{\'e}na}, P. and {M{\'e}rand}, A. and {Messina}, S. and {Molli{\`e}re}, P. and {Monnier}, J.~D. and {Ott}, T. and {Otten}, G. and {Paumard}, T. and {Paladini}, C. and {Perraut}, K. and {Perrin}, G. and {Pueyo}, L. and {Pfuhl}, O. and {Rodet}, L. and {Rodriguez-Coira}, G. and {Rousset}, G. and {Samland}, M. and {Shangguan}, J. and {Schmidt}, T. and {Straub}, O. and {Straubmeier}, C. and {Stolker}, T. and {Vigan}, A. and {Vincent}, F. and {Widmann}, F. and {Woillez}, J. and {GRAVITY Collaboration}},
        title = "{Unveiling the {\ensuremath{\beta}} Pictoris system, coupling high contrast imaging, interferometric, and radial velocity data}",
      journal = {\aap},
     keywords = {techniques: high angular resolution, techniques: radial velocities, planets and satellites: detection, planets and satellites: fundamental parameters},
         year = 2020,
        month = oct,
       volume = {642},
          eid = {A18},
        pages = {A18},
          doi = {10.1051/0004-6361/202038823},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...642A..18L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Morzinski2015,
       author = {{Morzinski}, Katie M. and {Males}, Jared R. and {Skemer}, Andy J. and {Close}, Laird M. and {Hinz}, Phil M. and {Rodigas}, T.~J. and {Puglisi}, Alfio and {Esposito}, Simone and {Riccardi}, Armando and {Pinna}, Enrico and {Xompero}, Marco and {Briguglio}, Runa and {Bailey}, Vanessa P. and {Follette}, Katherine B. and {Kopon}, Derek and {Weinberger}, Alycia J. and {Wu}, Ya-Lin},
        title = "{Magellan Adaptive Optics First-light Observations of the Exoplanet {\ensuremath{\beta}} Pic b. II. 3-5 {\ensuremath{\mu}}m Direct Imaging with MagAO+Clio, and the Empirical Bolometric Luminosity of a Self-luminous Giant Planet}",
      journal = {\apj},
     keywords = {instrumentation: adaptive optics, planetary systems, planets and satellites: individual: Beta Pictoris b, stars: individual: Beta Pictoris, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = dec,
       volume = {815},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.1088/0004-637X/815/2/108},
archivePrefix = {arXiv},
       eprint = {1511.02894},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...815..108M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Chilcote2015,
       author = {{Chilcote}, Jeffrey and {Barman}, Travis and {Fitzgerald}, Michael P. and {Graham}, James R. and {Larkin}, James E. and {Macintosh}, Bruce and {Bauman}, Brian and {Burrows}, Adam S. and {Cardwell}, Andrew and {De Rosa}, Robert J. and {Dillon}, Daren and {Doyon}, Ren{\'e} and {Dunn}, Jennifer and {Erikson}, Darren and {Gavel}, Donald and {Goodsell}, Stephen J. and {Hartung}, Markus and {Hibon}, Pascale and {Ingraham}, Patrick and {Kalas}, Paul and {Konopacky}, Quinn and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marley}, Mark S. and {Marois}, Christian and {Millar-Blanchaer}, Max and {Morzinski}, Katie and {Norton}, Andrew and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall and {Poyneer}, Lisa and {Pueyo}, Laurent and {Rantakyr{\"o}}, Fredrik T. and {Sadakuni}, Naru and {Saddlemyer}, Leslie and {Savransky}, Dmitry and {Serio}, Andrew and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, R{\'e}mi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{The First H-band Spectrum of the Giant Planet {\ensuremath{\beta}} Pictoris b}",
      journal = {\apjl},
     keywords = {infrared: general, instrumentation: adaptive optics, planetary systems, stars: individual: beta Pictoris, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = jan,
       volume = {798},
       number = {1},
          eid = {L3},
        pages = {L3},
          doi = {10.1088/2041-8205/798/1/L3},
archivePrefix = {arXiv},
       eprint = {1407.4469},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798L...3C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bonnefoy2014,
       author = {{Bonnefoy}, M. and {Marleau}, G. -D. and {Galicher}, R. and {Beust}, H. and {Lagrange}, A. -M. and {Baudino}, J. -L. and {Chauvin}, G. and {Borgniet}, S. and {Meunier}, N. and {Rameau}, J. and {Boccaletti}, A. and {Cumming}, A. and {Helling}, C. and {Homeier}, D. and {Allard}, F. and {Delorme}, P.},
        title = "{Physical and orbital properties of {\ensuremath{\beta}} Pictoris b}",
      journal = {\aap},
     keywords = {techniques: photometric, techniques: spectroscopic, planetary systems, stars: individual:{\ensuremath{\beta}}Pic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = jul,
       volume = {567},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/201424041},
archivePrefix = {arXiv},
       eprint = {1407.4001},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...567L...9B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baudino2015,
       author = {{Baudino}, J. -L. and {B{\'e}zard}, B. and {Boccaletti}, A. and {Bonnefoy}, M. and {Lagrange}, A. -M. and {Galicher}, R.},
        title = "{Interpreting the photometry and spectroscopy of directly imaged planets: a new atmospheric model applied to {\ensuremath{\beta}} Pictoris b and SPHERE observations}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, planets and satellites: gaseous planets, stars: individual: beta Pictoris, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {582},
          eid = {A83},
        pages = {A83},
          doi = {10.1051/0004-6361/201526332},
archivePrefix = {arXiv},
       eprint = {1504.04876},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..83B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonnefoy2013,
       author = {{Bonnefoy}, M. and {Boccaletti}, A. and {Lagrange}, A. -M. and {Allard}, F. and {Mordasini}, C. and {Beust}, H. and {Chauvin}, G. and {Girard}, J.~H.~V. and {Homeier}, D. and {Apai}, D. and {Lacour}, S. and {Rouan}, D.},
        title = "{The near-infrared spectral energy distribution of {\ensuremath{\beta}} Pictoris b}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, techniques: photometric, planetary systems, stars: individual:{\ensuremath{\beta}}Pic b, planets and satellites: atmospheres, planets and satellites: fundamental parameters, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = jul,
       volume = {555},
          eid = {A107},
        pages = {A107},
          doi = {10.1051/0004-6361/201220838},
archivePrefix = {arXiv},
       eprint = {1302.1160},
 primaryClass = {astro-ph.EP},
       adsurl ={https://ui.adsabs.harvard.edu/abs/2013A&A...555A.107B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Currie2013,
       author = {{Currie}, Thayne and {Burrows}, Adam and {Madhusudhan}, Nikku and {Fukagawa}, Misato and {Girard}, Julien H. and {Dawson}, Rebekah and {Murray-Clay}, Ruth and {Kenyon}, Scott and {Kuchner}, Marc and {Matsumura}, Soko and {Jayawardhana}, Ray and {Chambers}, John and {Bromley}, Ben},
        title = "{A Combined Very Large Telescope and Gemini Study of the Atmosphere of the Directly Imaged Planet, {\ensuremath{\beta}} Pictoris b}",
      journal = {\apj},
     keywords = {planetary systems, stars: early-type, stars: individual: beta Pictoris, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {776},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.1088/0004-637X/776/1/15},
archivePrefix = {arXiv},
       eprint = {1306.0610},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...776...15C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018Snellen&Brown,
       author = {{Snellen}, I.~A.~G. and {Brown}, A.~G.~A.},
        title = "{The mass of the young planet Beta Pictoris b through the astrometric motion of its host star}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = aug,
       volume = {2},
        pages = {883-886},
          doi = {10.1038/s41550-018-0561-6},
archivePrefix = {arXiv},
       eprint = {1808.06257},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..883S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lagrange2010,
       author = {{Lagrange}, A. -M. and {Bonnefoy}, M. and {Chauvin}, G. and {Apai}, D. and {Ehrenreich}, D. and {Boccaletti}, A. and {Gratadour}, D. and {Rouan}, D. and {Mouillet}, D. and {Lacour}, S. and {Kasper}, M.},
        title = "{A Giant Planet Imaged in the Disk of the Young Star {\ensuremath{\beta}} Pictoris}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jul,
       volume = {329},
       number = {5987},
        pages = {57},
          doi = {10.1126/science.1187187},
archivePrefix = {arXiv},
       eprint = {1006.3314},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Sci...329...57L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{GravityCollaboration2020,
       author = {{GRAVITY Collaboration} and {Nowak}, M. and {Lacour}, S. and {Molli{\`e}re}, P. and {Wang}, J. and {Charnay}, B. and {van Dishoeck}, E.~F. and {Abuter}, R. and {Amorim}, A. and {Berger}, J.~P. and {Beust}, H. and {Bonnefoy}, M. and {Bonnet}, H. and {Brandner}, W. and {Buron}, A. and {Cantalloube}, F. and {Collin}, C. and {Chapron}, F. and {Cl{\'e}net}, Y. and {Coud{\'e} Du Foresto}, V. and {de Zeeuw}, P.~T. and {Dembet}, R. and {Dexter}, J. and {Duvert}, G. and {Eckart}, A. and {Eisenhauer}, F. and {F{\"o}rster Schreiber}, N.~M. and {F{\'e}dou}, P. and {Garcia Lopez}, R. and {Gao}, F. and {Gendron}, E. and {Genzel}, R. and {Gillessen}, S. and {Hau{\ss}mann}, F. and {Henning}, T. and {Hippler}, S. and {Hubert}, Z. and {Jocou}, L. and {Kervella}, P. and {Lagrange}, A. -M. and {Lapeyr{\`e}re}, V. and {Le Bouquin}, J. -B. and {L{\'e}na}, P. and {Maire}, A. -L. and {Ott}, T. and {Paumard}, T. and {Paladini}, C. and {Perraut}, K. and {Perrin}, G. and {Pueyo}, L. and {Pfuhl}, O. and {Rabien}, S. and {Rau}, C. and {Rodr{\'\i}guez-Coira}, G. and {Rousset}, G. and {Scheithauer}, S. and {Shangguan}, J. and {Straub}, O. and {Straubmeier}, C. and {Sturm}, E. and {Tacconi}, L.~J. and {Vincent}, F. and {Widmann}, F. and {Wieprecht}, E. and {Wiezorrek}, E. and {Woillez}, J. and {Yazici}, S. and {Ziegler}, D.},
        title = "{Peering into the formation history of {\ensuremath{\beta}} Pictoris b with VLTI/GRAVITY long-baseline interferometry}",
      journal = {\aap},
     keywords = {planets and satellites: formation, planets and satellites: atmospheres, techniques: interferometric, stars: individual: {\ensuremath{\beta}} Pictoris, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jan,
       volume = {633},
          eid = {A110},
        pages = {A110},
          doi = {10.1051/0004-6361/201936898},
archivePrefix = {arXiv},
       eprint = {1912.04651},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...633A.110G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zuckerman2006,
       author = {{Zuckerman}, B. and {Bessell}, M.~S. and {Song}, Inseok and {Kim}, S.},
        title = "{The Carina-Near Moving Group}",
      journal = {\apjl},
     keywords = {open clusters and associations: individual (HR 3070 moving group), Stars: Evolution, Stars: Kinematics, Stars: Pre-Main-Sequence, Astrophysics},
         year = 2006,
        month = oct,
       volume = {649},
       number = {2},
        pages = {L115-L118},
          doi = {10.1086/508060},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609041},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...649L.115Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Yang2016,
       author = {{Yang}, Hao and {Apai}, D{\'a}niel and {Marley}, Mark S. and {Karalidi}, Theodora and {Flateau}, Davin and {Showman}, Adam P. and {Metchev}, Stanimir and {Buenzli}, Esther and {Radigan}, Jacqueline and {Artigau}, {\'E}tienne and {Lowrance}, Patrick J. and {Burgasser}, Adam J.},
        title = "{Extrasolar Storms: Pressure-dependent Changes in Light-curve Phase in Brown Dwarfs from Simultaneous HST and Spitzer Observations}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, stars: atmospheres, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = jul,
       volume = {826},
       number = {1},
          eid = {8},
        pages = {8},
          doi = {10.3847/0004-637X/826/1/8},
archivePrefix = {arXiv},
       eprint = {1605.02708},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826....8Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Artigau2006,
       author = {{Artigau}, {\'E}tienne and {Doyon}, Ren{\'e} and {Lafreni{\`e}re}, David and {Nadeau}, Daniel and {Robert}, Jasmin and {Albert}, Lo{\"\i}c},
        title = "{Discovery of the Brightest T Dwarf in the Northern Hemisphere}",
      journal = {\apjl},
     keywords = {stars: individual (SIMP J013656.5+093347), Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = nov,
       volume = {651},
       number = {1},
        pages = {L57-L60},
          doi = {10.1086/509146},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609419},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...651L..57A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Metchev2013,
       author = {{Metchev}, S. and {Apai}, D. and {Radigan}, J. and {Artigau}, {\'E}. and {Heinze}, A. and {Helling}, C. and {Homeier}, D. and {Littlefair}, S. and {Morley}, C. and {Skemer}, A. and {Stark}, C.},
        title = "{Clouds in brown dwarfs and giant planets}",
      journal = {Astronomische Nachrichten},
     keywords = {stars: low-mass, brown dwarfs, stars: rotation, stars: variables: general, planetary systems},
         year = 2013,
        month = feb,
       volume = {334},
       number = {1-2},
        pages = {40-43},
          doi = {10.1002/asna.201211776},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013AN....334...40M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Croll2016,
       author = {{Croll}, Bryce and {Muirhead}, Philip S. and {Lichtman}, Jack and {Han}, Eunkyu and {Dalba}, Paul A. and {Radigan}, Jacqueline},
        title = "{Long-term, Multiwavelength Light Curves of Ultra-Cool Dwarfs: II. The evolving Light Curves of the T2.5 SIMP 0136 \& the Uncorrelated Light Curves of the M9 TVLM 513}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = sep,
          eid = {arXiv:1609.03587},
        pages = {arXiv:1609.03587},
archivePrefix = {arXiv},
       eprint = {1609.03587},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv160903587C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Artigau2009,
       author = {{Artigau}, {\'E}tienne and {Bouchard}, Sandie and {Doyon}, Ren{\'e} and {Lafreni{\`e}re}, David},
        title = "{Photometric Variability of the T2.5 Brown Dwarf SIMP J013656.5+093347: Evidence for Evolving Weather Patterns}",
      journal = {\apj},
     keywords = {stars: individual: SIMP J013656.5+093347, stars: low-mass, brown dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = aug,
       volume = {701},
       number = {2},
        pages = {1534-1539},
          doi = {10.1088/0004-637X/701/2/1534},
archivePrefix = {arXiv},
       eprint = {0906.3514},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...701.1534A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gizis2015,
       author = {{Gizis}, John E. and {Dettman}, Kyle G. and {Burgasser}, Adam J. and {Camnasio}, Sara and {Alam}, Munazza and {Filippazzo}, Joseph C. and {Cruz}, Kelle L. and {Metchev}, Stanimir and {Berger}, Edo and {Williams}, Peter K.~G.},
        title = "{Kepler Monitoring of an L Dwarf. II. Clouds with Multi-year Lifetimes}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: activity, stars: atmospheres, stars: individual: WISEP J190648.47+401106.8, starspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = nov,
       volume = {813},
       number = {2},
          eid = {104},
        pages = {104},
          doi = {10.1088/0004-637X/813/2/104},
archivePrefix = {arXiv},
       eprint = {1509.07186},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...813..104G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Mohanty&Basri2003,
       author = {{Mohanty}, Subhanjoy and {Basri}, Gibor},
        title = "{Rotation and Activity in Mid-M to L Field Dwarfs}",
      journal = {\apj},
     keywords = {Stars: Activity, Stars: Low-Mass, Brown Dwarfs, Stars: Rotation, Astrophysics},
         year = 2003,
        month = jan,
       volume = {583},
       number = {1},
        pages = {451-472},
          doi = {10.1086/345097},
archivePrefix = {arXiv},
       eprint = {astro-ph/0201455},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...583..451M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Reiners&Basri2008,
       author = {{Reiners}, A. and {Basri}, G.},
        title = "{Chromospheric Activity, Rotation, and Rotational Braking in M and L Dwarfs}",
      journal = {\apj},
     keywords = {stars: activity, stars: flare, stars: late-type, stars: low-mass, brown dwarfs, stars: rotation, Astrophysics},
         year = 2008,
        month = sep,
       volume = {684},
       number = {2},
        pages = {1390-1403},
          doi = {10.1086/590073},
archivePrefix = {arXiv},
       eprint = {0805.1059},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...684.1390R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Martin1999,
       author = {{Mart{\'\i}n}, Eduardo L. and {Delfosse}, Xavier and {Basri}, Gibor and {Goldman}, Bertrand and {Forveille}, Thierry and {Zapatero Osorio}, Maria Rosa},
        title = "{Spectroscopic Classification of Late-M and L Field Dwarfs}",
      journal = {\aj},
     keywords = {STARS: EVOLUTION, STARS: FUNDAMENTAL PARAMETERS, STARS: LOW-MASS, BROWN DWARFS},
         year = 1999,
        month = nov,
       volume = {118},
       number = {5},
        pages = {2466-2482},
          doi = {10.1086/301107},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999AJ....118.2466M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dupuy2023,
       author = {{Dupuy}, Trent J. and {Liu}, Michael C. and {Evans}, Elise L. and {Best}, William M.~J. and {Pearce}, Logan A. and {Sanghi}, Aniket and {Phillips}, Mark W. and {Bardalez Gagliuffi}, Daniella C.},
        title = "{On the masses, age, and architecture of the VHS J1256-1257AB b system}",
      journal = {\mnras},
     keywords = {astrometry, planetary systems, binaries: visual, brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2023,
        month = feb,
       volume = {519},
       number = {2},
        pages = {1688-1694},
          doi = {10.1093/mnras/stac3557},
archivePrefix = {arXiv},
       eprint = {2208.08448},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.519.1688D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@INPROCEEDINGS{Allard2011,
       author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B.},
        title = "{Model Atmospheres From Very Low Mass Stars to Brown Dwarfs}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {16th Cambridge Workshop on Cool Stars, Stellar Systems, and the Sun},
         year = 2011,
       editor = {{Johns-Krull}, Christopher and {Browning}, Matthew K. and {West}, Andrew A.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {448},
        month = dec,
        pages = {91},
archivePrefix = {arXiv},
       eprint = {1011.5405},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ASPC..448...91A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bryan2018,
       author = {{Bryan}, Marta L. and {Benneke}, Bj{\"o}rn and {Knutson}, Heather A. and {Batygin}, Konstantin and {Bowler}, Brendan P.},
        title = "{Constraints on the spin evolution of young planetary-mass companions}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = dec,
       volume = {2},
        pages = {138-144},
          doi = {10.1038/s41550-017-0325-8},
archivePrefix = {arXiv},
       eprint = {1712.00457},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..138B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miles2022,
       author = {{Miles}, Brittany E. and {Biller}, Beth A. and {Patapis}, Polychronis and {Worthen}, Kadin and {Rickman}, Emily and {Hoch}, Kielan K.~W. and {Skemer}, Andrew and {Perrin}, Marshall D. and {Chen}, Christine H. and {Mukherjee}, Sagnick and {Morley}, Caroline V. and {Moran}, Sarah E. and {Bonnefoy}, Mickael and {Petrus}, Simon and {Carter}, Aarynn L. and {Choquet}, Elodie and {Hinkley}, Sasha and {Ward-Duong}, Kimberly and {Leisenring}, Jarron M. and {Millar-Blanchaer}, Maxwell A. and {Pueyo}, Laurent and {Ray}, Shrishmoy and {Stapelfeldt}, Karl R. and {Stone}, Jordan M. and {Wang}, Jason J. and {Absil}, Olivier and {Balmer}, William O. and {Boccaletti}, Anthony and {Bonavita}, Mariangela and {Booth}, Mark and {Bowler}, Brendan P. and {Chauvin}, Gael and {Christiaens}, Valentin and {Currie}, Thayne and {Danielski}, Camilla and {Fortney}, Jonathan J. and {Girard}, Julien H. and {Greenbaum}, Alexandra Z. and {Henning}, Thomas and {Hines}, Dean C. and {Janson}, Markus and {Kalas}, Paul and {Kammerer}, Jens and {Kenworthy}, Matthew A. and {Kervella}, Pierre and {Lagage}, Pierre-Olivier and {Lew}, Ben W.~P. and {Liu}, Michael C. and {Macintosh}, Bruce and {Marino}, Sebastian and {Marley}, Mark S. and {Marois}, Christian and {Matthews}, Elisabeth C. and {Matthews}, Brenda C. and {Mawet}, Dimitri and {McElwain}, Michael W. and {Metchev}, Stanimir and {Meyer}, Michael R. and {Molliere}, Paul and {Pantin}, Eric and {Rebollido}, Andreas Quirrenbachm Isabel and {Ren}, Bin B. and {Vasist}, Malavika and {Wyatt}, Mark C. and {Zhou}, Yifan and {Briesemeister}, Zackery W. and {Bryan}, Marta L. and {Calissendorff}, Per and {Catalloube}, Faustine and {Cugno}, Gabriele and {De Furio}, Matthew and {Dupuy}, Trent J. and {Factor}, Samuel M. and {Faherty}, Jacqueline K. and {Fitzgerald}, Michael P. and {Franson}, Kyle and {Gonzales}, Eileen C. and {Hood}, Callie E. and {Howe}, Alex R. and {Kraus}, Adam L. and {Kuzuhara}, Masayuki and {Lawson}, Kellen and {Lazzoni}, Cecilia and {Liu}, Pengyu and {Llop-Sayson}, Jorge and {Lloyd}, James P. and {Martinez}, Raquel A. and {Mazoyer}, Johan and {Quanz}, Sascha P. and {Adams Redai}, Jea and {Samland}, Matthias and {Schlieder}, Joshua E. and {Tamura}, Motohide and {Tan}, Xianyu and {Uyama}, Taichi and {Vigan}, Arthur and {Vos}, Johanna M. and {Wagner}, Kevin and {Wolff}, Schuyler G. and {Ygouf}, Marie and {Zhang}, Keming and {Zhang}, Zhoujian},
        title = "{The JWST Early Release Science Program for Direct Observations of Exoplanetary Systems II: A 1 to 20 Micron Spectrum of the Planetary-Mass Companion VHS 1256-1257 b}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = sep,
          eid = {arXiv:2209.00620},
        pages = {arXiv:2209.00620},
archivePrefix = {arXiv},
       eprint = {2209.00620},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220900620M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dupuy2020,
       author = {{Dupuy}, Trent J. and {Liu}, Michael C. and {Magnier}, Eugene A. and {Best}, William M.~J. and {Baraffe}, Isabelle and {Chabrier}, Gilles and {Forveille}, Thierry and {Metchev}, Stanimir A. and {Tremblin}, Pascal},
        title = "{The Parallax of VHS J1256-1257 from CFHT and Pan-STARRS-1}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Brown dwarfs, 185, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = apr,
       volume = {4},
       number = {4},
          eid = {54},
        pages = {54},
          doi = {10.3847/2515-5172/ab8942},
archivePrefix = {arXiv},
       eprint = {2004.05180},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020RNAAS...4...54D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Petrus2022,
       author = {{Petrus}, Simon and {Chauvin}, Ga{\"e}l and {Bonnefoy}, Micka{\"e}l and {Tremblin}, Pascal and {Charnay}, Benjamin and {Delorme}, Philippe and {Marleau}, Gabriel-Dominique and {Bayo}, Amelia and {Manjavacas}, Elena and {Lagrange}, Anne-Marie and {Molli{\`e}re}, Paul and {Palma-Bifani}, Paulina and {Biller James-S. Jenkins}, Beth},
        title = "{X-SHYNE: X-shooter spectra of young exoplanet analogs. I. A medium-resolution 0.65-2.5$\mathrm{\mu m}$ one-shot spectrum of VHS\textbackslash,1256-1257 b}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jul,
          eid = {arXiv:2207.06622},
        pages = {arXiv:2207.06622},
archivePrefix = {arXiv},
       eprint = {2207.06622},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220706622P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gauza2015,
       author = {{Gauza}, Bartosz and {B{\'e}jar}, Victor J.~S. and {P{\'e}rez-Garrido}, Antonio and {Zapatero Osorio}, Maria Rosa and {Lodieu}, Nicolas and {Rebolo}, Rafael and {Pall{\'e}}, Enric and {Nowak}, Grzegorz},
        title = "{Discovery of a Young Planetary Mass Companion to the Nearby M Dwarf VHS J125601.92-125723.9}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: planetary systems, stars: imaging, stars: individual: VHS J125601.92-125723.9, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = may,
       volume = {804},
       number = {2},
          eid = {96},
        pages = {96},
          doi = {10.1088/0004-637X/804/2/96},
archivePrefix = {arXiv},
       eprint = {1505.00806},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...804...96G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@Article{Matplotlib,
  Author    = {Hunter, J. D.},
  Title     = {Matplotlib: A 2D graphics environment},
  Journal   = {Computing in Science \& Engineering},
  Volume    = {9},
  Number    = {3},
  Pages     = {90--95},
  abstract  = {Matplotlib is a 2D graphics package used for Python for
  application development, interactive scripting, and publication-quality
  image generation across user interfaces and operating systems.},
  publisher = {IEEE COMPUTER SOC},
  doi       = {10.1109/MCSE.2007.55},
  year      = 2007
}

@inproceedings{Pandas, 
  title={Data structures for statistical computing in python}, 
  author={McKinney, Wes and others}, 
  booktitle={Proceedings of the 9th Python in Science Conference}, 
  volume={445}, 
  pages={51--56}, 
  year={2010}, 
  organization={Austin, TX} 
}

@article{astropy:2013,
Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
Adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..33A},
Archiveprefix = {arXiv},
Author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and {Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and {Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and {Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and {Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and {Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and {Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and {Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and {Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and {Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and {Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and {Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and {Servillat}, M. and {Streicher}, O.},
Doi = {10.1051/0004-6361/201322068},
Eid = {A33},
Eprint = {1307.6212},
Journal = {\aap},
Keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
Month = oct,
Pages = {A33},
Primaryclass = {astro-ph.IM},
Title = {{Astropy: A community Python package for astronomy}},
Volume = 558,
Year = 2013,
Bdsk-Url-1 = {https://dx.doi.org/10.1051/0004-6361/201322068}}

@ARTICLE{astropy:2018,
       author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and
         {Sip{\H{o}}cz}, B.~M. and {G{\"u}nther}, H.~M. and {Lim}, P.~L. and
         {Crawford}, S.~M. and {Conseil}, S. and {Shupe}, D.~L. and
         {Craig}, M.~W. and {Dencheva}, N. and {Ginsburg}, A. and {Vand
        erPlas}, J.~T. and {Bradley}, L.~D. and {P{\'e}rez-Su{\'a}rez}, D. and
         {de Val-Borro}, M. and {Aldcroft}, T.~L. and {Cruz}, K.~L. and
         {Robitaille}, T.~P. and {Tollerud}, E.~J. and {Ardelean}, C. and
         {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and {Bakanov}, A.~V. and
         {Bamford}, S.~P. and {Barentsen}, G. and {Barmby}, P. and
         {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and {Boquien}, M. and
         {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
         {Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
         {Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'\i}guez}, J.~L. and
         {Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
         {Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
         {Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
         {Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
         {Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and
         {Garrison}, L.~H. and {Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and
         {Gommers}, R. and {Greco}, J.~P. and {Greenfield}, P. and
         {Groener}, A.~M. and {Grollier}, F. and {Hagen}, A. and {Hirst}, P. and
         {Homeier}, D. and {Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and
         {Hunkeler}, J.~S. and {Ivezi{\'c}}, {\v{Z}}. and {Jain}, A. and
         {Jenness}, T. and {Kanarek}, G. and {Kendrew}, S. and {Kern}, N.~S. and
         {Kerzendorf}, W.~E. and {Khvalko}, A. and {King}, J. and {Kirkby}, D. and
         {Kulkarni}, A.~M. and {Kumar}, A. and {Lee}, A. and {Lenz}, D. and
         {Littlefair}, S.~P. and {Ma}, Z. and {Macleod}, D.~M. and
         {Mastropietro}, M. and {McCully}, C. and {Montagnac}, S. and
         {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and {Muna}, D. and
         {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
         {Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
         {Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
         {Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
         {Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and
         {Sakurikar}, P. and {Seifert}, M. and {Sherbert}, L.~E. and
         {Sherwood-Taylor}, H. and {Shih}, A.~Y. and {Sick}, J. and
         {Silbiger}, M.~T. and {Singanamalla}, S. and {Singer}, L.~P. and
         {Sladen}, P.~H. and {Sooley}, K.~A. and {Sornarajah}, S. and
         {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
         {Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
         {van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
         {Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
         {Zabalza}, V. and {Astropy Contributors}},
        title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
      journal = {\aj},
     keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = sep,
       volume = {156},
       number = {3},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-3881/aabc4f},
archivePrefix = {arXiv},
       eprint = {1801.02634},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hoch2022,
       author = {{Hoch}, Kielan K.~W. and {Konopacky}, Quinn M. and {Barman}, Travis S. and {Theissen}, Christopher A. and {Brock}, Laci and {Perrin}, Marshall D. and {Ruffio}, Jean-Baptiste and {Macintosh}, Bruce and {Marois}, Christian},
        title = "{Moderate-resolution K-band Spectroscopy of the Substellar Companion VHS 1256 b}",
      journal = {\aj},
     keywords = {Direct imaging, Exoplanet atmospheres, High resolution spectroscopy, Exoplanet formation, Brown dwarfs, 387, 487, 2096, 492, 185, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = oct,
       volume = {164},
       number = {4},
          eid = {155},
        pages = {155},
          doi = {10.3847/1538-3881/ac84d4},
archivePrefix = {arXiv},
       eprint = {2207.03819},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....164..155H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skrutskie2006,
       author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
        title = "{The Two Micron All Sky Survey (2MASS)}",
      journal = {\aj},
     keywords = {Catalogs, Infrared: General, Surveys},
         year = 2006,
        month = feb,
       volume = {131},
       number = {2},
        pages = {1163-1183},
          doi = {10.1086/498708},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....131.1163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Rich2016,
       author = {{Rich}, Evan A. and {Currie}, Thayne and {Wisniewski}, John P. and {Hashimoto}, Jun and {Brandt}, Timothy D. and {Carson}, Joseph C. and {Kuzuhara}, Masayuki and {Uyama}, Taichi},
        title = "{Thermal Infrared Imaging and Atmospheric Modeling of VHS J125601.92-125723.9 b: Evidence for Moderately Thick Clouds and Equilibrium Carbon Chemistry in a Hierarchical Triple System}",
      journal = {\apj},
     keywords = {binaries: general, brown dwarfs, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {830},
       number = {2},
          eid = {114},
        pages = {114},
          doi = {10.3847/0004-637X/830/2/114},
archivePrefix = {arXiv},
       eprint = {1607.06007},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...830..114R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@ARTICLE{Cutri2014,
    author = {{Cutri}, R. ~M.},
    title = "{VizieR Online Data Catalog}",
    journal = {VizieR Online Data Catalog},
    year = 2014,
    volume = {2328}
    }


@ARTICLE{Lawrence2012,
       author = {{Lawrence}, A. and {Warren}, S.~J. and {Almaini}, O. and {Edge}, A.~C. and {Hambly}, N.~C. and {Jameson}, R.~F. and {Lucas}, P. and {Casali}, M. and {Adamson}, A. and {Dye}, S. and {Emerson}, J.~P. and {Foucaud}, S. and {Hewett}, P. and {Hirst}, P. and {Hodgkin}, S.~T. and {Irwin}, M.~J. and {Lodieu}, N. and {McMahon}, R.~G. and {Simpson}, C. and {Smail}, I. and {Mortlock}, D. and {Folger}, M.},
        title = "{VizieR Online Data Catalog: UKIDSS-DR8 LAS, GCS and DXS Surveys (Lawrence+ 2012)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Surveys, Infrared sources, Photometry: infrared},
         year = 2012,
        month = mar,
          eid = {II/314},
        pages = {II/314},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012yCat.2314....0L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Marois2010,
       author = {{Marois}, Christian and {Zuckerman}, B. and {Konopacky}, Quinn M. and {Macintosh}, Bruce and {Barman}, Travis},
        title = "{Images of a fourth planet orbiting HR 8799}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = dec,
       volume = {468},
       number = {7327},
        pages = {1080-1083},
          doi = {10.1038/nature09684},
archivePrefix = {arXiv},
       eprint = {1011.4918},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.468.1080M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marois2008,
       author = {{Marois}, Christian and {Macintosh}, Bruce and {Barman}, Travis and {Zuckerman}, B. and {Song}, Inseok and {Patience}, Jennifer and {Lafreni{\`e}re}, David and {Doyon}, Ren{\'e}},
        title = "{Direct Imaging of Multiple Planets Orbiting the Star HR 8799}",
      journal = {Science},
     keywords = {Astrophysics},
         year = 2008,
        month = nov,
       volume = {322},
       number = {5906},
        pages = {1348},
          doi = {10.1126/science.1166585},
archivePrefix = {arXiv},
       eprint = {0811.2606},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008Sci...322.1348M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skemer2012,
       author = {{Skemer}, Andrew J. and {Hinz}, Philip M. and {Esposito}, Simone and {Burrows}, Adam and {Leisenring}, Jarron and {Skrutskie}, Michael and {Desidera}, Silvano and {Mesa}, Dino and {Arcidiacono}, Carmelo and {Mannucci}, Filippo and {Rodigas}, Timothy J. and {Close}, Laird and {McCarthy}, Don and {Kulesa}, Craig and {Agapito}, Guido and {Apai}, Daniel and {Argomedo}, Javier and {Bailey}, Vanessa and {Boutsia}, Konstantina and {Briguglio}, Runa and {Brusa}, Guido and {Busoni}, Lorenzo and {Claudi}, Riccardo and {Eisner}, Joshua and {Fini}, Luca and {Follette}, Katherine B. and {Garnavich}, Peter and {Gratton}, Raffaele and {Guerra}, Juan Carlos and {Hill}, John M. and {Hoffmann}, William F. and {Jones}, Terry and {Krejny}, Megan and {Males}, Jared and {Masciadri}, Elena and {Meyer}, Michael R. and {Miller}, Douglas L. and {Morzinski}, Katie and {Nelson}, Matthew and {Pinna}, Enrico and {Puglisi}, Alfio and {Quanz}, Sascha P. and {Quiros-Pacheco}, Fernando and {Riccardi}, Armando and {Stefanini}, Paolo and {Vaitheeswaran}, Vidhya and {Wilson}, John C. and {Xompero}, Marco},
        title = "{First Light LBT AO Images of HR 8799 bcde at 1.6 and 3.3 {\ensuremath{\mu}}m: New Discrepancies between Young Planets and Old Brown Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, instrumentation: adaptive optics, planetary systems, planets and satellites: atmospheres, stars: individual: HR 8799, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2012,
        month = jul,
       volume = {753},
       number = {1},
          eid = {14},
        pages = {14},
          doi = {10.1088/0004-637X/753/1/14},
archivePrefix = {arXiv},
       eprint = {1203.2615},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...753...14S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gozdziewski2020,
       author = {{Go{\'z}dziewski}, Krzysztof and {Migaszewski}, Cezary},
        title = "{An Exact, Generalized Laplace Resonance in the HR 8799 Planetary System}",
      journal = {\apjl},
     keywords = {Exoplanet dynamics, Exoplanet systems, Exoplanet detection methods, 490, 484, 489, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = oct,
       volume = {902},
       number = {2},
          eid = {L40},
        pages = {L40},
          doi = {10.3847/2041-8213/abb881},
archivePrefix = {arXiv},
       eprint = {2009.07006},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...902L..40G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



Corinne and {Schultheis}, Mathias},
       series = {EAS Publications Series},
       volume = {57},
        month = nov,
        pages = {3-43},
          doi = {10.1051/eas/1257001},
archivePrefix = {arXiv},
       eprint = {1206.1021},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012EAS....57....3A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{Chilcote2017,
       author = {{Chilcote}, Jeffrey and {Pueyo}, Laurent and {De Rosa}, Robert J. and {Vargas}, Jeffrey and {Macintosh}, Bruce and {Bailey}, Vanessa P. and {Barman}, Travis and {Bauman}, Brian and {Bruzzone}, Sebastian and {Bulger}, Joanna and {Burrows}, Adam S. and {Cardwell}, Andrew and {Chen}, Christine H. and {Cotten}, Tara and {Dillon}, Daren and {Doyon}, Rene and {Draper}, Zachary H. and {Duch{\^e}ne}, Gaspard and {Dunn}, Jennifer and {Erikson}, Darren and {Fitzgerald}, Michael P. and {Follette}, Katherine B. and {Gavel}, Donald and {Goodsell}, Stephen J. and {Graham}, James R. and {Greenbaum}, Alexandra Z. and {Hartung}, Markus and {Hibon}, Pascale and {Hung}, Li-Wei and {Ingraham}, Patrick and {Kalas}, Paul and {Konopacky}, Quinn and {Larkin}, James E. and {Maire}, J{\'e}r{\^o}me and {Marchis}, Franck and {Marley}, Mark S. and {Marois}, Christian and {Metchev}, Stanimir and {Millar-Blanchaer}, Maxwell A. and {Morzinski}, Katie M. and {Nielsen}, Eric L. and {Norton}, Andrew and {Oppenheimer}, Rebecca and {Palmer}, David and {Patience}, Jennifer and {Perrin}, Marshall and {Poyneer}, Lisa and {Rajan}, Abhijith and {Rameau}, Julien and {Rantakyr{\"o}}, Fredrik T. and {Sadakuni}, Naru and {Saddlemyer}, Leslie and {Savransky}, Dmitry and {Schneider}, Adam C. and {Serio}, Andrew and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Soummer}, Remi and {Thomas}, Sandrine and {Wallace}, J. Kent and {Wang}, Jason J. and {Ward-Duong}, Kimberly and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{1-2.4 {\ensuremath{\mu}}m Near-IR Spectrum of the Giant Planet {\ensuremath{\beta}} Pictoris b Obtained with the Gemini Planet Imager}",
      journal = {\aj},
     keywords = {instrumentation: adaptive optics, planetary systems, stars: individual: beta Pictoris, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = apr,
       volume = {153},
       number = {4},
          eid = {182},
        pages = {182},
          doi = {10.3847/1538-3881/aa63e9},
archivePrefix = {arXiv},
       eprint = {1703.00011},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....153..182C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Burgasser2003,
       author = {{Burgasser}, Adam J. and {McElwain}, Michael W. and {Kirkpatrick}, J. Davy},
        title = "{The 2MASS Wide-Field T Dwarf Search. II. Discovery of Three T Dwarfs in the Southern Hemisphere}",
      journal = {\aj},
     keywords = {Infrared Radiation, Galaxy: Solar Neighborhood, stars: individual (2MASS J03480772-6022270), stars: individual (2MASS J05160945-0445499), stars: individual (2MASS J22282889-4310262), Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2003,
        month = nov,
       volume = {126},
       number = {5},
        pages = {2487-2494},
          doi = {10.1086/378608},
archivePrefix = {arXiv},
       eprint = {astro-ph/0307374},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003AJ....126.2487B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ZapateroOsorio2006,
       author = {{Zapatero Osorio}, M.~R. and {Mart{\'\i}n}, E.~L. and {Bouy}, H. and {Tata}, R. and {Deshpande}, R. and {Wainscoat}, R.~J.},
        title = "{Spectroscopic Rotational Velocities of Brown Dwarfs}",
      journal = {\apj},
     keywords = {stars: individual (DENIS-P J0255.0-4700), stars: individual (GL 570D), Stars: Individual: Alphanumeric: LP 944-20, stars: individual ([Pleiades] PPl 1), stars: individual (SDSS J053951.99-005902.0), stars: individual (SDSS J134646.45-003150.4), stars: individual (SDSS J162414.37+002915.6), stars: individual (SDSSp J125453.90-012247.4), stars: individual (2MASS J00361617+1821104), stars: individual (2MASS J03341218-4953322), stars: individual (2MASS J04151954-0935066), stars: individual (2MASS J05591914-1404488), stars: individual (2MASS J12171110-0311131), stars: individual (2MASS J15031961+2525196), stars: individual (2MASS J15530228+1532369AB), stars: individual (2MASS J16322911+1904407), stars: individual (2MASS J17281150+3948593AB), stars: individual (2MASS J22244381-0158521), stars: individual (vB 10), Stars: Low-Mass, Brown Dwarfs, Stars: Rotation, Astrophysics},
         year = 2006,
        month = aug,
       volume = {647},
       number = {2},
        pages = {1405-1412},
          doi = {10.1086/505484},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603194},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...647.1405Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Stephens2009,
       author = {{Stephens}, D.~C. and {Leggett}, S.~K. and {Cushing}, Michael C. and {Marley}, Mark S. and {Saumon}, D. and {Geballe}, T.~R. and {Golimowski}, David A. and {Fan}, Xiaohui and {Noll}, K.~S.},
        title = "{The 0.8-14.5 {\ensuremath{\mu}}m Spectra of Mid-L to Mid-T Dwarfs: Diagnostics of Effective Temperature, Grain Sedimentation, Gas Transport, and Surface Gravity}",
      journal = {\apj},
     keywords = {stars: individual: 2MASS J00361617+1821104 2MASS J05591914{\textendash}1404488 2MASS J08251968+2115521 2MASS J09083803+5032088 2MASS J15074769{\textendash}1627386 2MASS J22244381{\textendash}0158521 2MASS J22443167+2043433 2MASS J22541892+3123498 DENIS-P J025503.3{\textendash}470049 SDSS J000013.54+255418.6 SDSS J075840.32+324723.3 SDSS J080531.83+481233.1 SDSS J085758.44+570851.4 SDSS J105213.50+442255.6AB SDSS J111009.99+011613.0 SDSS J115553.85+ 055957.5 SDSS J120747.17+024424.8 SDSS J125453.90{\textendash}012247.5 SDSS J133148.88{\textendash}011652.5 SDSS J151643.00+305344.3 SDSS J152039.82+354619.8, stars: low-mass, brown dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = sep,
       volume = {702},
       number = {1},
        pages = {154-170},
          doi = {10.1088/0004-637X/702/1/154},
archivePrefix = {arXiv},
       eprint = {0906.2991},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...702..154S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Kirkpatrick2014,
       author = {{Kirkpatrick}, J. Davy and {Schneider}, Adam and {Fajardo-Acosta}, Sergio and {Gelino}, Christopher R. and {Mace}, Gregory N. and {Wright}, Edward L. and {Logsdon}, Sarah E. and {McLean}, Ian S. and {Cushing}, Michael C. and {Skrutskie}, Michael F. and {Eisenhardt}, Peter R. and {Stern}, Daniel and {Balokovi{\'c}}, Mislav and {Burgasser}, Adam J. and {Faherty}, Jacqueline K. and {Lansbury}, George B. and {Rich}, J.~A. and {Skrzypek}, Nathalie and {Fowler}, John W. and {Cutri}, Roc M. and {Masci}, Frank J. and {Conrow}, Tim and {Grillmair}, Carl J. and {McCallon}, Howard L. and {Beichman}, Charles A. and {Marsh}, Kenneth A.},
        title = "{The AllWISE Motion Survey and the Quest for Cold Subdwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, catalogs, solar neighborhood, stars: fundamental parameters, stars: low-mass, subdwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = mar,
       volume = {783},
       number = {2},
          eid = {122},
        pages = {122},
          doi = {10.1088/0004-637X/783/2/122},
archivePrefix = {arXiv},
       eprint = {1402.0661},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...783..122K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lawrence2007,
       author = {{Lawrence}, A. and {Warren}, S.~J. and {Almaini}, O. and {Edge}, A.~C. and {Hambly}, N.~C. and {Jameson}, R.~F. and {Lucas}, P. and {Casali}, M. and {Adamson}, A. and {Dye}, S. and {Emerson}, J.~P. and {Foucaud}, S. and {Hewett}, P. and {Hirst}, P. and {Hodgkin}, S.~T. and {Irwin}, M.~J. and {Lodieu}, N. and {McMahon}, R.~G. and {Simpson}, C. and {Smail}, I. and {Mortlock}, D. and {Folger}, M.},
        title = "{The UKIRT Infrared Deep Sky Survey (UKIDSS)}",
      journal = {\mnras},
     keywords = {surveys, infrared: general, Astrophysics},
         year = 2007,
        month = aug,
       volume = {379},
       number = {4},
        pages = {1599-1617},
          doi = {10.1111/j.1365-2966.2007.12040.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0604426},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.379.1599L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\textbf{}

@ARTICLE{Skrutskie2006,
       author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
        title = "{The Two Micron All Sky Survey (2MASS)}",
      journal = {\aj},
     keywords = {Catalogs, Infrared: General, Surveys},
         year = 2006,
        month = feb,
       volume = {131},
       number = {2},
        pages = {1163-1183},
          doi = {10.1086/498708},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....131.1163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gagne2017,
       author = {{Gagn{\'e}}, Jonathan and {Faherty}, Jacqueline K. and {Burgasser}, Adam J. and {Artigau}, {\'E}tienne and {Bouchard}, Sandie and {Albert}, Lo{\"\i}c and {Lafreni{\`e}re}, David and {Doyon}, Ren{\'e} and {Bardalez Gagliuffi}, Daniella C.},
        title = "{SIMP J013656.5+093347 Is Likely a Planetary-mass Object in the Carina-Near Moving Group}",
      journal = {\apjl},
     keywords = {brown dwarfs, planets and satellites: atmospheres, stars: individual: SIMP J013656.5+093347, stars: kinematics and dynamics, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = may,
       volume = {841},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.3847/2041-8213/aa70e2},
archivePrefix = {arXiv},
       eprint = {1705.01625},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...841L...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Burgasser2010,
       author = {{Burgasser}, Adam J. and {Cruz}, Kelle L. and {Cushing}, Michael and {Gelino}, Christopher R. and {Looper}, Dagny L. and {Faherty}, Jacqueline K. and {Kirkpatrick}, J. Davy and {Reid}, I. Neill},
        title = "{SpeX Spectroscopy of Unresolved Very Low Mass Binaries. I. Identification of 17 Candidate Binaries Straddling the L Dwarf/T Dwarf Transition}",
      journal = {\apj},
     keywords = {binaries: general, brown dwarfs, stars: fundamental parameters, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {2},
        pages = {1142-1169},
          doi = {10.1088/0004-637X/710/2/1142},
archivePrefix = {arXiv},
       eprint = {0912.3808},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710.1142B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Cutri2003,
       author = {{Cutri}, R.~M. and {Skrutskie}, M.~F. and {van Dyk}, S. and {Beichman}, C.~A. and {Carpenter}, J.~M. and {Chester}, T. and {Cambresy}, L. and {Evans}, T. and {Fowler}, J. and {Gizis}, J. and {Howard}, E. and {Huchra}, J. and {Jarrett}, T. and {Kopan}, E.~L. and {Kirkpatrick}, J.~D. and {Light}, R.~M. and {Marsh}, K.~A. and {McCallon}, H. and {Schneider}, S. and {Stiening}, R. and {Sykes}, M. and {Weinberg}, M. and {Wheaton}, W.~A. and {Wheelock}, S. and {Zacarias}, N.},
        title = "{VizieR Online Data Catalog: 2MASS All-Sky Catalog of Point Sources (Cutri+ 2003)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Infrared sources, Photometry: infrared, Surveys},
         year = 2003,
        month = jun,
          eid = {II/246},
        pages = {II/246},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003yCat.2246....0C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Barnes2014,
       author = {{Barnes}, J.~R. and {Jenkins}, J.~S. and {Jones}, H.~R.~A. and {Jeffers}, S.~V. and {Rojo}, P. and {Arriagada}, P. and {Jord{\'a}n}, A. and {Minniti}, D. and {Tuomi}, M. and {Pinfield}, D. and {Anglada-Escud{\'e}}, G.},
        title = "{Precision radial velocities of 15 M5-M9 dwarfs}",
      journal = {\mnras},
     keywords = {techniques: radial velocities, planets and satellites: detection, stars: activity, stars: atmospheres, stars: low-mass, planetary systems, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = apr,
       volume = {439},
       number = {3},
        pages = {3094-3113},
          doi = {10.1093/mnras/stu172},
archivePrefix = {arXiv},
       eprint = {1401.5350},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.439.3094B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Costa2006,
       author = {{Costa}, Edgardo and {M{\'e}ndez}, Ren{\'e} A. and {Jao}, W. -C. and {Henry}, Todd J. and {Subasavage}, John P. and {Ianna}, Philip A.},
        title = "{The Solar Neighborhood. XVI. Parallaxes from CTIOPI: Final Results from the 1.5 m Telescope Program}",
      journal = {\aj},
     keywords = {Astrometry, Galaxy: Solar Neighborhood, Stars: Distances, Stars: Fundamental Parameters, Techniques: Photometric},
         year = 2006,
        month = sep,
       volume = {132},
       number = {3},
        pages = {1234-1247},
          doi = {10.1086/505706},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....132.1234C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Agol2021,
       author = {{Agol}, Eric and {Dorn}, Caroline and {Grimm}, Simon L. and {Turbet}, Martin and {Ducrot}, Elsa and {Delrez}, Laetitia and {Gillon}, Micha{\"e}l and {Demory}, Brice-Olivier and {Burdanov}, Artem and {Barkaoui}, Khalid and {Benkhaldoun}, Zouhair and {Bolmont}, Emeline and {Burgasser}, Adam and {Carey}, Sean and {de Wit}, Julien and {Fabrycky}, Daniel and {Foreman-Mackey}, Daniel and {Haldemann}, Jonas and {Hernandez}, David M. and {Ingalls}, James and {Jehin}, Emmanuel and {Langford}, Zachary and {Leconte}, J{\'e}r{\'e}my and {Lederer}, Susan M. and {Luger}, Rodrigo and {Malhotra}, Renu and {Meadows}, Victoria S. and {Morris}, Brett M. and {Pozuelos}, Francisco J. and {Queloz}, Didier and {Raymond}, Sean N. and {Selsis}, Franck and {Sestovic}, Marko and {Triaud}, Amaury H.~M.~J. and {Van Grootel}, Valerie},
        title = "{Refining the Transit-timing and Photometric Analysis of TRAPPIST-1: Masses, Radii, Densities, Dynamics, and Ephemerides}",
      journal = {\psj},
     keywords = {Extrasolar rocky planets, Exoplanet dynamics, Infrared photometry, Habitable planets, Transit timing variation method, Transit photometry, Exoplanet astronomy, Planetary interior, Fundamental parameters of stars, Markov chain Monte Carlo, N-body simulations, Few-body systems, 511, 490, 792, 695, 1710, 1709, 486, 1248, 555, 1889, 1083, 531, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = feb,
       volume = {2},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.3847/PSJ/abd022},
archivePrefix = {arXiv},
       eprint = {2010.01074},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021PSJ.....2....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Husser2013,
       author = {{Husser}, T. -O. and {Wende-von Berg}, S. and {Dreizler}, S. and {Homeier}, D. and {Reiners}, A. and {Barman}, T. and {Hauschildt}, P.~H.},
        title = "{A new extensive library of PHOENIX stellar atmospheres and synthetic spectra}",
      journal = {\aap},
     keywords = {stars: atmospheres, convection, stars: late-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = may,
       volume = {553},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201219058},
archivePrefix = {arXiv},
       eprint = {1303.5632},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...553A...6H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wenger2000,
       author = {{Wenger}, M. and {Ochsenbein}, F. and {Egret}, D. and {Dubois}, P. and {Bonnarel}, F. and {Borde}, S. and {Genova}, F. and {Jasniewicz}, G. and {Lalo{\"e}}, S. and {Lesteven}, S. and {Monier}, R.},
        title = "{The SIMBAD astronomical database. The CDS reference database for astronomical objects}",
      journal = {\aaps},
     keywords = {ASTRONOMICAL DATA BASES: MISCELLANEOUS, CATALOGS, Astrophysics},
         year = 2000,
        month = apr,
       volume = {143},
        pages = {9-22},
          doi = {10.1051/aas:2000332},
archivePrefix = {arXiv},
       eprint = {astro-ph/0002110},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&AS..143....9W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Mawet2019,
       author = {{Mawet}, Dimitri and {Fitzgerald}, Michael and {Konopacky}, Quinn and {Beichman}, Charles and {Jovanovic}, Nemanja and {Dekany}, Richard and {Hover}, David and {Chisholm}, Eric and {Ciardi}, David and {Artigau}, {\'E}tienne and {Banyal}, Ravinder and {Beatty}, Thomas and {Benneke}, Bj{\"o}rn and {Blake}, Geoffrey A. and {Burgasser}, Adam and {Canalizo}, Gabriela and {Chen}, Guo and {Do}, Tuan and {Doppmann}, Greg and {Doyon}, Ren{\'e} and {Dressing}, Courtney and {Fang}, Min and {Greene}, Thomas and {Hillenbrand}, Lynne and {Howard}, Andrew and {Kane}, Stephen and {Kataria}, Tiffany and {Kempton}, Eliza and {Knutson}, Heather and {Kotani}, Takayuki and {Lafreni{\`e}re}, David and {Liu}, Chao and {Nishiyama}, Shogo and {Pandey}, Gajendra and {Plavchan}, Peter and {Prato}, Lisa and {Rajaguru}, S.~P. and {Robertson}, Paul and {Salyk}, Colette and {Sato}, Bun'ei and {Schlawin}, Everett and {Sengupta}, Sujan and {Sivarani}, Thirupathi and {Skidmore}, Warren and {Tamura}, Motohide and {Terada}, Hiroshi and {Vasisht}, Gautam and {Wang}, Ji and {Zhang}, Hui},
        title = "{High-resolution Infrared Spectrograph for Exoplanet Characterization with the Keck and Thirty Meter Telescopes}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Bulletin of the American Astronomical Society},
         year = 2019,
       volume = {51},
        month = sep,
          eid = {134},
        pages = {134},
archivePrefix = {arXiv},
       eprint = {1908.03623},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019BAAS...51g.134M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Brandl2021,
       author = {{Brandl}, B. and {Bettonvil}, F. and {van Boekel}, R. and {Glauser}, A. and {Quanz}, S. and {Absil}, O. and {Amorim}, A. and {Feldt}, M. and {Glasse}, A. and {G{\"u}del}, M. and {Ho}, P. and {Labadie}, L. and {Meyer}, M. and {Pantin}, E. and {van Winckel}, H. and {METIS Consortium}},
        title = "{METIS: The Mid-infrared ELT Imager and Spectrograph}",
      journal = {The Messenger},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = mar,
       volume = {182},
        pages = {22-26},
          doi = {10.18727/0722-6691/5218},
archivePrefix = {arXiv},
       eprint = {2103.11208},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021Msngr.182...22B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Szentgyorgyi2018,
       author = {{Szentgyorgyi}, Andrew and {Baldwin}, Daniel and {Barnes}, Stuart and {Bean}, Jacob and {Ben-Ami}, Sagi and {Brennan}, Patricia and {Budynkiewicz}, Jamie and {Catropa}, Daniel and {Chun}, Moo-Young and {Conroy}, Charlie and {Contos}, Adam and {Crane}, Jeffrey D. and {Durusky}, Daniel and {Epps}, Harland and {Evans}, Ian and {Evans}, Janet and {Fishman}, Valery and {Frebel}, Anna and {Gauron}, Thomas and {Guzman}, Dani and {Hare}, Tyson and {Jang}, Bi-Ho and {Jang}, Jeong-Gyun and {Jordan}, Andres and {Kim}, Jihun and {Kim}, Kang-Min and {Kim}, Yunjong and {Lee}, Sungho and {Lopez-Morales}, Mercedes and {Mendes de Oliveira}, Claudia and {McCracken}, Kenneth and {McMuldroch}, Stuart and {Miller}, Joseph and {Mueller}, Mark and {Oh}, Jae Sok and {Onyuksel}, Cem and {Park}, Byeong-Gon and {Park}, Chan and {Park}, Sung-Joon and {Paxson}, Charles and {Phillips}, David and {Plummer}, David and {Podgorski}, William and {Rubin}, Adam and {Seifahrt}, Andreas and {Stark}, Daniel and {Steiner}, Joao and {Uomoto}, Alan and {Walsworth}, Ronald and {Yu}, Young-Sam},
        title = "{The GMT-consortium large earth finder (G-CLEF): an optical echelle spectrograph for the Giant Magellan Telescope (GMT)}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy VII},
         year = 2018,
       editor = {{Evans}, Christopher J. and {Simard}, Luc and {Takami}, Hideki},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {10702},
        month = jul,
          eid = {107021R},
        pages = {107021R},
          doi = {10.1117/12.2313539},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018SPIE10702E..1RS},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Plummer2022,
       author = {{Plummer}, Michael K. and {Wang}, Ji},
        title = "{A Unified Spectroscopic and Photometric Model to Infer Surface Inhomogeneity: Application to Luhman 16B}",
      journal = {\apj},
     keywords = {Doppler imaging, M dwarf stars, Brown dwarfs, Spectrophotometry, Exoplanet atmospheres, 400, 982, 185, 1556, 487, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jul,
       volume = {933},
       number = {2},
          eid = {163},
        pages = {163},
          doi = {10.3847/1538-4357/ac75b9},
archivePrefix = {arXiv},
       eprint = {2206.01770},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...933..163P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{zhang14,
       author = {{Zhang}, Xi and {Showman}, Adam P.},
        title = "{Atmospheric Circulation of Brown Dwarfs: Jets, Vortices, and Time Variability}",
      journal = {\apjl},
     keywords = {brown dwarfs, methods: numerical, stars: atmospheres, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = jun,
       volume = {788},
       number = {1},
          eid = {L6},
        pages = {L6},
          doi = {10.1088/2041-8205/788/1/L6},
archivePrefix = {arXiv},
       eprint = {1403.2143},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...788L...6Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rossiter1924,
       author = {{Rossiter}, R.~A.},
        title = "{On the detection of an effect of rotation during eclipse in the velocity of the brighter component of beta Lyrae, and on the constancy of velocity of this system.}",
      journal = {\apj},
         year = 1924,
        month = jul,
       volume = {60},
        pages = {15-21},
          doi = {10.1086/142825},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ApJ....60...15R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oppenheimer1998,
       author = {{Oppenheimer}, B.~R. and {Kulkarni}, S.~R. and {Matthews}, K. and {van Kerkwijk}, M.~H.},
        title = "{The Spectrum of the Brown Dwarf Gliese 229B}",
      journal = {\apj},
     keywords = {STARS: CIRCUMSTELLAR MATTER, LINE: IDENTIFICATION, STARS: INDIVIDUAL NAME: GLIESE 229B, STARS: LOW-MASS, BROWN DWARFS, Stars: Circumstellar Matter, Line: Identification, Stars: Individual: Name: Gliese 229B, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 1998,
        month = aug,
       volume = {502},
       number = {2},
        pages = {932-943},
          doi = {10.1086/305928},
archivePrefix = {arXiv},
       eprint = {astro-ph/9802299},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...502..932O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{McLaughlin1924ApJ,
       author = {{McLaughlin}, D.~B.},
        title = "{Some results of a spectrographic study of the Algol system.}",
      journal = {\apj},
         year = 1924,
        month = jul,
       volume = {60},
        pages = {22-31},
          doi = {10.1086/142826},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ApJ....60...22M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Tan&Showman19,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric Variability Driven by Radiative Cloud Feedback in Brown Dwarfs and Directly Imaged Extrasolar Giant Planets}",
      journal = {\apj},
     keywords = {brown dwarfs, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, radiative transfer, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2019,
        month = apr,
       volume = {874},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.3847/1538-4357/ab0c07},
archivePrefix = {arXiv},
       eprint = {1809.06467},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874..111T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tan22,
       author = {{Tan}, Xianyu},
        title = "{Jet streams and tracer mixing in the atmospheres of brown dwarfs and isolated young giant planets}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, brown dwarfs},
         year = 2022,
        month = feb,
          doi = {10.1093/mnras/stac344},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.tmp..360T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mukherjee21,
       author = {{Mukherjee}, Sagnick and {Fortney}, Jonathan J. and {Jensen-Clem}, Rebecca and {Tan}, Xianyu and {Marley}, Mark S. and {Batalha}, Natasha E.},
        title = "{Modeling Polarization Signals from Cloudy Brown Dwarfs Luhman 16 A and B in Three Dimensions}",
      journal = {\apj},
     keywords = {185, 2180, 112, 1278, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = dec,
       volume = {923},
       number = {1},
          eid = {113},
        pages = {113},
          doi = {10.3847/1538-4357/ac2d92},
archivePrefix = {arXiv},
       eprint = {2110.05739},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923..113M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tan21b,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric circulation of brown dwarfs and directly imaged exoplanets driven by cloud radiative feedback: global and equatorial dynamics}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
       volume = {502},
       number = {2},
        pages = {2198-2219},
          doi = {10.1093/mnras/stab097},
archivePrefix = {arXiv},
       eprint = {2101.04417},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502.2198T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tan21a,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric circulation of brown dwarfs and directly imaged exoplanets driven by cloud radiative feedback: effects of rotation}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2021,
        month = mar,
       volume = {502},
       number = {1},
        pages = {678-699},
          doi = {10.1093/mnras/stab060},
archivePrefix = {arXiv},
       eprint = {2005.12152},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502..678T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{showman20,
       author = {{Showman}, Adam P. and {Tan}, Xianyu and {Parmentier}, Vivien},
        title = "{Atmospheric Dynamics of Hot Giant Planets and Brown Dwarfs}",
      journal = {\ssr},
     keywords = {Exoplanets, Giant planets, Hot Jupiters, Jupiter, Saturn, Brown dwarfs, Atmospheric dynamics, Turbulence, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {216},
       number = {8},
          eid = {139},
        pages = {139},
          doi = {10.1007/s11214-020-00758-8},
archivePrefix = {arXiv},
       eprint = {2007.15363},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SSRv..216..139S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{showman&kaspi13,
       author = {{Showman}, Adam P. and {Kaspi}, Yohai},
        title = "{Atmospheric Dynamics of Brown Dwarfs and Directly Imaged Giant Planets}",
      journal = {\apj},
     keywords = {brown dwarfs, convection, methods: numerical, stars: low-mass, turbulence, waves, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {776},
       number = {2},
          eid = {85},
        pages = {85},
          doi = {10.1088/0004-637X/776/2/85},
archivePrefix = {arXiv},
       eprint = {1210.7573},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...776...85S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{triaud17,
       author = {{Triaud}, Amaury H.~M.~J.},
        title = "{The Rossiter-McLaughlin Effect in Exoplanet Research}",
     keywords = {Physics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Handbook of Exoplanets},
         year = 2018,
       editor = {{Deeg}, Hans J. and {Belmonte}, Juan Antonio},
          eid = {2},
        pages = {2},
          doi = {10.1007/978-3-319-55333-7\_2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018haex.bookE...2T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{watson19,
       author = {{Watson}, C.~A. and {de Mooij}, E.~J.~W. and {Steeghs}, D. and {Marsh}, T.~R. and {Brogi}, M. and {Gibson}, N.~P. and {Matthews}, S.},
        title = "{Doppler tomography as a tool for detecting exoplanet atmospheres}",
      journal = {\mnras},
     keywords = {line: profiles, techniques: spectroscopic, planets and satellites: atmospheres, planets and satellites: individual: {\ensuremath{\tau}} Boo-b, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {490},
       number = {2},
        pages = {1991-2006},
          doi = {10.1093/mnras/stz2679},
archivePrefix = {arXiv},
       eprint = {1909.09219},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.490.1991W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{kochokhov10,
       author = {{Kochukhov}, O. and {Makaganiuk}, V. and {Piskunov}, N.},
        title = "{Least-squares deconvolution of the stellar intensity and polarization spectra}",
      journal = {\aap},
     keywords = {magnetic fields, line: formation, polarization, stars: atmospheres, methods: data analysis, methods: numerical, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = dec,
       volume = {524},
          eid = {A5},
        pages = {A5},
          doi = {10.1051/0004-6361/201015429},
archivePrefix = {arXiv},
       eprint = {1008.5115},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...524A...5K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{karalidi15,
       author = {{Karalidi}, Theodora and {Apai}, D{\'a}niel and {Schneider}, Glenn and {Hanson}, Jake R. and {Pasachoff}, Jay M.},
        title = "{Aeolus: A Markov Chain Monte Carlo Code for Mapping Ultracool Atmospheres. An Application on Jupiter and Brown Dwarf HST Light Curves}",
      journal = {\apj},
     keywords = {methods: statistical, planets and satellites: individual: Jupiter, stars: individual: 2MASS J21392676+0220226, 2MASS J0136565+093347, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = nov,
       volume = {814},
       number = {1},
          eid = {65},
        pages = {65},
          doi = {10.1088/0004-637X/814/1/65},
archivePrefix = {arXiv},
       eprint = {1510.04251},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...814...65K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{karalidi16,
       author = {{Karalidi}, Theodora and {Apai}, D{\'a}niel and {Marley}, Mark S. and {Buenzli}, Esther},
        title = "{Maps of Evolving Cloud Structures in Luhman 16AB from HST Time-resolved Spectroscopy}",
      journal = {\apj},
     keywords = {methods: statistical, stars: individual: WISE J104915.57-531906.1, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = jul,
       volume = {825},
       number = {2},
          eid = {90},
        pages = {90},
          doi = {10.3847/0004-637X/825/2/90},
archivePrefix = {arXiv},
       eprint = {1605.01682},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...825...90K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{donati97,
       author = {{Donati}, J. -F. and {Brown}, S.~F.},
        title = "{Zeeman-Doppler imaging of active stars. V. Sensitivity of maximum entropy magnetic maps to field orientation.}",
      journal = {\aap},
     keywords = {STARS: MAGNETIC FIELDS, STARS: IMAGING, STARS: ACTIVITY, LINE: PROFILES, POLARIZATION, METHODS: OBSERVATIONAL},
         year = 1997,
        month = oct,
       volume = {326},
        pages = {1135-1142},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997A&A...326.1135D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{crossfield14,
       author = {{Crossfield}, I.~J.~M. and {Biller}, B. and {Schlieder}, J.~E. and {Deacon}, N.~R. and {Bonnefoy}, M. and {Homeier}, D. and {Allard}, F. and {Buenzli}, E. and {Henning}, Th. and {Brandner}, W. and {Goldman}, B. and {Kopytova}, T.},
        title = "{A global cloud map of the nearest known brown dwarf}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = jan,
       volume = {505},
       number = {7485},
        pages = {654-656},
          doi = {10.1038/nature12955},
archivePrefix = {arXiv},
       eprint = {1401.8145},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014Natur.505..654C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{apai21,
       author = {{Apai}, D{\'a}niel and {Nardiello}, Domenico and {Bedin}, Luigi R.},
        title = "{TESS Observations of the Luhman 16 AB Brown Dwarf System: Rotational Periods, Lightcurve Evolution, and Zonal Circulation}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Atmospheric circulation, T dwarfs, Atmospheric variability, Stellar rotation, Photometry, 487, 112, 1679, 2119, 1629, 1234, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jan,
       volume = {906},
       number = {1},
          eid = {64},
        pages = {64},
          doi = {10.3847/1538-4357/abcb97},
archivePrefix = {arXiv},
       eprint = {2101.02253},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...906...64A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{speagle20,
       author = {{Speagle}, Joshua S.},
        title = "{DYNESTY: a dynamic nested sampling package for estimating Bayesian posteriors and evidences}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, Astrophysics - Instrumentation and Methods for Astrophysics, Statistics - Computation},
         year = 2020,
        month = apr,
       volume = {493},
       number = {3},
        pages = {3132-3158},
          doi = {10.1093/mnras/staa278},
archivePrefix = {arXiv},
       eprint = {1904.02180},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.3132S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Skilling2004,
       author = {{Skilling}, John},
        title = "{Nested Sampling}",
     keywords = {02.50.Tt, Inference methods},
    booktitle = {Bayesian Inference and Maximum Entropy Methods in Science and Engineering: 24th International Workshop on Bayesian Inference and Maximum Entropy Methods in Science and Engineering},
         year = 2004,
       editor = {{Fischer}, Rainer and {Preuss}, Roland and {Toussaint}, Udo Von},
       series = {American Institute of Physics Conference Series},
       volume = {735},
        month = nov,
        pages = {395-405},
          doi = {10.1063/1.1835238},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004AIPC..735..395S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{skilling06,
    author  = {{Skilling}, John},
    title   = "Nested Sampling for General Bayesian Computation",
    year    = "2006",
    journal = {Bayesian Analysis},
    volume  = {1},
    issue = {4},
    pages   = {833-860},
    doi = {10.1214/06-BA127}
}

@ARTICLE{Buenzli15a,
       author = {{Buenzli}, Esther and {Saumon}, Didier and {Marley}, Mark S. and {Apai}, D{\'a}niel and {Radigan}, Jacqueline and {Bedin}, Luigi R. and {Reid}, I. Neill and {Morley}, Caroline V.},
        title = "{Cloud Structure of the Nearest Brown Dwarfs: Spectroscopic Variability of Luhman 16AB from the Hubble Space Telescope}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: atmospheres, stars: individual: WISE J104915.57-531906.1 Luhman 16AB, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = jan,
       volume = {798},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.1088/0004-637X/798/2/127},
archivePrefix = {arXiv},
       eprint = {1411.0003},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798..127B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{perryman18,
       author = {{Perryman}, Michael},
        title = "{The Exoplanet Handbook}",
         year = 2018,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018exha.book.....P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{kasting93,
       author = {{Kasting}, James F. and {Whitmire}, Daniel P. and {Reynolds}, Ray T.},
        title = "{Habitable Zones around Main Sequence Stars}",
      journal = {\icarus},
         year = 1993,
        month = jan,
       volume = {101},
       number = {1},
        pages = {108-128},
          doi = {10.1006/icar.1993.1010},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993Icar..101..108K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{kopparapu13,
       author = {{Kopparapu}, Ravi Kumar and {Ramirez}, Ramses and {Kasting}, James F. and {Eymet}, Vincent and {Robinson}, Tyler D. and {Mahadevan}, Suvrath and {Terrien}, Ryan C. and {Domagal-Goldman}, Shawn and {Meadows}, Victoria and {Deshpande}, Rohit},
        title = "{Habitable Zones around Main-sequence Stars: New Estimates}",
      journal = {\apj},
     keywords = {planetary systems, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = mar,
       volume = {765},
       number = {2},
          eid = {131},
        pages = {131},
          doi = {10.1088/0004-637X/765/2/131},
archivePrefix = {arXiv},
       eprint = {1301.6674},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...765..131K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{zendejas10,
       author = {{Zendejas}, J. and {Segura}, A. and {Raga}, A.~C.},
        title = "{Atmospheric mass loss by stellar wind from planets around main sequence M stars}",
      journal = {\icarus},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = dec,
       volume = {210},
       number = {2},
        pages = {539-544},
          doi = {10.1016/j.icarus.2010.07.013},
archivePrefix = {arXiv},
       eprint = {1006.0021},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Icar..210..539Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{tarter07,
       author = {{Tarter}, Jill C. and {Backus}, Peter R. and {Mancinelli}, Rocco L. and {Aurnou}, Jonathan M. and {Backman}, Dana E. and {Basri}, Gibor S. and {Boss}, Alan P. and {Clarke}, Andrew and {Deming}, Drake and {Doyle}, Laurance R. and {Feigelson}, Eric D. and {Freund}, Friedmann and {Grinspoon}, David H. and {Haberle}, Robert M. and {Hauck}, Steven A., II and {Heath}, Martin J. and {Henry}, Todd J. and {Hollingsworth}, Jeffery L. and {Joshi}, Manoj M. and {Kilston}, Steven and {Liu}, Michael C. and {Meikle}, Erik and {Reid}, I. Neill and {Rothschild}, Lynn J. and {Scalo}, John and {Segura}, Antigona and {Tang}, Carol M. and {Tiedje}, James M. and {Turnbull}, Margaret C. and {Walkowicz}, Lucianne M. and {Weber}, Arthur L. and {Young}, Richard E.},
        title = "{A Reappraisal of The Habitability of Planets around M Dwarf Stars}",
      journal = {Astrobiology},
     keywords = {Astrophysics},
         year = 2007,
        month = mar,
       volume = {7},
       number = {1},
        pages = {30-65},
          doi = {10.1089/ast.2006.0124},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609799},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AsBio...7...30T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{scalo07,
       author = {{Scalo}, John and {Kaltenegger}, Lisa and {Segura}, Ant Gona and {Fridlund}, Malcolm and {Ribas}, Ignasi and {Kulikov}, Yu. N. and {Grenfell}, John L. and {Rauer}, Hieke and {Odert}, Petra and {Leitzinger}, Martin and {Selsis}, F. and {Khodachenko}, Maxim L. and {Eiroa}, Carlos and {Kasting}, Jim and {Lammer}, Helmut},
        title = "{M Stars as Targets for Terrestrial Exoplanet Searches And Biosignature Detection}",
      journal = {Astrobiology},
         year = 2007,
        month = feb,
       volume = {7},
       number = {1},
        pages = {85-166},
          doi = {10.1089/ast.2006.0125},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AsBio...7...85S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{schuessler&solanki92,
       author = {{Schuessler}, M. and {Solanki}, S.~K.},
        title = "{Why rapid rotators have polar spots.}",
      journal = {\aap},
     keywords = {Cool Stars, Magnetic Stars, Starspots, Stellar Rotation, Computational Astrophysics, Coriolis Effect, Stellar Models, Astrophysics},
         year = 1992,
        month = oct,
       volume = {264},
        pages = {L13-L16},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...264L..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{granzer00,
       author = {{Schuessler}, M. and {Solanki}, S.~K.},
        title = "{Why rapid rotators have polar spots.}",
      journal = {\aap},
     keywords = {Cool Stars, Magnetic Stars, Starspots, Stellar Rotation, Computational Astrophysics, Coriolis Effect, Stellar Models, Astrophysics},
         year = 1992,
        month = oct,
       volume = {264},
        pages = {L13-L16},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...264L..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{yadav15,
       author = {{Yadav}, Rakesh K. and {Gastine}, Thomas and {Christensen}, Ulrich R. and {Reiners}, Ansgar},
        title = "{Formation of starspots in self-consistent global dynamo models: Polar spots on cool stars}",
      journal = {\aap},
     keywords = {starspots, stars: magnetic field, stars: rotation, stars: interiors, dynamo, convection, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jan,
       volume = {573},
          eid = {A68},
        pages = {A68},
          doi = {10.1051/0004-6361/201424589},
archivePrefix = {arXiv},
       eprint = {1407.3187},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..68Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier1998,
       author = {{Strassmeier}, K.~G. and {Bartus}, J. and {Kovari}, Zs. and {Weber}, M. and {Washuettl}, A.},
        title = "{Doppler imaging of stellar surface structure. VIII. The effectively single and rapidly-rotating G8-giant HD 51066 = CM Camelopardalis}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: IMAGING, STARS: INDIVIDUAL: HD 51066, STARS: LATE-TYPE, STARSPOTS},
         year = 1998,
        month = aug,
       volume = {336},
        pages = {587-603},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...336..587S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{strassmeier&rice98,
       author = {{Strassmeier}, K.~G. and {Rice}, J.~B.},
        title = "{Doppler imaging of stellar surface structure. IX. A high-resolution image of the weak-lined T Tauri star HDE 283572 = V987 Tauri}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARSPOTS, STARS: IMAGING, STARS: INDIVIDUAL: HDE 283572, STARS: LATE-TYPE},
         year = 1998,
        month = nov,
       volume = {339},
        pages = {497-506},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...339..497S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{jarvinen08,
       author = {{J{\"a}rvinen}, S.~P. and {Korhonen}, H. and {Berdyugina}, S.~V. and {Ilyin}, I. and {Strassmeier}, K.~G. and {Weber}, M. and {Savanov}, I. and {Tuominen}, I.},
        title = "{Magnetic activity on V889 Herculis. Combining photometry and spectroscopy}",
      journal = {\aap},
     keywords = {stars: imaging, stars: activity, stars: starspots, stars: individual: V889 Her},
         year = 2008,
        month = sep,
       volume = {488},
       number = {3},
        pages = {1047-1055},
          doi = {10.1051/0004-6361:200809837},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...488.1047J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{berdyugina98,
       author = {{Berdyugina}, Svetlana V.},
        title = "{Surface imaging by the Occamian approach. Basic principles, simulations, and tests}",
      journal = {\aap},
     keywords = {STARS: IMAGING, STARS: ACTIVITY, METHODS: DATA ANALYSIS},
         year = 1998,
        month = oct,
       volume = {338},
        pages = {97-105},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...338...97B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{barnes15,
       author = {{Barnes}, J.~R. and {Jeffers}, S.~V. and {Jones}, H.~R.~A. and {Pavlenko}, Ya. V. and {Jenkins}, J.~S. and {Haswell}, C.~A. and {Lohr}, M.~E.},
        title = "{Starspot Distributions on Fully Convective M Dwarfs: Implications for Radial Velocity Planet Searches}",
      journal = {\apj},
     keywords = {methods: data analysis, planets and satellites: detection, stars: individual: GJ 791.2A, LP 944-20, stars: late-type, starspots, techniques: spectroscopic, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = oct,
       volume = {812},
       number = {1},
          eid = {42},
        pages = {42},
          doi = {10.1088/0004-637X/812/1/42},
archivePrefix = {arXiv},
       eprint = {1509.05284},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...812...42B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{barnes17,
       author = {{Barnes}, J.~R. and {Jeffers}, S.~V. and {Haswell}, C.~A. and {Jones}, H.~R.~A. and {Shulyak}, D. and {Pavlenko}, Ya. V. and {Jenkins}, J.~S.},
        title = "{Surprisingly different star-spot distributions on the near equal-mass equal-rotation-rate stars in the M dwarf binary GJ 65 AB}",
      journal = {\mnras},
     keywords = {techniques: imaging spectroscopy, techniques: spectroscopic, stars: atmospheres, stars: imaging, stars: low-mass, starspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = oct,
       volume = {471},
       number = {1},
        pages = {811-823},
          doi = {10.1093/mnras/stx1482},
archivePrefix = {arXiv},
       eprint = {1706.03979},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471..811B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{rimmer18,
    author = "Paul B. Rimmer and Jianfeng Xu and Samantha J. Thompson and Ed Gillen and John D. Sutherland and Didier Queloz",
    title = "The origin of RNA precursors on exoplanets",
    journal = "Science Advances",
    volume = "4",
    issue = "8",
    pages = "eear3302",
    month = "August",
    year = "2018"
}

@article{gunther20,
       author = {{G{\"u}nther}, Maximilian N. and {Zhan}, Zhuchang and {Seager}, Sara and {Rimmer}, Paul B. and {Ranjan}, Sukrit and {Stassun}, Keivan G. and {Oelkers}, Ryan J. and {Daylan}, Tansu and {Newton}, Elisabeth and {Kristiansen}, Martti H. and {Olah}, Katalin and {Gillen}, Edward and {Rappaport}, Saul and {Ricker}, George R. and {Vanderspek}, Roland K. and {Latham}, David W. and {Winn}, Joshua N. and {Jenkins}, Jon M. and {Glidden}, Ana and {Fausnaugh}, Michael and {Levine}, Alan M. and {Dittmann}, Jason A. and {Quinn}, Samuel N. and {Krishnamurthy}, Akshata and {Ting}, Eric B.},
        title = "{Stellar Flares from the First TESS Data Release: Exploring a New Sample of M Dwarfs}",
      journal = {\aj},
     keywords = {1166, 498, 695, 1367, 1603, 1580, 696, 511, 74, 2079, 487, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = feb,
       volume = {159},
       number = {2},
          eid = {60},
        pages = {60},
          doi = {10.3847/1538-3881/ab5d3a},
archivePrefix = {arXiv},
       eprint = {1901.00443},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159...60G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{zeldes21,
       author = {{Zeldes}, Jesse and {Hinkle}, Jason T. and {Shappee}, Benjamin J. and {Avallone}, Ellis A. and {Schmidt}, Sarah J. and {van Saders}, Jennifer L. and {Way}, Zachary and {Kochanek}, Christopher S. and {Holoien}, Thomas W. -S.},
        title = "{Flares Big and Small: a K2 and TESS View of ASAS-SN Superflares}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.04501},
        pages = {arXiv:2109.04501},
archivePrefix = {arXiv},
       eprint = {2109.04501},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210904501Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{ramsay21,
       author = {{Ramsay}, Gavin and {Kolotkov}, Dmitrii and {Doyle}, J. Gerry and {Doyle}, Lauren},
        title = "{Transiting Exoplanet Survey Satellite (TESS) Observations of Flares and Quasi-Periodic Pulsations from Low-Mass Stars and Potential Impact on Exoplanets}",
      journal = {\solphys},
     keywords = {Stars: activity, Stars: flare, Stars: low-mass, Stars: pulsations, Stars: magnetic fields, Planets and satellites: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = nov,
       volume = {296},
       number = {11},
          eid = {162},
        pages = {162},
          doi = {10.1007/s11207-021-01899-x},
archivePrefix = {arXiv},
       eprint = {2108.10670},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021SoPh..296..162R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ilin2021,
       author = {{Ilin}, Ekaterina and {Poppenhaeger}, Katja and {Schmidt}, Sarah J. and {J{\"a}rvinen}, Silva P. and {Newton}, Elisabeth R. and {Alvarado-G{\'o}mez}, Juli{\'a}n D. and {Pineda}, J. Sebastian and {Davenport}, James R.~A. and {Oshagh}, Mahmoudreza and {Ilyin}, Ilya},
        title = "{Giant white-light flares on fully convective stars occur at high latitudes}",
      journal = {\mnras},
     keywords = {stars: activity, stars: flare, stars: magnetic field, stars: low-mass, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {507},
       number = {2},
        pages = {1723-1745},
          doi = {10.1093/mnras/stab2159},
archivePrefix = {arXiv},
       eprint = {2108.01917},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.507.1723I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Wang17,
       author = {{Wang}, Ji and {Prato}, Lisa and {Mawet}, Dimitri},
        title = "{Time-resolved High Spectral Resolution Observation of 2MASSW J0746425+200032AB}",
      journal = {\apj},
     keywords = {binaries: spectroscopic, brown dwarfs, infrared: stars, methods: observational, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {838},
       number = {1},
          eid = {35},
        pages = {35},
          doi = {10.3847/1538-4357/aa6345},
archivePrefix = {arXiv},
       eprint = {1702.07769},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...838...35W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wang18,
       author = {{Wang}, Ji and {David}, Trevor J. and {Hillenbrand}, Lynne A. and {Mawet}, Dimitri and {Albrecht}, Simon and {Liu}, Zibo},
        title = "{EPIC 203868608: A Low-mass Quadruple Star System in the Upper Scorpius OB Association}",
      journal = {\apj},
     keywords = {binaries: close, binaries: eclipsing, binaries: spectroscopic, stars: late-type, stars: low-mass, techniques: radial velocities, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = oct,
       volume = {865},
       number = {2},
          eid = {141},
        pages = {141},
          doi = {10.3847/1538-4357/aadee8},
archivePrefix = {arXiv},
       eprint = {1809.01689},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865..141W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{donatelli&reichel14,
    author = "M. Donatelli and L. Reichel",
    title = "Square smoothing regularization matrices with accurate boundary conditions",
    journal = "Journal of Computational and Applied Mathematics",
    volume = "272",
    pages = "334-349",
    month = "December",
    year = "2014"
}

@article{PaiAsnodkar22,
       author = {{Pai Asnodkar}, Anusha and {Wang}, Ji and {Gaudi}, B. Scott and {Cauley}, P. Wilson and {Eastman}, Jason D. and {Ilyin}, Ilya and {Strassmeier}, Klaus and {Beatty}, Thomas},
        title = "{KELT-9 as an Eclipsing Double-lined Spectroscopic Binary: A Unique and Self-consistent Solution to the System}",
      journal = {\aj},
     keywords = {486, 487, 498, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = feb,
       volume = {163},
       number = {2},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-3881/ac32c7},
archivePrefix = {arXiv},
       eprint = {2110.15275},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....163...40P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zhang2020,
       author = {{Zhang}, Xi},
        title = "{Atmospheric regimes and trends on exoplanets and brown dwarfs}",
      journal = {Research in Astronomy and Astrophysics},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {20},
       number = {7},
          eid = {099},
        pages = {099},
          doi = {10.1088/1674-4527/20/7/99},
archivePrefix = {arXiv},
       eprint = {2006.13384},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020RAA....20...99Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Luger2019,
       author = {{Luger}, Rodrigo and {Agol}, Eric and {Foreman-Mackey}, Daniel and {Fleming}, David P. and {Lustig-Yaeger}, Jacob and {Deitrick}, Russell},
        title = "{starry: Analytic Occultation Light Curves}",
      journal = {\aj},
     keywords = {eclipses, methods: analytical, occultations, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {157},
       number = {2},
          eid = {64},
        pages = {64},
          doi = {10.3847/1538-3881/aae8e5},
archivePrefix = {arXiv},
       eprint = {1810.06559},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157...64L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{luger21a,
       author = {{Luger}, Rodrigo and {Bedell}, Megan and {Foreman-Mackey}, Daniel and {Crossfield}, Ian J.~M. and {Zhao}, Lily L. and {Hogg}, David W.},
        title = "{Mapping stellar surfaces III: An Efficient, Scalable, and Open-Source Doppler Imaging Model}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = oct,
          eid = {arXiv:2110.06271},
        pages = {arXiv:2110.06271},
archivePrefix = {arXiv},
       eprint = {2110.06271},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv211006271L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{higson19,
       author = {{Higson}, Edward and {Handley}, Will and {Hobson}, Mike and {Lasenby}, Anthony},
        title = "{Dynamic nested sampling: an improved algorithm for parameter estimation and evidence calculation}",
      journal = {Statistics and Computing},
     keywords = {Statistics - Computation, Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Data Analysis, Statistics and Probability, Statistics - Methodology, Statistics - Computation, Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Data Analysis, Statistics and Probability, Statistics - Methodology},
         year = 2019,
        month = sep,
       volume = {29},
       number = {5},
        pages = {891-913},
          doi = {10.1007/s11222-018-9844-0},
archivePrefix = {arXiv},
       eprint = {1704.03459},
 primaryClass = {stat.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019S&C....29..891H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{luhman13,
       author = {{Luhman}, K.~L.},
        title = "{Discovery of a Binary Brown Dwarf at 2 pc from the Sun}",
      journal = {\apjl},
     keywords = {brown dwarfs, infrared: stars, proper motions, solar neighborhood, stars: low-mass, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.1088/2041-8205/767/1/L1},
archivePrefix = {arXiv},
       eprint = {1303.2401},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767L...1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{kniazev13,
       author = {{Kniazev}, A.~Y. and {Vaisanen}, P. and {Mu{\v{z}}i{\'c}}, K. and {Mehner}, A. and {Boffin}, H.~M.~J. and {Kurtev}, R. and {Melo}, C. and {Ivanov}, V.~D. and {Girard}, J. and {Mawet}, D. and {Schmidtobreick}, L. and {Huelamo}, N. and {Borissova}, J. and {Minniti}, D. and {Ishibashi}, K. and {Potter}, S.~B. and {Beletsky}, Y. and {Buckley}, D.~A.~H. and {Crawford}, S. and {Gulbis}, A.~A.~S. and {Kotze}, P. and {Miszalski}, B. and {Pickering}, T.~E. and {Romero Colmenero}, E. and {Williams}, T.~B.},
        title = "{Characterization of the nearby L/T Binary Brown Dwarf WISE J104915.57-531906.1 at 2 pc from the Sun}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, solar neighborhood, stars: individual: G 171{\textendash}22 HD 55383 WISE J104915.57{\textendash}531906.1, stars: low-mass, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = jun,
       volume = {770},
       number = {2},
          eid = {124},
        pages = {124},
          doi = {10.1088/0004-637X/770/2/124},
archivePrefix = {arXiv},
       eprint = {1303.7171},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...770..124K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{burgasser13,
       author = {{Burgasser}, Adam J. and {Sheppard}, Scott S. and {Luhman}, K.~L.},
        title = "{Resolved Near-infrared Spectroscopy of WISE J104915.57-531906.1AB: A Flux-reversal Binary at the L dwarf/T Dwarf Transition}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57{\textendash}531906.1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = aug,
       volume = {772},
       number = {2},
          eid = {129},
        pages = {129},
          doi = {10.1088/0004-637X/772/2/129},
archivePrefix = {arXiv},
       eprint = {1303.7283},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...772..129B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garcia17,
       author = {{Garcia}, E. Victor and {Ammons}, S. Mark and {Salama}, Maissa and {Crossfield}, Ian and {Bendek}, Eduardo and {Chilcote}, Jeffrey and {Garrel}, Vincent and {Graham}, James R. and {Kalas}, Paul and {Konopacky}, Quinn and {Lu}, Jessica R. and {Macintosh}, Bruce and {Marin}, Eduardo and {Marois}, Christian and {Nielsen}, Eric and {Neichel}, Beno{\^\i}t and {Pham}, Don and {De Rosa}, Robert J. and {Ryan}, Dominic M. and {Service}, Maxwell and {Sivo}, Gaetano},
        title = "{Individual, Model-independent Masses of the Closest Known Brown Dwarf Binary to the Sun}",
      journal = {\apj},
     keywords = {astrometry, binaries: visual, brown dwarfs, stars: fundamental parameters, stars: individual: WISE J104915.57{\textendash}531906.1, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = sep,
       volume = {846},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/aa844f},
archivePrefix = {arXiv},
       eprint = {1708.02714},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...846...97G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{morley12,
       author = {{Morley}, Caroline V. and {Fortney}, Jonathan J. and {Marley}, Mark S. and {Visscher}, Channon and {Saumon}, Didier and {Leggett}, S.~K.},
        title = "{Neglected Clouds in T and Y Dwarf Atmospheres}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = sep,
       volume = {756},
       number = {2},
          eid = {172},
        pages = {172},
          doi = {10.1088/0004-637X/756/2/172},
archivePrefix = {arXiv},
       eprint = {1206.4313},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...756..172M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{faherty14,
       author = {{Faherty}, Jacqueline K. and {Beletsky}, Yuri and {Burgasser}, Adam J. and {Tinney}, Chris and {Osip}, David J. and {Filippazzo}, Joseph C. and {Simcoe}, Robert A.},
        title = "{Signatures of Cloud, Temperature, and Gravity from Spectra of the Closest Brown Dwarfs}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57-531906.1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = aug,
       volume = {790},
       number = {2},
          eid = {90},
        pages = {90},
          doi = {10.1088/0004-637X/790/2/90},
archivePrefix = {arXiv},
       eprint = {1406.1518},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...790...90F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lazorenko18,
       author = {{Lazorenko}, P.~F. and {Sahlmann}, J.},
        title = "{Updated astrometry and masses of the LUH 16 brown dwarf binary}",
      journal = {\aap},
     keywords = {astrometry, brown dwarfs, binaries: visual, parallaxes, stars: individual: WISE J104915.57-531906.1, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A111},
        pages = {A111},
          doi = {10.1051/0004-6361/201833626},
archivePrefix = {arXiv},
       eprint = {1808.07835},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A.111L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sahlmann15,
       author = {{Sahlmann}, J. and {Lazorenko}, P.~F.},
        title = "{Mass ratio of the 2 pc binary brown dwarf LUH 16 and limits on planetary companions from astrometry}",
      journal = {\mnras},
     keywords = {astrometry, parallaxes, binaries: visual, brown dwarfs, stars: individual: WISE J104915.57-531906.1, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {453},
       number = {1},
        pages = {L103-L107},
          doi = {10.1093/mnrasl/slv113},
archivePrefix = {arXiv},
       eprint = {1506.07994},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453L.103S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lodieu15,
       author = {{Lodieu}, N. and {Zapatero Osorio}, M.~R. and {Rebolo}, R. and {B{\'e}jar}, V.~J.~S. and {Pavlenko}, Y. and {P{\'e}rez-Garrido}, A.},
        title = "{VLT X-Shooter spectroscopy of the nearest brown dwarf binary}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, brown dwarfs, binaries: general, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {581},
          eid = {A73},
        pages = {A73},
          doi = {10.1051/0004-6361/201424933},
archivePrefix = {arXiv},
       eprint = {1506.08848},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...581A..73L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gillon13,
       author = {{Gillon}, M. and {Triaud}, A.~H.~M.~J. and {Jehin}, E. and {Delrez}, L. and {Opitom}, C. and {Magain}, P. and {Lendl}, M. and {Queloz}, D.},
        title = "{Fast-evolving weather for the coolest of our two new substellar neighbours}",
      journal = {\aap},
     keywords = {brown dwarfs, stars: individual: WISE-J104915.57-531906.1, solar neighborhood, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = jul,
       volume = {555},
          eid = {L5},
        pages = {L5},
          doi = {10.1051/0004-6361/201321620},
archivePrefix = {arXiv},
       eprint = {1304.0481},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...555L...5G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heinze21,
       author = {{Heinze}, A.~N. and {Metchev}, Stanimir and {Kurtev}, Radostin and {Gillon}, Michael},
        title = "{Weather on Other Worlds. VI. Optical Spectrophotometry of Luhman 16B Reveals Large-amplitude Variations in the Alkali Lines}",
      journal = {\apj},
     keywords = {Brown dwarfs, Atmospheric clouds, Exoplanet atmospheric variability, Variable stars, Spectrophotometry, Time series analysis, 185, 2180, 2020, 1761, 1556, 1916, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.3847/1538-4357/ac178b},
archivePrefix = {arXiv},
       eprint = {2107.10995},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920..108H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ammons&garcia19,
       author = {{Ammons}, Stephen M. and {Garcia}, Victor},
        title = "{Independent Masses for the Luhman 16AB Binary Brown Dwarf System from Gemini GEMS}",
    booktitle = {American Astronomical Society Meeting Abstracts \#233},
         year = 2019,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {233},
        month = jan,
          eid = {114.07},
        pages = {114.07},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AAS...23311407A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bedin17,
       author = {{Bedin}, L.~R. and {Pourbaix}, D. and {Apai}, D. and {Burgasser}, A.~J. and {Buenzli}, E. and {Boffin}, H.~M.~J. and {Libralato}, M.},
        title = "{Hubble Space Telescope astrometry of the closest brown dwarf binary system - I. Overview and improved orbit$^{★}$}",
      journal = {\mnras},
     keywords = {astrometry, binaries: visual, brown dwarfs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = sep,
       volume = {470},
       number = {1},
        pages = {1140-1155},
          doi = {10.1093/mnras/stx1177},
archivePrefix = {arXiv},
       eprint = {1706.00657},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1140B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{biller13,
       author = {{Biller}, Beth A. and {Crossfield}, Ian J.~M. and {Mancini}, Luigi and {Ciceri}, Simona and {Southworth}, John and {Kopytova}, Taisiya G. and {Bonnefoy}, Micka{\"e}l and {Deacon}, Niall R. and {Schlieder}, Joshua E. and {Buenzli}, Esther and {Brandner}, Wolfgang and {Allard}, France and {Homeier}, Derek and {Freytag}, Bernd and {Bailer-Jones}, Coryn A.~L. and {Greiner}, Jochen and {Henning}, Thomas and {Goldman}, Bertrand},
        title = "{Weather on the Nearest Brown Dwarfs: Resolved Simultaneous Multi-wavelength Variability Monitoring of WISE J104915.57-531906.1AB}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {778},
       number = {1},
          eid = {L10},
        pages = {L10},
          doi = {10.1088/2041-8205/778/1/L10},
archivePrefix = {arXiv},
       eprint = {1310.5144},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...778L..10B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{burgasser14,
       author = {{Burgasser}, Adam J. and {Gillon}, Micha{\"e}l and {Faherty}, Jacqueline K. and {Radigan}, Jacqueline and {Triaud}, Amaury H.~M.~J. and {Plavchan}, Peter and {Street}, Rachel and {Jehin}, E. and {Delrez}, L. and {Opitom}, C.},
        title = "{A Monitoring Campaign for Luhman 16AB. I. Detection of Resolved Near-infrared Spectroscopic Variability}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57-531906.1AB Luhman 16AB, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = apr,
       volume = {785},
       number = {1},
          eid = {48},
        pages = {48},
          doi = {10.1088/0004-637X/785/1/48},
archivePrefix = {arXiv},
       eprint = {1402.2342},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...785...48B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hoeijmakers2019,
       author = {{Hoeijmakers}, H.~J. and {Ehrenreich}, D. and {Kitzmann}, D. and
         {Allart}, R. and {Grimm}, S.~L. and {Seidel}, J.~V. and
         {Wyttenbach}, A. and {Pino}, L. and {Nielsen}, L.~D. and {Fisher}, C. and
         {Rimmer}, P.~B. and {Bourrier}, V. and {Cegla}, H.~M. and {Lavie}, B. and
         {Lovis}, C. and {Patzer}, A.~B.~C. and {Stock}, J.~W. and
         {Pepe}, F.~A. and {Heng}, Kevin},
        title = "{A spectral survey of an ultra-hot Jupiter. Detection of metals in the transmission spectrum of KELT-9 b}",
      journal = {\aap},
     keywords = {planets and satellites: gaseous planets, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A165},
        pages = {A165},
          doi = {10.1051/0004-6361/201935089},
archivePrefix = {arXiv},
       eprint = {1905.02096},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A.165H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaudi2017,
       author = {{Gaudi}, B. Scott and {Stassun}, Keivan G. and {Collins}, Karen A. and
         {Beatty}, Thomas G. and {Zhou}, George and {Latham}, David W. and
         {Bieryla}, Allyson and {Eastman}, Jason D. and {Siverd}, Robert J. and
         {Crepp}, Justin R. and {Gonzales}, Erica J. and {Stevens}, Daniel J. and
         {Buchhave}, Lars A. and {Pepper}, Joshua and {Johnson}, Marshall C. and
         {Colon}, Knicole D. and {Jensen}, Eric L.~N. and
         {Rodriguez}, Joseph E. and {Bozza}, Valerio and
         {Novati}, Sebastiano Calchi and {D'Ago}, Giuseppe and
         {Dumont}, Mary T. and {Ellis}, Tyler and {Gaillard}, Clement and
         {Jang-Condell}, Hannah and {Kasper}, David H. and {Fukui}, Akihiko and
         {Gregorio}, Joao and {Ito}, Ayaka and {Kielkopf}, John F. and
         {Manner}, Mark and {Matt}, Kyle and {Narita}, Norio and
         {Oberst}, Thomas E. and {Reed}, Phillip A. and {Scarpetta}, Gaetano and
         {Stephens}, Denice C. and {Yeigh}, Rex R. and {Zambelli}, Roberto and
         {Fulton}, B.~J. and {Howard}, Andrew W. and {James}, David J. and
         {Penny}, Matthew and {Bayliss}, Daniel and {Curtis}, Ivan A. and
         {Depoy}, D.~L. and {Esquerdo}, Gilbert A. and {Gould}, Andrew and
         {Joner}, Michael D. and {Kuhn}, Rudolf B. and
         {Labadie-Bartz}, Jonathan and {Lund}, Michael B. and
         {Marshall}, Jennifer L. and {McLeod}, Kim K. and {Pogge}, Richard W. and
         {Relles}, Howard and {Stockdale}, Christopher and {Tan}, T.~G. and
         {Trueblood}, Mark and {Trueblood}, Patricia},
        title = "{A giant planet undergoing extreme-ultraviolet irradiation by its hot massive-star host}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jun,
       volume = {546},
       number = {7659},
        pages = {514-518},
          doi = {10.1038/nature22392},
archivePrefix = {arXiv},
       eprint = {1706.06723},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Natur.546..514G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lund2017,
       author = {{Lund}, Michael B. and {Rodriguez}, Joseph E. and {Zhou}, George and {Gaudi}, B. Scott and {Stassun}, Keivan G. and {Johnson}, Marshall C. and {Bieryla}, Allyson and {Oelkers}, Ryan J. and {Stevens}, Daniel J. and {Collins}, Karen A. and {Penev}, Kaloyan and {Quinn}, Samuel N. and {Latham}, David W. and {Villanueva}, Steven, Jr. and {Eastman}, Jason D. and {Kielkopf}, John F. and {Oberst}, Thomas E. and {Jensen}, Eric L.~N. and {Cohen}, David H. and {Joner}, Michael D. and {Stephens}, Denise C. and {Relles}, Howard and {Corfini}, Giorgio and {Gregorio}, Joao and {Zambelli}, Roberto and {Esquerdo}, Gilbert A. and {Calkins}, Michael L. and {Berlind}, Perry and {Ciardi}, David R. and {Dressing}, Courtney and {Patel}, Rahul and {Gagnon}, Patrick and {Gonzales}, Erica and {Beatty}, Thomas G. and {Siverd}, Robert J. and {Labadie-Bartz}, Jonathan and {Kuhn}, Rudolf B. and {Col{\'o}n}, Knicole D. and {James}, David and {Pepper}, Joshua and {Fulton}, Benjamin J. and {McLeod}, Kim K. and {Stockdale}, Christopher and {Calchi Novati}, Sebastiano and {DePoy}, D.~L. and {Gould}, Andrew and {Marshall}, Jennifer L. and {Trueblood}, Mark and {Trueblood}, Patricia and {Johnson}, John A. and {Wright}, Jason and {McCrady}, Nate and {Wittenmyer}, Robert A. and {Johnson}, Samson A. and {Sergi}, Anthony and {Wilson}, Maurice and {Sliski}, David H.},
        title = "{KELT-20b: A Giant Planet with a Period of P {\ensuremath{\sim}} 3.5 days Transiting the V {\ensuremath{\sim}} 7.6 Early A Star HD 185603}",
      journal = {\aj},
     keywords = {methods: observational, planets and satellites: detection, planets and satellites: gaseous planets, stars: individual (HD 185603), techniques: photometric, techniques: radial velocities, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = nov,
       volume = {154},
       number = {5},
          eid = {194},
        pages = {194},
          doi = {10.3847/1538-3881/aa8f95},
archivePrefix = {arXiv},
       eprint = {1707.01518},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..194L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Talens2018,
       author = {{Talens}, G.~J.~J. and {Justesen}, A.~B. and {Albrecht}, S. and {McCormac}, J. and {Van Eylen}, V. and {Otten}, G.~P.~P.~L. and {Murgas}, F. and {Palle}, E. and {Pollacco}, D. and {Stuik}, R. and {Spronck}, J.~F.~P. and {Lesage}, A. -L. and {Grundahl}, F. and {Fredslund Andersen}, M. and {Antoci}, V. and {Snellen}, I.~A.~G.},
        title = "{MASCARA-2 b. A hot Jupiter transiting the m$_{V}$ = 7.6 A-star HD 185603}",
      journal = {\aap},
     keywords = {planetary systems, stars: individual: MASCARA-2 (HD 185603, HIP 96618), Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = apr,
       volume = {612},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201731512},
archivePrefix = {arXiv},
       eprint = {1707.01500},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...612A..57T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@book{gray_2005, place={Cambridge}, edition={3}, title={The Observation and Analysis of Stellar Photospheres}, DOI={10.1017/CBO9781316036570}, publisher={Cambridge University Press}, author={Gray, David F.}, year={2005}}

@ARTICLE{Cauley2019,
       author = {{Cauley}, P. Wilson and {Shkolnik}, Evgenya L. and {Ilyin}, Ilya and
         {Strassmeier}, Klaus G. and {Redfield}, Seth and {Jensen}, Adam},
        title = "{Atmospheric Dynamics and the Variable Transit of KELT-9 b}",
      journal = {\aj},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, stars: flare, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {157},
       number = {2},
          eid = {69},
        pages = {69},
          doi = {10.3847/1538-3881/aaf725},
archivePrefix = {arXiv},
       eprint = {1810.05776},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157...69C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{Madhusudhan2018,
       author = {{Madhusudhan}, Nikku},
        title = "{Atmospheric Retrieval of Exoplanets}",
     keywords = {Physics, Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {Handbook of Exoplanets},
         year = 2018,
       editor = {{Deeg}, Hans J. and {Belmonte}, Juan Antonio},
          eid = {104},
        pages = {104},
          doi = {10.1007/978-3-319-55333-7_104},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018haex.bookE.104M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Madhusudhan2019,
       author = {{Madhusudhan}, Nikku},
        title = "{Exoplanetary Atmospheres: Key Insights, Challenges, and Prospects}",
      journal = {\araa},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = aug,
       volume = {57},
        pages = {617-663},
          doi = {10.1146/annurev-astro-081817-051846},
archivePrefix = {arXiv},
       eprint = {1904.03190},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ARA&A..57..617M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2008,
       author = {{Showman}, Adam P. and {Cooper}, Curtis S. and {Fortney}, Jonathan J. and {Marley}, Mark S.},
        title = "{Atmospheric Circulation of Hot Jupiters: Three-dimensional Circulation Models of HD 209458b and HD 189733b with Simplified Forcing}",
      journal = {\apj},
     keywords = {atmospheric effects, methods: numerical, planets and satellites: general, planets and satellites: individual: HD 209458b, Astrophysics},
         year = 2008,
        month = jul,
       volume = {682},
       number = {1},
        pages = {559-576},
          doi = {10.1086/589325},
archivePrefix = {arXiv},
       eprint = {0802.0327},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...682..559S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2011,
       author = {{Showman}, Adam P. and {Polvani}, Lorenzo M.},
        title = "{Equatorial Superrotation on Tidally Locked Exoplanets}",
      journal = {\apj},
     keywords = {hydrodynamics, methods: analytical, methods: numerical, planets and satellites: atmospheres, planets and satellites: individual: HD 189733b, waves, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = sep,
       volume = {738},
       number = {1},
          eid = {71},
        pages = {71},
          doi = {10.1088/0004-637X/738/1/71},
archivePrefix = {arXiv},
       eprint = {1103.3101},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...738...71S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2013,
       author = {{Showman}, Adam P. and {Fortney}, Jonathan J. and {Lewis}, Nikole K. and {Shabram}, Megan},
        title = "{Doppler Signatures of the Atmospheric Circulation on Hot Jupiters}",
      journal = {\apj},
     keywords = {atmospheric effects, hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: general, planets and satellites: individual: HD 189733b HD 209458b GJ 436b, waves, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = jan,
       volume = {762},
       number = {1},
          eid = {24},
        pages = {24},
          doi = {10.1088/0004-637X/762/1/24},
archivePrefix = {arXiv},
       eprint = {1207.5639},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...762...24S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kataria2016,
       author = {{Kataria}, Tiffany and {Sing}, David K. and {Lewis}, Nikole K. and {Visscher}, Channon and {Showman}, Adam P. and {Fortney}, Jonathan J. and {Marley}, Mark S.},
        title = "{The Atmospheric Circulation of a Nine-hot-Jupiter Sample: Probing Circulation and Chemistry over a Wide Phase Space}",
      journal = {\apj},
     keywords = {atmospheric effects, methods: numerical, planets and satellites: general, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = apr,
       volume = {821},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.3847/0004-637X/821/1/9},
archivePrefix = {arXiv},
       eprint = {1602.06733},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...821....9K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wong2020,
       author = {{Wong}, Ian and {Shporer}, Avi and {Kitzmann}, Daniel and {Morris}, Brett M. and {Heng}, Kevin and {Hoeijmakers}, H. Jens and {Demory}, Brice-Olivier and {Ahlers}, John P. and {Mansfield}, Megan and {Bean}, Jacob L. and {Daylan}, Tansu and {Fetherolf}, Tara and {Rodriguez}, Joseph E. and {Benneke}, Bj{\"o}rn and {Ricker}, George R. and {Latham}, David W. and {Vanderspek}, Roland and {Seager}, Sara and {Winn}, Joshua N. and {Jenkins}, Jon M. and {Burke}, Christopher J. and {Christiansen}, Jessie L. and {Essack}, Zahra and {Rose}, Mark E. and {Smith}, Jeffrey C. and {Tenenbaum}, Peter and {Yahalomi}, Daniel},
        title = "{Exploring the Atmospheric Dynamics of the Extreme Ultrahot Jupiter KELT-9b Using TESS Photometry}",
      journal = {\aj},
     keywords = {Hot Jupiters, Photometry, Exoplanet astronomy, 753, 1234, 486, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = aug,
       volume = {160},
       number = {2},
          eid = {88},
        pages = {88},
          doi = {10.3847/1538-3881/aba2cb},
archivePrefix = {arXiv},
       eprint = {1910.01607},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160...88W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Louden2015,
       author = {{Louden}, Tom and {Wheatley}, Peter J.},
        title = "{Spatially Resolved Eastward Winds and Rotation of HD 189733b}",
      journal = {\apjl},
     keywords = {atmospheric effects, celestial mechanics, planets and satellites: atmospheres, planets and satellites: individual: HD 189733b, stars: individual: HD 189733, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = dec,
       volume = {814},
       number = {2},
          eid = {L24},
        pages = {L24},
          doi = {10.1088/2041-8205/814/2/L24},
archivePrefix = {arXiv},
       eprint = {1511.03689},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...814L..24L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brogi2016,
       author = {{Brogi}, M. and {de Kok}, R.~J. and {Albrecht}, S. and {Snellen}, I.~A.~G. and {Birkby}, J.~L. and {Schwarz}, H.},
        title = "{Rotation and Winds of Exoplanet HD 189733 b Measured with High-dispersion Transmission Spectroscopy}",
      journal = {\apj},
     keywords = {planets and satellites: atmospheres, planets and satellites: fundamental parameters, planets and satellites: individual: HD 189733 b, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = feb,
       volume = {817},
       number = {2},
          eid = {106},
        pages = {106},
          doi = {10.3847/0004-637X/817/2/106},
archivePrefix = {arXiv},
       eprint = {1512.05175},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817..106B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Snellen2010,
       author = {{Snellen}, Ignas A.~G. and {de Kok}, Remco J. and {de Mooij}, Ernst J.~W. and {Albrecht}, Simon},
        title = "{The orbital motion, absolute mass and high-altitude winds of exoplanet HD209458b}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jun,
       volume = {465},
       number = {7301},
        pages = {1049-1051},
          doi = {10.1038/nature09111},
archivePrefix = {arXiv},
       eprint = {1006.4364},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.465.1049S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kempton2012,
       author = {{Miller-Ricci Kempton}, Eliza and {Rauscher}, Emily},
        title = "{Constraining High-speed Winds in Exoplanet Atmospheres through Observations of Anomalous Doppler Shifts during Transit}",
      journal = {\apj},
     keywords = {planetary systems, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = jun,
       volume = {751},
       number = {2},
          eid = {117},
        pages = {117},
          doi = {10.1088/0004-637X/751/2/117},
archivePrefix = {arXiv},
       eprint = {1109.2270},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...751..117M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fu2017,
       author = {{Fu}, Guangwei and {Deming}, Drake and {Knutson}, Heather and {Madhusudhan}, Nikku and {Mandell}, Avi and {Fraine}, Jonathan},
        title = "{Statistical Analysis of Hubble/WFC3 Transit Spectroscopy of Extrasolar Planets}",
      journal = {\apjl},
     keywords = {planets and satellites: atmospheres, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = oct,
       volume = {847},
       number = {2},
          eid = {L22},
        pages = {L22},
          doi = {10.3847/2041-8213/aa8e40},
archivePrefix = {arXiv},
       eprint = {1709.07385},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...847L..22F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Crossfield2017,
       author = {{Crossfield}, Ian J.~M. and {Kreidberg}, Laura},
        title = "{Trends in Atmospheric Properties of Neptune-size Exoplanets}",
      journal = {\aj},
     keywords = {eclipses, methods: statistical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = dec,
       volume = {154},
       number = {6},
          eid = {261},
        pages = {261},
          doi = {10.3847/1538-3881/aa9279},
archivePrefix = {arXiv},
       eprint = {1708.00016},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..261C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sheppard2017,
       author = {{Sheppard}, Kyle B. and {Mandell}, Avi M. and {Tamburo}, Patrick and {Gandhi}, Siddharth and {Pinhas}, Arazi and {Madhusudhan}, Nikku and {Deming}, Drake},
        title = "{Evidence for a Dayside Thermal Inversion and High Metallicity for the Hot Jupiter WASP-18b}",
      journal = {\apjl},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: gaseous planets, planets and satellites: individual: WASP-18b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = dec,
       volume = {850},
       number = {2},
          eid = {L32},
        pages = {L32},
          doi = {10.3847/2041-8213/aa9ae9},
archivePrefix = {arXiv},
       eprint = {1711.10491},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...850L..32S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Evans2017,
       author = {{Evans}, Thomas M. and {Sing}, David K. and {Kataria}, Tiffany and {Goyal}, Jayesh and {Nikolov}, Nikolay and {Wakeford}, Hannah R. and {Deming}, Drake and {Marley}, Mark S. and {Amundsen}, David S. and {Ballester}, Gilda E. and {Barstow}, Joanna K. and {Ben-Jaffel}, Lotfi and {Bourrier}, Vincent and {Buchhave}, Lars A. and {Cohen}, Ofer and {Ehrenreich}, David and {Garc{\'\i}a Mu{\~n}oz}, Antonio and {Henry}, Gregory W. and {Knutson}, Heather and {Lavvas}, Panayotis and {Lecavelier Des Etangs}, Alain and {Lewis}, Nikole K. and {L{\'o}pez-Morales}, Mercedes and {Mandell}, Avi M. and {Sanz-Forcada}, Jorge and {Tremblin}, Pascal and {Lupu}, Roxana},
        title = "{An ultrahot gas-giant exoplanet with a stratosphere}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = aug,
       volume = {548},
       number = {7665},
        pages = {58-61},
          doi = {10.1038/nature23266},
archivePrefix = {arXiv},
       eprint = {1708.01076},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Natur.548...58E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haynes2015,
       author = {{Haynes}, Korey and {Mandell}, Avi M. and {Madhusudhan}, Nikku and {Deming}, Drake and {Knutson}, Heather},
        title = "{Spectroscopic Evidence for a Temperature Inversion in the Dayside Atmosphere of Hot Jupiter WASP-33b}",
      journal = {\apj},
     keywords = {eclipses, planetary systems, techniques: photometric, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = jun,
       volume = {806},
       number = {2},
          eid = {146},
        pages = {146},
          doi = {10.1088/0004-637X/806/2/146},
archivePrefix = {arXiv},
       eprint = {1505.01490},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...806..146H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pino2020,
       author = {{Pino}, Lorenzo and {D{\'e}sert}, Jean-Michel and {Brogi}, Matteo and {Malavolta}, Luca and {Wyttenbach}, Aur{\'e}lien and {Line}, Michael and {Hoeijmakers}, Jens and {Fossati}, Luca and {Bonomo}, Aldo Stefano and {Nascimbeni}, Valerio and {Panwar}, Vatsal and {Affer}, Laura and {Benatti}, Serena and {Biazzo}, Katia and {Bignamini}, Andrea and {Borsa}, Franscesco and {Carleo}, Ilaria and {Claudi}, Riccardo and {Cosentino}, Rosario and {Covino}, Elvira and {Damasso}, Mario and {Desidera}, Silvano and {Giacobbe}, Paolo and {Harutyunyan}, Avet and {Lanza}, Antonino Francesco and {Leto}, Giuseppe and {Maggio}, Antonio and {Maldonado}, Jesus and {Mancini}, Luigi and {Micela}, Giuseppina and {Molinari}, Emilio and {Pagano}, Isabella and {Piotto}, Giampaolo and {Poretti}, Ennio and {Rainer}, Monica and {Scandariato}, Gaetano and {Sozzetti}, Alessandro and {Allart}, Romain and {Borsato}, Luca and {Bruno}, Giovanni and {Di Fabrizio}, Luca and {Ehrenreich}, David and {Fiorenzano}, Aldo and {Frustagli}, Giuseppe and {Lavie}, Baptiste and {Lovis}, Christophe and {Magazz{\`u}}, Antonio and {Nardiello}, Domenico and {Pedani}, Marco and {Smareglia}, Riccardo},
        title = "{Neutral Iron Emission Lines from the Dayside of KELT-9b: The GAPS Program with HARPS-N at TNG XX}",
      journal = {\apjl},
     keywords = {487, 2021, 2096, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = may,
       volume = {894},
       number = {2},
          eid = {L27},
        pages = {L27},
          doi = {10.3847/2041-8213/ab8c44},
archivePrefix = {arXiv},
       eprint = {2004.11335},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...894L..27P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nugroho2017,
       author = {{Nugroho}, Stevanus K. and {Kawahara}, Hajime and {Masuda}, Kento and {Hirano}, Teruyuki and {Kotani}, Takayuki and {Tajitsu}, Akito},
        title = "{High-resolution Spectroscopic Detection of TiO and a Stratosphere in the Day-side of WASP-33b}",
      journal = {\aj},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: individual (WASP-33b), techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = dec,
       volume = {154},
       number = {6},
          eid = {221},
        pages = {221},
          doi = {10.3847/1538-3881/aa9433},
archivePrefix = {arXiv},
       eprint = {1710.05276},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..221N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier2015,
       author = {{Strassmeier}, K.~G. and {Ilyin}, I. and {J{\"a}rvinen}, A. and {Weber}, M. and {Woche}, M. and {Barnes}, S.~I. and {Bauer}, S. -M. and {Beckert}, E. and {Bittner}, W. and {Bredthauer}, R. and {Carroll}, T.~A. and {Denker}, C. and {Dionies}, F. and {DiVarano}, I. and {D{\"o}scher}, D. and {Fechner}, T. and {Feuerstein}, D. and {Granzer}, T. and {Hahn}, T. and {Harnisch}, G. and {Hofmann}, A. and {Lesser}, M. and {Paschke}, J. and {Pankratow}, S. and {Plank}, V. and {Pl{\"u}schke}, D. and {Popow}, E. and {Sablowski}, D.},
        title = "{PEPSI: The high-resolution {\'e}chelle spectrograph and polarimeter for the Large Binocular Telescope}",
      journal = {Astronomische Nachrichten},
     keywords = {instrumentation: spectrographs, instrumentation: polarimeters, instrumentation: detectors, techniques: spectroscopic, stars: individual (HD 194937, {\ensuremath{\tau}} Cet, {\ensuremath{\alpha}} Cyg), Sun: photosphere, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = may,
       volume = {336},
       number = {4},
        pages = {324},
          doi = {10.1002/asna.201512172},
archivePrefix = {arXiv},
       eprint = {1505.06492},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AN....336..324S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kochukhov2010,
       author = {{Kochukhov}, O. and {Makaganiuk}, V. and {Piskunov}, N.},
        title = "{Least-squares deconvolution of the stellar intensity and polarization spectra}",
      journal = {\aap},
     keywords = {magnetic fields, line: formation, polarization, stars: atmospheres, methods: data analysis, methods: numerical, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = dec,
       volume = {524},
          eid = {A5},
        pages = {A5},
          doi = {10.1051/0004-6361/201015429},
archivePrefix = {arXiv},
       eprint = {1008.5115},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...524A...5K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Borsa2019,
       author = {{Borsa}, F. and {Rainer}, M. and {Bonomo}, A.~S. and {Barbato}, D. and {Fossati}, L. and {Malavolta}, L. and {Nascimbeni}, V. and {Lanza}, A.~F. and {Esposito}, M. and {Affer}, L. and {Andreuzzi}, G. and {Benatti}, S. and {Biazzo}, K. and {Bignamini}, A. and {Brogi}, M. and {Carleo}, I. and {Claudi}, R. and {Cosentino}, R. and {Covino}, E. and {Damasso}, M. and {Desidera}, S. and {Garrido Rubio}, A. and {Giacobbe}, P. and {Gonz{\'a}lez-{\'A}lvarez}, E. and {Harutyunyan}, A. and {Knapic}, C. and {Leto}, G. and {Ligi}, R. and {Maggio}, A. and {Maldonado}, J. and {Mancini}, L. and {Fiorenzano}, A.~F.~M. and {Masiero}, S. and {Micela}, G. and {Molinari}, E. and {Pagano}, I. and {Pedani}, M. and {Piotto}, G. and {Pino}, L. and {Poretti}, E. and {Scandariato}, G. and {Smareglia}, R. and {Sozzetti}, A.},
        title = "{The GAPS Programme with HARPS-N at TNG. XIX. Atmospheric Rossiter-McLaughlin effect and improved parameters of KELT-9b}",
      journal = {\aap},
     keywords = {planetary systems, techniques: spectroscopic, techniques: radial velocities, planets and satellites: atmospheres, stars: individual: KELT-9, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = nov,
       volume = {631},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201935718},
archivePrefix = {arXiv},
       eprint = {1907.10078},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...631A..34B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tan2019,
       author = {{Tan}, Xianyu and {Komacek}, Thaddeus D.},
        title = "{The Atmospheric Circulation of Ultra-hot Jupiters}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Hot Jupiters, Hydrodynamics, 753, 487, 1963, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = nov,
       volume = {886},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/ab4a76},
archivePrefix = {arXiv},
       eprint = {1910.01622},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886...26T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Roth2021,
       author = {{Roth}, A. and {Drummond}, B. and {H{\'e}brard}, E. and {Tremblin}, P. and {Goyal}, J. and {Mayne}, N.},
        title = "{Pseudo-2D modelling of heat redistribution through H$_{2}$ thermal dissociation/recombination: Consequences for ultra-hot jupiters}",
      journal = {\mnras},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = may,
          doi = {10.1093/mnras/stab1256},
archivePrefix = {arXiv},
       eprint = {2104.14376},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.tmp.1239R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Casasayas-Barris2019,
       author = {{Casasayas-Barris}, N. and {Pall{\'e}}, E. and {Yan}, F. and {Chen}, G. and {Kohl}, S. and {Stangret}, M. and {Parviainen}, H. and {Helling}, Ch. and {Watanabe}, N. and {Czesla}, S. and {Fukui}, A. and {Monta{\~n}{\'e}s-Rodr{\'\i}guez}, P. and {Nagel}, E. and {Narita}, N. and {Nortmann}, L. and {Nowak}, G. and {Schmitt}, J.~H.~M.~M. and {Zapatero Osorio}, M.~R.},
        title = "{Atmospheric characterization of the ultra-hot Jupiter MASCARA-2b/KELT-20b. Detection of Ca II, Fe II, Na I, and the Balmer series of H (H{\ensuremath{\alpha}}, H{\ensuremath{\beta}}, and H{\ensuremath{\gamma}}) with high-dispersion transit spectroscopy (Corrigendum)}",
      journal = {\aap},
     keywords = {planetary systems, methods: observational, techniques: spectroscopic, planets and satellites: individual: MASCARA-2b, planets and satellites: individual: KELT-20b - errata, addenda},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {C6},
        pages = {C6},
          doi = {10.1051/0004-6361/201935623e},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640C...6C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2017,
       author = {{Yan}, F. and {Pall{\'e}}, E. and {Fosbury}, R.~A.~E. and {Petr-Gotzens}, M.~G. and {Henning}, Th.},
        title = "{Effect of the stellar absorption line centre-to-limb variation on exoplanet transmission spectrum observations}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, techniques: spectroscopic, stars: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jul,
       volume = {603},
          eid = {A73},
        pages = {A73},
          doi = {10.1051/0004-6361/201630144},
archivePrefix = {arXiv},
       eprint = {1703.07585},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...603A..73Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Yan2015,
       author = {{Yan}, F. and {Fosbury}, R.~A.~E. and {Petr-Gotzens}, M.~G. and {Zhao}, G. and {Pall{\'e}}, E.},
        title = "{The centre-to-limb variations of solar Fraunhofer lines imprinted upon lunar eclipse spectra. Implications for exoplanet transit observations}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, Earth, Moon, eclipses, stars: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {574},
          eid = {A94},
        pages = {A94},
          doi = {10.1051/0004-6361/201425220},
archivePrefix = {arXiv},
       eprint = {1501.02306},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...574A..94Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2018,
       author = {{Yan}, Fei and {Henning}, Thomas},
        title = "{An extended hydrogen envelope of the extremely hot giant exoplanet KELT-9b}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = jul,
       volume = {2},
        pages = {714-718},
          doi = {10.1038/s41550-018-0503-3},
archivePrefix = {arXiv},
       eprint = {1807.00869},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..714Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2019,
       author = {{Yan}, F. and {Casasayas-Barris}, N. and {Molaverdikhani}, K. and {Alonso-Floriano}, F.~J. and {Reiners}, A. and {Pall{\'e}}, E. and {Henning}, Th. and {Molli{\`e}re}, P. and {Chen}, G. and {Nortmann}, L. and {Snellen}, I.~A.~G. and {Ribas}, I. and {Quirrenbach}, A. and {Caballero}, J.~A. and {Amado}, P.~J. and {Azzaro}, M. and {Bauer}, F.~F. and {Cort{\'e}s Contreras}, M. and {Czesla}, S. and {Khalafinejad}, S. and {Lara}, L.~M. and {L{\'o}pez-Puertas}, M. and {Montes}, D. and {Nagel}, E. and {Oshagh}, M. and {S{\'a}nchez-L{\'o}pez}, A. and {Stangret}, M. and {Zechmeister}, M.},
        title = "{Ionized calcium in the atmospheres of two ultra-hot exoplanets WASP-33b and KELT-9b}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, techniques: spectroscopic, planets and satellites: individual: WASP-33b, planets and satellites: individual: KELT-9b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = dec,
       volume = {632},
          eid = {A69},
        pages = {A69},
          doi = {10.1051/0004-6361/201936396},
archivePrefix = {arXiv},
       eprint = {1911.00380},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...632A..69Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyttenbach2020,
       author = {{Wyttenbach}, A. and {Molli{\`e}re}, P. and {Ehrenreich}, D. and {Cegla}, H.~M. and {Bourrier}, V. and {Lovis}, C. and {Pino}, L. and {Allart}, R. and {Seidel}, J.~V. and {Hoeijmakers}, H.~J. and {Nielsen}, L.~D. and {Lavie}, B. and {Pepe}, F. and {Bonfils}, X. and {Snellen}, I.~A.~G.},
        title = "{Mass-loss rate and local thermodynamic state of the KELT-9 b thermosphere from the hydrogen Balmer series}",
      journal = {\aap},
     keywords = {planetary systems, planets and satellites: atmospheres, planets and satellites: individual: KELT-9 b, techniques: spectroscopic, instrumentation: spectrographs, methods: observational, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jun,
       volume = {638},
          eid = {A87},
        pages = {A87},
          doi = {10.1051/0004-6361/201937316},
archivePrefix = {arXiv},
       eprint = {2004.13733},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...638A..87W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Faigler2011,
       author = {{Faigler}, S. and {Mazeh}, T.},
        title = "{Photometric detection of non-transiting short-period low-mass companions through the beaming, ellipsoidal and reflection effects in Kepler and CoRoT light curves}",
      journal = {\mnras},
     keywords = {methods: data analysis, binaries: eclipsing, binaries: general, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = aug,
       volume = {415},
       number = {4},
        pages = {3921-3928},
          doi = {10.1111/j.1365-2966.2011.19011.x},
archivePrefix = {arXiv},
       eprint = {1106.2713},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.415.3921F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eastman2010,
       author = {{Eastman}, Jason and {Siverd}, Robert and {Gaudi}, B. Scott},
        title = "{Achieving Better Than 1 Minute Accuracy in the Heliocentric and Barycentric Julian Dates}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = aug,
       volume = {122},
       number = {894},
        pages = {935},
          doi = {10.1086/655938},
archivePrefix = {arXiv},
       eprint = {1005.4415},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010PASP..122..935E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Eastman2012,
       author = {{Eastman}, Jason},
        title = "{Time Utilities}",
     keywords = {Software},
         year = 2012,
        month = jun,
          eid = {ascl:1206.012},
        pages = {ascl:1206.012},
archivePrefix = {ascl},
       eprint = {1206.012},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ascl.soft06012E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eastman2019,
       author = {{Eastman}, Jason D. and {Rodriguez}, Joseph E. and {Agol}, Eric and {Stassun}, Keivan G. and {Beatty}, Thomas G. and {Vanderburg}, Andrew and {Gaudi}, B. Scott and {Collins}, Karen A. and {Luger}, Rodrigo},
        title = "{EXOFASTv2: A public, generalized, publication-quality exoplanet modeling code}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jul,
          eid = {arXiv:1907.09480},
        pages = {arXiv:1907.09480},
archivePrefix = {arXiv},
       eprint = {1907.09480},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190709480E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Claret2017,
       author = {{Claret}, A.},
        title = "{Limb and gravity-darkening coefficients for the TESS satellite at several metallicities, surface gravities, and microturbulent velocities}",
      journal = {\aap},
     keywords = {planetary systems, stars: atmospheres, binaries: eclipsing, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {600},
          eid = {A30},
        pages = {A30},
          doi = {10.1051/0004-6361/201629705},
archivePrefix = {arXiv},
       eprint = {1804.10295},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...600A..30C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beltz2021a,
       author = {{Beltz}, Hayley and {Rauscher}, Emily and {Brogi}, Matteo and {Kempton}, Eliza M. -R.},
        title = "{A Significant Increase in Detection of High-resolution Emission Spectra Using a Three-dimensional Atmospheric Model of a Hot Jupiter}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, High resolution spectroscopy, Hot Jupiters, Hydrodynamical simulations, Radiative transfer simulations, 487, 2096, 753, 767, 1967, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jan,
       volume = {161},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.3847/1538-3881/abb67b},
archivePrefix = {arXiv},
       eprint = {2009.09030},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Donatelli2014,
title = {Square smoothing regularization matrices with accurate boundary conditions},
journal = {Journal of Computational and Applied Mathematics},
volume = {272},
pages = {334-349},
year = {2014},
issn = {0377-0427},
doi = {https://doi.org/10.1016/j.cam.2013.08.015},
url = {https://www.sciencedirect.com/science/article/pii/S0377042713004202},
author = {M. Donatelli and L. Reichel},
keywords = {Tikhonov regularization, Regularization matrix, Boundary conditions},
abstract = {This paper is concerned with the solution of large-scale linear discrete ill-posed problems. The determination of a meaningful approximate solution of these problems requires regularization. We discuss regularization by the Tikhonov method and by truncated iteration. The choice of regularization matrix in Tikhonov regularization may significantly affect the quality of the computed approximate solution. The present paper describes the construction of square regularization matrices from finite difference equations with a focus on the boundary conditions. The regularization matrices considered have a structure that makes them easy to apply in iterative methods, including methods based on the Arnoldi process. Numerical examples illustrate the properties and effectiveness of the regularization matrices described.}
}

@ARTICLE{Donati1997,
       author = {{Donati}, J. -F. and {Semel}, M. and {Carter}, B.~D. and {Rees}, D.~E. and {Collier Cameron}, A.},
        title = "{Spectropolarimetric observations of active stars}",
      journal = {\mnras},
     keywords = {Stellar Spectra, Polarimetry, Stellar Atmospheres, Astronomical Spectroscopy, Late Stars, Astronomy, LINE: PROFILES, POLARIZATION, STARS: ACTIVITY, STARS: ATMOSPHERES, STARS: LATE-TYPE, STARS: MAGNETIC FIELDS},
         year = 1997,
        month = nov,
       volume = {291},
       number = {4},
        pages = {658-682},
          doi = {10.1093/mnras/291.4.658},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997MNRAS.291..658D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Molliere2019,
       author = {{Molli{\`e}re}, P. and {Wardenier}, J.~P. and {van Boekel}, R. and {Henning}, Th. and {Molaverdikhani}, K. and {Snellen}, I.~A.~G.},
        title = "{petitRADTRANS. A Python radiative transfer package for exoplanet characterization and retrieval}",
      journal = {\aap},
     keywords = {methods: numerical, planets and satellites: atmospheres, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/201935470},
archivePrefix = {arXiv},
       eprint = {1904.11504},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A..67M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{Palme2014,
       author = {{Palme}, H. and {Lodders}, K. and {Jones}, A.},
        title = "{Solar System Abundances of the Elements}",
    booktitle = {Planets, Asteriods, Comets and The Solar System},
         year = 2014,
       editor = {{Davis}, Andrew M.},
       volume = {2},
        pages = {15-36},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014pacs.book...15P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Pakhomov2017,
       author = {{Pakhomov}, Yu. and {Piskunov}, N. and {Ryabchikova}, T.},
        title = "{VALD3: Current Developments}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Stars: From Collapse to Collapse},
         year = 2017,
       editor = {{Balega}, Yu. Yu. and {Kudryavtsev}, D.~O. and {Romanyuk}, I.~I. and {Yakunin}, I.~A.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {510},
        month = jun,
        pages = {518},
archivePrefix = {arXiv},
       eprint = {1710.10854},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ASPC..510..518P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Valenti2012,
       author = {{Valenti}, J.~A. and {Piskunov}, N.},
        title = "{SME: Spectroscopy Made Easy}",
     keywords = {Software},
         year = 2012,
        month = feb,
          eid = {ascl:1202.013},
        pages = {ascl:1202.013},
archivePrefix = {ascl},
       eprint = {1202.013},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ascl.soft02013V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Valenti1996,
       author = {{Valenti}, J.~A. and {Piskunov}, N.},
        title = "{Spectroscopy made easy: A new tool for fitting observations with synthetic spectra.}",
      journal = {\aaps},
     keywords = {RADIATIVE TRANSFER, METHODS: NUMERICAL, TECHNIQUES: SPECTROSCOPIC, STARS: FUNDAMENTAL PARAMETERS, SUN: FUNDAMENTAL PARAMETERS, ATOMIC DATA},
         year = 1996,
        month = sep,
       volume = {118},
        pages = {595-603},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..118..595V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CollierCameron2010,
       author = {{Collier Cameron}, A. and {Bruce}, V.~A. and {Miller}, G.~R.~M. and {Triaud}, A.~H.~M.~J. and {Queloz}, D.},
        title = "{Line-profile tomography of exoplanet transits - I. The Doppler shadow of HD 189733b}",
      journal = {\mnras},
     keywords = {techniques: spectroscopic, stars: activity, binaries: eclipsing, planetary systems, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = mar,
       volume = {403},
       number = {1},
        pages = {151-158},
          doi = {10.1111/j.1365-2966.2009.16131.x},
archivePrefix = {arXiv},
       eprint = {0911.5361},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.403..151C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Foreman-Mackey2013,
       author = {{Foreman-Mackey}, Daniel and {Hogg}, David W. and {Lang}, Dustin and {Goodman}, Jonathan},
        title = "{emcee: The MCMC Hammer}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Computational Physics, Statistics - Computation},
         year = 2013,
        month = mar,
       volume = {125},
       number = {925},
        pages = {306},
          doi = {10.1086/670067},
archivePrefix = {arXiv},
       eprint = {1202.3665},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PASP..125..306F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seager2003,
       author = {{Seager}, S. and {Mall{\'e}n-Ornelas}, G.},
        title = "{A Unique Solution of Planet and Star Parameters from an Extrasolar Planet Transit Light Curve}",
      journal = {\apj},
     keywords = {Stars: Binaries: Eclipsing, Stars: Planetary Systems, Techniques: Photometric, Astrophysics},
         year = 2003,
        month = mar,
       volume = {585},
       number = {2},
        pages = {1038-1055},
          doi = {10.1086/346105},
archivePrefix = {arXiv},
       eprint = {astro-ph/0206228},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...585.1038S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Torres2010,
       author = {{Torres}, G. and {Andersen}, J. and {Gim{\'e}nez}, A.},
        title = "{Accurate masses and radii of normal stars: modern results and applications}",
      journal = {\aapr},
     keywords = {Stars: fundamental parameters, Stars: binaries: eclipsing, Stars: binaries: spectroscopic, Stars: interiors, Stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = feb,
       volume = {18},
       number = {1-2},
        pages = {67-126},
          doi = {10.1007/s00159-009-0025-1},
archivePrefix = {arXiv},
       eprint = {0908.2624},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&ARv..18...67T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tayar2020,
       author = {{Tayar}, Jamie and {Claytor}, Zachary R. and {Huber}, Daniel and {van Saders}, Jennifer},
        title = "{A Guide to Realistic Uncertainties on Fundamental Properties of Solar-Type Exoplanet Host Stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.07957},
        pages = {arXiv:2012.07957},
archivePrefix = {arXiv},
       eprint = {2012.07957},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201207957T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RodriguezMartinez2021,
       author = {{Rodriguez Martinez}, Romy and {Stevens}, Daniel J. and {Gaudi}, B. Scott and {Schulze}, Joseph G. and {Panero}, Wendy R. and {Johnson}, Jennifer A. and {Wang}, Ji},
        title = "{Analytic Estimates of the Achievable Precision on the Physical Properties of Transiting Planets Using Purely Empirical Measurements}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jan,
          eid = {arXiv:2101.09289},
        pages = {arXiv:2101.09289},
archivePrefix = {arXiv},
       eprint = {2101.09289},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210109289R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ahlers2020,
       author = {{Ahlers}, John P. and {Johnson}, Marshall C. and {Stassun}, Keivan G. and {Col{\'o}n}, Knicole D. and {Barnes}, Jason W. and {Stevens}, Daniel J. and {Beatty}, Thomas and {Gaudi}, B. Scott and {Collins}, Karen A. and {Rodriguez}, Joseph E. and {Ricker}, George and {Vanderspek}, Roland and {Latham}, David and {Seager}, Sara and {Winn}, Joshua and {Jenkins}, Jon M. and {Caldwell}, Douglas A. and {Goeke}, Robert F. and {Osborn}, Hugh P. and {Paegert}, Martin and {Rowden}, Pam and {Tenenbaum}, Peter},
        title = "{KELT-9 b's Asymmetric TESS Transit Caused by Rapid Stellar Rotation and Spin-Orbit Misalignment}",
      journal = {\aj},
     keywords = {Exoplanets, Hot Jupiters, Exoplanet evolution, Stellar rotation, Gravity darkening, von Zeipel theorem, Exoplanet astronomy, Transit photometry, 1709, 498, 491, 1781, 680, 1629, 486, 753, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {160},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.3847/1538-3881/ab8fa3},
archivePrefix = {arXiv},
       eprint = {2004.14812},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160....4A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Loeb2003,
       author = {{Loeb}, Abraham and {Gaudi}, B. Scott},
        title = "{Periodic Flux Variability of Stars due to the Reflex Doppler Effect Induced by Planetary Companions}",
      journal = {\apjl},
     keywords = {Stars: Planetary Systems, Techniques: Photometric, Astrophysics},
         year = 2003,
        month = may,
       volume = {588},
       number = {2},
        pages = {L117-L120},
          doi = {10.1086/375551},
archivePrefix = {arXiv},
       eprint = {astro-ph/0303212},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...588L.117L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Giacobbe2021,
       author = {{Giacobbe}, Paolo and {Brogi}, Matteo and {Gandhi}, Siddharth and {Cubillos}, Patricio E. and {Bonomo}, Aldo S. and {Sozzetti}, Alessandro and {Fossati}, Luca and {Guilluy}, Gloria and {Carleo}, Ilaria and {Rainer}, Monica and {Harutyunyan}, Avet and {Borsa}, Francesco and {Pino}, Lorenzo and {Nascimbeni}, Valerio and {Benatti}, Serena and {Biazzo}, Katia and {Bignamini}, Andrea and {Chubb}, Katy L. and {Claudi}, Riccardo and {Cosentino}, Rosario and {Covino}, Elvira and {Damasso}, Mario and {Desidera}, Silvano and {Fiorenzano}, Aldo F.~M. and {Ghedina}, Adriano and {Lanza}, Antonino F. and {Leto}, Giuseppe and {Maggio}, Antonio and {Malavolta}, Luca and {Maldonado}, Jesus and {Micela}, Giuseppina and {Molinari}, Emilio and {Pagano}, Isabella and {Pedani}, Marco and {Piotto}, Giampaolo and {Poretti}, Ennio and {Scandariato}, Gaetano and {Yurchenko}, Sergei N. and {Fantinel}, Daniela and {Galli}, Alberto and {Lodi}, Marcello and {Sanna}, Nicoletta and {Tozzi}, Andrea},
        title = "{Five carbon- and nitrogen-bearing species in a hot giant planet's atmosphere}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
          eid = {arXiv:2104.03352},
        pages = {arXiv:2104.03352},
archivePrefix = {arXiv},
       eprint = {2104.03352},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210403352G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Murray-Clay2009,
       author = {{Murray-Clay}, Ruth A. and {Chiang}, Eugene I. and {Murray}, Norman},
        title = "{Atmospheric Escape From Hot Jupiters}",
      journal = {\apj},
     keywords = {hydrodynamics, planetary systems, stars: individual: HD 209458, Astrophysics},
         year = 2009,
        month = mar,
       volume = {693},
       number = {1},
        pages = {23-42},
          doi = {10.1088/0004-637X/693/1/23},
archivePrefix = {arXiv},
       eprint = {0811.0006},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...693...23M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GarciaMunoz2019,
       author = {{Garc{\'\i}a Mu{\~n}oz}, A. and {Schneider}, P.~C.},
        title = "{Rapid Escape of Ultra-hot Exoplanet Atmospheres Driven by Hydrogen Balmer Absorption}",
      journal = {\apjl},
     keywords = {Exoplanet atmospheres, Aeronomy, Exoplanet evolution, Radiative transfer, 487, 22, 491, 1335, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = oct,
       volume = {884},
       number = {2},
          eid = {L43},
        pages = {L43},
          doi = {10.3847/2041-8213/ab498d},
archivePrefix = {arXiv},
       eprint = {1910.00267},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884L..43G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Erkaev2007,
       author = {{Erkaev}, N.~V. and {Kulikov}, Yu. N. and {Lammer}, H. and {Selsis}, F. and {Langmayr}, D. and {Jaritz}, G.~F. and {Biernat}, H.~K.},
        title = "{Roche lobe effects on the atmospheric loss from ``Hot Jupiters''}",
      journal = {\aap},
     keywords = {hydrodynamics, atmospheric effects, stars: activity, planets and satellites: general, Astrophysics},
         year = 2007,
        month = sep,
       volume = {472},
       number = {1},
        pages = {329-334},
          doi = {10.1051/0004-6361:20066929},
archivePrefix = {arXiv},
       eprint = {astro-ph/0612729},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...472..329E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krenn2021,
       author = {{Krenn}, Andreas F. and {Fossati}, Luca and {Kubyshkina}, Daria and {Lammer}, Helmut},
        title = "{A critical assessment of the applicability of the energy-limited approximation for estimating exoplanetary mass-loss rates}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.05858},
        pages = {arXiv:2105.05858},
archivePrefix = {arXiv},
       eprint = {2105.05858},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210505858K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kubyshkina2018,
       author = {{Kubyshkina}, D. and {Fossati}, L. and {Erkaev}, N.~V. and {Cubillos}, P.~E. and {Johnstone}, C.~P. and {Kislyakova}, K.~G. and {Lammer}, H. and {Lendl}, M. and {Odert}, P.},
        title = "{Overcoming the Limitations of the Energy-limited Approximation for Planet Atmospheric Escape}",
      journal = {\apjl},
     keywords = {planets and satellites: atmospheres, planets and satellites: gaseous planets, planets and satellites: general, planets and satellites: physical evolution, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = oct,
       volume = {866},
       number = {2},
          eid = {L18},
        pages = {L18},
          doi = {10.3847/2041-8213/aae586},
archivePrefix = {arXiv},
       eprint = {1810.06920},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...866L..18K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanz-Forcada2011,
       author = {{Sanz-Forcada}, J. and {Micela}, G. and {Ribas}, I. and {Pollock}, A.~M.~T. and {Eiroa}, C. and {Velasco}, A. and {Solano}, E. and {Garc{\'\i}a-{\'A}lvarez}, D.},
        title = "{Estimation of the XUV radiation onto close planets and their evaporation}",
      journal = {\aap},
     keywords = {planetary systems, stars: coronae, astrobiology, X-rays: stars, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = aug,
       volume = {532},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201116594},
archivePrefix = {arXiv},
       eprint = {1105.0550},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...532A...6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia2016,
       author = {{Gaia Collaboration} and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Milligan}, D.~J. and {Panem}, C. and {Poinsignon}, V. and {Pourbaix}, D. and {Randich}, S. and {Sarri}, G. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Valette}, V. and {van Leeuwen}, F. and {Walton}, N.~A. and {Aerts}, C. and {Arenou}, F. and {Cropper}, M. and {Drimmel}, R. and {H{\o}g}, E. and {Katz}, D. and {Lattanzi}, M.~G. and {O'Mullane}, W. and {Grebel}, E.~K. and {Holland}, A.~D. and {Huc}, C. and {Passot}, X. and {Bramante}, L. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Hern{\'a}ndez}, J. and {Jean-Antoine-Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Panuzzo}, P. and {Portell}, J. and {Richards}, P.~J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Torra}, J. and {Els}, S.~G. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Lock}, T. and {Mercier}, E. and {Altmann}, M. and {Andrae}, R. and {Astraatmadja}, T.~L. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Cowell}, S. and {Creevey}, O. and {Cuypers}, J. and {Davidson}, M. and {De Ridder}, J. and {de Torres}, A. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fr{\'e}mat}, Y. and {Garc{\'\i}a-Torres}, M. and {Gosset}, E. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hauser}, M. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Huckle}, H.~E. and {Hutton}, A. and {Jasniewicz}, G. and {Jordan}, S. and {Kontizas}, M. and {Korn}, A.~J. and {Lanzafame}, A.~C. and {Manteiga}, M. and {Moitinho}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Smith}, K.~W. and {Sozzetti}, A. and {Thuillot}, W. and {van Reeven}, W. and {Viala}, Y. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aguado}, J.~J. and {Allan}, P.~M. and {Allasia}, W. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Ant{\'o}n}, S. and {Arcay}, B. and {Atzei}, A. and {Ayache}, L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Barache}, C. and {Barata}, C. and {Barbier}, A. and {Barblan}, F. and {Baroni}, M. and {Barrado y Navascu{\'e}s}, D. and {Barros}, M. and {Barstow}, M.~A. and {Becciani}, U. and {Bellazzini}, M. and {Bellei}, G. and {Bello Garc{\'\i}a}, A. and {Belokurov}, V. and {Bendjoya}, P. and {Berihuete}, A. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Billebaud}, F. and {Blagorodnova}, N. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bouy}, H. and {Bragaglia}, A. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Bucciarelli}, B. and {Budnik}, F. and {Burgess}, P. and {Burgon}, R. and {Burlacu}, A. and {Busonero}, D. and {Buzzi}, R. and {Caffau}, E. and {Cambras}, J. and {Campbell}, H. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carlucci}, T. and {Carrasco}, J.~M. and {Castellani}, M. and {Charlot}, P. and {Charnas}, J. and {Charvet}, P. and {Chassat}, F. and {Chiavassa}, A. and {Clotet}, M. and {Cocozza}, G. and {Collins}, R.~S. and {Collins}, P. and {Costigan}, G. and {Crifo}, F. and {Cross}, N.~J.~G. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {De Cat}, P. and {de Felice}, F. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {di Marco}, F. and {Di Matteo}, P. and {Diakite}, S. and {Distefano}, E. and {Dolding}, C. and {Dos Anjos}, S. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Dzigan}, Y. and {Ecale}, E. and {Edvardsson}, B. and {Enke}, H. and {Erdmann}, M. and {Escolar}, D. and {Espina}, M. and {Evans}, N.~W. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Faye}, F. and {Federici}, L. and {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fouesneau}, M. and {Fraile}, E. and {Fraser}, M. and {Fuchs}, J. and {Furnell}, R. and {Gai}, M. and {Galleti}, S. and {Galluccio}, L. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Gar{\'e}}, P. and {Garofalo}, A. and {Garralda}, N. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guerrier}, A. and {Guillout}, P. and {Guiraud}, J. and {G{\'u}rpide}, A. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Haigron}, R. and {Hatzidimitriou}, D. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Hobbs}, D. and {Hofmann}, W. and {Holl}, B. and {Holland}, G. and {Hunt}, J.~A.~S. and {Hypki}, A. and {Icardi}, V. and {Irwin}, M. and {Jevardat de Fombelle}, G. and {Jofr{\'e}}, P. and {Jonker}, P.~G. and {Jorissen}, A. and {Julbe}, F. and {Karampelas}, A. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Koubsky}, P. and {Kowalczyk}, A. and {Krone-Martins}, A. and {Kudryashova}, M. and {Kull}, I. and {Bachchan}, R.~K. and {Lacoste-Seris}, F. and {Lanza}, A.~F. and {Lavigne}, J. -B. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lemaitre}, V. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\"o}ffler}, W. and {L{\'o}pez}, M. and {Lopez-Lozano}, A. and {Lorenz}, D. and {Loureiro}, T. and {MacDonald}, I. and {Magalh{\~a}es Fernandes}, T. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marie}, J. and {Marinoni}, S. and {Marrese}, P.~M. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Mart{\'\i}n-Fleitas}, J.~M. and {Martino}, M. and {Mary}, N. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Mestre}, A. and {Michalik}, D. and {Millar}, N.~R. and {Miranda}, B.~M.~H. and {Molina}, D. and {Molinaro}, R. and {Molinaro}, M. and {Moln{\'a}r}, L. and {Moniez}, M. and {Montegriffo}, P. and {Monteiro}, D. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morley}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Narbonne}, J. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {Ord{\'e}novic}, C. and {Ordieres-Mer{\'e}}, J. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Parsons}, P. and {Paulsen}, T. and {Pecoraro}, M. and {Pedrosa}, R. and {Pentik{\"a}inen}, H. and {Pereira}, J. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Ragaini}, S. and {Rago}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Ranalli}, P. and {Rauw}, G. and {Read}, A. and {Regibo}, S. and {Renk}, F. and {Reyl{\'e}}, C. and {Ribeiro}, R.~A. and {Rimoldini}, L. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rudolph}, A. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sarasso}, M. and {Savietto}, H. and {Schnorhk}, A. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {Segransan}, D. and {Serpell}, E. and {Shih}, I. -C. and {Smareglia}, R. and {Smart}, R.~L. and {Smith}, C. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Tingley}, B. and {Trager}, S.~C. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Valentini}, G. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Varadi}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Via}, T. and {Vicente}, D. and {Vogt}, S. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Weingrill}, K. and {Werner}, D. and {Wevers}, T. and {Whitehead}, G. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T. and {Alecu}, A. and {Allen}, M. and {Allende Prieto}, C. and {Amorim}, A. and {Anglada-Escud{\'e}}, G. and {Arsenijevic}, V. and {Azaz}, S. and {Balm}, P. and {Beck}, M. and {Bernstein}, H. -H. and {Bigot}, L. and {Bijaoui}, A. and {Blasco}, C. and {Bonfigli}, M. and {Bono}, G. and {Boudreault}, S. and {Bressan}, A. and {Brown}, S. and {Brunet}, P. -M. and {Bunclark}, P. and {Buonanno}, R. and {Butkevich}, A.~G. and {Carret}, C. and {Carrion}, C. and {Chemin}, L. and {Ch{\'e}reau}, F. and {Corcione}, L. and {Darmigny}, E. and {de Boer}, K.~S. and {de Teodoro}, P. and {de Zeeuw}, P.~T. and {Delle Luche}, C. and {Domingues}, C.~D. and {Dubath}, P. and {Fodor}, F. and {Fr{\'e}zouls}, B. and {Fries}, A. and {Fustes}, D. and {Fyfe}, D. and {Gallardo}, E. and {Gallegos}, J. and {Gardiol}, D. and {Gebran}, M. and {Gomboc}, A. and {G{\'o}mez}, A. and {Grux}, E. and {Gueguen}, A. and {Heyrovsky}, A. and {Hoar}, J. and {Iannicola}, G. and {Isasi Parache}, Y. and {Janotto}, A. -M. and {Joliet}, E. and {Jonckheere}, A. and {Keil}, R. and {Kim}, D. -W. and {Klagyivik}, P. and {Klar}, J. and {Knude}, J. and {Kochukhov}, O. and {Kolka}, I. and {Kos}, J. and {Kutka}, A. and {Lainey}, V. and {LeBouquin}, D. and {Liu}, C. and {Loreggia}, D. and {Makarov}, V.~V. and {Marseille}, M.~G. and {Martayan}, C. and {Martinez-Rubi}, O. and {Massart}, B. and {Meynadier}, F. and {Mignot}, S. and {Munari}, U. and {Nguyen}, A. -T. and {Nordlander}, T. and {Ocvirk}, P. and {O'Flaherty}, K.~S. and {Olias Sanz}, A. and {Ortiz}, P. and {Osorio}, J. and {Oszkiewicz}, D. and {Ouzounis}, A. and {Palmer}, M. and {Park}, P. and {Pasquato}, E. and {Peltzer}, C. and {Peralta}, J. and {P{\'e}turaud}, F. and {Pieniluoma}, T. and {Pigozzi}, E. and {Poels}, J. and {Prat}, G. and {Prod'homme}, T. and {Raison}, F. and {Rebordao}, J.~M. and {Risquez}, D. and {Rocca-Volmerange}, B. and {Rosen}, S. and {Ruiz-Fuertes}, M.~I. and {Russo}, F. and {Sembay}, S. and {Serraller Vizcaino}, I. and {Short}, A. and {Siebert}, A. and {Silva}, H. and {Sinachopoulos}, D. and {Slezak}, E. and {Soffel}, M. and {Sosnowska}, D. and {Strai{\v{z}}ys}, V. and {ter Linden}, M. and {Terrell}, D. and {Theil}, S. and {Tiede}, C. and {Troisi}, L. and {Tsalmantza}, P. and {Tur}, D. and {Vaccari}, M. and {Vachier}, F. and {Valles}, P. and {Van Hamme}, W. and {Veltz}, L. and {Virtanen}, J. and {Wallut}, J. -M. and {Wichmann}, R. and {Wilkinson}, M.~I. and {Ziaeepour}, H. and {Zschocke}, S.},
        title = "{The Gaia mission}",
      journal = {\aap},
     keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = nov,
       volume = {595},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201629272},
archivePrefix = {arXiv},
       eprint = {1609.04153},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...595A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia2020,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, techniques: radial velocities, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202039657},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ehrenreich2020,
       author = {{Ehrenreich}, David and {Lovis}, Christophe and {Allart}, Romain and {Zapatero Osorio}, Mar{\'\i}a Rosa and {Pepe}, Francesco and {Cristiani}, Stefano and {Rebolo}, Rafael and {Santos}, Nuno C. and {Borsa}, Francesco and {Demangeon}, Olivier and {Dumusque}, Xavier and {Gonz{\'a}lez Hern{\'a}ndez}, Jonay I. and {Casasayas-Barris}, N{\'u}ria and {S{\'e}gransan}, Damien and {Sousa}, S{\'e}rgio and {Abreu}, Manuel and {Adibekyan}, Vardan and {Affolter}, Michael and {Allende Prieto}, Carlos and {Alibert}, Yann and {Aliverti}, Matteo and {Alves}, David and {Amate}, Manuel and {Avila}, Gerardo and {Baldini}, Veronica and {Bandy}, Timothy and {Benz}, Willy and {Bianco}, Andrea and {Bolmont}, {\'E}meline and {Bouchy}, Fran{\c{c}}ois and {Bourrier}, Vincent and {Broeg}, Christopher and {Cabral}, Alexandre and {Calderone}, Giorgio and {Pall{\'e}}, Enric and {Cegla}, H.~M. and {Cirami}, Roberto and {Coelho}, Jo{\~a}o M.~P. and {Conconi}, Paolo and {Coretti}, Igor and {Cumani}, Claudio and {Cupani}, Guido and {Dekker}, Hans and {Delabre}, Bernard and {Deiries}, Sebastian and {D'Odorico}, Valentina and {Di Marcantonio}, Paolo and {Figueira}, Pedro and {Fragoso}, Ana and {Genolet}, Ludovic and {Genoni}, Matteo and {G{\'e}nova Santos}, Ricardo and {Hara}, Nathan and {Hughes}, Ian and {Iwert}, Olaf and {Kerber}, Florian and {Knudstrup}, Jens and {Landoni}, Marco and {Lavie}, Baptiste and {Lizon}, Jean-Louis and {Lendl}, Monika and {Lo Curto}, Gaspare and {Maire}, Charles and {Manescau}, Antonio and {Martins}, C.~J.~A.~P. and {M{\'e}gevand}, Denis and {Mehner}, Andrea and {Micela}, Giusi and {Modigliani}, Andrea and {Molaro}, Paolo and {Monteiro}, Manuel and {Monteiro}, Mario and {Moschetti}, Manuele and {M{\"u}ller}, Eric and {Nunes}, Nelson and {Oggioni}, Luca and {Oliveira}, Ant{\'o}nio and {Pariani}, Giorgio and {Pasquini}, Luca and {Poretti}, Ennio and {Rasilla}, Jos{\'e} Luis and {Redaelli}, Edoardo and {Riva}, Marco and {Santana Tschudi}, Samuel and {Santin}, Paolo and {Santos}, Pedro and {Segovia Milla}, Alex and {Seidel}, Julia V. and {Sosnowska}, Danuta and {Sozzetti}, Alessandro and {Span{\`o}}, Paolo and {Su{\'a}rez Mascare{\~n}o}, Alejandro and {Tabernero}, Hugo and {Tenegi}, Fabio and {Udry}, St{\'e}phane and {Zanutta}, Alessio and {Zerbi}, Filippo},
        title = "{Nightside condensation of iron in an ultrahot giant exoplanet}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = mar,
       volume = {580},
       number = {7805},
        pages = {597-601},
          doi = {10.1038/s41586-020-2107-1},
archivePrefix = {arXiv},
       eprint = {2003.05528},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.580..597E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kesseli2021,
       author = {{Kesseli}, Aurora Y. and {Snellen}, I.~A.~G.},
        title = "{Confirmation of Asymmetric Iron Absorption in WASP-76b with HARPS}",
      journal = {\apjl},
     keywords = {Exoplanet atmospheres, Hot Jupiters, Exoplanet atmospheric composition, 487, 753, 2021, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = feb,
       volume = {908},
       number = {1},
          eid = {L17},
        pages = {L17},
          doi = {10.3847/2041-8213/abe047},
archivePrefix = {arXiv},
       eprint = {2102.01095},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...908L..17K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lothringer2018,
       author = {{Lothringer}, Joshua D. and {Barman}, Travis and {Koskinen}, Tommi},
        title = "{Extremely Irradiated Hot Jupiters: Non-oxide Inversions, H$^{-}$ Opacity, and Thermal Dissociation of Molecules}",
      journal = {\apj},
     keywords = {methods: numerical, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = oct,
       volume = {866},
       number = {1},
          eid = {27},
        pages = {27},
          doi = {10.3847/1538-4357/aadd9e},
archivePrefix = {arXiv},
       eprint = {1805.00038},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...866...27L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Kirk2019,
	doi = {10.3847/1538-3881/ab397d},
	url = {https://doi.org/10.3847/1538-3881/ab397d},
	year = 2019,
	month = {sep},
	publisher = {American Astronomical Society},
	volume = {158},
	number = {4},
	pages = {144},
	author = {James Kirk and Mercedes L{\'{o}}pez-Morales and Peter J. Wheatley and Ian C. Weaver and Ian Skillen and Tom Louden and James McCormac and N{\'{e}}stor Espinoza},
	title = {{LRG}-{BEASTS}: Transmission Spectroscopy and Retrieval Analysis of the Highly Inflated Saturn-mass Planet {WASP}-39b},
	journal = {The Astronomical Journal},
	abstract = {We present a ground-based transmission spectrum and comprehensive retrieval analysis of the highly inflated Saturn-mass planet WASP-39b. We obtained low-resolution spectra (R ≈ 400) of a transit of WASP-39b using the ACAM instrument on the 4.2 m William Herschel Telescope as part of the LRG-BEASTS survey. Our transmission spectrum is in good agreement with previous ground- and space-based observations of WASP-39b, and covers a wavelength range of 4000–9000 Å. Previous analyses of this exoplanet have retrieved water abundances that span more than four orders of magnitude, which in turn lead to conclusions of a subsolar or highly supersolar atmospheric metallicity. In order to determine the cause of the large discrepancies in the literature regarding WASP-39b’s atmospheric metallicity, we performed retrieval analyses of all literature data sets. Our retrievals, which assume equilibrium chemistry, recovered highly supersolar metallicities for all data sets. When running our retrievals on a combined spectrum, spanning 0.3–5 μm, we recovered an atmospheric metallicity of × solar. We find that stellar activity has a negligible effect on the derived abundances and instead conclude that different assumptions made during retrieval analyses lead to the reported water abundances that differ by orders of magnitude. This in turn has significant consequences for the conclusions we draw. This is the fourth planet to be observed as part of the LRG-BEASTS survey, which is demonstrating that 4 m class telescopes can obtain low-resolution transmission spectra with precisions of around one atmospheric scale height.}
}

@ARTICLE{Mansfield2020,
       author = {{Mansfield}, Megan and {Bean}, Jacob L. and {Stevenson}, Kevin B. and {Komacek}, Thaddeus D. and {Bell}, Taylor J. and {Tan}, Xianyu and {Malik}, Matej and {Beatty}, Thomas G. and {Wong}, Ian and {Cowan}, Nicolas B. and {Dang}, Lisa and {D{\'e}sert}, Jean-Michel and {Fortney}, Jonathan J. and {Gaudi}, B. Scott and {Keating}, Dylan and {Kempton}, Eliza M. -R. and {Kreidberg}, Laura and {Line}, Michael R. and {Parmentier}, Vivien and {Stassun}, Keivan G. and {Swain}, Mark R. and {Zellem}, Robert T.},
        title = "{Evidence for H2 Dissociation and Recombination Heat Transport in the Atmosphere of KELT-9b}",
      journal = {\apjl},
     keywords = {Hot Jupiters, Exoplanet atmospheres, 753, 487, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {L15},
        pages = {L15},
          doi = {10.3847/2041-8213/ab5b09},
archivePrefix = {arXiv},
       eprint = {1910.01567},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888L..15M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek2020,
       author = {{Komacek}, Thaddeus D. and {Showman}, Adam P.},
        title = "{Temporal Variability in Hot Jupiter Atmospheres}",
      journal = {\apj},
     keywords = {Hydrodynamics, Computational methods, Exoplanets, Exoplanet atmospheres, Exoplanet atmospheric variability, 1963, 1965, 498, 487, 2020, Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2020,
        month = jan,
       volume = {888},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/1538-4357/ab5b0b},
archivePrefix = {arXiv},
       eprint = {1910.09523},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888....2K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rogers2014,
       author = {{Rogers}, T.~M. and {Komacek}, T.~D.},
        title = "{Magnetic Effects in Hot Jupiter Atmospheres}",
      journal = {\apj},
     keywords = {hydrodynamics, magnetohydrodynamics: MHD, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = oct,
       volume = {794},
       number = {2},
          eid = {132},
        pages = {132},
          doi = {10.1088/0004-637X/794/2/132},
archivePrefix = {arXiv},
       eprint = {1409.0519},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...794..132R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rogers2017,
       author = {{Rogers}, T.~M. and {McElwaine}, J.~N.},
        title = "{The Hottest Hot Jupiters May Host Atmospheric Dynamos}",
      journal = {\apjl},
     keywords = {dynamo, magnetohydrodynamics: MHD, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jun,
       volume = {841},
       number = {2},
          eid = {L26},
        pages = {L26},
          doi = {10.3847/2041-8213/aa72da},
archivePrefix = {arXiv},
       eprint = {1704.04197},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...841L..26R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Knutson2007,
       author = {{Knutson}, Heather A. and {Charbonneau}, David and {Allen}, Lori E. and {Fortney}, Jonathan J. and {Agol}, Eric and {Cowan}, Nicolas B. and {Showman}, Adam P. and {Cooper}, Curtis S. and {Megeath}, S. Thomas},
        title = "{A map of the day-night contrast of the extrasolar planet HD 189733b}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2007,
        month = may,
       volume = {447},
       number = {7141},
        pages = {183-186},
          doi = {10.1038/nature05782},
archivePrefix = {arXiv},
       eprint = {0705.0993},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007Natur.447..183K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaudi2007,
       author = {{Gaudi}, B. Scott and {Winn}, Joshua N.},
        title = "{Prospects for the Characterization and Confirmation of Transiting Exoplanets via the Rossiter-McLaughlin Effect}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Rotation, Astrophysics},
         year = 2007,
        month = jan,
       volume = {655},
       number = {1},
        pages = {550-563},
          doi = {10.1086/509910},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608071},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...655..550G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ohta2005,
       author = {{Ohta}, Yasuhiro and {Taruya}, Atsushi and {Suto}, Yasushi},
        title = "{The Rossiter-McLaughlin Effect and Analytic Radial Velocity Curves for Transiting Extrasolar Planetary Systems}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Individual: Henry Draper Number: HD 209458, Techniques: Spectroscopic, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {1118-1135},
          doi = {10.1086/428344},
archivePrefix = {arXiv},
       eprint = {astro-ph/0410499},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622.1118O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Queloz2000,
       author = {{Queloz}, D. and {Eggenberger}, A. and {Mayor}, M. and {Perrier}, C. and {Beuzit}, J.~L. and {Naef}, D. and {Sivan}, J.~P. and {Udry}, S.},
        title = "{Detection of a spectroscopic transit by the planet orbiting the star HD209458}",
      journal = {\aap},
     keywords = {STARS: BINARIES: SPECTROSCOPIC, STARS: BINARIES: ECLIPSING, STARS: INDIVIDUAL: HD209458, STARS: PLANETARY SYSTEMS, Astrophysics},
         year = 2000,
        month = jul,
       volume = {359},
        pages = {L13-L17},
archivePrefix = {arXiv},
       eprint = {astro-ph/0006213},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...359L..13Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Czesla2015,
       author = {{Czesla}, S. and {Klocov{\'a}}, T. and {Khalafinejad}, S. and {Wolter}, U. and {Schmitt}, J.~H.~M.~M.},
        title = "{The center-to-limb variation across the Fraunhofer lines of HD 189733. Sampling the stellar spectrum using a transiting planet}",
      journal = {\aap},
     keywords = {planets and satellites: individual: HD 189733b, planets and satellites: atmospheres, stars: activity, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {582},
          eid = {A51},
        pages = {A51},
          doi = {10.1051/0004-6361/201526386},
archivePrefix = {arXiv},
       eprint = {1509.05657},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..51C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stenflo2015,
       author = {{Stenflo}, J.~O.},
        title = "{FTS atlas of the Sun's spectrally resolved center-to-limb variation}",
      journal = {\aap},
     keywords = {Sun: atmosphere, atlases, line: profiles, techniques: spectroscopic, radiative transfer, polarization, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jan,
       volume = {573},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201424685},
archivePrefix = {arXiv},
       eprint = {1410.8474},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..74S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fossati2021,
       author = {{Fossati}, L. and {Young}, M.~E. and {Shulyak}, D. and {Koskinen}, T. and {Huang}, C. and {Cubillos}, P.~E. and {France}, K. and {Sreejith}, A.~G.},
        title = "{Non-local thermodynamic equilibrium effects determine the upper atmospheric temperature structure of the ultra-hot Jupiter KELT-9b}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jun,
          eid = {arXiv:2106.11263},
        pages = {arXiv:2106.11263},
archivePrefix = {arXiv},
       eprint = {2106.11263},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210611263F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lefevre2022,
       author = {{Lef{\`e}vre}, Maxence and {Tan}, Xianyu and {Lee}, Elspeth K.~H. and {Pierrehumbert}, R.~T.},
        title = "{Cloud-convection feedback in brown dwarfs atmosphere}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = mar,
          eid = {arXiv:2203.08625},
        pages = {arXiv:2203.08625},
archivePrefix = {arXiv},
       eprint = {2203.08625},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220308625L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Rossiter1924,
       author = {{Rossiter}, R.~A.},
        title = "{On the detection of an effect of rotation during eclipse in the velocity of the brigher component of beta Lyrae, and on the constancy of velocity of this system.}",
      journal = {\apj},
         year = 1924,
        month = jul,
       volume = {60},
        pages = {15-21},
          doi = {10.1086/142825},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ApJ....60...15R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McLaughlin1924,
       author = {{McLaughlin}, D.~B.},
        title = "{Some results of a spectrographic study of the Algol system.}",
      journal = {\apj},
         year = 1924,
        month = jul,
       volume = {60},
        pages = {22-31},
          doi = {10.1086/142826},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ApJ....60...22M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stevens2018,
       author = {{Stevens}, Daniel J. and {Gaudi}, B. Scott and {Stassun}, Keivan G.},
        title = "{Measuring Model-independent Masses and Radii of Single-lined Eclipsing Binaries: Analytic Precision Estimates}",
      journal = {\apj},
     keywords = {binaries: eclipsing, methods: analytical, planetary systems, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = jul,
       volume = {862},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.3847/1538-4357/aaccf5},
archivePrefix = {arXiv},
       eprint = {1712.05046},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...862...53S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Popper1980,
       author = {{Popper}, D.~M.},
        title = "{Stellar masses.}",
      journal = {\araa},
     keywords = {Astronomical Catalogs, Eclipsing Binary Stars, Stellar Mass, Stellar Spectra, B Stars, Giant Stars, Main Sequence Stars, O Stars, Astrophysics},
         year = 1980,
        month = jan,
       volume = {18},
        pages = {115-164},
          doi = {10.1146/annurev.aa.18.090180.000555},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980ARA&A..18..115P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harmanec1988,
       author = {{Harmanec}, Petr},
        title = "{Stellar Masses and Radii Based on Modern Binary Data}",
      journal = {Bulletin of the Astronomical Institutes of Czechoslovakia},
     keywords = {Early Stars, Eclipsing Binary Stars, Stellar Mass, Stellar Rotation, B Stars, Light Curve, Main Sequence Stars, Stellar Magnitude, Stellar Spectra, Stellar Temperature, Astrophysics},
         year = 1988,
        month = dec,
       volume = {39},
        pages = {329},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988BAICz..39..329H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andersen1991,
       author = {{Andersen}, J.},
        title = "{Accurate masses and radii of normal stars}",
      journal = {\aapr},
     keywords = {Eclipsing Binary Stars, Stellar Mass, Stellar Spectrophotometry, Stellar Structure, Abundance, Stellar Evolution, Stellar Models, Stellar Physics, Astrophysics, Stars: binaries: general, stars: diameters of, stars: evolution of, stars: luminosities of, stars: mass of, stars: structure of},
         year = 1991,
        month = jan,
       volume = {3},
       number = {2},
        pages = {91-126},
          doi = {10.1007/BF00873538},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991A&ARv...3...91A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{scipy2020,
  author  = {Virtanen, Pauli and Gommers, Ralf and Oliphant, Travis E. and
            Haberland, Matt and Reddy, Tyler and Cournapeau, David and
            Burovski, Evgeni and Peterson, Pearu and Weckesser, Warren and
            Bright, Jonathan and {van der Walt}, St{\'e}fan J. and
            Brett, Matthew and Wilson, Joshua and Millman, K. Jarrod and
            Mayorov, Nikolay and Nelson, Andrew R. J. and Jones, Eric and
            Kern, Robert and Larson, Eric and Carey, C J and
            Polat, {\.I}lhan and Feng, Yu and Moore, Eric W. and
            {VanderPlas}, Jake and Laxalde, Denis and Perktold, Josef and
            Cimrman, Robert and Henriksen, Ian and Quintero, E. A. and
            Harris, Charles R. and Archibald, Anne M. and
            Ribeiro, Ant{\^o}nio H. and Pedregosa, Fabian and
            {van Mulbregt}, Paul and {SciPy 1.0 Contributors}},
  title   = {{{SciPy} 1.0: Fundamental Algorithms for Scientific
            Computing in Python}},
  journal = {Nature Methods},
  year    = {2020},
  volume  = {17},
  pages   = {261--272},
  adsurl  = {https://rdcu.be/b08Wh},
  doi     = {10.1038/s41592-019-0686-2},
}


@ARTICLE{Perna2010,
       author = {{Perna}, Rosalba and {Menou}, Kristen and {Rauscher}, Emily},
        title = "{Magnetic Drag on Hot Jupiter Atmospheric Winds}",
      journal = {\apj},
     keywords = {planets and satellites: atmospheres, planets and satellites: individual: HD 209458b, planets and satellites: magnetic fields, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = aug,
       volume = {719},
       number = {2},
        pages = {1421-1426},
          doi = {10.1088/0004-637X/719/2/1421},
archivePrefix = {arXiv},
       eprint = {1003.3838},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...719.1421P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Savel2021,
       author = {{Savel}, Arjun B. and {Kempton}, Eliza M. -R. and {Malik}, Matej and {Komacek}, Thaddeus D. and {Bean}, Jacob L. and {May}, Erin M. and {Stevenson}, Kevin B. and {Mansfield}, Megan and {Rauscher}, Emily},
        title = "{No umbrella needed: Confronting the hypothesis of iron rain on WASP-76b with post-processed general circulation models}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = aug,
          eid = {arXiv:2109.00163},
        pages = {arXiv:2109.00163},
archivePrefix = {arXiv},
       eprint = {2109.00163},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210900163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Flowers2019,
       author = {{Flowers}, Erin and {Brogi}, Matteo and {Rauscher}, Emily and {Kempton}, Eliza M. -R. and {Chiavassa}, Andrea},
        title = "{The High-resolution Transmission Spectrum of HD 189733b Interpreted with Atmospheric Doppler Shifts from Three-dimensional General Circulation Models}",
      journal = {\aj},
     keywords = {hydrodynamics, planets and satellites: atmospheres, planets and satellites: gaseous planets, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = may,
       volume = {157},
       number = {5},
          eid = {209},
        pages = {209},
          doi = {10.3847/1538-3881/ab164c},
archivePrefix = {arXiv},
       eprint = {1810.06099},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..209F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cauley2021,
       author = {{Cauley}, P. Wilson and {Wang}, Ji and {Shkolnik}, Evgenya L. and {Ilyin}, Ilya and {Strassmeier}, Klaus G. and {Redfield}, Seth and {Jensen}, Adam G.},
        title = "{Time-resolved Rotational Velocities in the Upper Atmosphere of WASP-33 b}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanets, Hot Jupiters, 487, 498, 753, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = mar,
       volume = {161},
       number = {3},
          eid = {152},
        pages = {152},
          doi = {10.3847/1538-3881/abde43},
archivePrefix = {arXiv},
       eprint = {2010.02118},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..152C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek2016,
       author = {{Komacek}, Thaddeus D. and {Showman}, Adam P.},
        title = "{Atmospheric Circulation of Hot Jupiters: Dayside-Nightside Temperature Differences}",
      journal = {\apj},
     keywords = {hydrodynamics, methods: analytical, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = apr,
       volume = {821},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.3847/0004-637X/821/1/16},
archivePrefix = {arXiv},
       eprint = {1601.00069},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...821...16K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rauscher2013,
       author = {{Rauscher}, Emily and {Menou}, Kristen},
        title = "{Three-dimensional Atmospheric Circulation Models of HD 189733b and HD 209458b with Consistent Magnetic Drag and Ohmic Dissipation}",
      journal = {\apj},
     keywords = {hydrodynamics, magnetic fields, methods: numerical, planets and satellites: individual: HD 189733b HD 209458b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = feb,
       volume = {764},
       number = {1},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/764/1/103},
archivePrefix = {arXiv},
       eprint = {1208.2274},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...764..103R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Beltz2021b,
       author = {{Beltz}, Hayley and {Rauscher}, Emily and {Roman}, Michael and {Guilliat}, Abigail},
        title = "{Exploring the Effects of Active Magnetic Drag in a GCM of the Ultra-Hot Jupiter WASP-76b}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.13371},
        pages = {arXiv:2109.13371},
archivePrefix = {arXiv},
       eprint = {2109.13371},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210913371B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lothringer2019,
       author = {{Lothringer}, Joshua D. and {Barman}, Travis},
        title = "{The Influence of Host Star Spectral Type on Ultra-hot Jupiter Atmospheres}",
      journal = {\apj},
     keywords = {methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = may,
       volume = {876},
       number = {1},
          eid = {69},
        pages = {69},
          doi = {10.3847/1538-4357/ab1485},
archivePrefix = {arXiv},
       eprint = {1903.12183},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...876...69L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{TESS2015,
       author = {{Ricker}, George R. and {Winn}, Joshua N. and {Vanderspek}, Roland and {Latham}, David W. and {Bakos}, G{\'a}sp{\'a}r {\'A}. and {Bean}, Jacob L. and {Berta-Thompson}, Zachory K. and {Brown}, Timothy M. and {Buchhave}, Lars and {Butler}, Nathaniel R. and {Butler}, R. Paul and {Chaplin}, William J. and {Charbonneau}, David and {Christensen-Dalsgaard}, J{\o}rgen and {Clampin}, Mark and {Deming}, Drake and {Doty}, John and {De Lee}, Nathan and {Dressing}, Courtney and {Dunham}, Edward W. and {Endl}, Michael and {Fressin}, Francois and {Ge}, Jian and {Henning}, Thomas and {Holman}, Matthew J. and {Howard}, Andrew W. and {Ida}, Shigeru and {Jenkins}, Jon M. and {Jernigan}, Garrett and {Johnson}, John Asher and {Kaltenegger}, Lisa and {Kawai}, Nobuyuki and {Kjeldsen}, Hans and {Laughlin}, Gregory and {Levine}, Alan M. and {Lin}, Douglas and {Lissauer}, Jack J. and {MacQueen}, Phillip and {Marcy}, Geoffrey and {McCullough}, Peter R. and {Morton}, Timothy D. and {Narita}, Norio and {Paegert}, Martin and {Palle}, Enric and {Pepe}, Francesco and {Pepper}, Joshua and {Quirrenbach}, Andreas and {Rinehart}, Stephen A. and {Sasselov}, Dimitar and {Sato}, Bun'ei and {Seager}, Sara and {Sozzetti}, Alessandro and {Stassun}, Keivan G. and {Sullivan}, Peter and {Szentgyorgyi}, Andrew and {Torres}, Guillermo and {Udry}, Stephane and {Villasenor}, Joel},
        title = "{Transiting Exoplanet Survey Satellite (TESS)}",
      journal = {Journal of Astronomical Telescopes, Instruments, and Systems},
         year = 2015,
        month = jan,
       volume = {1},
          eid = {014003},
        pages = {014003},
          doi = {10.1117/1.JATIS.1.1.014003},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015JATIS...1a4003R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ambikasaran2014,
author = {{Ambikasaran}, S. and {Foreman-Mackey}, D. and
{Greengard}, L. and {Hogg}, D.~W. and {O'Neil}, M.},
title = "{Fast Direct Methods for Gaussian Processes}",
year = 2014,
month = mar,
url = http://arxiv.org/abs/1403.6015
}

@ARTICLE{Charbonneau2005,
       author = {{Charbonneau}, David and {Allen}, Lori E. and {Megeath}, S. Thomas and {Torres}, Guillermo and {Alonso}, Roi and {Brown}, Timothy M. and {Gilliland}, Ronald L. and {Latham}, David W. and {Mandushev}, Georgi and {O'Donovan}, Francis T. and {Sozzetti}, Alessandro},
        title = "{Detection of Thermal Emission from an Extrasolar Planet}",
      journal = {\apj},
     keywords = {Stars: Binaries: Eclipsing, Infrared: Stars, Stars: Planetary Systems, Stars: Individual: Alphanumeric: TrES-1, Techniques: Photometric, Astrophysics},
         year = 2005,
        month = jun,
       volume = {626},
       number = {1},
        pages = {523-529},
          doi = {10.1086/429991},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503457},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...626..523C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hindle2021,
       author = {{Hindle}, A.~W. and {Bushby}, P.~J. and {Rogers}, T.~M.},
        title = "{Observational Consequences of Shallow-water Magnetohydrodynamics on Hot Jupiters}",
      journal = {\apjl},
     keywords = {Magnetohydrodynamics, Astrophysical fluid dynamics, Hot Jupiters, Exoplanet dynamics, Exoplanet atmospheres, Exoplanet atmospheric variability, 1964, 101, 753, 490, 487, 2020, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jul,
       volume = {916},
       number = {1},
          eid = {L8},
        pages = {L8},
          doi = {10.3847/2041-8213/ac0fec},
archivePrefix = {arXiv},
       eprint = {2107.10848},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...916L...8H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fromang2016,
       author = {{Fromang}, S{\'e}bastien and {Leconte}, Jeremy and {Heng}, Kevin},
        title = "{Shear-driven instabilities and shocks in the atmospheres of hot Jupiters}",
      journal = {\aap},
     keywords = {hydrodynamics, instabilities, shock waves, methods: numerical, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = jul,
       volume = {591},
          eid = {A144},
        pages = {A144},
          doi = {10.1051/0004-6361/201527600},
archivePrefix = {arXiv},
       eprint = {1603.02794},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...591A.144F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Menou2020,
       author = {{Menou}, Kristen},
        title = "{Hot Jupiter atmospheric flows at high resolution}",
      journal = {\mnras},
     keywords = {astrochemistry, diffusion, hydrodynamics, radiative transfer, turbulence, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = apr,
       volume = {493},
       number = {4},
        pages = {5038-5044},
          doi = {10.1093/mnras/staa532},
archivePrefix = {arXiv},
       eprint = {1911.00084},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.5038M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wardenier2021,
       author = {{Wardenier}, Joost P. and {Parmentier}, Vivien and {Lee}, Elspeth K.~H. and {Line}, Michael R. and {Gharib-Nezhad}, Ehsan},
        title = "{Decomposing the iron cross-correlation signal of the ultra-hot Jupiter WASP-76b in transmission using 3D Monte Carlo radiative transfer}",
      journal = {\mnras},
     keywords = {radiative transfer, methods: numerical, planets and satellites: individual: WASP-76b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
       volume = {506},
       number = {1},
        pages = {1258-1283},
          doi = {10.1093/mnras/stab1797},
archivePrefix = {arXiv},
       eprint = {2105.11034},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.506.1258W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2020,
       author = {{Showman}, Adam P. and {Tan}, Xianyu and {Parmentier}, Vivien},
        title = "{Atmospheric Dynamics of Hot Giant Planets and Brown Dwarfs}",
      journal = {\ssr},
     keywords = {Exoplanets, Giant planets, Hot Jupiters, Jupiter, Saturn, Brown dwarfs, Atmospheric dynamics, Turbulence, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {216},
       number = {8},
          eid = {139},
        pages = {139},
          doi = {10.1007/s11214-020-00758-8},
archivePrefix = {arXiv},
       eprint = {2007.15363},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SSRv..216..139S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993JAnSc..41..439S,
       author = {{Shuster}, Malcolm D.},
        title = "{Survey of attitude representations}",
      journal = {Journal of the Astronautical Sciences},
     keywords = {Attitude Control, Flight Mechanics, Kinematic Equations, Satellite Orientation, Satellite Rotation, Covariance, Errors, Kinematics, Transformations (Mathematics), Astronautics (General)},
         year = 1993,
        month = oct,
       volume = {41},
       number = {4},
        pages = {439-517},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993JAnSc..41..439S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993JGCD...16..393S,
       author = {{Shuster}, Malcolm D.},
        title = "{Attitude determination in higher dimensions}",
      journal = {Journal of Guidance Control Dynamics},
     keywords = {Attitude Control, Matrices (Mathematics), Algorithms, Three Dimensional Models, Space Communications, Spacecraft Communications, Command and Tracking},
         year = 1993,
        month = apr,
       volume = {16},
       number = {2},
        pages = {393-395},
          doi = {10.2514/3.21018},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993JGCD...16..393S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993fmet.symp..259S,
       author = {{Shuster}, Malcolm D.},
        title = "{Attitude analysis in Flatland: The plane truth}",
     keywords = {Attitude (Inclination), Euclidean Geometry, Orbit Calculation, Quaternions, Attitude Indicators, Satellite Attitude Control, Two Dimensional Models, Astrodynamics},
    booktitle = {Flight Mechanics/Estimation Theory Symposium},
         year = 1993,
        month = feb,
        pages = {259-274},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993fmet.symp..259S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shuster1993,
       author = {{Shuster}, M.~D.},
        title = "{The kinematic equation for the rotation vector}",
      journal = {IEEE Transactions on Aerospace Electronic Systems},
         year = 1993,
        month = jan,
       volume = {29},
       number = {1},
        pages = {263-267},
          doi = {10.1109/7.249140},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ITAES..29..263S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eriksson2019,
       author = {{Eriksson}, Simon C. and {Janson}, Markus and {Calissendorff}, Per},
        title = "{Detection of new strongly variable brown dwarfs in the L/T transition}",
      journal = {\aap},
     keywords = {brown dwarfs, stars: individual: 2MASS J22153705+2110554, stars: variables: general, stars: low-mass, infrared: stars, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = sep,
       volume = {629},
          eid = {A145},
        pages = {A145},
          doi = {10.1051/0004-6361/201935671},
archivePrefix = {arXiv},
       eprint = {1910.02638},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...629A.145E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley&Ackerman2001,
       author = {{Marley}, M.~S. and {Ackerman}, A.~S.},
        title = "{The Role of Clouds in Brown Dwarf and Extrasolar Giant Planet Atmospheres}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = 2001,
        month = mar,
          eid = {astro-ph/0103269},
        pages = {astro-ph/0103269},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103269},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001astro.ph..3269M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremblin2016,
       author = {{Tremblin}, P. and {Amundsen}, D.~S. and {Chabrier}, G. and {Baraffe}, I. and {Drummond}, B. and {Hinkley}, S. and {Mourier}, P. and {Venot}, O.},
        title = "{Cloudless Atmospheres for L/T Dwarfs and Extrasolar Giant Planets}",
      journal = {\apjl},
     keywords = {brown dwarfs, methods: numerical, methods: observational, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = feb,
       volume = {817},
       number = {2},
          eid = {L19},
        pages = {L19},
          doi = {10.3847/2041-8205/817/2/L19},
archivePrefix = {arXiv},
       eprint = {1601.03652},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817L..19T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burgasser2002,
       author = {{Burgasser}, Adam J. and {Marley}, Mark S. and {Ackerman}, Andrew S. and {Saumon}, Didier and {Lodders}, Katharina and {Dahn}, Conard C. and {Harris}, Hugh C. and {Kirkpatrick}, J. Davy},
        title = "{Evidence of Cloud Disruption in the L/T Dwarf Transition}",
      journal = {\apjl},
     keywords = {Infrared: Stars, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: SDSS J1254-0122, Stars: Individual: Alphanumeric: 2MASS J0559-1404, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2002,
        month = jun,
       volume = {571},
       number = {2},
        pages = {L151-L154},
          doi = {10.1086/341343},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205051},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...571L.151B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Radigan2014b,
       author = {{Radigan}, Jacqueline},
        title = "{An Independent Analysis of the Brown Dwarf Atmosphere Monitoring (BAM) Data: Large-amplitude Variability is Rare Outside the L/T Transition}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = dec,
       volume = {797},
       number = {2},
          eid = {120},
        pages = {120},
          doi = {10.1088/0004-637X/797/2/120},
archivePrefix = {arXiv},
       eprint = {1408.5919},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...797..120R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Radigan2014a,
       author = {{Radigan}, Jacqueline and {Lafreni{\`e}re}, David and {Jayawardhana}, Ray and {Artigau}, Etienne},
        title = "{Strong Brightness Variations Signal Cloudy-to-clear Transition of Brown Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = oct,
       volume = {793},
       number = {2},
          eid = {75},
        pages = {75},
          doi = {10.1088/0004-637X/793/2/75},
archivePrefix = {arXiv},
       eprint = {1404.3247},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...793...75R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Girardin2013,
       author = {{Girardin}, F. and {Artigau}, {\'E}. and {Doyon}, R.},
        title = "{In Search of Dust Clouds: Photometric Monitoring of a Sample of Late L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: SDSS J105213.51+442255.7 SDSSp J125453.90{\textendash}012247.4, stars: low-mass, stars: variables: general, techniques: photometric},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/767/1/61},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767...61G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Paudel2018,
       author = {{Paudel}, Rishi R. and {Gizis}, John E. and {Mullan}, D.~J. and {Schmidt}, Sarah J. and {Burgasser}, Adam J. and {Williams}, Peter K.~G. and {Berger}, Edo},
        title = "{K2 Ultracool Dwarfs Survey. III. White Light Flares Are Ubiquitous in M6-L0 Dwarfs}",
      journal = {\apj},
     keywords = {stars: activity, stars: flare, stars: individual: 2MASS J12321827-0951502, TRAPPIST-1, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = may,
       volume = {858},
       number = {1},
          eid = {55},
        pages = {55},
          doi = {10.3847/1538-4357/aab8fe},
archivePrefix = {arXiv},
       eprint = {1803.07708},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...858...55P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Paudel2020,
       author = {{Paudel}, R.~R. and {Gizis}, J.~E. and {Mullan}, D.~J. and {Schmidt}, S.~J. and {Burgasser}, A.~J. and {Williams}, P.~K.~G.},
        title = "{K2 Ultracool Dwarfs Survey - VI. White light superflares observed on an L5 dwarf and flare rates of L dwarfs}",
      journal = {\mnras},
     keywords = {stars: activity, stars: flare, stars: individual: VVV BD001, 2MASS J08585891+1804463, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jun,
       volume = {494},
       number = {4},
        pages = {5751-5760},
          doi = {10.1093/mnras/staa1137},
archivePrefix = {arXiv},
       eprint = {2004.10579},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.5751P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Chabrier2000,
       author = {{Chabrier}, G. and {Baraffe}, I. and {Allard}, F. and {Hauschildt}, P.},
        title = "{Evolutionary Models for Very Low-Mass Stars and Brown Dwarfs with Dusty Atmospheres}",
      journal = {\apj},
     keywords = {Hertzsprung-Russell, Stars: Evolution, Stars: Low-Mass, Brown Dwarfs, Stars: Luminosity Function, Mass Function, Astrophysics},
         year = 2000,
        month = oct,
       volume = {542},
       number = {1},
        pages = {464-472},
          doi = {10.1086/309513},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005557},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...542..464C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dupuy2017,
       author = {{Dupuy}, Trent J. and {Liu}, Michael C.},
        title = "{Individual Dynamical Masses of Ultracool Dwarfs}",
      journal = {\apjs},
     keywords = {astrometry, binaries: close, brown dwarfs, fundamental parameters, parallaxes, stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = aug,
       volume = {231},
       number = {2},
          eid = {15},
        pages = {15},
          doi = {10.3847/1538-4365/aa5e4c},
archivePrefix = {arXiv},
       eprint = {1703.05775},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJS..231...15D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows2006,
       author = {{Burrows}, Adam and {Sudarsky}, David and {Hubeny}, Ivan},
        title = "{L and T Dwarf Models and the L to T Transition}",
      journal = {\apj},
     keywords = {Infrared: Stars, Molecular Processes, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = apr,
       volume = {640},
       number = {2},
        pages = {1063-1077},
          doi = {10.1086/500293},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509066},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...640.1063B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kirkpatrick2005,
       author = {{Kirkpatrick}, J. Davy},
        title = "{New Spectral Types L and T}",
      journal = {\araa},
         year = 2005,
        month = sep,
       volume = {43},
       number = {1},
        pages = {195-245},
          doi = {10.1146/annurev.astro.42.053102.134017},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ARA&A..43..195K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cushing2008,
       author = {{Cushing}, Michael C. and {Marley}, Mark S. and {Saumon}, D. and {Kelly}, Brandon C. and {Vacca}, William D. and {Rayner}, John T. and {Freedman}, Richard S. and {Lodders}, Katharina and {Roellig}, Thomas L.},
        title = "{Atmospheric Parameters of Field L and T Dwarfs}",
      journal = {\apj},
     keywords = {infrared: stars, radiative transfer, stars: fundamental parameters, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = may,
       volume = {678},
       number = {2},
        pages = {1372-1395},
          doi = {10.1086/526489},
archivePrefix = {arXiv},
       eprint = {0711.0801},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...678.1372C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Tsuji1996b,
       author = {{Tsuji}, T. and {Ohnaka}, K. and {Aoki}, W. and {Nakajima}, T.},
        title = "{Evolution of dusty photospheres through red to brown dwarfs: how dust forms in very low mass objects.}",
      journal = {\aap},
     keywords = {EQUATION OF STATE, MOLECULAR PROCESSES, STARS: ATMOSPHERES, STARS: FUNDAMENTAL PARAMETERS, STARS: LATE-TYPE, STARS: LOW-MASS, BROWN DWARFS},
         year = 1996,
        month = apr,
       volume = {308},
        pages = {L29-L32},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...308L..29T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Allard2001,
       author = {{Allard}, France and {Hauschildt}, Peter H. and {Alexander}, David R. and {Tamanai}, Akemi and {Schweitzer}, Andreas},
        title = "{The Limiting Effects of Dust in Brown Dwarf Model Atmospheres}",
      journal = {\apj},
     keywords = {Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2001,
        month = jul,
       volume = {556},
       number = {1},
        pages = {357-372},
          doi = {10.1086/321547},
archivePrefix = {arXiv},
       eprint = {astro-ph/0104256},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...556..357A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Marley2002,
       author = {{Marley}, Mark S. and {Seager}, S. and {Saumon}, D. and {Lodders}, Katharina and {Ackerman}, Andrew S. and {Freedman}, Richard S. and {Fan}, Xiaohui},
        title = "{Clouds and Chemistry: Ultracool Dwarf Atmospheric Properties from Optical and Infrared Colors}",
      journal = {\apj},
     keywords = {Stars: Atmospheres, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2002,
        month = mar,
       volume = {568},
       number = {1},
        pages = {335-342},
          doi = {10.1086/338800},
archivePrefix = {arXiv},
       eprint = {astro-ph/0105438},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...568..335M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Noll2000,
       author = {{Noll}, Keith S. and {Geballe}, T.~R. and {Leggett}, S.~K. and {Marley}, Mark S.},
        title = "{The Onset of Methane in L Dwarfs}",
      journal = {\apjl},
     keywords = {Infrared: Stars, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2000,
        month = oct,
       volume = {541},
       number = {2},
        pages = {L75-L78},
          doi = {10.1086/312906},
archivePrefix = {arXiv},
       eprint = {astro-ph/0007449},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...541L..75N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Buenzli2014,
       author = {{Buenzli}, Esther and {Apai}, D{\'a}niel and {Radigan}, Jacqueline and {Reid}, I. Neill and {Flateau}, Davin},
        title = "{Brown Dwarf Photospheres are Patchy: A Hubble Space Telescope Near-infrared Spectroscopic Survey Finds Frequent Low-level Variability}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = feb,
       volume = {782},
       number = {2},
          eid = {77},
        pages = {77},
          doi = {10.1088/0004-637X/782/2/77},
archivePrefix = {arXiv},
       eprint = {1312.5294},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...782...77B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reimers2008,
       author = {{Reiners}, A. and {Basri}, G.},
        title = "{Chromospheric Activity, Rotation, and Rotational Braking in M and L Dwarfs}",
      journal = {\apj},
     keywords = {stars: activity, stars: flare, stars: late-type, stars: low-mass, brown dwarfs, stars: rotation, Astrophysics},
         year = 2008,
        month = sep,
       volume = {684},
       number = {2},
        pages = {1390-1403},
          doi = {10.1086/590073},
archivePrefix = {arXiv},
       eprint = {0805.1059},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...684.1390R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Enoch2003,
       author = {{Enoch}, Melissa L. and {Brown}, Michael E. and {Burgasser}, Adam J.},
        title = "{Photometric Variability at the L/T Dwarf Boundary}",
      journal = {\aj},
     keywords = {stars: individual (2MASSW J0030300-145033), stars: individual (SDSSp J015141.69+124429.6), Stars: Low-Mass, Brown Dwarfs, Stars: Variables: Other, Astrophysics},
         year = 2003,
        month = aug,
       volume = {126},
       number = {2},
        pages = {1006-1016},
          doi = {10.1086/376598},
archivePrefix = {arXiv},
       eprint = {astro-ph/0305048},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003AJ....126.1006E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Girardin2013,
       author = {{Girardin}, F. and {Artigau}, {\'E}. and {Doyon}, R.},
        title = "{In Search of Dust Clouds: Photometric Monitoring of a Sample of Late L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: SDSS J105213.51+442255.7 SDSSp J125453.90{\textendash}012247.4, stars: low-mass, stars: variables: general, techniques: photometric},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/767/1/61},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767...61G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jones&Tsuji1997,
       author = {{Jones}, Hugh R.~A. and {Tsuji}, Takashi},
        title = "{Spectral Evidence for Dust in Late-Type M Dwarfs}",
      journal = {\apjl},
     keywords = {EQUATION OF STATE, MOLECULAR PROCESSES, STARS: ATMOSPHERES, STARS: FUNDAMENTAL PARAMETERS, STARS: LATE-TYPE, INFRARED: STARS, STARS: LOW-MASS, BROWN DWARFS, Equation of State, Infrared: Stars, Molecular Processes, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 1997,
        month = may,
       volume = {480},
       number = {1},
        pages = {L39-L41},
          doi = {10.1086/310619},
archivePrefix = {arXiv},
       eprint = {astro-ph/9702108},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...480L..39J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley2010,
       author = {{Marley}, Mark S. and {Saumon}, Didier and {Goldblatt}, Colin},
        title = "{A Patchy Cloud Model for the L to T Dwarf Transition}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = nov,
       volume = {723},
       number = {1},
        pages = {L117-L121},
          doi = {10.1088/2041-8205/723/1/L117},
archivePrefix = {arXiv},
       eprint = {1009.6217},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...723L.117M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Metchev2015,
       author = {{Metchev}, Stanimir A. and {Heinze}, Aren and {Apai}, D{\'a}niel and {Flateau}, Davin and {Radigan}, Jacqueline and {Burgasser}, Adam and {Marley}, Mark S. and {Artigau}, {\'E}tienne and {Plavchan}, Peter and {Goldman}, Bertrand},
        title = "{Weather on Other Worlds. II. Survey Results: Spots are Ubiquitous on L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: low-mass, stars: rotation, starspots, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {154},
        pages = {154},
          doi = {10.1088/0004-637X/799/2/154},
archivePrefix = {arXiv},
       eprint = {1411.3051},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..154M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Apai2017,
       author = {{Apai}, D. and {Karalidi}, T. and {Marley}, M.~S. and {Yang}, H. and {Flateau}, D. and {Metchev}, S. and {Cowan}, N.~B. and {Buenzli}, E. and {Burgasser}, A.~J. and {Radigan}, J. and {Artigau}, E. and {Lowrance}, P.},
        title = "{Zones, spots, and planetary-scale waves beating in brown dwarf atmospheres}",
      journal = {Science},
     keywords = {ASTRONOMY, GEOCHEM PHYS, PLANET SCI},
         year = 2017,
        month = aug,
       volume = {357},
       number = {6352},
        pages = {683-687},
          doi = {10.1126/science.aam9848},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Sci...357..683A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Goncharskii1982,
       author = {{Goncharskii}, A.~V. and {Stepanov}, V.~V. and {Khokhlova}, V.~L. and {Yagola}, A.~G.},
        title = "{Mapping of chemical elements on the surfaces of Ap stars. I. Solution of the inverse problem of finding local profiles of spectral lines}",
      journal = {\sovast},
         year = 1982,
        month = dec,
       volume = {26},
        pages = {690-696},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982SvA....26..690G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goncharskii1977,
       author = {{Goncharskii}, A.~V. and {Stepanov}, V.~V. and {Kokhlova}, V.~L. and {Yagola}, A.~G.},
        title = "{Reconstruction of local line profiles from those observed in an Ap spectrum.}",
      journal = {Pisma v Astronomicheskii Zhurnal},
         year = 1977,
        month = jun,
       volume = {3},
        pages = {278},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977PAZh....3..278G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Deutsch1958,
       author = {{Deutsch}, A.~J.},
        title = "{Harmonic Analysis of the Periodic Spectrum Variables}",
    booktitle = {Electromagnetic Phenomena in Cosmical Physics},
         year = 1958,
       editor = {{Lehnert}, B.},
       volume = {6},
        month = jan,
        pages = {209},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1958IAUS....6..209D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Deutsch1970,
       author = {{Deutsch}, Armin J.},
        title = "{Harmonic Analysis of Rigidly Rotating AP Stars}",
      journal = {\apj},
         year = 1970,
        month = mar,
       volume = {159},
        pages = {985},
          doi = {10.1086/150376},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970ApJ...159..985D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Falk1974,
       author = {{Falk}, Alfred E. and {Wehlau}, William H.},
        title = "{Harmonic Analysis of the Line Profiles of an Oblique Rotator}",
      journal = {\apj},
         year = 1974,
        month = sep,
       volume = {192},
        pages = {409-416},
          doi = {10.1086/153072},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ApJ...192..409F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Khokhlova1976,
       author = {{Khokhlova}, V.~L.},
        title = "{Mapping of ``spots'' on the surface of Ap stars by means of line profiles}",
      journal = {\sovast},
         year = 1976,
        month = apr,
       volume = {19},
        pages = {576},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1976SvA....19..576K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vogt&Penrod1983,
       author = {{Vogt}, S.~S. and {Penrod}, G.~D.},
        title = "{Doppler imaging of spotted stars : application to the RS Canum Venaticorum star HR 1099.}",
      journal = {\pasp},
     keywords = {Binary Stars, Imaging Techniques, Starspots, Coronal Holes, Doppler Effect, Line Spectra, Mapping, Stellar Rotation, Astrophysics},
         year = 1983,
        month = sep,
       volume = {95},
        pages = {565-576},
          doi = {10.1086/131208},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983PASP...95..565V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Donati1999,
       author = {{Donati}, J. -F.},
        title = "{Magnetic cycles of HR 1099 and LQ Hydrae}",
      journal = {\mnras},
     keywords = {LINE: PROFILES, STARS: ACTIVITY, BINARIES: GENERAL, STARS: IMAGING, STARS: MAGNETIC FIELDS, STARS: ROTATION},
         year = 1999,
        month = jan,
       volume = {302},
       number = {3},
        pages = {457-481},
          doi = {10.1046/j.1365-8711.1999.02096.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999MNRAS.302..457D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier1999a,
       author = {{Strassmeier}, K.~G. and {Lupinek}, S. and {Dempsey}, R.~C. and {Rice}, J.~B.},
        title = "{Doppler imaging of stellar surface structure. X. The FK Comae-type star HD 199178 = V 1794 Cygni}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: IMAGING, STARS: INDIVIDUAL: HD 199178, STARS: LATE-TYPE, STARS: STARSPOTS},
         year = 1999,
        month = jul,
       volume = {347},
        pages = {212-224},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&A...347..212S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier1999b,
       author = {{Strassmeier}, K.~G.},
        title = "{Doppler imaging of stellar surface structure. XI. The super starspots on the K0 giant HD 12545: larger than the entire Sun}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: IMAGING, STARS: INDIVIDUAL: HD 12545, STARS: LATE-TYPE, STARS: STARSPOTS},
         year = 1999,
        month = jul,
       volume = {347},
        pages = {225-234},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&A...347..225S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CollierCameron&Unruh1994,
       author = {{Collier Cameron}, A. and {Unruh}, Y.~C.},
        title = "{Doppler images of AB Doradus in 1992 January.}",
      journal = {\mnras},
         year = 1994,
        month = aug,
       volume = {269},
        pages = {814-836},
          doi = {10.1093/mnras/269.3.814},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994MNRAS.269..814C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hatzes1995,
       author = {{Hatzes}, Artie P.},
        title = "{Doppler Imaging of the Cool SPOT Distribution on the Weak T Tauri Star V410 Tauri}",
      journal = {\apj},
     keywords = {LINE: PROFILES, STARS: ACTIVITY, STARS: CHROMOSPHERES, STARS: INDIVIDUAL CONSTELLATION NAME: V410 TAURI, STARS: PRE-MAIN-SEQUENCE},
         year = 1995,
        month = oct,
       volume = {451},
        pages = {784},
          doi = {10.1086/176265},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...451..784H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barnes&CollierCameron2001a,
       author = {{Barnes}, J.~R. and {Collier Cameron}, A. and {James}, D.~J. and {Donati}, J. -F.},
        title = "{Doppler images from dual-site observations of southern rapidly rotating stars - II. Starspot patterns and differential rotation on Speedy Mic}",
      journal = {\mnras},
     keywords = {LINE: PROFILES, METHODS: DATA ANALYSIS, TECHNIQUES: MISCELLANEOUS, STARS: ACTIVITY, STARS: INDIVIDUAL: SPEEDY MIC (HD 197890), STARS: LATE-TYPE},
         year = 2001,
        month = jun,
       volume = {324},
       number = {1},
        pages = {231-242},
          doi = {10.1046/j.1365-8711.2001.04309.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.324..231B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Zaire2021,
       author = {{Zaire}, B. and {Donati}, J. -F. and {Klein}, B.},
        title = "{Magnetic field and activity phenomena of the K2 dwarf V471 Tau}",
      journal = {\mnras},
     keywords = {magnetic fields, techniques: polarimetric, binaries: eclipsing, stars: imaging, stars: individual: V471 Tau, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jun,
       volume = {504},
       number = {2},
        pages = {1969-1988},
          doi = {10.1093/mnras/stab1019},
archivePrefix = {arXiv},
       eprint = {2104.02619},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.504.1969Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Finociety2021,
       author = {{Finociety}, B. and {Donati}, J. -F. and {Klein}, B. and {Zaire}, B. and {Lehmann}, L. and {Moutou}, C. and {Bouvier}, J. and {Alencar}, S.~H.~P. and {Yu}, L. and {Grankin}, K. and {Artigau}, {\'E}. and {Doyon}, R. and {Delfosse}, X. and {Fouqu{\'e}}, P. and {H{\'e}brard}, G. and {Jardine}, M. and {K{\'o}sp{\'a}l}, {\'A}. and {M{\'e}nard}, F. and {M{\'e}nard}, F. and {SLS consortium}},
        title = "{The T Tauri star V410 Tau in the eyes of SPIRou and TESS}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, stars: activity, stars: imaging, stars: individual: V410 Tau, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = dec,
       volume = {508},
       number = {3},
        pages = {3427-3445},
          doi = {10.1093/mnras/stab2778},
archivePrefix = {arXiv},
       eprint = {2109.11755},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.508.3427F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barnes&CollierCameron2001b,
       author = {{Barnes}, J.~R. and {Collier Cameron}, A.},
        title = "{Starspot patterns on the M dwarfs HK Aqr and RE 1816 +541}",
      journal = {\mnras},
     keywords = {LINE: PROFILES, METHODS: DATA ANALYSIS, STARS: ACTIVITY, STARS: IMAGING, STARS: LATE-TYPE, STARS: SPOTS},
         year = 2001,
        month = sep,
       volume = {326},
       number = {3},
        pages = {950-958},
          doi = {10.1046/j.1365-8711.2001.04649.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.326..950B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barnes2004,
       author = {{Barnes}, J.~R. and {James}, D.~J. and {Collier Cameron}, A.},
        title = "{Differential rotation and star-spot evolution on HK Aqr in 2001 and 2002}",
      journal = {\mnras},
     keywords = {line: profiles, methods: data analysis, techniques: miscellaneous, stars: activity, stars: individual: HK Aqr (Gl 890), stars: late-type},
         year = 2004,
        month = aug,
       volume = {352},
       number = {2},
        pages = {589-599},
          doi = {10.1111/j.1365-2966.2004.07949.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.352..589B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fegley&Lodders1996,
       author = {{Fegley}, Bruce, Jr. and {Lodders}, Katharina},
        title = "{Atmospheric Chemistry of the Brown Dwarf Gliese 229B: Thermochemical Equilibrium Predictions}",
      journal = {\apjl},
     keywords = {INFRARED: STARS, STARS: ABUNDANCES, STARS: ATMOSPHERES, STARS: LOW-MASS, BROWN DWARFS, STARS: INDIVIDUAL NAME: GLIESE 229B},
         year = 1996,
        month = nov,
       volume = {472},
        pages = {L37},
          doi = {10.1086/310356},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...472L..37F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Noll1997,
       author = {{Noll}, Keith S. and {Geballe}, T.~R. and {Marley}, Mark S.},
        title = "{Detection of Abundant Carbon Monoxide in the Brown Dwarf Gliese 229B}",
      journal = {\apjl},
     keywords = {INFRARED: STARS, STARS: LOW-MASS, BROWN DWARFS, STARS: INDIVIDUAL NAME: GLIESE 229B, Infrared: Stars, Stars: Individual: Name: Gliese 229B, Stars: Low-Mass, Brown Dwarfs},
         year = 1997,
        month = nov,
       volume = {489},
       number = {1},
        pages = {L87-L90},
          doi = {10.1086/310954},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...489L..87N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Griffith&Yelle1999,
       author = {{Griffith}, Caitlin A. and {Yelle}, Roger V.},
        title = "{Disequilibrium Chemistry in a Brown Dwarf's Atmosphere: Carbon Monoxide in Gliese 229B}",
      journal = {\apjl},
     keywords = {CONVECTION, PLANETS AND SATELLITES: GENERAL, STARS: ATMOSPHERES, STARS: INDIVIDUAL: NAME: GLIESE 229B, STARS: LOW-MASS, BROWN DWARFS, Convection, Planets and Satellites: General, Stars: Atmospheres, Stars: Individual: Name: Gliese 229B, Stars: Low-Mass, Brown Dwarfs},
         year = 1999,
        month = jul,
       volume = {519},
       number = {1},
        pages = {L85-L88},
          doi = {10.1086/312103},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...519L..85G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon2000,
       author = {{Saumon}, D. and {Geballe}, T.~R. and {Leggett}, S.~K. and {Marley}, M.~S. and {Freedman}, R.~S. and {Lodders}, K. and {Fegley}, B., Jr. and {Sengupta}, S.~K.},
        title = "{Molecular Abundances in the Atmosphere of the T Dwarf GL 229B}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Individual: Alphanumeric: Gl 229B, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2000,
        month = sep,
       volume = {541},
       number = {1},
        pages = {374-389},
          doi = {10.1086/309410},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003353},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...541..374S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Saumon2006,
       author = {{Saumon}, D. and {Marley}, M.~S. and {Cushing}, M.~C. and {Leggett}, S.~K. and {Roellig}, T.~L. and {Lodders}, K. and {Freedman}, R.~S.},
        title = "{Ammonia as a Tracer of Chemical Equilibrium in the T7.5 Dwarf Gliese 570D}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Individual: Name: Gliese 570D, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = aug,
       volume = {647},
       number = {1},
        pages = {552-557},
          doi = {10.1086/505419},
archivePrefix = {arXiv},
       eprint = {astro-ph/0605563},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...647..552S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon2007,
       author = {{Saumon}, D. and {Marley}, M.~S. and {Leggett}, S.~K. and {Geballe}, T.~R. and {Stephens}, D. and {Golimowski}, D.~A. and {Cushing}, M.~C. and {Fan}, X. and {Rayner}, J.~T. and {Lodders}, K. and {Freedman}, R.~S.},
        title = "{Physical Parameters of Two Very Cool T Dwarfs}",
      journal = {\apj},
     keywords = {stars: individual (2MASS J04151954-0935066), stars: individual (2MASS J12171110-0311131), stars: individual (Gl 570D), Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = feb,
       volume = {656},
       number = {2},
        pages = {1136-1149},
          doi = {10.1086/510557},
archivePrefix = {arXiv},
       eprint = {astro-ph/0611062},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...656.1136S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hubeny&Burrows2007,
       author = {{Hubeny}, Ivan and {Burrows}, Adam},
        title = "{A Systematic Study of Departures from Chemical Equilibrium in the Atmospheres of Substellar Mass Objects}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Individual: Name: Gliese 570D, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {1248-1261},
          doi = {10.1086/522107},
archivePrefix = {arXiv},
       eprint = {0705.3922},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669.1248H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2007a,
       author = {{Leggett}, S.~K. and {Saumon}, D. and {Marley}, M.~S. and {Geballe}, T.~R. and {Golimowski}, D.~A. and {Stephens}, D. and {Fan}, X.},
        title = "{3.6-7.9 {\ensuremath{\mu}}m Photometry of L and T Dwarfs and the Prevalence of Vertical Mixing in their Atmospheres}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = feb,
       volume = {655},
       number = {2},
        pages = {1079-1094},
          doi = {10.1086/510014},
archivePrefix = {arXiv},
       eprint = {astro-ph/0610214},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...655.1079L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2007b,
       author = {{Leggett}, S.~K. and {Marley}, M.~S. and {Freedman}, R. and {Saumon}, D. and {Liu}, Michael C. and {Geballe}, T.~R. and {Golimowski}, D.~A. and {Stephens}, D.~C.},
        title = "{Physical and Spectral Characteristics of the T8 and Later Type Dwarfs}",
      journal = {\apj},
     keywords = {Infrared: Stars, stars: individual (2MASS J04151954-0935066), stars: individual (2MASS J09393548-2448279), stars: individual (2MASS J11145133-2618235), stars: individual (HD 3651B), stars: individual (Gl 570D), Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = sep,
       volume = {667},
       number = {1},
        pages = {537-548},
          doi = {10.1086/519948},
archivePrefix = {arXiv},
       eprint = {0705.2602},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...667..537L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2008,
       author = {{Leggett}, S.~K. and {Saumon}, D. and {Albert}, Loic and {Cushing}, Michael C. and {Liu}, Michael C. and {Luhman}, K.~L. and {Marley}, M.~S. and {Kirkpatrick}, J. Davy and {Roellig}, Thomas L. and {Allers}, K.~N.},
        title = "{HN Peg B: A Test of Models of the L to T Dwarf Transition}",
      journal = {\apj},
     keywords = {binaries: visual, stars: individual: 2MASS J21442847+1446077 HN Peg HN Peg B, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = aug,
       volume = {682},
       number = {2},
        pages = {1256-1263},
          doi = {10.1086/589146},
archivePrefix = {arXiv},
       eprint = {0804.1386},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...682.1256L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Freytag2010,
       author = {{Freytag}, B. and {Allard}, F. and {Ludwig}, H. -G. and {Homeier}, D. and {Steffen}, M.},
        title = "{The role of convection, overshoot, and gravity waves for the transport of dust in M dwarf and brown dwarf atmospheres}",
      journal = {\aap},
     keywords = {brown dwarfs, hydrodynamics, convection, waves, stars: atmospheres, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = apr,
       volume = {513},
          eid = {A19},
        pages = {A19},
          doi = {10.1051/0004-6361/200913354},
archivePrefix = {arXiv},
       eprint = {1002.3437},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...513A..19F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hirano2011,
       author = {{Hirano}, Teruyuki and {Suto}, Yasushi and {Winn}, Joshua N. and {Taruya}, Atsushi and {Narita}, Norio and {Albrecht}, Simon and {Sato}, Bun'ei},
        title = "{Improved Modeling of the Rossiter-McLaughlin Effect for Transiting Exoplanets}",
      journal = {\apj},
     keywords = {planets and satellites: general, planets and satellites: formation, stars: rotation, techniques: radial velocities, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = dec,
       volume = {742},
       number = {2},
          eid = {69},
        pages = {69},
          doi = {10.1088/0004-637X/742/2/69},
archivePrefix = {arXiv},
       eprint = {1108.4430},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...742...69H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Albrecht2007,
       author = {{Albrecht}, S. and {Reffert}, S. and {Quirrenbach}, A. and {Mitchell}, D.~S. and {Snellen}, I.},
        title = "{The Rossiter-McLaughlin Effect in the Eclipsing Binary System V1143 Cyg -- First Results}",
    booktitle = {Solar and Stellar Physics Through Eclipses},
         year = 2007,
       editor = {{Demircan}, O. and {Selam}, S.~O. and {Albayrak}, B.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {370},
        month = may,
        pages = {218},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ASPC..370..218A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Johnson2014,
       author = {{Johnson}, Marshall C. and {Cochran}, William D. and {Albrecht}, Simon and {Dodson-Robinson}, Sarah E. and {Winn}, Joshua N. and {Gullikson}, Kevin},
        title = "{A Misaligned Prograde Orbit for Kepler-13 Ab via Doppler Tomography}",
      journal = {\apj},
     keywords = {line: profiles, planetary systems, planets and satellites: individual: Kepler-13 Ab, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = jul,
       volume = {790},
       number = {1},
          eid = {30},
        pages = {30},
          doi = {10.1088/0004-637X/790/1/30},
archivePrefix = {arXiv},
       eprint = {1406.0512},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...790...30J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Molliere2020,
       author = {{Molli{\`e}re}, P. and {Stolker}, T. and {Lacour}, S. and {Otten}, G.~P.~P.~L. and {Shangguan}, J. and {Charnay}, B. and {Molyarova}, T. and {Nowak}, M. and {Henning}, Th. and {Marleau}, G. -D. and {Semenov}, D.~A. and {van Dishoeck}, E. and {Eisenhauer}, F. and {Garcia}, P. and {Garcia Lopez}, R. and {Girard}, J.~H. and {Greenbaum}, A.~Z. and {Hinkley}, S. and {Kervella}, P. and {Kreidberg}, L. and {Maire}, A. -L. and {Nasedkin}, E. and {Pueyo}, L. and {Snellen}, I.~A.~G. and {Vigan}, A. and {Wang}, J. and {de Zeeuw}, P.~T. and {Zurlo}, A.},
        title = "{Retrieving scattering clouds and disequilibrium chemistry in the atmosphere of HR 8799e}",
      journal = {\aap},
     keywords = {methods: numerical, planets and satellites: atmospheres, radiative transfer, instrumentation: spectrographs, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {A131},
        pages = {A131},
          doi = {10.1051/0004-6361/202038325},
archivePrefix = {arXiv},
       eprint = {2006.09394},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640A.131M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Barman2015,
       author = {{Barman}, Travis S. and {Konopacky}, Quinn M. and {Macintosh}, Bruce and {Marois}, Christian},
        title = "{Simultaneous Detection of Water, Methane, and Carbon Monoxide in the Atmosphere of Exoplanet HR8799b}",
      journal = {\apj},
     keywords = {brown dwarfs, planetary systems, stars: atmospheres, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = may,
       volume = {804},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/804/1/61},
archivePrefix = {arXiv},
       eprint = {1503.03539},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...804...61B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Konopacky2013,
       author = {{Konopacky}, Quinn M. and {Barman}, Travis S. and {Macintosh}, Bruce A. and {Marois}, Christian},
        title = "{Detection of Carbon Monoxide and Water Absorption Lines in an Exoplanet Atmosphere}",
      journal = {Science},
     keywords = {ASTRONOMY Astronomy, Ecology, Chemistry, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = mar,
       volume = {339},
       number = {6126},
        pages = {1398-1401},
          doi = {10.1126/science.1232003},
archivePrefix = {arXiv},
       eprint = {1303.3280},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013Sci...339.1398K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skemer2014,
       author = {{Skemer}, Andrew J. and {Marley}, Mark S. and {Hinz}, Philip M. and {Morzinski}, Katie M. and {Skrutskie}, Michael F. and {Leisenring}, Jarron M. and {Close}, Laird M. and {Saumon}, Didier and {Bailey}, Vanessa P. and {Briguglio}, Runa and {Defrere}, Denis and {Esposito}, Simone and {Follette}, Katherine B. and {Hill}, John M. and {Males}, Jared R. and {Puglisi}, Alfio and {Rodigas}, Timothy J. and {Xompero}, Marco},
        title = "{Directly Imaged L-T Transition Exoplanets in the Mid-infrared}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: planetary systems, instrumentation: adaptive optics, planets and satellites: atmospheres, planets and satellites: gaseous planets, stars: individual: HR 8799 2M1207 b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = sep,
       volume = {792},
       number = {1},
          eid = {17},
        pages = {17},
          doi = {10.1088/0004-637X/792/1/17},
archivePrefix = {arXiv},
       eprint = {1311.2085},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...792...17S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Currie2014,
       author = {{Currie}, Thayne and {Burrows}, Adam and {Girard}, Julien H. and {Cloutier}, Ryan and {Fukagawa}, Misato and {Sorahana}, Satoko and {Kuchner}, Marc and {Kenyon}, Scott J. and {Madhusudhan}, Nikku and {Itoh}, Yoichi and {Jayawardhana}, Ray and {Matsumura}, Soko and {Pyo}, Tae-Soo},
        title = "{Deep Thermal Infrared Imaging of HR 8799 bcde: New Atmospheric Constraints and Limits on a Fifth Planet}",
      journal = {\apj},
     keywords = {planetary systems, planets and satellites: atmospheres, planets and satellites: composition, stars: early-type, stars: individual: HR 8799, techniques: high angular resolution, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = nov,
       volume = {795},
       number = {2},
          eid = {133},
        pages = {133},
          doi = {10.1088/0004-637X/795/2/133},
archivePrefix = {arXiv},
       eprint = {1409.5134},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...795..133C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lavie2017,
       author = {{Lavie}, Baptiste and {Mendon{\c{c}}a}, Jo{\~a}o M. and {Mordasini}, Christoph and {Malik}, Matej and {Bonnefoy}, Micka{\"e}l and {Demory}, Brice-Olivier and {Oreshenko}, Maria and {Grimm}, Simon L. and {Ehrenreich}, David and {Heng}, Kevin},
        title = "{HELIOS-RETRIEVAL: An Open-source, Nested Sampling Atmospheric Retrieval Code; Application to the HR 8799 Exoplanets and Inferred Constraints for Planet Formation}",
      journal = {\aj},
     keywords = {methods: statistical, planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: formation, planets and satellites: gaseous planets, planets and satellites: individual: HR 8799, Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2017,
        month = sep,
       volume = {154},
       number = {3},
          eid = {91},
        pages = {91},
          doi = {10.3847/1538-3881/aa7ed8},
archivePrefix = {arXiv},
       eprint = {1610.03216},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154...91L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Kass&Raftery1995,
author = { Robert E.   Kass  and  Adrian E.   Raftery },
title = {Bayes Factors},
journal = {Journal of the American Statistical Association},
volume = {90},
number = {430},
pages = {773-795},
year  = {1995},
publisher = {Taylor & Francis},
doi = {10.1080/01621459.1995.10476572},

URL = { 
        https://www.tandfonline.com/doi/abs/10.1080/01621459.1995.10476572
    
},
eprint = { 
        https://www.tandfonline.com/doi/pdf/10.1080/01621459.1995.10476572
    
}

}


@ARTICLE{Bonnefoy2016,
       author = {{Bonnefoy}, M. and {Zurlo}, A. and {Baudino}, J.~L. and {Lucas}, P. and {Mesa}, D. and {Maire}, A. -L. and {Vigan}, A. and {Galicher}, R. and {Homeier}, D. and {Marocco}, F. and {Gratton}, R. and {Chauvin}, G. and {Allard}, F. and {Desidera}, S. and {Kasper}, M. and {Moutou}, C. and {Lagrange}, A. -M. and {Antichi}, J. and {Baruffolo}, A. and {Baudrand}, J. and {Beuzit}, J. -L. and {Boccaletti}, A. and {Cantalloube}, F. and {Carbillet}, M. and {Charton}, J. and {Claudi}, R.~U. and {Costille}, A. and {Dohlen}, K. and {Dominik}, C. and {Fantinel}, D. and {Feautrier}, P. and {Feldt}, M. and {Fusco}, T. and {Gigan}, P. and {Girard}, J.~H. and {Gluck}, L. and {Gry}, C. and {Henning}, T. and {Janson}, M. and {Langlois}, M. and {Madec}, F. and {Magnard}, Y. and {Maurel}, D. and {Mawet}, D. and {Meyer}, M.~R. and {Milli}, J. and {Moeller-Nilsson}, O. and {Mouillet}, D. and {Pavlov}, A. and {Perret}, D. and {Pujet}, P. and {Quanz}, S.~P. and {Rochat}, S. and {Rousset}, G. and {Roux}, A. and {Salasnich}, B. and {Salter}, G. and {Sauvage}, J. -F. and {Schmid}, H.~M. and {Sevin}, A. and {Soenke}, C. and {Stadler}, E. and {Turatto}, M. and {Udry}, S. and {Vakili}, F. and {Wahhaj}, Z. and {Wildi}, F.},
        title = "{First light of the VLT planet finder SPHERE. IV. Physical and chemical properties of the planets around HR8799}",
      journal = {\aap},
     keywords = {instrumentation: high angular resolution, stars: individual: HR8799, planets and satellites: atmospheres, planets and satellites: detection, techniques: imaging spectroscopy, planets and satellites: fundamental parameters, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = mar,
       volume = {587},
          eid = {A58},
        pages = {A58},
          doi = {10.1051/0004-6361/201526906},
archivePrefix = {arXiv},
       eprint = {1511.04082},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...587A..58B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Chauvin2017,
       author = {{Chauvin}, G. and {Desidera}, S. and {Lagrange}, A. -M. and {Vigan}, A. and {Feldt}, M. and {Gratton}, R. and {Langlois}, M. and {Cheetham}, A. and {Bonnefoy}, M. and {Meyer}, M.},
        title = "{SHINE, The SpHere INfrared survey for Exoplanets}",
     keywords = {Imaging and spectroscopy, Planets: physical parameters, atmospheres and formation},
    booktitle = {SF2A-2017: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics},
         year = 2017,
       editor = {{Reyl{\'e}}, C. and {Di Matteo}, P. and {Herpin}, F. and {Lagadec}, E. and {Lan{\c{c}}on}, A. and {Meliani}, Z. and {Royer}, F.},
        month = dec,
        pages = {Di},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017sf2a.conf..331C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeRosa2016,
       author = {{De Rosa}, Robert J. and {Rameau}, Julien and {Patience}, Jenny and {Graham}, James R. and {Doyon}, Ren{\'e} and {Lafreni{\`e}re}, David and {Macintosh}, Bruce and {Pueyo}, Laurent and {Rajan}, Abhijith and {Wang}, Jason J. and {Ward-Duong}, Kimberly and {Hung}, Li-Wei and {Maire}, J{\'e}r{\^o}me and {Nielsen}, Eric L. and {Ammons}, S. Mark and {Bulger}, Joanna and {Cardwell}, Andrew and {Chilcote}, Jeffrey K. and {Galvez}, Ramon L. and {Gerard}, Benjamin L. and {Goodsell}, Stephen and {Hartung}, Markus and {Hibon}, Pascale and {Ingraham}, Patrick and {Johnson-Groh}, Mara and {Kalas}, Paul and {Konopacky}, Quinn M. and {Marchis}, Franck and {Marois}, Christian and {Metchev}, Stanimir and {Morzinski}, Katie M. and {Oppenheimer}, Rebecca and {Perrin}, Marshall D. and {Rantakyr{\"o}}, Fredrik T. and {Savransky}, Dmitry and {Thomas}, Sandrine},
        title = "{Spectroscopic Characterization of HD 95086 b with the Gemini Planet Imager}",
      journal = {\apj},
     keywords = {infrared: planetary systems, instrumentation: adaptive optics, planets and satellites: atmospheres, stars: individual: HD 95086, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = jun,
       volume = {824},
       number = {2},
          eid = {121},
        pages = {121},
          doi = {10.3847/0004-637X/824/2/121},
archivePrefix = {arXiv},
       eprint = {1604.01411},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824..121D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Currie2011,
       author = {{Currie}, Thayne and {Burrows}, Adam and {Itoh}, Yoichi and {Matsumura}, Soko and {Fukagawa}, Misato and {Apai}, Daniel and {Madhusudhan}, Nikku and {Hinz}, Philip M. and {Rodigas}, T.~J. and {Kasper}, Markus and {Pyo}, T. -S. and {Ogino}, Satoshi},
        title = "{A Combined Subaru/VLT/MMT 1-5 {\ensuremath{\mu}}m Study of Planets Orbiting HR 8799: Implications for Atmospheric Properties, Masses, and Formation}",
      journal = {\apj},
     keywords = {brown dwarfs, instrumentation: adaptive optics, planetary systems, stars: individual: HR 8799, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = mar,
       volume = {729},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.1088/0004-637X/729/2/128},
archivePrefix = {arXiv},
       eprint = {1101.1973},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...729..128C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Madhusudhan2011,
       author = {{Madhusudhan}, Nikku and {Burrows}, Adam and {Currie}, Thayne},
        title = "{Model Atmospheres for Massive Gas Giants with Thick Clouds: Application to the HR 8799 Planets and Predictions for Future Detections}",
      journal = {\apj},
     keywords = {planetary systems, planets and satellites: general, planets and satellites: individual: HR 8799b HR 8799c HR 8799d, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = aug,
       volume = {737},
       number = {1},
          eid = {34},
        pages = {34},
          doi = {10.1088/0004-637X/737/1/34},
archivePrefix = {arXiv},
       eprint = {1102.5089},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737...34M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Galicher2011,
       author = {{Galicher}, Rapha{\"e}l and {Marois}, Christian and {Macintosh}, Bruce and {Barman}, Travis and {Konopacky}, Quinn},
        title = "{M-band Imaging of the HR 8799 Planetary System Using an Innovative LOCI-based Background Subtraction Technique}",
      journal = {\apjl},
     keywords = {instrumentation: high angular resolution, methods: data analysis, methods: observational, planetary systems, planets and satellites: atmospheres, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = oct,
       volume = {739},
       number = {2},
          eid = {L41},
        pages = {L41},
          doi = {10.1088/2041-8205/739/2/L41},
archivePrefix = {arXiv},
       eprint = {1107.0967},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...739L..41G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Tuomi2019,
       author = {{Tuomi}, M. and {Jones}, H.~R.~A. and {Butler}, R.~P. and {Arriagada}, P. and {Vogt}, S.~S. and {Burt}, J. and {Laughlin}, G. and {Holden}, B. and {Shectman}, S.~A. and {Crane}, J.~D. and {Thompson}, I. and {Keiser}, S. and {Jenkins}, J.~S. and {Berdi{\~n}as}, Z. and {Diaz}, M. and {Kiraga}, M. and {Barnes}, J.~R.},
        title = "{Frequency of planets orbiting M dwarfs in the Solar neighbourhood}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jun,
          eid = {arXiv:1906.04644},
        pages = {arXiv:1906.04644},
archivePrefix = {arXiv},
       eprint = {1906.04644},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190604644T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mulders2015a,
       author = {{Mulders}, Gijs D. and {Pascucci}, Ilaria and {Apai}, D{\'a}niel},
        title = "{A Stellar-mass-dependent Drop in Planet Occurrence Rates}",
      journal = {\apj},
     keywords = {planetary systems, planet-star interactions, planets and satellites: formation, protoplanetary disks, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = jan,
       volume = {798},
       number = {2},
          eid = {112},
        pages = {112},
          doi = {10.1088/0004-637X/798/2/112},
archivePrefix = {arXiv},
       eprint = {1406.7356},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798..112M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mulders2015b,
       author = {{Mulders}, Gijs D. and {Pascucci}, Ilaria and {Apai}, D{\'a}niel},
        title = "{An Increase in the Mass of Planetary Systems around Lower-mass Stars}",
      journal = {\apj},
     keywords = {planets and satellites: formation, planetary systems, protoplanetary disks, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = dec,
       volume = {814},
       number = {2},
          eid = {130},
        pages = {130},
          doi = {10.1088/0004-637X/814/2/130},
archivePrefix = {arXiv},
       eprint = {1510.02481},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...814..130M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mulders2021,
       author = {{Mulders}, Gijs D. and {Dr{\k{a}}{\.z}kowska}, Joanna and {van der Marel}, Nienke and {Ciesla}, Fred J. and {Pascucci}, Ilaria},
        title = "{Why Do M Dwarfs Have More Transiting Planets?}",
      journal = {\apjl},
     keywords = {Exoplanets, Exoplanet formation, Planet formation, Planetary system formation, Protoplanetary disks, 498, 492, 1241, 1257, 1300, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.3847/2041-8213/ac2947},
archivePrefix = {arXiv},
       eprint = {2110.02971},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920L...1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Howard2012,
       author = {{Howard}, Andrew W. and {Marcy}, Geoffrey W. and {Bryson}, Stephen T. and {Jenkins}, Jon M. and {Rowe}, Jason F. and {Batalha}, Natalie M. and {Borucki}, William J. and {Koch}, David G. and {Dunham}, Edward W. and {Gautier}, Thomas N., III and {Van Cleve}, Jeffrey and {Cochran}, William D. and {Latham}, David W. and {Lissauer}, Jack J. and {Torres}, Guillermo and {Brown}, Timothy M. and {Gilliland}, Ronald L. and {Buchhave}, Lars A. and {Caldwell}, Douglas A. and {Christensen-Dalsgaard}, J{\o}rgen and {Ciardi}, David and {Fressin}, Francois and {Haas}, Michael R. and {Howell}, Steve B. and {Kjeldsen}, Hans and {Seager}, Sara and {Rogers}, Leslie and {Sasselov}, Dimitar D. and {Steffen}, Jason H. and {Basri}, Gibor S. and {Charbonneau}, David and {Christiansen}, Jessie and {Clarke}, Bruce and {Dupree}, Andrea and {Fabrycky}, Daniel C. and {Fischer}, Debra A. and {Ford}, Eric B. and {Fortney}, Jonathan J. and {Tarter}, Jill and {Girouard}, Forrest R. and {Holman}, Matthew J. and {Johnson}, John Asher and {Klaus}, Todd C. and {Machalek}, Pavel and {Moorhead}, Althea V. and {Morehead}, Robert C. and {Ragozzine}, Darin and {Tenenbaum}, Peter and {Twicken}, Joseph D. and {Quinn}, Samuel N. and {Isaacson}, Howard and {Shporer}, Avi and {Lucas}, Philip W. and {Walkowicz}, Lucianne M. and {Welsh}, William F. and {Boss}, Alan and {Devore}, Edna and {Gould}, Alan and {Smith}, Jeffrey C. and {Morris}, Robert L. and {Prsa}, Andrej and {Morton}, Timothy D. and {Still}, Martin and {Thompson}, Susan E. and {Mullally}, Fergal and {Endl}, Michael and {MacQueen}, Phillip J.},
        title = "{Planet Occurrence within 0.25 AU of Solar-type Stars from Kepler}",
      journal = {\apjs},
     keywords = {planetary systems, stars: statistics, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = aug,
       volume = {201},
       number = {2},
          eid = {15},
        pages = {15},
          doi = {10.1088/0067-0049/201/2/15},
archivePrefix = {arXiv},
       eprint = {1103.2541},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJS..201...15H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sabotta2021,
       author = {{Sabotta}, S. and {Schlecker}, M. and {Chaturvedi}, P. and {Guenther}, E.~W. and {Mu{\~n}oz Rodr{\'\i}guez}, I. and {Mu{\~n}oz S{\'a}nchez}, J.~C. and {Caballero}, J.~A. and {Shan}, Y. and {Reffert}, S. and {Ribas}, I. and {Reiners}, A. and {Hatzes}, A.~P. and {Amado}, P.~J. and {Klahr}, H. and {Morales}, J.~C. and {Quirrenbach}, A. and {Henning}, Th. and {Dreizler}, S. and {Pall{\'e}}, E. and {Perger}, M. and {Azzaro}, M. and {Jeffers}, S.~V. and {Kaminski}, A. and {K{\"u}rster}, M. and {Lafarga}, M. and {Montes}, D. and {Passegger}, V.~M. and {Zechmeister}, M.},
        title = "{The CARMENES search for exoplanets around M dwarfs. Planet occurrence rates from a subsample of 71 stars}",
      journal = {\aap},
     keywords = {planetary systems, techniques: radial velocities, methods: data analysis, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
       volume = {653},
          eid = {A114},
        pages = {A114},
          doi = {10.1051/0004-6361/202140968},
archivePrefix = {arXiv},
       eprint = {2107.03802},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...653A.114S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vos2022b,
       author = {{Vos}, Johanna M. and {Burningham}, Ben and {Faherty}, Jacqueline K. and {Alejandro}, Sherelyn and {Gonzales}, Eileen and {Calamari}, Emily and {Bardalez Gagliuffi}, Daniella and {Visscher}, Channon and {Tan}, Xianyu and {Morley}, Caroline V. and {Marley}, Mark and {Gemma}, Marina E. and {Whiteford}, Niall and {Gaarn}, Josefine and {Park}, Grace},
        title = "{Patchy Forsterite Clouds in the Atmospheres of Two Highly Variable Exoplanet Analogs}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = dec,
          eid = {arXiv:2212.07399},
        pages = {arXiv:2212.07399},
archivePrefix = {arXiv},
       eprint = {2212.07399},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv221207399V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Khokhlova1986,
       author = {{Khokhlova}, V.~L. and {Rice}, J.~B. and {Wehlau}, W.~H.},
        title = "{Distribution of Chemical Elements over the Surface of the Magnetic AP Star Theta Aurigae}",
      journal = {\apj},
     keywords = {A Stars, Magnetic Stars, Peculiar Stars, Stellar Composition, Abundance, Chromium, Iron, Line Spectra, Spatial Distribution, Astrophysics, LINE PROFILES, STARS: ABUNDANCES, STARS: INDIVIDUAL CONSTELLATION NAME: THETA AURIGAE, STARS: PECULIAR A, STARS: SPECTRUM VARIABLES},
         year = 1986,
        month = aug,
       volume = {307},
        pages = {768},
          doi = {10.1086/164462},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986ApJ...307..768K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Khokhlova1985,
       author = {{Khokhlova}, V.~L.},
        title = "{Magnetic AP stars}",
      journal = {\apspr},
     keywords = {A Stars, Magnetic Stars, Peculiar Stars, Stellar Composition, Stellar Spectra, Helium, Hertzsprung-Russell Diagram, Stellar Physics, Astrophysics},
         year = 1985,
        month = jan,
       volume = {4},
        pages = {99-159},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ASPRv...4...99K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Albrecht2022,
       author = {{Albrecht}, Ethan M. and {Jensen}, Audra M. and {Jensen}, Erik G. and {Wilson}, Kody A. and {Plummer}, Michael K. and {Key}, Joshua A. and {O'Keefe}, Daniel S. and {Chun}, Francis K. and {Strong}, David M. and {Schuetz-Christy}, Casey P.},
        title = "{Near-Simultaneous Observations of a Geosynchronous Satellite Using Two Telescopes and Multiple Optical Filters}",
      journal = {Journal of the Astronautical Sciences},
     keywords = {Space domain awareness, Geosynchronous satellites, Polarization, Stokes parameters, Slitless Spectroscopy, Photometry, Near-simultaneous imagery, Non-resolved imagery},
         year = 2022,
        month = feb,
       volume = {69},
       number = {1},
        pages = {120-138},
          doi = {10.1007/s40295-021-00292-x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022JAnSc..69..120A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhou2020b,
       author = {{Zhou}, Yifan and {Bowler}, Brendan P. and {Morley}, Caroline V. and {Apai}, D{\'a}niel and {Kataria}, Tiffany and {Bryan}, Marta L. and {Benneke}, Bj{\"o}rn},
        title = "{Spectral Variability of VHS J1256-1257b from 1 to 5 {\ensuremath{\mu}}m}",
      journal = {\aj},
     keywords = {Brown dwarfs, L dwarfs, Atmospheric variability, Light curves, Exoplanet atmospheres, Time series analysis, Photometry, Spectrophotometry, 185, 894, 2119, 918, 487, 1916, 1234, 1556, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {160},
       number = {2},
          eid = {77},
        pages = {77},
          doi = {10.3847/1538-3881/ab9e04},
archivePrefix = {arXiv},
       eprint = {2004.05168},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160...77Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Biller2018,
       author = {{Biller}, Beth A. and {Vos}, Johanna and {Buenzli}, Esther and {Allers}, Katelyn and {Bonnefoy}, Micka{\"e}l and {Charnay}, Benjamin and {B{\'e}zard}, Bruno and {Allard}, France and {Homeier}, Derek and {Bonavita}, Mariangela and {Brandner}, Wolfgang and {Crossfield}, Ian and {Dupuy}, Trent and {Henning}, Thomas and {Kopytova}, Taisiya and {Liu}, Michael C. and {Manjavacas}, Elena and {Schlieder}, Joshua},
        title = "{Simultaneous Multiwavelength Variability Characterization of the Free-floating Planetary-mass Object PSO J318.5-22}",
      journal = {\aj},
     keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = feb,
       volume = {155},
       number = {2},
          eid = {95},
        pages = {95},
          doi = {10.3847/1538-3881/aaa5a6},
archivePrefix = {arXiv},
       eprint = {1712.03746},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....155...95B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Buenzli2012,
       author = {{Buenzli}, Esther and {Apai}, D{\'a}niel and {Morley}, Caroline V. and {Flateau}, Davin and {Showman}, Adam P. and {Burrows}, Adam and {Marley}, Mark S. and {Lewis}, Nikole K. and {Reid}, I. Neill},
        title = "{Vertical Atmospheric Structure in a Variable Brown Dwarf: Pressure-dependent Phase Shifts in Simultaneous Hubble Space Telescope-Spitzer Light Curves}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: atmospheres, stars: individual: 2MASS J22282889{\textendash}4310262, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = dec,
       volume = {760},
       number = {2},
          eid = {L31},
        pages = {L31},
          doi = {10.1088/2041-8205/760/2/L31},
archivePrefix = {arXiv},
       eprint = {1210.6654},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...760L..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schlawin2017,
       author = {{Schlawin}, E. and {Burgasser}, Adam J. and {Karalidi}, T. and {Gizis}, J.~E. and {Teske}, J.},
        title = "{Spectral Variability of Two Rapidly Rotating Brown Dwarfs: 2MASS J08354256-0819237 and 2MASS J18212815+1414010}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, stars: individual: 2MASS J08354256-0819237, 2MASS J18212815+1414010, stars: late-type, techniques: spectroscopic, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = nov,
       volume = {849},
       number = {2},
          eid = {163},
        pages = {163},
          doi = {10.3847/1538-4357/aa90b8},
archivePrefix = {arXiv},
       eprint = {1709.06565},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...849..163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Yang2015,
       author = {{Yang}, Hao and {Apai}, D{\'a}niel and {Marley}, Mark S. and {Saumon}, Didier and {Morley}, Caroline V. and {Buenzli}, Esther and {Artigau}, {\'E}tienne and {Radigan}, Jacqueline and {Metchev}, Stanimir and {Burgasser}, Adam J. and {Mohanty}, Subhanjoy and {Lowrance}, Patrick J. and {Showman}, Adam P. and {Karalidi}, Theodora and {Flateau}, Davin and {Heinze}, Aren N.},
        title = "{HST Rotational Spectral Mapping of Two L-type Brown Dwarfs: Variability in and out of Water Bands indicates High-altitude Haze Layers}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: atmospheres, stars: individual: 2MASS J18212815+1414010 2MASS J15074769-1627386 2MASS J01365662+0933473, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jan,
       volume = {798},
       number = {1},
          eid = {L13},
        pages = {L13},
          doi = {10.1088/2041-8205/798/1/L13},
archivePrefix = {arXiv},
       eprint = {1411.2911},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798L..13Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Manjavacas2021,
       author = {{Manjavacas}, Elena and {Karalidi}, Theodora and {Vos}, Johanna M. and {Biller}, Beth A. and {Lew}, Ben W.~P.},
        title = "{Revealing the Vertical Cloud Structure of a Young Low-mass Brown Dwarf, an Analog to the {\ensuremath{\beta}}-Pictoris b Directly Imaged Exoplanet, through Keck I/MOSFIRE Spectrophotometric Variability}",
      journal = {\aj},
     keywords = {L dwarfs, 894, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = nov,
       volume = {162},
       number = {5},
          eid = {179},
        pages = {179},
          doi = {10.3847/1538-3881/ac174c},
archivePrefix = {arXiv},
       eprint = {2107.12368},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....162..179M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lew2020b,
       author = {{Lew}, Ben W.~P. and {Apai}, D{\'a}niel and {Marley}, Mark and {Saumon}, Didier and {Schneider}, Glenn and {Zhou}, Yifan and {Cowan}, Nicolas B. and {Karalidi}, Theodora and {Manjavacas}, Elena and {Bedin}, L.~R. and {Miles-P{\'a}ez}, Paulo A.},
        title = "{Cloud Atlas: Unraveling the Vertical Cloud Structure with the Time-series Spectrophotometry of an Unusually Red Brown Dwarf}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Exoplanet atmospheric variability, Brown dwarfs, Clouds, 487, 2020, 185, 258, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = nov,
       volume = {903},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.3847/1538-4357/abb81d},
archivePrefix = {arXiv},
       eprint = {2009.10714},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...903...15L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhou2020,
       author = {{Zhou}, Yifan and {Apai}, D{\'a}niel and {Bedin}, Luigi R. and {Lew}, Ben W.~P. and {Schneider}, Glenn and {Burgasser}, Adam J. and {Manjavacas}, Elena and {Karalidi}, Theodora and {Metchev}, Stanimir and {Miles-P{\'a}ez}, Paulo A. and {Cowan}, Nicolas B. and {Lowrance}, Patrick J. and {Radigan}, Jacqueline},
        title = "{Cloud Atlas: High-precision HST/WFC3/IR Time-resolved Observations of Directly Imaged Exoplanet HD 106906b}",
      journal = {\aj},
     keywords = {1093, 487, 2020, 387, 80, 1916, 756, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = apr,
       volume = {159},
       number = {4},
          eid = {140},
        pages = {140},
          doi = {10.3847/1538-3881/ab6f65},
archivePrefix = {arXiv},
       eprint = {2001.08304},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159..140Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lew2020a,
       author = {{Lew}, Ben W.~P. and {Apai}, D{\'a}niel and {Zhou}, Yifan and {Radigan}, Jacqueline and {Marley}, Mark and {Schneider}, Glenn and {Cowan}, Nicolas B. and {Miles-P{\'a}ez}, Paulo A. and {Manjavacas}, Elena and {Karalidi}, Theodora and {Bedin}, L.~R. and {Lowrance}, Patrick J. and {Burgasser}, Adam J.},
        title = "{Cloud Atlas: Weak Color Modulations Due to Rotation in the Planetary-mass Companion GU Psc b and 11 Other Brown Dwarfs}",
      journal = {\aj},
     keywords = {185, 487, 1244, 2020, 1679, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = mar,
       volume = {159},
       number = {3},
          eid = {125},
        pages = {125},
          doi = {10.3847/1538-3881/ab5f59},
archivePrefix = {arXiv},
       eprint = {1912.02812},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....159..125L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MilesPaez2019,
       author = {{Miles-P{\'a}ez}, Paulo A. and {Metchev}, Stanimir and {Apai}, D{\'a}niel and {Zhou}, Yifan and {Manjavacas}, Elena and {Karalidi}, Theodora and {Lew}, Ben W.~P. and {Burgasser}, Adam J. and {Bedin}, Luigi R. and {Cowan}, Nicolas and {Lowrance}, Patrick J. and {Marley}, Mark S. and {Radigan}, Jacqueline and {Schneider}, Glenn},
        title = "{Cloud Atlas: Variability in and out of the Water Band in the Planetary-mass HD 203030B Points to Cloud Sedimentation in Low-gravity L Dwarfs}",
      journal = {\apj},
     keywords = {Brown dwarfs, Light curves, Exoplanet atmospheres, 185, 918, 487, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = oct,
       volume = {883},
       number = {2},
          eid = {181},
        pages = {181},
          doi = {10.3847/1538-4357/ab3d25},
archivePrefix = {arXiv},
       eprint = {1908.09403},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...883..181M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Manjavacas2019b,
       author = {{Manjavacas}, Elena and {Apai}, D{\'a}niel and {Lew}, Ben W.~P. and {Zhou}, Yifan and {Schneider}, Glenn and {Burgasser}, Adam J. and {Karalidi}, Theodora and {Miles-P{\'a}ez}, Paulo A. and {Lowrance}, Patrick J. and {Cowan}, Nicolas and {Bedin}, Luigi R. and {Marley}, Mark S. and {Metchev}, Stan and {Radigan}, Jacqueline},
        title = "{Cloud Atlas: Rotational Spectral Modulations and Potential Sulfide Clouds in the Planetary-mass, Late T-type Companion Ross 458C}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = apr,
       volume = {875},
       number = {2},
          eid = {L15},
        pages = {L15},
          doi = {10.3847/2041-8213/ab13b9},
archivePrefix = {arXiv},
       eprint = {1903.10702},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...875L..15M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhou2019,
       author = {{Zhou}, Yifan and {Apai}, D{\'a}niel and {Lew}, Ben W.~P. and {Schneider}, Glenn and {Manjavacas}, Elena and {Bedin}, Luigi R. and {Cowan}, Nicolas B. and {Marley}, Mark S. and {Radigan}, Jacqueline and {Karalidi}, Theodora and {Lowrance}, Patrick J. and {Miles-P{\'a}ez}, Paulo A. and {Metchev}, Stanimir and {Burgasser}, Adam J.},
        title = "{Cloud Atlas: High-contrast Time-resolved Observations of Planetary-mass Companions}",
      journal = {\aj},
     keywords = {methods: observational, planetary systems, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {157},
       number = {3},
          eid = {128},
        pages = {128},
          doi = {10.3847/1538-3881/ab037f},
archivePrefix = {arXiv},
       eprint = {1902.00085},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..128Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Manjavacas2019a,
       author = {{Manjavacas}, Elena and {Apai}, D{\'a}niel and {Zhou}, Yifan and {Lew}, Ben W.~P. and {Schneider}, Glenn and {Metchev}, Stan and {Miles-P{\'a}ez}, Paulo A. and {Radigan}, Jacqueline and {Marley}, Mark S. and {Cowan}, Nicolas and {Karalidi}, Theodora and {Burgasser}, Adam J. and {Bedin}, Luigi R. and {Lowrance}, Patrick J. and {Kauffmann}, Parker},
        title = "{Cloud Atlas: Hubble Space Telescope Near-infrared Spectral Library of Brown Dwarfs, Planetary-mass Companions, and Hot Jupiters}",
      journal = {\aj},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = mar,
       volume = {157},
       number = {3},
          eid = {101},
        pages = {101},
          doi = {10.3847/1538-3881/aaf88f},
archivePrefix = {arXiv},
       eprint = {1812.03963},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..101M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhou2018,
       author = {{Zhou}, Yifan and {Apai}, D{\'a}niel and {Metchev}, Stanimir and {Lew}, Ben W.~P. and {Schneider}, Glenn and {Marley}, Mark S. and {Karalidi}, Theodora and {Manjavacas}, Elena and {Bedin}, Luigi R. and {Cowan}, Nicolas B. and {Miles-P{\'a}ez}, Paulo A. and {Lowrance}, Patrick J. and {Radigan}, Jacqueline and {Burgasser}, Adam J.},
        title = "{Cloud Atlas: Rotational Modulations in the L/T Transition Brown Dwarf Companion HN Peg B}",
      journal = {\aj},
     keywords = {brown dwarfs, methods: observational, stars: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = mar,
       volume = {155},
       number = {3},
          eid = {132},
        pages = {132},
          doi = {10.3847/1538-3881/aaabbd},
archivePrefix = {arXiv},
       eprint = {1801.09757},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....155..132Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Manjavacas2018,
       author = {{Manjavacas}, Elena and {Apai}, D{\'a}niel and {Zhou}, Yifan and {Karalidi}, Theodora and {Lew}, Ben W.~P. and {Schneider}, Glenn and {Cowan}, Nicolas and {Metchev}, Stan and {Miles-P{\'a}ez}, Paulo A. and {Burgasser}, Adam J. and {Radigan}, Jacqueline and {Bedin}, Luigi R. and {Lowrance}, Patrick J. and {Marley}, Mark S.},
        title = "{Cloud Atlas: Discovery of Rotational Spectral Modulations in a Low-mass, L-type Brown Dwarf Companion to a Star}",
      journal = {\aj},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = jan,
       volume = {155},
       number = {1},
          eid = {11},
        pages = {11},
          doi = {10.3847/1538-3881/aa984f},
archivePrefix = {arXiv},
       eprint = {1710.08433},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....155...11M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lew2016,
       author = {{Lew}, Ben W.~P. and {Apai}, Daniel and {Zhou}, Yifan and {Schneider}, Glenn and {Burgasser}, Adam J. and {Karalidi}, Theodora and {Yang}, Hao and {Marley}, Mark S. and {Cowan}, Nicolas B. and {Bedin}, Luigi R. and {Metchev}, Stanimir A. and {Radigan}, Jacqueline and {Lowrance}, Patrick J.},
        title = "{Cloud Atlas: Discovery of Patchy Clouds and High-amplitude Rotational Modulations in a Young, Extremely Red L-type Brown Dwarf}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: atmospheres, stars: individual: WISEP J004701.06+680352.1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {829},
       number = {2},
          eid = {L32},
        pages = {L32},
          doi = {10.3847/2041-8205/829/2/L32},
archivePrefix = {arXiv},
       eprint = {1609.04804},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...829L..32L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zink2020,
       author = {{Zink}, Jon K. and {Hardegree-Ullman}, Kevin K. and {Christiansen}, Jessie L. and {Petigura}, Erik A. and {Dressing}, Courtney D. and {Schlieder}, Joshua E. and {Ciardi}, David R. and {Crossfield}, Ian J.~M.},
        title = "{Scaling K2. III. Comparable Planet Occurrence in the FGK Samples of Campaign 5 and Kepler}",
      journal = {\aj},
     keywords = {Exoplanet catalogs, Dwarf stars, 488, 2053, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {160},
       number = {2},
          eid = {94},
        pages = {94},
          doi = {10.3847/1538-3881/aba123},
archivePrefix = {arXiv},
       eprint = {2006.16261},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160...94Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wang2020,
       author = {{Wang}, Ji and {Wang}, Jason J. and {Ma}, Bo and {Chilcote}, Jeffrey and {Ertel}, Steve and {Guyon}, Olivier and {Ilyin}, Ilya and {Jovanovic}, Nemanja and {Kalas}, Paul and {Lozi}, Julien and {Macintosh}, Bruce and {Strassmeier}, Klaus G. and {Stone}, Jordan},
        title = "{On the Chemical Abundance of HR 8799 and the Planet c}",
      journal = {\aj},
     keywords = {Exoplanet atmospheric composition, Planetary atmospheres, Direct imaging, Stellar atmospheres, Coronagraphic imaging, Exoplanet detection methods, Chemically peculiar stars, Peculiar variable stars, Chemical abundances, Abundance ratios, Stellar abundances, Chemically peculiar giant stars, 2021, 1244, 387, 1584, 313, 489, 226, 1202, 224, 11, 1577, 1201, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = sep,
       volume = {160},
       number = {3},
          eid = {150},
        pages = {150},
          doi = {10.3847/1538-3881/ababa7},
archivePrefix = {arXiv},
       eprint = {2007.02810},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160..150W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Claret2012,
       author = {{Claret}, A. and {Hauschildt}, P.~H. and {Witte}, S.},
        title = "{New limb-darkening coefficients for PHOENIX/1D model atmospheres. I. Calculations for 1500 K {\ensuremath{\leq}} T$_{eff}$ {\ensuremath{\leq}} 4800 K Kepler, CoRot, Spitzer, uvby, UBVRIJHK, Sloan, and 2MASS photometric systems}",
      journal = {\aap},
     keywords = {stars: atmospheres, binaries: eclipsing, brown dwarfs, planetary systems, stars: late-type},
         year = 2012,
        month = oct,
       volume = {546},
          eid = {A14},
        pages = {A14},
          doi = {10.1051/0004-6361/201219849},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...546A..14C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Buenzli15b,
       author = {{Buenzli}, Esther and {Marley}, Mark. S. and {Apai}, D{\'a}niel and {Saumon}, Didier and {Biller}, Beth A. and {Crossfield}, Ian J.~M. and {Radigan}, Jacqueline},
        title = "{Cloud Structure of the Nearest Brown Dwarfs. II. High-amplitude Variability for Luhman 16 A and B in and out of the 0.99 {\ensuremath{\mu}}m FeH feature}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: atmospheres, stars: individual: WISE J104915.57{\textendash}531906.1, Luhman 16AB, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {812},
       number = {2},
          eid = {163},
        pages = {163},
          doi = {10.1088/0004-637X/812/2/163},
archivePrefix = {arXiv},
       eprint = {1509.06148},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...812..163B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Saumon1996,
       author = {{Saumon}, D. and {Hubbard}, W.~B. and {Burrows}, A. and {Guillot}, T. and {Lunine}, J.~I. and {Chabrier}, G.},
        title = "{A Theory of Extrasolar Giant Planets}",
      journal = {\apj},
     keywords = {STARS: PLANETARY SYSTEMS, Astrophysics},
         year = 1996,
        month = apr,
       volume = {460},
        pages = {993},
          doi = {10.1086/177027},
archivePrefix = {arXiv},
       eprint = {astro-ph/9510046},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...460..993S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beichman2010,
       author = {{Beichman}, Charles A. and {Krist}, John and {Trauger}, John T. and {Greene}, Tom and {Oppenheimer}, Ben and {Sivaramakrishnan}, Anand and {Doyon}, Ren{\'e} and {Boccaletti}, Anthony and {Barman}, Travis S. and {Rieke}, Marcia},
        title = "{Imaging Young Giant Planets From Ground and Space}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = feb,
       volume = {122},
       number = {888},
        pages = {162},
          doi = {10.1086/651057},
archivePrefix = {arXiv},
       eprint = {1001.0351},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010PASP..122..162B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


}



@ARTICLE{Bowler2016,
       author = {{Bowler}, Brendan P.},
        title = "{Imaging Extrasolar Giant Planets}",
      journal = {\pasp},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {128},
       number = {968},
        pages = {102001},
          doi = {10.1088/1538-3873/128/968/102001},
archivePrefix = {arXiv},
       eprint = {1605.02731},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PASP..128j2001B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wang2017b,
       author = {{Wang}, Ji and {Mawet}, Dimitri and {Ruane}, Garreth and {Hu}, Renyu and {Benneke}, Bj{\"o}rn},
        title = "{Observing Exoplanets with High Dispersion Coronagraphy. I. The Scientific Potential of Current and Next-generation Large Ground and Space Telescopes}",
      journal = {\aj},
     keywords = {brown dwarfs, instrumentation: spectrographs, planetary systems, techniques: high angular resolution, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = apr,
       volume = {153},
       number = {4},
          eid = {183},
        pages = {183},
          doi = {10.3847/1538-3881/aa6474},
archivePrefix = {arXiv},
       eprint = {1703.00582},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....153..183W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Tan&Showman19,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric Variability Driven by Radiative Cloud Feedback in Brown Dwarfs and Directly Imaged Extrasolar Giant Planets}",
      journal = {\apj},
     keywords = {brown dwarfs, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, radiative transfer, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2019,
        month = apr,
       volume = {874},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.3847/1538-4357/ab0c07},
archivePrefix = {arXiv},
       eprint = {1809.06467},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874..111T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Apai2013,
       author = {{Apai}, D{\'a}niel and {Radigan}, Jacqueline and {Buenzli}, Esther and {Burrows}, Adam and {Reid}, Iain Neill and {Jayawardhana}, Ray},
        title = "{HST Spectral Mapping of L/T Transition Brown Dwarfs Reveals Cloud Thickness Variations}",
      journal = {\apj},
     keywords = {brown dwarfs, planetary systems, planets and satellites: individual: Jupiter, stars: atmospheres, stars: low-mass, starspots, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = may,
       volume = {768},
       number = {2},
          eid = {121},
        pages = {121},
          doi = {10.1088/0004-637X/768/2/121},
archivePrefix = {arXiv},
       eprint = {1303.4151},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...768..121A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{tan22,
       author = {{Tan}, Xianyu},
        title = "{Jet streams and tracer mixing in the atmospheres of brown dwarfs and isolated young giant planets}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, brown dwarfs},
         year = 2022,
        month = feb,
          doi = {10.1093/mnras/stac344},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.tmp..360T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mukherjee21,
       author = {{Mukherjee}, Sagnick and {Fortney}, Jonathan J. and {Jensen-Clem}, Rebecca and {Tan}, Xianyu and {Marley}, Mark S. and {Batalha}, Natasha E.},
        title = "{Modeling Polarization Signals from Cloudy Brown Dwarfs Luhman 16 A and B in Three Dimensions}",
      journal = {\apj},
     keywords = {185, 2180, 112, 1278, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = dec,
       volume = {923},
       number = {1},
          eid = {113},
        pages = {113},
          doi = {10.3847/1538-4357/ac2d92},
archivePrefix = {arXiv},
       eprint = {2110.05739},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923..113M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tan21b,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric circulation of brown dwarfs and directly imaged exoplanets driven by cloud radiative feedback: global and equatorial dynamics}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
       volume = {502},
       number = {2},
        pages = {2198-2219},
          doi = {10.1093/mnras/stab097},
archivePrefix = {arXiv},
       eprint = {2101.04417},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502.2198T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tan21a,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric circulation of brown dwarfs and directly imaged exoplanets driven by cloud radiative feedback: effects of rotation}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2021,
        month = mar,
       volume = {502},
       number = {1},
        pages = {678-699},
          doi = {10.1093/mnras/stab060},
archivePrefix = {arXiv},
       eprint = {2005.12152},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502..678T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{showman20,
       author = {{Showman}, Adam P. and {Tan}, Xianyu and {Parmentier}, Vivien},
        title = "{Atmospheric Dynamics of Hot Giant Planets and Brown Dwarfs}",
      journal = {\ssr},
     keywords = {Exoplanets, Giant planets, Hot Jupiters, Jupiter, Saturn, Brown dwarfs, Atmospheric dynamics, Turbulence, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {216},
       number = {8},
          eid = {139},
        pages = {139},
          doi = {10.1007/s11214-020-00758-8},
archivePrefix = {arXiv},
       eprint = {2007.15363},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SSRv..216..139S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{showman19,
       author = {{Showman}, Adam P. and {Tan}, Xianyu and {Zhang}, Xi},
        title = "{Atmospheric Circulation of Brown Dwarfs and Jupiter- and Saturn-like Planets: Zonal Jets, Long-term Variability, and QBO-type Oscillations}",
      journal = {\apj},
     keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: individual: Jupiter, Saturn, turbulence, waves, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = sep,
       volume = {883},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.3847/1538-4357/ab384a},
archivePrefix = {arXiv},
       eprint = {1807.08433},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...883....4S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{showman&kaspi13,
       author = {{Showman}, Adam P. and {Kaspi}, Yohai},
        title = "{Atmospheric Dynamics of Brown Dwarfs and Directly Imaged Giant Planets}",
      journal = {\apj},
     keywords = {brown dwarfs, convection, methods: numerical, stars: low-mass, turbulence, waves, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {776},
       number = {2},
          eid = {85},
        pages = {85},
          doi = {10.1088/0004-637X/776/2/85},
archivePrefix = {arXiv},
       eprint = {1210.7573},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...776...85S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{triaud17,
       author = {{Triaud}, Amaury H.~M.~J.},
        title = "{The Rossiter-McLaughlin Effect in Exoplanet Research}",
     keywords = {Physics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Handbook of Exoplanets},
         year = 2018,
       editor = {{Deeg}, Hans J. and {Belmonte}, Juan Antonio},
          eid = {2},
        pages = {2},
          doi = {10.1007/978-3-319-55333-7\_2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018haex.bookE...2T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{watson19,
       author = {{Watson}, C.~A. and {de Mooij}, E.~J.~W. and {Steeghs}, D. and {Marsh}, T.~R. and {Brogi}, M. and {Gibson}, N.~P. and {Matthews}, S.},
        title = "{Doppler tomography as a tool for detecting exoplanet atmospheres}",
      journal = {\mnras},
     keywords = {line: profiles, techniques: spectroscopic, planets and satellites: atmospheres, planets and satellites: individual: {\ensuremath{\tau}} Boo-b, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {490},
       number = {2},
        pages = {1991-2006},
          doi = {10.1093/mnras/stz2679},
archivePrefix = {arXiv},
       eprint = {1909.09219},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.490.1991W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{karalidi15,
       author = {{Karalidi}, Theodora and {Apai}, D{\'a}niel and {Schneider}, Glenn and {Hanson}, Jake R. and {Pasachoff}, Jay M.},
        title = "{Aeolus: A Markov Chain Monte Carlo Code for Mapping Ultracool Atmospheres. An Application on Jupiter and Brown Dwarf HST Light Curves}",
      journal = {\apj},
     keywords = {methods: statistical, planets and satellites: individual: Jupiter, stars: individual: 2MASS J21392676+0220226, 2MASS J0136565+093347, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = nov,
       volume = {814},
       number = {1},
          eid = {65},
        pages = {65},
          doi = {10.1088/0004-637X/814/1/65},
archivePrefix = {arXiv},
       eprint = {1510.04251},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...814...65K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{donati97,
       author = {{Donati}, J. -F. and {Brown}, S.~F.},
        title = "{Zeeman-Doppler imaging of active stars. V. Sensitivity of maximum entropy magnetic maps to field orientation.}",
      journal = {\aap},
     keywords = {STARS: MAGNETIC FIELDS, STARS: IMAGING, STARS: ACTIVITY, LINE: PROFILES, POLARIZATION, METHODS: OBSERVATIONAL},
         year = 1997,
        month = oct,
       volume = {326},
        pages = {1135-1142},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997A&A...326.1135D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{vogt87,
       author = {{Vogt}, Steven S. and {Penrod}, G. Donald and {Hatzes}, Artie P.},
        title = "{Doppler Images of Rotating Stars Using Maximum Entropy Image Reconstruction}",
      journal = {\apj},
     keywords = {Doppler Effect, Image Reconstruction, Maximum Entropy Method, Peculiar Stars, Stellar Rotation, Stellar Spectra, Computational Grids, Iterative Solution, Line Spectra, Signal To Noise Ratios, Spatial Resolution, Spectral Resolution, Starspots, Astronomy, LINE PROFILES, STARS: PECULIAR A, STARS: ROTATION},
         year = 1987,
        month = oct,
       volume = {321},
        pages = {496},
          doi = {10.1086/165647},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987ApJ...321..496V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Radigan2012,
       author = {{Radigan}, Jacqueline and {Jayawardhana}, Ray and {Lafreni{\`e}re}, David and {Artigau}, {\'E}tienne and {Marley}, Mark and {Saumon}, Didier},
        title = "{Large-amplitude Variations of an L/T Transition Brown Dwarf: Multi-wavelength Observations of Patchy, High-contrast Cloud Features}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: 2MASS J21392676+0220226, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = may,
       volume = {750},
       number = {2},
          eid = {105},
        pages = {105},
          doi = {10.1088/0004-637X/750/2/105},
archivePrefix = {arXiv},
       eprint = {1201.3403},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...750..105R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek2017,
       author = {{Komacek}, Thaddeus D. and {Youdin}, Andrew N.},
        title = "{Structure and Evolution of Internally Heated Hot Jupiters}",
      journal = {\apj},
     keywords = {methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, planets and satellites: individual: HD 209458b, planets and satellites: interiors, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = aug,
       volume = {844},
       number = {2},
          eid = {94},
        pages = {94},
          doi = {10.3847/1538-4357/aa7b75},
archivePrefix = {arXiv},
       eprint = {1706.07605},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...844...94K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tan&Komacek2019,
       author = {{Tan}, Xianyu and {Komacek}, Thaddeus D.},
        title = "{The Atmospheric Circulation of Ultra-hot Jupiters}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Hot Jupiters, Hydrodynamics, 753, 487, 1963, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = nov,
       volume = {886},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/ab4a76},
archivePrefix = {arXiv},
       eprint = {1910.01622},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886...26T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tan&Showman2020,
       author = {{Tan}, Xianyu and {Showman}, Adam P.},
        title = "{Atmospheric Circulation of Tidally Locked Gas Giants with Increasing Rotation and Implications for White Dwarf-Brown Dwarf Systems}",
      journal = {\apj},
     keywords = {Brown dwarfs, Exoplanet atmospheres, White dwarf stars, Hydrodynamics, Hot Jupiters, 185, 487, 1799, 1963, 753, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = oct,
       volume = {902},
       number = {1},
          eid = {27},
        pages = {27},
          doi = {10.3847/1538-4357/abb3d4},
archivePrefix = {arXiv},
       eprint = {2001.06269},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...902...27T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lee2020,
       author = {{Lee}, Elspeth K.~H. and {Casewell}, Sarah L. and {Chubb}, Katy L. and {Hammond}, Mark and {Tan}, Xianyu and {Tsai}, Shang-Min and {Pierrehumbert}, Raymond T.},
        title = "{Simplified 3D GCM modelling of the irradiated brown dwarf WD 0137-349B}",
      journal = {\mnras},
     keywords = {binaries: close, Brown dwarfs, stars: individual: WD 0137‑349B, Radiative transfer, planets and satellites: atmospheres, stars: atmospheres, radiative transfer, brown dwarfs, stars: individual: WD 0137-349B, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {496},
       number = {4},
        pages = {4674-4687},
          doi = {10.1093/mnras/staa1882},
archivePrefix = {arXiv},
       eprint = {2001.06558},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.4674L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Oppenheimer1998,
       author = {{Oppenheimer}, B.~R. and {Kulkarni}, S.~R. and {Matthews}, K. and {van Kerkwijk}, M.~H.},
        title = "{The Spectrum of the Brown Dwarf Gliese 229B}",
      journal = {\apj},
     keywords = {STARS: CIRCUMSTELLAR MATTER, LINE: IDENTIFICATION, STARS: INDIVIDUAL NAME: GLIESE 229B, STARS: LOW-MASS, BROWN DWARFS, Stars: Circumstellar Matter, Line: Identification, Stars: Individual: Name: Gliese 229B, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 1998,
        month = aug,
       volume = {502},
       number = {2},
        pages = {932-943},
          doi = {10.1086/305928},
archivePrefix = {arXiv},
       eprint = {astro-ph/9802299},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...502..932O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Hellier2001,
       author = {{Hellier}, Coel},
        title = "{Cataclysmic Variable Stars}",
         year = 2001,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001cvs..book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@article{perryman18,
       author = {{Perryman}, Michael},
        title = "{The Exoplanet Handbook}",
         year = 2018,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018exha.book.....P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{tarter07,
       author = {{Tarter}, Jill C. and {Backus}, Peter R. and {Mancinelli}, Rocco L. and {Aurnou}, Jonathan M. and {Backman}, Dana E. and {Basri}, Gibor S. and {Boss}, Alan P. and {Clarke}, Andrew and {Deming}, Drake and {Doyle}, Laurance R. and {Feigelson}, Eric D. and {Freund}, Friedmann and {Grinspoon}, David H. and {Haberle}, Robert M. and {Hauck}, Steven A., II and {Heath}, Martin J. and {Henry}, Todd J. and {Hollingsworth}, Jeffery L. and {Joshi}, Manoj M. and {Kilston}, Steven and {Liu}, Michael C. and {Meikle}, Erik and {Reid}, I. Neill and {Rothschild}, Lynn J. and {Scalo}, John and {Segura}, Antigona and {Tang}, Carol M. and {Tiedje}, James M. and {Turnbull}, Margaret C. and {Walkowicz}, Lucianne M. and {Weber}, Arthur L. and {Young}, Richard E.},
        title = "{A Reappraisal of The Habitability of Planets around M Dwarf Stars}",
      journal = {Astrobiology},
     keywords = {Astrophysics},
         year = 2007,
        month = mar,
       volume = {7},
       number = {1},
        pages = {30-65},
          doi = {10.1089/ast.2006.0124},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609799},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AsBio...7...30T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







@article{schuessler&solanki92,
       author = {{Schuessler}, M. and {Solanki}, S.~K.},
        title = "{Why rapid rotators have polar spots.}",
      journal = {\aap},
     keywords = {Cool Stars, Magnetic Stars, Starspots, Stellar Rotation, Computational Astrophysics, Coriolis Effect, Stellar Models, Astrophysics},
         year = 1992,
        month = oct,
       volume = {264},
        pages = {L13-L16},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...264L..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{granzer00,
       author = {{Schuessler}, M. and {Solanki}, S.~K.},
        title = "{Why rapid rotators have polar spots.}",
      journal = {\aap},
     keywords = {Cool Stars, Magnetic Stars, Starspots, Stellar Rotation, Computational Astrophysics, Coriolis Effect, Stellar Models, Astrophysics},
         year = 1992,
        month = oct,
       volume = {264},
        pages = {L13-L16},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...264L..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{yadav15,
       author = {{Yadav}, Rakesh K. and {Gastine}, Thomas and {Christensen}, Ulrich R. and {Reiners}, Ansgar},
        title = "{Formation of starspots in self-consistent global dynamo models: Polar spots on cool stars}",
      journal = {\aap},
     keywords = {starspots, stars: magnetic field, stars: rotation, stars: interiors, dynamo, convection, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jan,
       volume = {573},
          eid = {A68},
        pages = {A68},
          doi = {10.1051/0004-6361/201424589},
archivePrefix = {arXiv},
       eprint = {1407.3187},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..68Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier1998,
       author = {{Strassmeier}, K.~G. and {Bartus}, J. and {Kovari}, Zs. and {Weber}, M. and {Washuettl}, A.},
        title = "{Doppler imaging of stellar surface structure. VIII. The effectively single and rapidly-rotating G8-giant HD 51066 = CM Camelopardalis}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: IMAGING, STARS: INDIVIDUAL: HD 51066, STARS: LATE-TYPE, STARSPOTS},
         year = 1998,
        month = aug,
       volume = {336},
        pages = {587-603},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...336..587S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{strassmeier&rice98,
       author = {{Strassmeier}, K.~G. and {Rice}, J.~B.},
        title = "{Doppler imaging of stellar surface structure. IX. A high-resolution image of the weak-lined T Tauri star HDE 283572 = V987 Tauri}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARSPOTS, STARS: IMAGING, STARS: INDIVIDUAL: HDE 283572, STARS: LATE-TYPE},
         year = 1998,
        month = nov,
       volume = {339},
        pages = {497-506},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...339..497S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{jarvinen08,
       author = {{J{\"a}rvinen}, S.~P. and {Korhonen}, H. and {Berdyugina}, S.~V. and {Ilyin}, I. and {Strassmeier}, K.~G. and {Weber}, M. and {Savanov}, I. and {Tuominen}, I.},
        title = "{Magnetic activity on V889 Herculis. Combining photometry and spectroscopy}",
      journal = {\aap},
     keywords = {stars: imaging, stars: activity, stars: starspots, stars: individual: V889 Her},
         year = 2008,
        month = sep,
       volume = {488},
       number = {3},
        pages = {1047-1055},
          doi = {10.1051/0004-6361:200809837},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...488.1047J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{berdyugina98,
       author = {{Berdyugina}, Svetlana V.},
        title = "{Surface imaging by the Occamian approach. Basic principles, simulations, and tests}",
      journal = {\aap},
     keywords = {STARS: IMAGING, STARS: ACTIVITY, METHODS: DATA ANALYSIS},
         year = 1998,
        month = oct,
       volume = {338},
        pages = {97-105},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...338...97B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{barnes17,
       author = {{Barnes}, J.~R. and {Jeffers}, S.~V. and {Haswell}, C.~A. and {Jones}, H.~R.~A. and {Shulyak}, D. and {Pavlenko}, Ya. V. and {Jenkins}, J.~S.},
        title = "{Surprisingly different star-spot distributions on the near equal-mass equal-rotation-rate stars in the M dwarf binary GJ 65 AB}",
      journal = {\mnras},
     keywords = {techniques: imaging spectroscopy, techniques: spectroscopic, stars: atmospheres, stars: imaging, stars: low-mass, starspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = oct,
       volume = {471},
       number = {1},
        pages = {811-823},
          doi = {10.1093/mnras/stx1482},
archivePrefix = {arXiv},
       eprint = {1706.03979},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471..811B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{rimmer18,
    author = "Paul B. Rimmer and Jianfeng Xu and Samantha J. Thompson and Ed Gillen and John D. Sutherland and Didier Queloz",
    title = "The origin of RNA precursors on exoplanets",
    journal = "Science Advances",
    volume = "4",
    issue = "8",
    pages = "eear3302",
    month = "August",
    year = "2018"
}


@article{zeldes21,
       author = {{Zeldes}, Jesse and {Hinkle}, Jason T. and {Shappee}, Benjamin J. and {Avallone}, Ellis A. and {Schmidt}, Sarah J. and {van Saders}, Jennifer L. and {Way}, Zachary and {Kochanek}, Christopher S. and {Holoien}, Thomas W. -S.},
        title = "{Flares Big and Small: a K2 and TESS View of ASAS-SN Superflares}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.04501},
        pages = {arXiv:2109.04501},
archivePrefix = {arXiv},
       eprint = {2109.04501},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210904501Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{ramsay21,
       author = {{Ramsay}, Gavin and {Kolotkov}, Dmitrii and {Doyle}, J. Gerry and {Doyle}, Lauren},
        title = "{Transiting Exoplanet Survey Satellite (TESS) Observations of Flares and Quasi-Periodic Pulsations from Low-Mass Stars and Potential Impact on Exoplanets}",
      journal = {\solphys},
     keywords = {Stars: activity, Stars: flare, Stars: low-mass, Stars: pulsations, Stars: magnetic fields, Planets and satellites: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = nov,
       volume = {296},
       number = {11},
          eid = {162},
        pages = {162},
          doi = {10.1007/s11207-021-01899-x},
archivePrefix = {arXiv},
       eprint = {2108.10670},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021SoPh..296..162R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{asnodkar22,
       author = {{Pai Asnodkar}, Anusha and {Wang}, Ji and {Gaudi}, B. Scott and {Cauley}, P. Wilson and {Eastman}, Jason D. and {Ilyin}, Ilya and {Strassmeier}, Klaus and {Beatty}, Thomas},
        title = "{KELT-9 as an Eclipsing Double-lined Spectroscopic Binary: A Unique and Self-consistent Solution to the System}",
      journal = {\aj},
     keywords = {486, 487, 498, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = feb,
       volume = {163},
       number = {2},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-3881/ac32c7},
archivePrefix = {arXiv},
       eprint = {2110.15275},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....163...40P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{gray22,
       author = {{Gray}, David F.},
        title = "{The Observation and Analysis of Stellar Photospheres}",
         year = 2008,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008oasp.book.....G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{luger19,
       author = {{Luger}, Rodrigo and {Agol}, Eric and {Foreman-Mackey}, Daniel and {Fleming}, David P. and {Lustig-Yaeger}, Jacob and {Deitrick}, Russell},
        title = "{starry: Analytic Occultation Light Curves}",
      journal = {\aj},
     keywords = {eclipses, methods: analytical, occultations, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {157},
       number = {2},
          eid = {64},
        pages = {64},
          doi = {10.3847/1538-3881/aae8e5},
archivePrefix = {arXiv},
       eprint = {1810.06559},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157...64L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{luger21c,
       author = {{Luger}, Rodrigo and {Foreman-Mackey}, Daniel and {Hedges}, Christina},
        title = "{Mapping Stellar Surfaces. II. An Interpretable Gaussian Process Model for Light Curves}",
      journal = {\aj},
     keywords = {Analytical mathematics, Time series analysis, Gaussian Processes regression, Starspots, 38, 1916, 1930, 1572, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = sep,
       volume = {162},
       number = {3},
          eid = {124},
        pages = {124},
          doi = {10.3847/1538-3881/abfdb9},
archivePrefix = {arXiv},
       eprint = {2102.01697},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....162..124L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{luger21d,
       author = {{Luger}, Rodrigo and {Foreman-Mackey}, Daniel and {Hedges}, Christina and {Hogg}, David W.},
        title = "{Mapping Stellar Surfaces. I. Degeneracies in the Rotational Light-curve Problem}",
      journal = {\aj},
     keywords = {Time series analysis, Light curves, Stellar surfaces, Starspots, 1916, 918, 1632, 1572, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = sep,
       volume = {162},
       number = {3},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-3881/abfdb8},
archivePrefix = {arXiv},
       eprint = {2102.00007},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....162..123L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{luger21b,
       author = {{Luger}, Rodrigo and {Foreman-Mackey}, Daniel and {Hedges}, Christina},
        title = "{starry\_process: Interpretable Gaussian processes for stellar light curves}",
      journal = {The Journal of Open Source Software},
     keywords = {Python, C, astronomy, C++, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = jul,
       volume = {6},
       number = {63},
          eid = {3071},
        pages = {3071},
          doi = {10.21105/joss.03071},
archivePrefix = {arXiv},
       eprint = {2102.01774},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021JOSS....6.3071L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{luhman13,
       author = {{Luhman}, K.~L.},
        title = "{Discovery of a Binary Brown Dwarf at 2 pc from the Sun}",
      journal = {\apjl},
     keywords = {brown dwarfs, infrared: stars, proper motions, solar neighborhood, stars: low-mass, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.1088/2041-8205/767/1/L1},
archivePrefix = {arXiv},
       eprint = {1303.2401},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767L...1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{kniazev13,
       author = {{Kniazev}, A.~Y. and {Vaisanen}, P. and {Mu{\v{z}}i{\'c}}, K. and {Mehner}, A. and {Boffin}, H.~M.~J. and {Kurtev}, R. and {Melo}, C. and {Ivanov}, V.~D. and {Girard}, J. and {Mawet}, D. and {Schmidtobreick}, L. and {Huelamo}, N. and {Borissova}, J. and {Minniti}, D. and {Ishibashi}, K. and {Potter}, S.~B. and {Beletsky}, Y. and {Buckley}, D.~A.~H. and {Crawford}, S. and {Gulbis}, A.~A.~S. and {Kotze}, P. and {Miszalski}, B. and {Pickering}, T.~E. and {Romero Colmenero}, E. and {Williams}, T.~B.},
        title = "{Characterization of the nearby L/T Binary Brown Dwarf WISE J104915.57-531906.1 at 2 pc from the Sun}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, solar neighborhood, stars: individual: G 171{\textendash}22 HD 55383 WISE J104915.57{\textendash}531906.1, stars: low-mass, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = jun,
       volume = {770},
       number = {2},
          eid = {124},
        pages = {124},
          doi = {10.1088/0004-637X/770/2/124},
archivePrefix = {arXiv},
       eprint = {1303.7171},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...770..124K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{burgasser13,
       author = {{Burgasser}, Adam J. and {Sheppard}, Scott S. and {Luhman}, K.~L.},
        title = "{Resolved Near-infrared Spectroscopy of WISE J104915.57-531906.1AB: A Flux-reversal Binary at the L dwarf/T Dwarf Transition}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57{\textendash}531906.1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = aug,
       volume = {772},
       number = {2},
          eid = {129},
        pages = {129},
          doi = {10.1088/0004-637X/772/2/129},
archivePrefix = {arXiv},
       eprint = {1303.7283},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...772..129B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garcia17,
       author = {{Garcia}, E. Victor and {Ammons}, S. Mark and {Salama}, Maissa and {Crossfield}, Ian and {Bendek}, Eduardo and {Chilcote}, Jeffrey and {Garrel}, Vincent and {Graham}, James R. and {Kalas}, Paul and {Konopacky}, Quinn and {Lu}, Jessica R. and {Macintosh}, Bruce and {Marin}, Eduardo and {Marois}, Christian and {Nielsen}, Eric and {Neichel}, Beno{\^\i}t and {Pham}, Don and {De Rosa}, Robert J. and {Ryan}, Dominic M. and {Service}, Maxwell and {Sivo}, Gaetano},
        title = "{Individual, Model-independent Masses of the Closest Known Brown Dwarf Binary to the Sun}",
      journal = {\apj},
     keywords = {astrometry, binaries: visual, brown dwarfs, stars: fundamental parameters, stars: individual: WISE J104915.57{\textendash}531906.1, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = sep,
       volume = {846},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/aa844f},
archivePrefix = {arXiv},
       eprint = {1708.02714},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...846...97G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{morley12,
       author = {{Morley}, Caroline V. and {Fortney}, Jonathan J. and {Marley}, Mark S. and {Visscher}, Channon and {Saumon}, Didier and {Leggett}, S.~K.},
        title = "{Neglected Clouds in T and Y Dwarf Atmospheres}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = sep,
       volume = {756},
       number = {2},
          eid = {172},
        pages = {172},
          doi = {10.1088/0004-637X/756/2/172},
archivePrefix = {arXiv},
       eprint = {1206.4313},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...756..172M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{faherty14,
       author = {{Faherty}, Jacqueline K. and {Beletsky}, Yuri and {Burgasser}, Adam J. and {Tinney}, Chris and {Osip}, David J. and {Filippazzo}, Joseph C. and {Simcoe}, Robert A.},
        title = "{Signatures of Cloud, Temperature, and Gravity from Spectra of the Closest Brown Dwarfs}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57-531906.1, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = aug,
       volume = {790},
       number = {2},
          eid = {90},
        pages = {90},
          doi = {10.1088/0004-637X/790/2/90},
archivePrefix = {arXiv},
       eprint = {1406.1518},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...790...90F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lazorenko18,
       author = {{Lazorenko}, P.~F. and {Sahlmann}, J.},
        title = "{Updated astrometry and masses of the LUH 16 brown dwarf binary}",
      journal = {\aap},
     keywords = {astrometry, brown dwarfs, binaries: visual, parallaxes, stars: individual: WISE J104915.57-531906.1, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A111},
        pages = {A111},
          doi = {10.1051/0004-6361/201833626},
archivePrefix = {arXiv},
       eprint = {1808.07835},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A.111L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sahlmann15,
       author = {{Sahlmann}, J. and {Lazorenko}, P.~F.},
        title = "{Mass ratio of the 2 pc binary brown dwarf LUH 16 and limits on planetary companions from astrometry}",
      journal = {\mnras},
     keywords = {astrometry, parallaxes, binaries: visual, brown dwarfs, stars: individual: WISE J104915.57-531906.1, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {453},
       number = {1},
        pages = {L103-L107},
          doi = {10.1093/mnrasl/slv113},
archivePrefix = {arXiv},
       eprint = {1506.07994},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453L.103S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lodieu15,
       author = {{Lodieu}, N. and {Zapatero Osorio}, M.~R. and {Rebolo}, R. and {B{\'e}jar}, V.~J.~S. and {Pavlenko}, Y. and {P{\'e}rez-Garrido}, A.},
        title = "{VLT X-Shooter spectroscopy of the nearest brown dwarf binary}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, brown dwarfs, binaries: general, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {581},
          eid = {A73},
        pages = {A73},
          doi = {10.1051/0004-6361/201424933},
archivePrefix = {arXiv},
       eprint = {1506.08848},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...581A..73L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gillon13,
       author = {{Gillon}, M. and {Triaud}, A.~H.~M.~J. and {Jehin}, E. and {Delrez}, L. and {Opitom}, C. and {Magain}, P. and {Lendl}, M. and {Queloz}, D.},
        title = "{Fast-evolving weather for the coolest of our two new substellar neighbours}",
      journal = {\aap},
     keywords = {brown dwarfs, stars: individual: WISE-J104915.57-531906.1, solar neighborhood, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = jul,
       volume = {555},
          eid = {L5},
        pages = {L5},
          doi = {10.1051/0004-6361/201321620},
archivePrefix = {arXiv},
       eprint = {1304.0481},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...555L...5G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heinze21,
       author = {{Heinze}, A.~N. and {Metchev}, Stanimir and {Kurtev}, Radostin and {Gillon}, Michael},
        title = "{Weather on Other Worlds. VI. Optical Spectrophotometry of Luhman 16B Reveals Large-amplitude Variations in the Alkali Lines}",
      journal = {\apj},
     keywords = {Brown dwarfs, Atmospheric clouds, Exoplanet atmospheric variability, Variable stars, Spectrophotometry, Time series analysis, 185, 2180, 2020, 1761, 1556, 1916, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.3847/1538-4357/ac178b},
archivePrefix = {arXiv},
       eprint = {2107.10995},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920..108H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ackerman&marley01,
       author = {{Ackerman}, Andrew S. and {Marley}, Mark S.},
        title = "{Precipitating Condensation Clouds in Substellar Atmospheres}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2001,
        month = aug,
       volume = {556},
       number = {2},
        pages = {872-884},
          doi = {10.1086/321540},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103423},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...556..872A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ammons&garcia19,
       author = {{Ammons}, Stephen M. and {Garcia}, Victor},
        title = "{Independent Masses for the Luhman 16AB Binary Brown Dwarf System from Gemini GEMS}",
    booktitle = {American Astronomical Society Meeting Abstracts \#233},
         year = 2019,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {233},
        month = jan,
          eid = {114.07},
        pages = {114.07},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AAS...23311407A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bedin17,
       author = {{Bedin}, L.~R. and {Pourbaix}, D. and {Apai}, D. and {Burgasser}, A.~J. and {Buenzli}, E. and {Boffin}, H.~M.~J. and {Libralato}, M.},
        title = "{Hubble Space Telescope astrometry of the closest brown dwarf binary system - I. Overview and improved orbit$^{★}$}",
      journal = {\mnras},
     keywords = {astrometry, binaries: visual, brown dwarfs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = sep,
       volume = {470},
       number = {1},
        pages = {1140-1155},
          doi = {10.1093/mnras/stx1177},
archivePrefix = {arXiv},
       eprint = {1706.00657},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1140B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{biller13,
       author = {{Biller}, Beth A. and {Crossfield}, Ian J.~M. and {Mancini}, Luigi and {Ciceri}, Simona and {Southworth}, John and {Kopytova}, Taisiya G. and {Bonnefoy}, Micka{\"e}l and {Deacon}, Niall R. and {Schlieder}, Joshua E. and {Buenzli}, Esther and {Brandner}, Wolfgang and {Allard}, France and {Homeier}, Derek and {Freytag}, Bernd and {Bailer-Jones}, Coryn A.~L. and {Greiner}, Jochen and {Henning}, Thomas and {Goldman}, Bertrand},
        title = "{Weather on the Nearest Brown Dwarfs: Resolved Simultaneous Multi-wavelength Variability Monitoring of WISE J104915.57-531906.1AB}",
      journal = {\apjl},
     keywords = {brown dwarfs, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = nov,
       volume = {778},
       number = {1},
          eid = {L10},
        pages = {L10},
          doi = {10.1088/2041-8205/778/1/L10},
archivePrefix = {arXiv},
       eprint = {1310.5144},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...778L..10B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{burgasser14,
       author = {{Burgasser}, Adam J. and {Gillon}, Micha{\"e}l and {Faherty}, Jacqueline K. and {Radigan}, Jacqueline and {Triaud}, Amaury H.~M.~J. and {Plavchan}, Peter and {Street}, Rachel and {Jehin}, E. and {Delrez}, L. and {Opitom}, C.},
        title = "{A Monitoring Campaign for Luhman 16AB. I. Detection of Resolved Near-infrared Spectroscopic Variability}",
      journal = {\apj},
     keywords = {binaries: visual, brown dwarfs, stars: individual: WISE J104915.57-531906.1AB Luhman 16AB, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = apr,
       volume = {785},
       number = {1},
          eid = {48},
        pages = {48},
          doi = {10.1088/0004-637X/785/1/48},
archivePrefix = {arXiv},
       eprint = {1402.2342},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...785...48B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hoeijmakers2019,
       author = {{Hoeijmakers}, H.~J. and {Ehrenreich}, D. and {Kitzmann}, D. and
         {Allart}, R. and {Grimm}, S.~L. and {Seidel}, J.~V. and
         {Wyttenbach}, A. and {Pino}, L. and {Nielsen}, L.~D. and {Fisher}, C. and
         {Rimmer}, P.~B. and {Bourrier}, V. and {Cegla}, H.~M. and {Lavie}, B. and
         {Lovis}, C. and {Patzer}, A.~B.~C. and {Stock}, J.~W. and
         {Pepe}, F.~A. and {Heng}, Kevin},
        title = "{A spectral survey of an ultra-hot Jupiter. Detection of metals in the transmission spectrum of KELT-9 b}",
      journal = {\aap},
     keywords = {planets and satellites: gaseous planets, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A165},
        pages = {A165},
          doi = {10.1051/0004-6361/201935089},
archivePrefix = {arXiv},
       eprint = {1905.02096},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A.165H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaudi2017,
       author = {{Gaudi}, B. Scott and {Stassun}, Keivan G. and {Collins}, Karen A. and
         {Beatty}, Thomas G. and {Zhou}, George and {Latham}, David W. and
         {Bieryla}, Allyson and {Eastman}, Jason D. and {Siverd}, Robert J. and
         {Crepp}, Justin R. and {Gonzales}, Erica J. and {Stevens}, Daniel J. and
         {Buchhave}, Lars A. and {Pepper}, Joshua and {Johnson}, Marshall C. and
         {Colon}, Knicole D. and {Jensen}, Eric L.~N. and
         {Rodriguez}, Joseph E. and {Bozza}, Valerio and
         {Novati}, Sebastiano Calchi and {D'Ago}, Giuseppe and
         {Dumont}, Mary T. and {Ellis}, Tyler and {Gaillard}, Clement and
         {Jang-Condell}, Hannah and {Kasper}, David H. and {Fukui}, Akihiko and
         {Gregorio}, Joao and {Ito}, Ayaka and {Kielkopf}, John F. and
         {Manner}, Mark and {Matt}, Kyle and {Narita}, Norio and
         {Oberst}, Thomas E. and {Reed}, Phillip A. and {Scarpetta}, Gaetano and
         {Stephens}, Denice C. and {Yeigh}, Rex R. and {Zambelli}, Roberto and
         {Fulton}, B.~J. and {Howard}, Andrew W. and {James}, David J. and
         {Penny}, Matthew and {Bayliss}, Daniel and {Curtis}, Ivan A. and
         {Depoy}, D.~L. and {Esquerdo}, Gilbert A. and {Gould}, Andrew and
         {Joner}, Michael D. and {Kuhn}, Rudolf B. and
         {Labadie-Bartz}, Jonathan and {Lund}, Michael B. and
         {Marshall}, Jennifer L. and {McLeod}, Kim K. and {Pogge}, Richard W. and
         {Relles}, Howard and {Stockdale}, Christopher and {Tan}, T.~G. and
         {Trueblood}, Mark and {Trueblood}, Patricia},
        title = "{A giant planet undergoing extreme-ultraviolet irradiation by its hot massive-star host}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jun,
       volume = {546},
       number = {7659},
        pages = {514-518},
          doi = {10.1038/nature22392},
archivePrefix = {arXiv},
       eprint = {1706.06723},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Natur.546..514G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lund2017,
       author = {{Lund}, Michael B. and {Rodriguez}, Joseph E. and {Zhou}, George and {Gaudi}, B. Scott and {Stassun}, Keivan G. and {Johnson}, Marshall C. and {Bieryla}, Allyson and {Oelkers}, Ryan J. and {Stevens}, Daniel J. and {Collins}, Karen A. and {Penev}, Kaloyan and {Quinn}, Samuel N. and {Latham}, David W. and {Villanueva}, Steven, Jr. and {Eastman}, Jason D. and {Kielkopf}, John F. and {Oberst}, Thomas E. and {Jensen}, Eric L.~N. and {Cohen}, David H. and {Joner}, Michael D. and {Stephens}, Denise C. and {Relles}, Howard and {Corfini}, Giorgio and {Gregorio}, Joao and {Zambelli}, Roberto and {Esquerdo}, Gilbert A. and {Calkins}, Michael L. and {Berlind}, Perry and {Ciardi}, David R. and {Dressing}, Courtney and {Patel}, Rahul and {Gagnon}, Patrick and {Gonzales}, Erica and {Beatty}, Thomas G. and {Siverd}, Robert J. and {Labadie-Bartz}, Jonathan and {Kuhn}, Rudolf B. and {Col{\'o}n}, Knicole D. and {James}, David and {Pepper}, Joshua and {Fulton}, Benjamin J. and {McLeod}, Kim K. and {Stockdale}, Christopher and {Calchi Novati}, Sebastiano and {DePoy}, D.~L. and {Gould}, Andrew and {Marshall}, Jennifer L. and {Trueblood}, Mark and {Trueblood}, Patricia and {Johnson}, John A. and {Wright}, Jason and {McCrady}, Nate and {Wittenmyer}, Robert A. and {Johnson}, Samson A. and {Sergi}, Anthony and {Wilson}, Maurice and {Sliski}, David H.},
        title = "{KELT-20b: A Giant Planet with a Period of P {\ensuremath{\sim}} 3.5 days Transiting the V {\ensuremath{\sim}} 7.6 Early A Star HD 185603}",
      journal = {\aj},
     keywords = {methods: observational, planets and satellites: detection, planets and satellites: gaseous planets, stars: individual (HD 185603), techniques: photometric, techniques: radial velocities, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = nov,
       volume = {154},
       number = {5},
          eid = {194},
        pages = {194},
          doi = {10.3847/1538-3881/aa8f95},
archivePrefix = {arXiv},
       eprint = {1707.01518},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..194L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Talens2018,
       author = {{Talens}, G.~J.~J. and {Justesen}, A.~B. and {Albrecht}, S. and {McCormac}, J. and {Van Eylen}, V. and {Otten}, G.~P.~P.~L. and {Murgas}, F. and {Palle}, E. and {Pollacco}, D. and {Stuik}, R. and {Spronck}, J.~F.~P. and {Lesage}, A. -L. and {Grundahl}, F. and {Fredslund Andersen}, M. and {Antoci}, V. and {Snellen}, I.~A.~G.},
        title = "{MASCARA-2 b. A hot Jupiter transiting the m$_{V}$ = 7.6 A-star HD 185603}",
      journal = {\aap},
     keywords = {planetary systems, stars: individual: MASCARA-2 (HD 185603, HIP 96618), Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = apr,
       volume = {612},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201731512},
archivePrefix = {arXiv},
       eprint = {1707.01500},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...612A..57T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@book{gray_2005, place={Cambridge}, edition={3}, title={The Observation and Analysis of Stellar Photospheres}, DOI={10.1017/CBO9781316036570}, publisher={Cambridge University Press}, author={Gray, David F.}, year={2005}}

@ARTICLE{Cauley2019,
       author = {{Cauley}, P. Wilson and {Shkolnik}, Evgenya L. and {Ilyin}, Ilya and
         {Strassmeier}, Klaus G. and {Redfield}, Seth and {Jensen}, Adam},
        title = "{Atmospheric Dynamics and the Variable Transit of KELT-9 b}",
      journal = {\aj},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, stars: flare, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {157},
       number = {2},
          eid = {69},
        pages = {69},
          doi = {10.3847/1538-3881/aaf725},
archivePrefix = {arXiv},
       eprint = {1810.05776},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157...69C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{Madhusudhan2018,
       author = {{Madhusudhan}, Nikku},
        title = "{Atmospheric Retrieval of Exoplanets}",
     keywords = {Physics, Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {Handbook of Exoplanets},
         year = 2018,
       editor = {{Deeg}, Hans J. and {Belmonte}, Juan Antonio},
          eid = {104},
        pages = {104},
          doi = {10.1007/978-3-319-55333-7_104},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018haex.bookE.104M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Madhusudhan2019,
       author = {{Madhusudhan}, Nikku},
        title = "{Exoplanetary Atmospheres: Key Insights, Challenges, and Prospects}",
      journal = {\araa},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = aug,
       volume = {57},
        pages = {617-663},
          doi = {10.1146/annurev-astro-081817-051846},
archivePrefix = {arXiv},
       eprint = {1904.03190},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ARA&A..57..617M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2008,
       author = {{Showman}, Adam P. and {Cooper}, Curtis S. and {Fortney}, Jonathan J. and {Marley}, Mark S.},
        title = "{Atmospheric Circulation of Hot Jupiters: Three-dimensional Circulation Models of HD 209458b and HD 189733b with Simplified Forcing}",
      journal = {\apj},
     keywords = {atmospheric effects, methods: numerical, planets and satellites: general, planets and satellites: individual: HD 209458b, Astrophysics},
         year = 2008,
        month = jul,
       volume = {682},
       number = {1},
        pages = {559-576},
          doi = {10.1086/589325},
archivePrefix = {arXiv},
       eprint = {0802.0327},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...682..559S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2011,
       author = {{Showman}, Adam P. and {Polvani}, Lorenzo M.},
        title = "{Equatorial Superrotation on Tidally Locked Exoplanets}",
      journal = {\apj},
     keywords = {hydrodynamics, methods: analytical, methods: numerical, planets and satellites: atmospheres, planets and satellites: individual: HD 189733b, waves, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = sep,
       volume = {738},
       number = {1},
          eid = {71},
        pages = {71},
          doi = {10.1088/0004-637X/738/1/71},
archivePrefix = {arXiv},
       eprint = {1103.3101},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...738...71S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2013,
       author = {{Showman}, Adam P. and {Fortney}, Jonathan J. and {Lewis}, Nikole K. and {Shabram}, Megan},
        title = "{Doppler Signatures of the Atmospheric Circulation on Hot Jupiters}",
      journal = {\apj},
     keywords = {atmospheric effects, hydrodynamics, methods: numerical, planets and satellites: atmospheres, planets and satellites: general, planets and satellites: individual: HD 189733b HD 209458b GJ 436b, waves, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = jan,
       volume = {762},
       number = {1},
          eid = {24},
        pages = {24},
          doi = {10.1088/0004-637X/762/1/24},
archivePrefix = {arXiv},
       eprint = {1207.5639},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...762...24S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kataria2016,
       author = {{Kataria}, Tiffany and {Sing}, David K. and {Lewis}, Nikole K. and {Visscher}, Channon and {Showman}, Adam P. and {Fortney}, Jonathan J. and {Marley}, Mark S.},
        title = "{The Atmospheric Circulation of a Nine-hot-Jupiter Sample: Probing Circulation and Chemistry over a Wide Phase Space}",
      journal = {\apj},
     keywords = {atmospheric effects, methods: numerical, planets and satellites: general, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = apr,
       volume = {821},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.3847/0004-637X/821/1/9},
archivePrefix = {arXiv},
       eprint = {1602.06733},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...821....9K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wong2020,
       author = {{Wong}, Ian and {Shporer}, Avi and {Kitzmann}, Daniel and {Morris}, Brett M. and {Heng}, Kevin and {Hoeijmakers}, H. Jens and {Demory}, Brice-Olivier and {Ahlers}, John P. and {Mansfield}, Megan and {Bean}, Jacob L. and {Daylan}, Tansu and {Fetherolf}, Tara and {Rodriguez}, Joseph E. and {Benneke}, Bj{\"o}rn and {Ricker}, George R. and {Latham}, David W. and {Vanderspek}, Roland and {Seager}, Sara and {Winn}, Joshua N. and {Jenkins}, Jon M. and {Burke}, Christopher J. and {Christiansen}, Jessie L. and {Essack}, Zahra and {Rose}, Mark E. and {Smith}, Jeffrey C. and {Tenenbaum}, Peter and {Yahalomi}, Daniel},
        title = "{Exploring the Atmospheric Dynamics of the Extreme Ultrahot Jupiter KELT-9b Using TESS Photometry}",
      journal = {\aj},
     keywords = {Hot Jupiters, Photometry, Exoplanet astronomy, 753, 1234, 486, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = aug,
       volume = {160},
       number = {2},
          eid = {88},
        pages = {88},
          doi = {10.3847/1538-3881/aba2cb},
archivePrefix = {arXiv},
       eprint = {1910.01607},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160...88W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Louden2015,
       author = {{Louden}, Tom and {Wheatley}, Peter J.},
        title = "{Spatially Resolved Eastward Winds and Rotation of HD 189733b}",
      journal = {\apjl},
     keywords = {atmospheric effects, celestial mechanics, planets and satellites: atmospheres, planets and satellites: individual: HD 189733b, stars: individual: HD 189733, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = dec,
       volume = {814},
       number = {2},
          eid = {L24},
        pages = {L24},
          doi = {10.1088/2041-8205/814/2/L24},
archivePrefix = {arXiv},
       eprint = {1511.03689},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...814L..24L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brogi2016,
       author = {{Brogi}, M. and {de Kok}, R.~J. and {Albrecht}, S. and {Snellen}, I.~A.~G. and {Birkby}, J.~L. and {Schwarz}, H.},
        title = "{Rotation and Winds of Exoplanet HD 189733 b Measured with High-dispersion Transmission Spectroscopy}",
      journal = {\apj},
     keywords = {planets and satellites: atmospheres, planets and satellites: fundamental parameters, planets and satellites: individual: HD 189733 b, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = feb,
       volume = {817},
       number = {2},
          eid = {106},
        pages = {106},
          doi = {10.3847/0004-637X/817/2/106},
archivePrefix = {arXiv},
       eprint = {1512.05175},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817..106B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Snellen2010,
       author = {{Snellen}, Ignas A.~G. and {de Kok}, Remco J. and {de Mooij}, Ernst J.~W. and {Albrecht}, Simon},
        title = "{The orbital motion, absolute mass and high-altitude winds of exoplanet HD209458b}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jun,
       volume = {465},
       number = {7301},
        pages = {1049-1051},
          doi = {10.1038/nature09111},
archivePrefix = {arXiv},
       eprint = {1006.4364},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.465.1049S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kempton2012,
       author = {{Miller-Ricci Kempton}, Eliza and {Rauscher}, Emily},
        title = "{Constraining High-speed Winds in Exoplanet Atmospheres through Observations of Anomalous Doppler Shifts during Transit}",
      journal = {\apj},
     keywords = {planetary systems, Astrophysics - Earth and Planetary Astrophysics},
         year = 2012,
        month = jun,
       volume = {751},
       number = {2},
          eid = {117},
        pages = {117},
          doi = {10.1088/0004-637X/751/2/117},
archivePrefix = {arXiv},
       eprint = {1109.2270},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...751..117M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kempton2014,
       author = {{Kempton}, Eliza M. -R. and {Perna}, Rosalba and {Heng}, Kevin},
        title = "{High Resolution Transmission Spectroscopy as a Diagnostic for Jovian Exoplanet Atmospheres: Constraints from Theoretical Models}",
      journal = {\apj},
     keywords = {methods: numerical, planetary systems, planets and satellites: atmospheres, planets and satellites: gaseous planets, radiative transfer, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = nov,
       volume = {795},
       number = {1},
          eid = {24},
        pages = {24},
          doi = {10.1088/0004-637X/795/1/24},
archivePrefix = {arXiv},
       eprint = {1409.1250},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...795...24K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Fu2017,
       author = {{Fu}, Guangwei and {Deming}, Drake and {Knutson}, Heather and {Madhusudhan}, Nikku and {Mandell}, Avi and {Fraine}, Jonathan},
        title = "{Statistical Analysis of Hubble/WFC3 Transit Spectroscopy of Extrasolar Planets}",
      journal = {\apjl},
     keywords = {planets and satellites: atmospheres, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = oct,
       volume = {847},
       number = {2},
          eid = {L22},
        pages = {L22},
          doi = {10.3847/2041-8213/aa8e40},
archivePrefix = {arXiv},
       eprint = {1709.07385},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...847L..22F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Crossfield2017,
       author = {{Crossfield}, Ian J.~M. and {Kreidberg}, Laura},
        title = "{Trends in Atmospheric Properties of Neptune-size Exoplanets}",
      journal = {\aj},
     keywords = {eclipses, methods: statistical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = dec,
       volume = {154},
       number = {6},
          eid = {261},
        pages = {261},
          doi = {10.3847/1538-3881/aa9279},
archivePrefix = {arXiv},
       eprint = {1708.00016},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..261C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sheppard2017,
       author = {{Sheppard}, Kyle B. and {Mandell}, Avi M. and {Tamburo}, Patrick and {Gandhi}, Siddharth and {Pinhas}, Arazi and {Madhusudhan}, Nikku and {Deming}, Drake},
        title = "{Evidence for a Dayside Thermal Inversion and High Metallicity for the Hot Jupiter WASP-18b}",
      journal = {\apjl},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: gaseous planets, planets and satellites: individual: WASP-18b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = dec,
       volume = {850},
       number = {2},
          eid = {L32},
        pages = {L32},
          doi = {10.3847/2041-8213/aa9ae9},
archivePrefix = {arXiv},
       eprint = {1711.10491},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...850L..32S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Evans2017,
       author = {{Evans}, Thomas M. and {Sing}, David K. and {Kataria}, Tiffany and {Goyal}, Jayesh and {Nikolov}, Nikolay and {Wakeford}, Hannah R. and {Deming}, Drake and {Marley}, Mark S. and {Amundsen}, David S. and {Ballester}, Gilda E. and {Barstow}, Joanna K. and {Ben-Jaffel}, Lotfi and {Bourrier}, Vincent and {Buchhave}, Lars A. and {Cohen}, Ofer and {Ehrenreich}, David and {Garc{\'\i}a Mu{\~n}oz}, Antonio and {Henry}, Gregory W. and {Knutson}, Heather and {Lavvas}, Panayotis and {Lecavelier Des Etangs}, Alain and {Lewis}, Nikole K. and {L{\'o}pez-Morales}, Mercedes and {Mandell}, Avi M. and {Sanz-Forcada}, Jorge and {Tremblin}, Pascal and {Lupu}, Roxana},
        title = "{An ultrahot gas-giant exoplanet with a stratosphere}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = aug,
       volume = {548},
       number = {7665},
        pages = {58-61},
          doi = {10.1038/nature23266},
archivePrefix = {arXiv},
       eprint = {1708.01076},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Natur.548...58E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haynes2015,
       author = {{Haynes}, Korey and {Mandell}, Avi M. and {Madhusudhan}, Nikku and {Deming}, Drake and {Knutson}, Heather},
        title = "{Spectroscopic Evidence for a Temperature Inversion in the Dayside Atmosphere of Hot Jupiter WASP-33b}",
      journal = {\apj},
     keywords = {eclipses, planetary systems, techniques: photometric, techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = jun,
       volume = {806},
       number = {2},
          eid = {146},
        pages = {146},
          doi = {10.1088/0004-637X/806/2/146},
archivePrefix = {arXiv},
       eprint = {1505.01490},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...806..146H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pino2020,
       author = {{Pino}, Lorenzo and {D{\'e}sert}, Jean-Michel and {Brogi}, Matteo and {Malavolta}, Luca and {Wyttenbach}, Aur{\'e}lien and {Line}, Michael and {Hoeijmakers}, Jens and {Fossati}, Luca and {Bonomo}, Aldo Stefano and {Nascimbeni}, Valerio and {Panwar}, Vatsal and {Affer}, Laura and {Benatti}, Serena and {Biazzo}, Katia and {Bignamini}, Andrea and {Borsa}, Franscesco and {Carleo}, Ilaria and {Claudi}, Riccardo and {Cosentino}, Rosario and {Covino}, Elvira and {Damasso}, Mario and {Desidera}, Silvano and {Giacobbe}, Paolo and {Harutyunyan}, Avet and {Lanza}, Antonino Francesco and {Leto}, Giuseppe and {Maggio}, Antonio and {Maldonado}, Jesus and {Mancini}, Luigi and {Micela}, Giuseppina and {Molinari}, Emilio and {Pagano}, Isabella and {Piotto}, Giampaolo and {Poretti}, Ennio and {Rainer}, Monica and {Scandariato}, Gaetano and {Sozzetti}, Alessandro and {Allart}, Romain and {Borsato}, Luca and {Bruno}, Giovanni and {Di Fabrizio}, Luca and {Ehrenreich}, David and {Fiorenzano}, Aldo and {Frustagli}, Giuseppe and {Lavie}, Baptiste and {Lovis}, Christophe and {Magazz{\`u}}, Antonio and {Nardiello}, Domenico and {Pedani}, Marco and {Smareglia}, Riccardo},
        title = "{Neutral Iron Emission Lines from the Dayside of KELT-9b: The GAPS Program with HARPS-N at TNG XX}",
      journal = {\apjl},
     keywords = {487, 2021, 2096, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = may,
       volume = {894},
       number = {2},
          eid = {L27},
        pages = {L27},
          doi = {10.3847/2041-8213/ab8c44},
archivePrefix = {arXiv},
       eprint = {2004.11335},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...894L..27P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nugroho2017,
       author = {{Nugroho}, Stevanus K. and {Kawahara}, Hajime and {Masuda}, Kento and {Hirano}, Teruyuki and {Kotani}, Takayuki and {Tajitsu}, Akito},
        title = "{High-resolution Spectroscopic Detection of TiO and a Stratosphere in the Day-side of WASP-33b}",
      journal = {\aj},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: individual (WASP-33b), techniques: spectroscopic, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = dec,
       volume = {154},
       number = {6},
          eid = {221},
        pages = {221},
          doi = {10.3847/1538-3881/aa9433},
archivePrefix = {arXiv},
       eprint = {1710.05276},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..221N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier2015,
       author = {{Strassmeier}, K.~G. and {Ilyin}, I. and {J{\"a}rvinen}, A. and {Weber}, M. and {Woche}, M. and {Barnes}, S.~I. and {Bauer}, S. -M. and {Beckert}, E. and {Bittner}, W. and {Bredthauer}, R. and {Carroll}, T.~A. and {Denker}, C. and {Dionies}, F. and {DiVarano}, I. and {D{\"o}scher}, D. and {Fechner}, T. and {Feuerstein}, D. and {Granzer}, T. and {Hahn}, T. and {Harnisch}, G. and {Hofmann}, A. and {Lesser}, M. and {Paschke}, J. and {Pankratow}, S. and {Plank}, V. and {Pl{\"u}schke}, D. and {Popow}, E. and {Sablowski}, D.},
        title = "{PEPSI: The high-resolution {\'e}chelle spectrograph and polarimeter for the Large Binocular Telescope}",
      journal = {Astronomische Nachrichten},
     keywords = {instrumentation: spectrographs, instrumentation: polarimeters, instrumentation: detectors, techniques: spectroscopic, stars: individual (HD 194937, {\ensuremath{\tau}} Cet, {\ensuremath{\alpha}} Cyg), Sun: photosphere, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = may,
       volume = {336},
       number = {4},
        pages = {324},
          doi = {10.1002/asna.201512172},
archivePrefix = {arXiv},
       eprint = {1505.06492},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AN....336..324S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Borsa2019,
       author = {{Borsa}, F. and {Rainer}, M. and {Bonomo}, A.~S. and {Barbato}, D. and {Fossati}, L. and {Malavolta}, L. and {Nascimbeni}, V. and {Lanza}, A.~F. and {Esposito}, M. and {Affer}, L. and {Andreuzzi}, G. and {Benatti}, S. and {Biazzo}, K. and {Bignamini}, A. and {Brogi}, M. and {Carleo}, I. and {Claudi}, R. and {Cosentino}, R. and {Covino}, E. and {Damasso}, M. and {Desidera}, S. and {Garrido Rubio}, A. and {Giacobbe}, P. and {Gonz{\'a}lez-{\'A}lvarez}, E. and {Harutyunyan}, A. and {Knapic}, C. and {Leto}, G. and {Ligi}, R. and {Maggio}, A. and {Maldonado}, J. and {Mancini}, L. and {Fiorenzano}, A.~F.~M. and {Masiero}, S. and {Micela}, G. and {Molinari}, E. and {Pagano}, I. and {Pedani}, M. and {Piotto}, G. and {Pino}, L. and {Poretti}, E. and {Scandariato}, G. and {Smareglia}, R. and {Sozzetti}, A.},
        title = "{The GAPS Programme with HARPS-N at TNG. XIX. Atmospheric Rossiter-McLaughlin effect and improved parameters of KELT-9b}",
      journal = {\aap},
     keywords = {planetary systems, techniques: spectroscopic, techniques: radial velocities, planets and satellites: atmospheres, stars: individual: KELT-9, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = nov,
       volume = {631},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201935718},
archivePrefix = {arXiv},
       eprint = {1907.10078},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...631A..34B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tan2019,
       author = {{Tan}, Xianyu and {Komacek}, Thaddeus D.},
        title = "{The Atmospheric Circulation of Ultra-hot Jupiters}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Hot Jupiters, Hydrodynamics, 753, 487, 1963, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = nov,
       volume = {886},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/ab4a76},
archivePrefix = {arXiv},
       eprint = {1910.01622},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886...26T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Roth2021,
       author = {{Roth}, A. and {Drummond}, B. and {H{\'e}brard}, E. and {Tremblin}, P. and {Goyal}, J. and {Mayne}, N.},
        title = "{Pseudo-2D modelling of heat redistribution through H$_{2}$ thermal dissociation/recombination: Consequences for ultra-hot jupiters}",
      journal = {\mnras},
     keywords = {planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = may,
          doi = {10.1093/mnras/stab1256},
archivePrefix = {arXiv},
       eprint = {2104.14376},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.tmp.1239R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Casasayas-Barris2019,
       author = {{Casasayas-Barris}, N. and {Pall{\'e}}, E. and {Yan}, F. and {Chen}, G. and {Kohl}, S. and {Stangret}, M. and {Parviainen}, H. and {Helling}, Ch. and {Watanabe}, N. and {Czesla}, S. and {Fukui}, A. and {Monta{\~n}{\'e}s-Rodr{\'\i}guez}, P. and {Nagel}, E. and {Narita}, N. and {Nortmann}, L. and {Nowak}, G. and {Schmitt}, J.~H.~M.~M. and {Zapatero Osorio}, M.~R.},
        title = "{Atmospheric characterization of the ultra-hot Jupiter MASCARA-2b/KELT-20b. Detection of Ca II, Fe II, Na I, and the Balmer series of H (H{\ensuremath{\alpha}}, H{\ensuremath{\beta}}, and H{\ensuremath{\gamma}}) with high-dispersion transit spectroscopy (Corrigendum)}",
      journal = {\aap},
     keywords = {planetary systems, methods: observational, techniques: spectroscopic, planets and satellites: individual: MASCARA-2b, planets and satellites: individual: KELT-20b - errata, addenda},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {C6},
        pages = {C6},
          doi = {10.1051/0004-6361/201935623e},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640C...6C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2017,
       author = {{Yan}, F. and {Pall{\'e}}, E. and {Fosbury}, R.~A.~E. and {Petr-Gotzens}, M.~G. and {Henning}, Th.},
        title = "{Effect of the stellar absorption line centre-to-limb variation on exoplanet transmission spectrum observations}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, techniques: spectroscopic, stars: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jul,
       volume = {603},
          eid = {A73},
        pages = {A73},
          doi = {10.1051/0004-6361/201630144},
archivePrefix = {arXiv},
       eprint = {1703.07585},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...603A..73Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Yan2015,
       author = {{Yan}, F. and {Fosbury}, R.~A.~E. and {Petr-Gotzens}, M.~G. and {Zhao}, G. and {Pall{\'e}}, E.},
        title = "{The centre-to-limb variations of solar Fraunhofer lines imprinted upon lunar eclipse spectra. Implications for exoplanet transit observations}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, Earth, Moon, eclipses, stars: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {574},
          eid = {A94},
        pages = {A94},
          doi = {10.1051/0004-6361/201425220},
archivePrefix = {arXiv},
       eprint = {1501.02306},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...574A..94Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2018,
       author = {{Yan}, Fei and {Henning}, Thomas},
        title = "{An extended hydrogen envelope of the extremely hot giant exoplanet KELT-9b}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = jul,
       volume = {2},
        pages = {714-718},
          doi = {10.1038/s41550-018-0503-3},
archivePrefix = {arXiv},
       eprint = {1807.00869},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..714Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yan2019,
       author = {{Yan}, F. and {Casasayas-Barris}, N. and {Molaverdikhani}, K. and {Alonso-Floriano}, F.~J. and {Reiners}, A. and {Pall{\'e}}, E. and {Henning}, Th. and {Molli{\`e}re}, P. and {Chen}, G. and {Nortmann}, L. and {Snellen}, I.~A.~G. and {Ribas}, I. and {Quirrenbach}, A. and {Caballero}, J.~A. and {Amado}, P.~J. and {Azzaro}, M. and {Bauer}, F.~F. and {Cort{\'e}s Contreras}, M. and {Czesla}, S. and {Khalafinejad}, S. and {Lara}, L.~M. and {L{\'o}pez-Puertas}, M. and {Montes}, D. and {Nagel}, E. and {Oshagh}, M. and {S{\'a}nchez-L{\'o}pez}, A. and {Stangret}, M. and {Zechmeister}, M.},
        title = "{Ionized calcium in the atmospheres of two ultra-hot exoplanets WASP-33b and KELT-9b}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, techniques: spectroscopic, planets and satellites: individual: WASP-33b, planets and satellites: individual: KELT-9b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = dec,
       volume = {632},
          eid = {A69},
        pages = {A69},
          doi = {10.1051/0004-6361/201936396},
archivePrefix = {arXiv},
       eprint = {1911.00380},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...632A..69Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wyttenbach2020,
       author = {{Wyttenbach}, A. and {Molli{\`e}re}, P. and {Ehrenreich}, D. and {Cegla}, H.~M. and {Bourrier}, V. and {Lovis}, C. and {Pino}, L. and {Allart}, R. and {Seidel}, J.~V. and {Hoeijmakers}, H.~J. and {Nielsen}, L.~D. and {Lavie}, B. and {Pepe}, F. and {Bonfils}, X. and {Snellen}, I.~A.~G.},
        title = "{Mass-loss rate and local thermodynamic state of the KELT-9 b thermosphere from the hydrogen Balmer series}",
      journal = {\aap},
     keywords = {planetary systems, planets and satellites: atmospheres, planets and satellites: individual: KELT-9 b, techniques: spectroscopic, instrumentation: spectrographs, methods: observational, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jun,
       volume = {638},
          eid = {A87},
        pages = {A87},
          doi = {10.1051/0004-6361/201937316},
archivePrefix = {arXiv},
       eprint = {2004.13733},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...638A..87W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Faigler2011,
       author = {{Faigler}, S. and {Mazeh}, T.},
        title = "{Photometric detection of non-transiting short-period low-mass companions through the beaming, ellipsoidal and reflection effects in Kepler and CoRoT light curves}",
      journal = {\mnras},
     keywords = {methods: data analysis, binaries: eclipsing, binaries: general, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = aug,
       volume = {415},
       number = {4},
        pages = {3921-3928},
          doi = {10.1111/j.1365-2966.2011.19011.x},
archivePrefix = {arXiv},
       eprint = {1106.2713},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.415.3921F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eastman2010,
       author = {{Eastman}, Jason and {Siverd}, Robert and {Gaudi}, B. Scott},
        title = "{Achieving Better Than 1 Minute Accuracy in the Heliocentric and Barycentric Julian Dates}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = aug,
       volume = {122},
       number = {894},
        pages = {935},
          doi = {10.1086/655938},
archivePrefix = {arXiv},
       eprint = {1005.4415},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010PASP..122..935E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Eastman2012,
       author = {{Eastman}, Jason},
        title = "{Time Utilities}",
     keywords = {Software},
         year = 2012,
        month = jun,
          eid = {ascl:1206.012},
        pages = {ascl:1206.012},
archivePrefix = {ascl},
       eprint = {1206.012},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ascl.soft06012E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eastman2019,
       author = {{Eastman}, Jason D. and {Rodriguez}, Joseph E. and {Agol}, Eric and {Stassun}, Keivan G. and {Beatty}, Thomas G. and {Vanderburg}, Andrew and {Gaudi}, B. Scott and {Collins}, Karen A. and {Luger}, Rodrigo},
        title = "{EXOFASTv2: A public, generalized, publication-quality exoplanet modeling code}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jul,
          eid = {arXiv:1907.09480},
        pages = {arXiv:1907.09480},
archivePrefix = {arXiv},
       eprint = {1907.09480},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190709480E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Claret2017,
       author = {{Claret}, A.},
        title = "{Limb and gravity-darkening coefficients for the TESS satellite at several metallicities, surface gravities, and microturbulent velocities}",
      journal = {\aap},
     keywords = {planetary systems, stars: atmospheres, binaries: eclipsing, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {600},
          eid = {A30},
        pages = {A30},
          doi = {10.1051/0004-6361/201629705},
archivePrefix = {arXiv},
       eprint = {1804.10295},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...600A..30C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beltz2021a,
       author = {{Beltz}, Hayley and {Rauscher}, Emily and {Brogi}, Matteo and {Kempton}, Eliza M. -R.},
        title = "{A Significant Increase in Detection of High-resolution Emission Spectra Using a Three-dimensional Atmospheric Model of a Hot Jupiter}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, High resolution spectroscopy, Hot Jupiters, Hydrodynamical simulations, Radiative transfer simulations, 487, 2096, 753, 767, 1967, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jan,
       volume = {161},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.3847/1538-3881/abb67b},
archivePrefix = {arXiv},
       eprint = {2009.09030},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Donatelli2014,
title = {Square smoothing regularization matrices with accurate boundary conditions},
journal = {Journal of Computational and Applied Mathematics},
volume = {272},
pages = {334-349},
year = {2014},
issn = {0377-0427},
doi = {https://doi.org/10.1016/j.cam.2013.08.015},
url = {https://www.sciencedirect.com/science/article/pii/S0377042713004202},
author = {M. Donatelli and L. Reichel},
keywords = {Tikhonov regularization, Regularization matrix, Boundary conditions},
abstract = {This paper is concerned with the solution of large-scale linear discrete ill-posed problems. The determination of a meaningful approximate solution of these problems requires regularization. We discuss regularization by the Tikhonov method and by truncated iteration. The choice of regularization matrix in Tikhonov regularization may significantly affect the quality of the computed approximate solution. The present paper describes the construction of square regularization matrices from finite difference equations with a focus on the boundary conditions. The regularization matrices considered have a structure that makes them easy to apply in iterative methods, including methods based on the Arnoldi process. Numerical examples illustrate the properties and effectiveness of the regularization matrices described.}
}


@ARTICLE{Molliere2019,
       author = {{Molli{\`e}re}, P. and {Wardenier}, J.~P. and {van Boekel}, R. and {Henning}, Th. and {Molaverdikhani}, K. and {Snellen}, I.~A.~G.},
        title = "{petitRADTRANS. A Python radiative transfer package for exoplanet characterization and retrieval}",
      journal = {\aap},
     keywords = {methods: numerical, planets and satellites: atmospheres, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/201935470},
archivePrefix = {arXiv},
       eprint = {1904.11504},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A..67M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{Palme2014,
       author = {{Palme}, H. and {Lodders}, K. and {Jones}, A.},
        title = "{Solar System Abundances of the Elements}",
    booktitle = {Planets, Asteriods, Comets and The Solar System},
         year = 2014,
       editor = {{Davis}, Andrew M.},
       volume = {2},
        pages = {15-36},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014pacs.book...15P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Pakhomov2017,
       author = {{Pakhomov}, Yu. and {Piskunov}, N. and {Ryabchikova}, T.},
        title = "{VALD3: Current Developments}",
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Stars: From Collapse to Collapse},
         year = 2017,
       editor = {{Balega}, Yu. Yu. and {Kudryavtsev}, D.~O. and {Romanyuk}, I.~I. and {Yakunin}, I.~A.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {510},
        month = jun,
        pages = {518},
archivePrefix = {arXiv},
       eprint = {1710.10854},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ASPC..510..518P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Valenti2012,
       author = {{Valenti}, J.~A. and {Piskunov}, N.},
        title = "{SME: Spectroscopy Made Easy}",
     keywords = {Software},
         year = 2012,
        month = feb,
          eid = {ascl:1202.013},
        pages = {ascl:1202.013},
archivePrefix = {ascl},
       eprint = {1202.013},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ascl.soft02013V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Valenti1996,
       author = {{Valenti}, J.~A. and {Piskunov}, N.},
        title = "{Spectroscopy made easy: A new tool for fitting observations with synthetic spectra.}",
      journal = {\aaps},
     keywords = {RADIATIVE TRANSFER, METHODS: NUMERICAL, TECHNIQUES: SPECTROSCOPIC, STARS: FUNDAMENTAL PARAMETERS, SUN: FUNDAMENTAL PARAMETERS, ATOMIC DATA},
         year = 1996,
        month = sep,
       volume = {118},
        pages = {595-603},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..118..595V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CollierCameron2010,
       author = {{Collier Cameron}, A. and {Bruce}, V.~A. and {Miller}, G.~R.~M. and {Triaud}, A.~H.~M.~J. and {Queloz}, D.},
        title = "{Line-profile tomography of exoplanet transits - I. The Doppler shadow of HD 189733b}",
      journal = {\mnras},
     keywords = {techniques: spectroscopic, stars: activity, binaries: eclipsing, planetary systems, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = mar,
       volume = {403},
       number = {1},
        pages = {151-158},
          doi = {10.1111/j.1365-2966.2009.16131.x},
archivePrefix = {arXiv},
       eprint = {0911.5361},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.403..151C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Foreman-Mackey2013,
       author = {{Foreman-Mackey}, Daniel and {Hogg}, David W. and {Lang}, Dustin and {Goodman}, Jonathan},
        title = "{emcee: The MCMC Hammer}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Computational Physics, Statistics - Computation},
         year = 2013,
        month = mar,
       volume = {125},
       number = {925},
        pages = {306},
          doi = {10.1086/670067},
archivePrefix = {arXiv},
       eprint = {1202.3665},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013PASP..125..306F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seager2003,
       author = {{Seager}, S. and {Mall{\'e}n-Ornelas}, G.},
        title = "{A Unique Solution of Planet and Star Parameters from an Extrasolar Planet Transit Light Curve}",
      journal = {\apj},
     keywords = {Stars: Binaries: Eclipsing, Stars: Planetary Systems, Techniques: Photometric, Astrophysics},
         year = 2003,
        month = mar,
       volume = {585},
       number = {2},
        pages = {1038-1055},
          doi = {10.1086/346105},
archivePrefix = {arXiv},
       eprint = {astro-ph/0206228},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...585.1038S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Torres2010,
       author = {{Torres}, G. and {Andersen}, J. and {Gim{\'e}nez}, A.},
        title = "{Accurate masses and radii of normal stars: modern results and applications}",
      journal = {\aapr},
     keywords = {Stars: fundamental parameters, Stars: binaries: eclipsing, Stars: binaries: spectroscopic, Stars: interiors, Stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = feb,
       volume = {18},
       number = {1-2},
        pages = {67-126},
          doi = {10.1007/s00159-009-0025-1},
archivePrefix = {arXiv},
       eprint = {0908.2624},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&ARv..18...67T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tayar2020,
       author = {{Tayar}, Jamie and {Claytor}, Zachary R. and {Huber}, Daniel and {van Saders}, Jennifer},
        title = "{A Guide to Realistic Uncertainties on Fundamental Properties of Solar-Type Exoplanet Host Stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.07957},
        pages = {arXiv:2012.07957},
archivePrefix = {arXiv},
       eprint = {2012.07957},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201207957T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RodriguezMartinez2021,
       author = {{Rodriguez Martinez}, Romy and {Stevens}, Daniel J. and {Gaudi}, B. Scott and {Schulze}, Joseph G. and {Panero}, Wendy R. and {Johnson}, Jennifer A. and {Wang}, Ji},
        title = "{Analytic Estimates of the Achievable Precision on the Physical Properties of Transiting Planets Using Purely Empirical Measurements}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jan,
          eid = {arXiv:2101.09289},
        pages = {arXiv:2101.09289},
archivePrefix = {arXiv},
       eprint = {2101.09289},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210109289R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ahlers2020,
       author = {{Ahlers}, John P. and {Johnson}, Marshall C. and {Stassun}, Keivan G. and {Col{\'o}n}, Knicole D. and {Barnes}, Jason W. and {Stevens}, Daniel J. and {Beatty}, Thomas and {Gaudi}, B. Scott and {Collins}, Karen A. and {Rodriguez}, Joseph E. and {Ricker}, George and {Vanderspek}, Roland and {Latham}, David and {Seager}, Sara and {Winn}, Joshua and {Jenkins}, Jon M. and {Caldwell}, Douglas A. and {Goeke}, Robert F. and {Osborn}, Hugh P. and {Paegert}, Martin and {Rowden}, Pam and {Tenenbaum}, Peter},
        title = "{KELT-9 b's Asymmetric TESS Transit Caused by Rapid Stellar Rotation and Spin-Orbit Misalignment}",
      journal = {\aj},
     keywords = {Exoplanets, Hot Jupiters, Exoplanet evolution, Stellar rotation, Gravity darkening, von Zeipel theorem, Exoplanet astronomy, Transit photometry, 1709, 498, 491, 1781, 680, 1629, 486, 753, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {160},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.3847/1538-3881/ab8fa3},
archivePrefix = {arXiv},
       eprint = {2004.14812},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AJ....160....4A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Loeb2003,
       author = {{Loeb}, Abraham and {Gaudi}, B. Scott},
        title = "{Periodic Flux Variability of Stars due to the Reflex Doppler Effect Induced by Planetary Companions}",
      journal = {\apjl},
     keywords = {Stars: Planetary Systems, Techniques: Photometric, Astrophysics},
         year = 2003,
        month = may,
       volume = {588},
       number = {2},
        pages = {L117-L120},
          doi = {10.1086/375551},
archivePrefix = {arXiv},
       eprint = {astro-ph/0303212},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...588L.117L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Giacobbe2021,
       author = {{Giacobbe}, Paolo and {Brogi}, Matteo and {Gandhi}, Siddharth and {Cubillos}, Patricio E. and {Bonomo}, Aldo S. and {Sozzetti}, Alessandro and {Fossati}, Luca and {Guilluy}, Gloria and {Carleo}, Ilaria and {Rainer}, Monica and {Harutyunyan}, Avet and {Borsa}, Francesco and {Pino}, Lorenzo and {Nascimbeni}, Valerio and {Benatti}, Serena and {Biazzo}, Katia and {Bignamini}, Andrea and {Chubb}, Katy L. and {Claudi}, Riccardo and {Cosentino}, Rosario and {Covino}, Elvira and {Damasso}, Mario and {Desidera}, Silvano and {Fiorenzano}, Aldo F.~M. and {Ghedina}, Adriano and {Lanza}, Antonino F. and {Leto}, Giuseppe and {Maggio}, Antonio and {Malavolta}, Luca and {Maldonado}, Jesus and {Micela}, Giuseppina and {Molinari}, Emilio and {Pagano}, Isabella and {Pedani}, Marco and {Piotto}, Giampaolo and {Poretti}, Ennio and {Scandariato}, Gaetano and {Yurchenko}, Sergei N. and {Fantinel}, Daniela and {Galli}, Alberto and {Lodi}, Marcello and {Sanna}, Nicoletta and {Tozzi}, Andrea},
        title = "{Five carbon- and nitrogen-bearing species in a hot giant planet's atmosphere}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
          eid = {arXiv:2104.03352},
        pages = {arXiv:2104.03352},
archivePrefix = {arXiv},
       eprint = {2104.03352},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210403352G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Murray-Clay2009,
       author = {{Murray-Clay}, Ruth A. and {Chiang}, Eugene I. and {Murray}, Norman},
        title = "{Atmospheric Escape From Hot Jupiters}",
      journal = {\apj},
     keywords = {hydrodynamics, planetary systems, stars: individual: HD 209458, Astrophysics},
         year = 2009,
        month = mar,
       volume = {693},
       number = {1},
        pages = {23-42},
          doi = {10.1088/0004-637X/693/1/23},
archivePrefix = {arXiv},
       eprint = {0811.0006},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...693...23M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GarciaMunoz2019,
       author = {{Garc{\'\i}a Mu{\~n}oz}, A. and {Schneider}, P.~C.},
        title = "{Rapid Escape of Ultra-hot Exoplanet Atmospheres Driven by Hydrogen Balmer Absorption}",
      journal = {\apjl},
     keywords = {Exoplanet atmospheres, Aeronomy, Exoplanet evolution, Radiative transfer, 487, 22, 491, 1335, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = oct,
       volume = {884},
       number = {2},
          eid = {L43},
        pages = {L43},
          doi = {10.3847/2041-8213/ab498d},
archivePrefix = {arXiv},
       eprint = {1910.00267},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884L..43G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Erkaev2007,
       author = {{Erkaev}, N.~V. and {Kulikov}, Yu. N. and {Lammer}, H. and {Selsis}, F. and {Langmayr}, D. and {Jaritz}, G.~F. and {Biernat}, H.~K.},
        title = "{Roche lobe effects on the atmospheric loss from ``Hot Jupiters''}",
      journal = {\aap},
     keywords = {hydrodynamics, atmospheric effects, stars: activity, planets and satellites: general, Astrophysics},
         year = 2007,
        month = sep,
       volume = {472},
       number = {1},
        pages = {329-334},
          doi = {10.1051/0004-6361:20066929},
archivePrefix = {arXiv},
       eprint = {astro-ph/0612729},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...472..329E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krenn2021,
       author = {{Krenn}, Andreas F. and {Fossati}, Luca and {Kubyshkina}, Daria and {Lammer}, Helmut},
        title = "{A critical assessment of the applicability of the energy-limited approximation for estimating exoplanetary mass-loss rates}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.05858},
        pages = {arXiv:2105.05858},
archivePrefix = {arXiv},
       eprint = {2105.05858},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210505858K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kubyshkina2018,
       author = {{Kubyshkina}, D. and {Fossati}, L. and {Erkaev}, N.~V. and {Cubillos}, P.~E. and {Johnstone}, C.~P. and {Kislyakova}, K.~G. and {Lammer}, H. and {Lendl}, M. and {Odert}, P.},
        title = "{Overcoming the Limitations of the Energy-limited Approximation for Planet Atmospheric Escape}",
      journal = {\apjl},
     keywords = {planets and satellites: atmospheres, planets and satellites: gaseous planets, planets and satellites: general, planets and satellites: physical evolution, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = oct,
       volume = {866},
       number = {2},
          eid = {L18},
        pages = {L18},
          doi = {10.3847/2041-8213/aae586},
archivePrefix = {arXiv},
       eprint = {1810.06920},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...866L..18K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanz-Forcada2011,
       author = {{Sanz-Forcada}, J. and {Micela}, G. and {Ribas}, I. and {Pollock}, A.~M.~T. and {Eiroa}, C. and {Velasco}, A. and {Solano}, E. and {Garc{\'\i}a-{\'A}lvarez}, D.},
        title = "{Estimation of the XUV radiation onto close planets and their evaporation}",
      journal = {\aap},
     keywords = {planetary systems, stars: coronae, astrobiology, X-rays: stars, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = aug,
       volume = {532},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201116594},
archivePrefix = {arXiv},
       eprint = {1105.0550},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...532A...6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia2016,
       author = {{Gaia Collaboration} and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Milligan}, D.~J. and {Panem}, C. and {Poinsignon}, V. and {Pourbaix}, D. and {Randich}, S. and {Sarri}, G. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Valette}, V. and {van Leeuwen}, F. and {Walton}, N.~A. and {Aerts}, C. and {Arenou}, F. and {Cropper}, M. and {Drimmel}, R. and {H{\o}g}, E. and {Katz}, D. and {Lattanzi}, M.~G. and {O'Mullane}, W. and {Grebel}, E.~K. and {Holland}, A.~D. and {Huc}, C. and {Passot}, X. and {Bramante}, L. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Hern{\'a}ndez}, J. and {Jean-Antoine-Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Panuzzo}, P. and {Portell}, J. and {Richards}, P.~J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Torra}, J. and {Els}, S.~G. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Lock}, T. and {Mercier}, E. and {Altmann}, M. and {Andrae}, R. and {Astraatmadja}, T.~L. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Cowell}, S. and {Creevey}, O. and {Cuypers}, J. and {Davidson}, M. and {De Ridder}, J. and {de Torres}, A. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fr{\'e}mat}, Y. and {Garc{\'\i}a-Torres}, M. and {Gosset}, E. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hauser}, M. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Huckle}, H.~E. and {Hutton}, A. and {Jasniewicz}, G. and {Jordan}, S. and {Kontizas}, M. and {Korn}, A.~J. and {Lanzafame}, A.~C. and {Manteiga}, M. and {Moitinho}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Smith}, K.~W. and {Sozzetti}, A. and {Thuillot}, W. and {van Reeven}, W. and {Viala}, Y. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aguado}, J.~J. and {Allan}, P.~M. and {Allasia}, W. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Ant{\'o}n}, S. and {Arcay}, B. and {Atzei}, A. and {Ayache}, L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Barache}, C. and {Barata}, C. and {Barbier}, A. and {Barblan}, F. and {Baroni}, M. and {Barrado y Navascu{\'e}s}, D. and {Barros}, M. and {Barstow}, M.~A. and {Becciani}, U. and {Bellazzini}, M. and {Bellei}, G. and {Bello Garc{\'\i}a}, A. and {Belokurov}, V. and {Bendjoya}, P. and {Berihuete}, A. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Billebaud}, F. and {Blagorodnova}, N. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bouy}, H. and {Bragaglia}, A. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Bucciarelli}, B. and {Budnik}, F. and {Burgess}, P. and {Burgon}, R. and {Burlacu}, A. and {Busonero}, D. and {Buzzi}, R. and {Caffau}, E. and {Cambras}, J. and {Campbell}, H. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carlucci}, T. and {Carrasco}, J.~M. and {Castellani}, M. and {Charlot}, P. and {Charnas}, J. and {Charvet}, P. and {Chassat}, F. and {Chiavassa}, A. and {Clotet}, M. and {Cocozza}, G. and {Collins}, R.~S. and {Collins}, P. and {Costigan}, G. and {Crifo}, F. and {Cross}, N.~J.~G. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {De Cat}, P. and {de Felice}, F. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {di Marco}, F. and {Di Matteo}, P. and {Diakite}, S. and {Distefano}, E. and {Dolding}, C. and {Dos Anjos}, S. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Dzigan}, Y. and {Ecale}, E. and {Edvardsson}, B. and {Enke}, H. and {Erdmann}, M. and {Escolar}, D. and {Espina}, M. and {Evans}, N.~W. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Faye}, F. and {Federici}, L. and {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fouesneau}, M. and {Fraile}, E. and {Fraser}, M. and {Fuchs}, J. and {Furnell}, R. and {Gai}, M. and {Galleti}, S. and {Galluccio}, L. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Gar{\'e}}, P. and {Garofalo}, A. and {Garralda}, N. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guerrier}, A. and {Guillout}, P. and {Guiraud}, J. and {G{\'u}rpide}, A. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Haigron}, R. and {Hatzidimitriou}, D. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Hobbs}, D. and {Hofmann}, W. and {Holl}, B. and {Holland}, G. and {Hunt}, J.~A.~S. and {Hypki}, A. and {Icardi}, V. and {Irwin}, M. and {Jevardat de Fombelle}, G. and {Jofr{\'e}}, P. and {Jonker}, P.~G. and {Jorissen}, A. and {Julbe}, F. and {Karampelas}, A. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Koubsky}, P. and {Kowalczyk}, A. and {Krone-Martins}, A. and {Kudryashova}, M. and {Kull}, I. and {Bachchan}, R.~K. and {Lacoste-Seris}, F. and {Lanza}, A.~F. and {Lavigne}, J. -B. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lemaitre}, V. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\"o}ffler}, W. and {L{\'o}pez}, M. and {Lopez-Lozano}, A. and {Lorenz}, D. and {Loureiro}, T. and {MacDonald}, I. and {Magalh{\~a}es Fernandes}, T. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marie}, J. and {Marinoni}, S. and {Marrese}, P.~M. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Mart{\'\i}n-Fleitas}, J.~M. and {Martino}, M. and {Mary}, N. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Mestre}, A. and {Michalik}, D. and {Millar}, N.~R. and {Miranda}, B.~M.~H. and {Molina}, D. and {Molinaro}, R. and {Molinaro}, M. and {Moln{\'a}r}, L. and {Moniez}, M. and {Montegriffo}, P. and {Monteiro}, D. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morley}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Narbonne}, J. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {Ord{\'e}novic}, C. and {Ordieres-Mer{\'e}}, J. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Parsons}, P. and {Paulsen}, T. and {Pecoraro}, M. and {Pedrosa}, R. and {Pentik{\"a}inen}, H. and {Pereira}, J. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Ragaini}, S. and {Rago}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Ranalli}, P. and {Rauw}, G. and {Read}, A. and {Regibo}, S. and {Renk}, F. and {Reyl{\'e}}, C. and {Ribeiro}, R.~A. and {Rimoldini}, L. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rudolph}, A. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sarasso}, M. and {Savietto}, H. and {Schnorhk}, A. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {Segransan}, D. and {Serpell}, E. and {Shih}, I. -C. and {Smareglia}, R. and {Smart}, R.~L. and {Smith}, C. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Tingley}, B. and {Trager}, S.~C. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Valentini}, G. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Varadi}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Via}, T. and {Vicente}, D. and {Vogt}, S. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Weingrill}, K. and {Werner}, D. and {Wevers}, T. and {Whitehead}, G. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T. and {Alecu}, A. and {Allen}, M. and {Allende Prieto}, C. and {Amorim}, A. and {Anglada-Escud{\'e}}, G. and {Arsenijevic}, V. and {Azaz}, S. and {Balm}, P. and {Beck}, M. and {Bernstein}, H. -H. and {Bigot}, L. and {Bijaoui}, A. and {Blasco}, C. and {Bonfigli}, M. and {Bono}, G. and {Boudreault}, S. and {Bressan}, A. and {Brown}, S. and {Brunet}, P. -M. and {Bunclark}, P. and {Buonanno}, R. and {Butkevich}, A.~G. and {Carret}, C. and {Carrion}, C. and {Chemin}, L. and {Ch{\'e}reau}, F. and {Corcione}, L. and {Darmigny}, E. and {de Boer}, K.~S. and {de Teodoro}, P. and {de Zeeuw}, P.~T. and {Delle Luche}, C. and {Domingues}, C.~D. and {Dubath}, P. and {Fodor}, F. and {Fr{\'e}zouls}, B. and {Fries}, A. and {Fustes}, D. and {Fyfe}, D. and {Gallardo}, E. and {Gallegos}, J. and {Gardiol}, D. and {Gebran}, M. and {Gomboc}, A. and {G{\'o}mez}, A. and {Grux}, E. and {Gueguen}, A. and {Heyrovsky}, A. and {Hoar}, J. and {Iannicola}, G. and {Isasi Parache}, Y. and {Janotto}, A. -M. and {Joliet}, E. and {Jonckheere}, A. and {Keil}, R. and {Kim}, D. -W. and {Klagyivik}, P. and {Klar}, J. and {Knude}, J. and {Kochukhov}, O. and {Kolka}, I. and {Kos}, J. and {Kutka}, A. and {Lainey}, V. and {LeBouquin}, D. and {Liu}, C. and {Loreggia}, D. and {Makarov}, V.~V. and {Marseille}, M.~G. and {Martayan}, C. and {Martinez-Rubi}, O. and {Massart}, B. and {Meynadier}, F. and {Mignot}, S. and {Munari}, U. and {Nguyen}, A. -T. and {Nordlander}, T. and {Ocvirk}, P. and {O'Flaherty}, K.~S. and {Olias Sanz}, A. and {Ortiz}, P. and {Osorio}, J. and {Oszkiewicz}, D. and {Ouzounis}, A. and {Palmer}, M. and {Park}, P. and {Pasquato}, E. and {Peltzer}, C. and {Peralta}, J. and {P{\'e}turaud}, F. and {Pieniluoma}, T. and {Pigozzi}, E. and {Poels}, J. and {Prat}, G. and {Prod'homme}, T. and {Raison}, F. and {Rebordao}, J.~M. and {Risquez}, D. and {Rocca-Volmerange}, B. and {Rosen}, S. and {Ruiz-Fuertes}, M.~I. and {Russo}, F. and {Sembay}, S. and {Serraller Vizcaino}, I. and {Short}, A. and {Siebert}, A. and {Silva}, H. and {Sinachopoulos}, D. and {Slezak}, E. and {Soffel}, M. and {Sosnowska}, D. and {Strai{\v{z}}ys}, V. and {ter Linden}, M. and {Terrell}, D. and {Theil}, S. and {Tiede}, C. and {Troisi}, L. and {Tsalmantza}, P. and {Tur}, D. and {Vaccari}, M. and {Vachier}, F. and {Valles}, P. and {Van Hamme}, W. and {Veltz}, L. and {Virtanen}, J. and {Wallut}, J. -M. and {Wichmann}, R. and {Wilkinson}, M.~I. and {Ziaeepour}, H. and {Zschocke}, S.},
        title = "{The Gaia mission}",
      journal = {\aap},
     keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = nov,
       volume = {595},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201629272},
archivePrefix = {arXiv},
       eprint = {1609.04153},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...595A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia2020,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, techniques: radial velocities, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202039657},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ehrenreich2020,
       author = {{Ehrenreich}, David and {Lovis}, Christophe and {Allart}, Romain and {Zapatero Osorio}, Mar{\'\i}a Rosa and {Pepe}, Francesco and {Cristiani}, Stefano and {Rebolo}, Rafael and {Santos}, Nuno C. and {Borsa}, Francesco and {Demangeon}, Olivier and {Dumusque}, Xavier and {Gonz{\'a}lez Hern{\'a}ndez}, Jonay I. and {Casasayas-Barris}, N{\'u}ria and {S{\'e}gransan}, Damien and {Sousa}, S{\'e}rgio and {Abreu}, Manuel and {Adibekyan}, Vardan and {Affolter}, Michael and {Allende Prieto}, Carlos and {Alibert}, Yann and {Aliverti}, Matteo and {Alves}, David and {Amate}, Manuel and {Avila}, Gerardo and {Baldini}, Veronica and {Bandy}, Timothy and {Benz}, Willy and {Bianco}, Andrea and {Bolmont}, {\'E}meline and {Bouchy}, Fran{\c{c}}ois and {Bourrier}, Vincent and {Broeg}, Christopher and {Cabral}, Alexandre and {Calderone}, Giorgio and {Pall{\'e}}, Enric and {Cegla}, H.~M. and {Cirami}, Roberto and {Coelho}, Jo{\~a}o M.~P. and {Conconi}, Paolo and {Coretti}, Igor and {Cumani}, Claudio and {Cupani}, Guido and {Dekker}, Hans and {Delabre}, Bernard and {Deiries}, Sebastian and {D'Odorico}, Valentina and {Di Marcantonio}, Paolo and {Figueira}, Pedro and {Fragoso}, Ana and {Genolet}, Ludovic and {Genoni}, Matteo and {G{\'e}nova Santos}, Ricardo and {Hara}, Nathan and {Hughes}, Ian and {Iwert}, Olaf and {Kerber}, Florian and {Knudstrup}, Jens and {Landoni}, Marco and {Lavie}, Baptiste and {Lizon}, Jean-Louis and {Lendl}, Monika and {Lo Curto}, Gaspare and {Maire}, Charles and {Manescau}, Antonio and {Martins}, C.~J.~A.~P. and {M{\'e}gevand}, Denis and {Mehner}, Andrea and {Micela}, Giusi and {Modigliani}, Andrea and {Molaro}, Paolo and {Monteiro}, Manuel and {Monteiro}, Mario and {Moschetti}, Manuele and {M{\"u}ller}, Eric and {Nunes}, Nelson and {Oggioni}, Luca and {Oliveira}, Ant{\'o}nio and {Pariani}, Giorgio and {Pasquini}, Luca and {Poretti}, Ennio and {Rasilla}, Jos{\'e} Luis and {Redaelli}, Edoardo and {Riva}, Marco and {Santana Tschudi}, Samuel and {Santin}, Paolo and {Santos}, Pedro and {Segovia Milla}, Alex and {Seidel}, Julia V. and {Sosnowska}, Danuta and {Sozzetti}, Alessandro and {Span{\`o}}, Paolo and {Su{\'a}rez Mascare{\~n}o}, Alejandro and {Tabernero}, Hugo and {Tenegi}, Fabio and {Udry}, St{\'e}phane and {Zanutta}, Alessio and {Zerbi}, Filippo},
        title = "{Nightside condensation of iron in an ultrahot giant exoplanet}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = mar,
       volume = {580},
       number = {7805},
        pages = {597-601},
          doi = {10.1038/s41586-020-2107-1},
archivePrefix = {arXiv},
       eprint = {2003.05528},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.580..597E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kesseli2021,
       author = {{Kesseli}, Aurora Y. and {Snellen}, I.~A.~G.},
        title = "{Confirmation of Asymmetric Iron Absorption in WASP-76b with HARPS}",
      journal = {\apjl},
     keywords = {Exoplanet atmospheres, Hot Jupiters, Exoplanet atmospheric composition, 487, 753, 2021, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = feb,
       volume = {908},
       number = {1},
          eid = {L17},
        pages = {L17},
          doi = {10.3847/2041-8213/abe047},
archivePrefix = {arXiv},
       eprint = {2102.01095},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...908L..17K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lothringer2018,
       author = {{Lothringer}, Joshua D. and {Barman}, Travis and {Koskinen}, Tommi},
        title = "{Extremely Irradiated Hot Jupiters: Non-oxide Inversions, H$^{-}$ Opacity, and Thermal Dissociation of Molecules}",
      journal = {\apj},
     keywords = {methods: numerical, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = oct,
       volume = {866},
       number = {1},
          eid = {27},
        pages = {27},
          doi = {10.3847/1538-4357/aadd9e},
archivePrefix = {arXiv},
       eprint = {1805.00038},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...866...27L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Kirk2019,
	doi = {10.3847/1538-3881/ab397d},
	url = {https://doi.org/10.3847/1538-3881/ab397d},
	year = 2019,
	month = {sep},
	publisher = {American Astronomical Society},
	volume = {158},
	number = {4},
	pages = {144},
	author = {James Kirk and Mercedes L{\'{o}}pez-Morales and Peter J. Wheatley and Ian C. Weaver and Ian Skillen and Tom Louden and James McCormac and N{\'{e}}stor Espinoza},
	title = {{LRG}-{BEASTS}: Transmission Spectroscopy and Retrieval Analysis of the Highly Inflated Saturn-mass Planet {WASP}-39b},
	journal = {The Astronomical Journal},
	abstract = {We present a ground-based transmission spectrum and comprehensive retrieval analysis of the highly inflated Saturn-mass planet WASP-39b. We obtained low-resolution spectra (R ≈ 400) of a transit of WASP-39b using the ACAM instrument on the 4.2 m William Herschel Telescope as part of the LRG-BEASTS survey. Our transmission spectrum is in good agreement with previous ground- and space-based observations of WASP-39b, and covers a wavelength range of 4000–9000 Å. Previous analyses of this exoplanet have retrieved water abundances that span more than four orders of magnitude, which in turn lead to conclusions of a subsolar or highly supersolar atmospheric metallicity. In order to determine the cause of the large discrepancies in the literature regarding WASP-39b’s atmospheric metallicity, we performed retrieval analyses of all literature data sets. Our retrievals, which assume equilibrium chemistry, recovered highly supersolar metallicities for all data sets. When running our retrievals on a combined spectrum, spanning 0.3–5 μm, we recovered an atmospheric metallicity of × solar. We find that stellar activity has a negligible effect on the derived abundances and instead conclude that different assumptions made during retrieval analyses lead to the reported water abundances that differ by orders of magnitude. This in turn has significant consequences for the conclusions we draw. This is the fourth planet to be observed as part of the LRG-BEASTS survey, which is demonstrating that 4 m class telescopes can obtain low-resolution transmission spectra with precisions of around one atmospheric scale height.}
}

@ARTICLE{Mansfield2020,
       author = {{Mansfield}, Megan and {Bean}, Jacob L. and {Stevenson}, Kevin B. and {Komacek}, Thaddeus D. and {Bell}, Taylor J. and {Tan}, Xianyu and {Malik}, Matej and {Beatty}, Thomas G. and {Wong}, Ian and {Cowan}, Nicolas B. and {Dang}, Lisa and {D{\'e}sert}, Jean-Michel and {Fortney}, Jonathan J. and {Gaudi}, B. Scott and {Keating}, Dylan and {Kempton}, Eliza M. -R. and {Kreidberg}, Laura and {Line}, Michael R. and {Parmentier}, Vivien and {Stassun}, Keivan G. and {Swain}, Mark R. and {Zellem}, Robert T.},
        title = "{Evidence for H2 Dissociation and Recombination Heat Transport in the Atmosphere of KELT-9b}",
      journal = {\apjl},
     keywords = {Hot Jupiters, Exoplanet atmospheres, 753, 487, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {L15},
        pages = {L15},
          doi = {10.3847/2041-8213/ab5b09},
archivePrefix = {arXiv},
       eprint = {1910.01567},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888L..15M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek2020,
       author = {{Komacek}, Thaddeus D. and {Showman}, Adam P.},
        title = "{Temporal Variability in Hot Jupiter Atmospheres}",
      journal = {\apj},
     keywords = {Hydrodynamics, Computational methods, Exoplanets, Exoplanet atmospheres, Exoplanet atmospheric variability, 1963, 1965, 498, 487, 2020, Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2020,
        month = jan,
       volume = {888},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/1538-4357/ab5b0b},
archivePrefix = {arXiv},
       eprint = {1910.09523},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888....2K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rogers2014,
       author = {{Rogers}, T.~M. and {Komacek}, T.~D.},
        title = "{Magnetic Effects in Hot Jupiter Atmospheres}",
      journal = {\apj},
     keywords = {hydrodynamics, magnetohydrodynamics: MHD, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = oct,
       volume = {794},
       number = {2},
          eid = {132},
        pages = {132},
          doi = {10.1088/0004-637X/794/2/132},
archivePrefix = {arXiv},
       eprint = {1409.0519},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...794..132R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rogers2017,
       author = {{Rogers}, T.~M. and {McElwaine}, J.~N.},
        title = "{The Hottest Hot Jupiters May Host Atmospheric Dynamos}",
      journal = {\apjl},
     keywords = {dynamo, magnetohydrodynamics: MHD, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jun,
       volume = {841},
       number = {2},
          eid = {L26},
        pages = {L26},
          doi = {10.3847/2041-8213/aa72da},
archivePrefix = {arXiv},
       eprint = {1704.04197},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...841L..26R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Knutson2007,
       author = {{Knutson}, Heather A. and {Charbonneau}, David and {Allen}, Lori E. and {Fortney}, Jonathan J. and {Agol}, Eric and {Cowan}, Nicolas B. and {Showman}, Adam P. and {Cooper}, Curtis S. and {Megeath}, S. Thomas},
        title = "{A map of the day-night contrast of the extrasolar planet HD 189733b}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2007,
        month = may,
       volume = {447},
       number = {7141},
        pages = {183-186},
          doi = {10.1038/nature05782},
archivePrefix = {arXiv},
       eprint = {0705.0993},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007Natur.447..183K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaudi2007,
       author = {{Gaudi}, B. Scott and {Winn}, Joshua N.},
        title = "{Prospects for the Characterization and Confirmation of Transiting Exoplanets via the Rossiter-McLaughlin Effect}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Rotation, Astrophysics},
         year = 2007,
        month = jan,
       volume = {655},
       number = {1},
        pages = {550-563},
          doi = {10.1086/509910},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608071},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...655..550G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ohta2005,
       author = {{Ohta}, Yasuhiro and {Taruya}, Atsushi and {Suto}, Yasushi},
        title = "{The Rossiter-McLaughlin Effect and Analytic Radial Velocity Curves for Transiting Extrasolar Planetary Systems}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Individual: Henry Draper Number: HD 209458, Techniques: Spectroscopic, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {1118-1135},
          doi = {10.1086/428344},
archivePrefix = {arXiv},
       eprint = {astro-ph/0410499},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622.1118O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Queloz2000,
       author = {{Queloz}, D. and {Eggenberger}, A. and {Mayor}, M. and {Perrier}, C. and {Beuzit}, J.~L. and {Naef}, D. and {Sivan}, J.~P. and {Udry}, S.},
        title = "{Detection of a spectroscopic transit by the planet orbiting the star HD209458}",
      journal = {\aap},
     keywords = {STARS: BINARIES: SPECTROSCOPIC, STARS: BINARIES: ECLIPSING, STARS: INDIVIDUAL: HD209458, STARS: PLANETARY SYSTEMS, Astrophysics},
         year = 2000,
        month = jul,
       volume = {359},
        pages = {L13-L17},
archivePrefix = {arXiv},
       eprint = {astro-ph/0006213},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...359L..13Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Czesla2015,
       author = {{Czesla}, S. and {Klocov{\'a}}, T. and {Khalafinejad}, S. and {Wolter}, U. and {Schmitt}, J.~H.~M.~M.},
        title = "{The center-to-limb variation across the Fraunhofer lines of HD 189733. Sampling the stellar spectrum using a transiting planet}",
      journal = {\aap},
     keywords = {planets and satellites: individual: HD 189733b, planets and satellites: atmospheres, stars: activity, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {582},
          eid = {A51},
        pages = {A51},
          doi = {10.1051/0004-6361/201526386},
archivePrefix = {arXiv},
       eprint = {1509.05657},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..51C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Morley2014,
       author = {{Morley}, Caroline V. and {Marley}, Mark S. and {Fortney}, Jonathan J. and {Lupu}, Roxana and {Saumon}, Didier and {Greene}, Tom and {Lodders}, Katharina},
        title = "{Water Clouds in Y Dwarfs and Exoplanets}",
      journal = {\apj},
     keywords = {brown dwarfs, planets and satellites: atmospheres, planets and satellites: detection, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = may,
       volume = {787},
       number = {1},
          eid = {78},
        pages = {78},
          doi = {10.1088/0004-637X/787/1/78},
archivePrefix = {arXiv},
       eprint = {1404.0005},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...787...78M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Burrows2003,
       author = {{Burrows}, Adam and {Sudarsky}, David and {Lunine}, Jonathan I.},
        title = "{Beyond the T Dwarfs: Theoretical Spectra, Colors, and Detectability of the Coolest Brown Dwarfs}",
      journal = {\apj},
     keywords = {Infrared: Stars, Molecular Processes, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2003,
        month = oct,
       volume = {596},
       number = {1},
        pages = {587-596},
          doi = {10.1086/377709},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304226},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...596..587B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Stenflo2015,
       author = {{Stenflo}, J.~O.},
        title = "{FTS atlas of the Sun's spectrally resolved center-to-limb variation}",
      journal = {\aap},
     keywords = {Sun: atmosphere, atlases, line: profiles, techniques: spectroscopic, radiative transfer, polarization, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jan,
       volume = {573},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201424685},
archivePrefix = {arXiv},
       eprint = {1410.8474},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..74S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tang2021,
       author = {{Tang}, Shih-Yun and {Robinson}, Tyler D. and {Marley}, Mark S. and {Batalha}, Natasha E. and {Lupu}, Roxana and {Prato}, L.},
        title = "{Impact of Water-latent Heat on the Thermal Structure of Ultra-cool Objects: Brown Dwarfs and Free-floating Planets}",
      journal = {\apj},
     keywords = {Brown dwarfs, Y dwarfs, Exoplanet atmospheres, Planetary atmospheres, Exoplanet structure, 185, 1827, 487, 1244, 495, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = nov,
       volume = {922},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/ac1e90},
archivePrefix = {arXiv},
       eprint = {2105.07000},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...922...26T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Fossati2021,
       author = {{Fossati}, L. and {Young}, M.~E. and {Shulyak}, D. and {Koskinen}, T. and {Huang}, C. and {Cubillos}, P.~E. and {France}, K. and {Sreejith}, A.~G.},
        title = "{Non-local thermodynamic equilibrium effects determine the upper atmospheric temperature structure of the ultra-hot Jupiter KELT-9b}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jun,
          eid = {arXiv:2106.11263},
        pages = {arXiv:2106.11263},
archivePrefix = {arXiv},
       eprint = {2106.11263},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210611263F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lefevre2022,
       author = {{Lef{\`e}vre}, Maxence and {Tan}, Xianyu and {Lee}, Elspeth K.~H. and {Pierrehumbert}, R.~T.},
        title = "{Cloud-convection feedback in brown dwarfs atmosphere}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = mar,
          eid = {arXiv:2203.08625},
        pages = {arXiv:2203.08625},
archivePrefix = {arXiv},
       eprint = {2203.08625},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220308625L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Wang2017a,
       author = {{Wang}, Ji and {Prato}, Lisa and {Mawet}, Dimitri},
        title = "{Time-resolved High Spectral Resolution Observation of 2MASSW J0746425+200032AB}",
      journal = {\apj},
     keywords = {binaries: spectroscopic, brown dwarfs, infrared: stars, methods: observational, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {838},
       number = {1},
          eid = {35},
        pages = {35},
          doi = {10.3847/1538-4357/aa6345},
archivePrefix = {arXiv},
       eprint = {1702.07769},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...838...35W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rossiter1924,
       author = {{Rossiter}, R.~A.},
        title = "{On the detection of an effect of rotation during eclipse in the velocity of the brigher component of beta Lyrae, and on the constancy of velocity of this system.}",
      journal = {\apj},
         year = 1924,
        month = jul,
       volume = {60},
        pages = {15-21},
          doi = {10.1086/142825},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ApJ....60...15R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McLaughlin1924,
       author = {{McLaughlin}, D.~B.},
        title = "{Some results of a spectrographic study of the Algol system.}",
      journal = {\apj},
         year = 1924,
        month = jul,
       volume = {60},
        pages = {22-31},
          doi = {10.1086/142826},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1924ApJ....60...22M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stevens2018,
       author = {{Stevens}, Daniel J. and {Gaudi}, B. Scott and {Stassun}, Keivan G.},
        title = "{Measuring Model-independent Masses and Radii of Single-lined Eclipsing Binaries: Analytic Precision Estimates}",
      journal = {\apj},
     keywords = {binaries: eclipsing, methods: analytical, planetary systems, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = jul,
       volume = {862},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.3847/1538-4357/aaccf5},
archivePrefix = {arXiv},
       eprint = {1712.05046},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...862...53S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Popper1980,
       author = {{Popper}, D.~M.},
        title = "{Stellar masses.}",
      journal = {\araa},
     keywords = {Astronomical Catalogs, Eclipsing Binary Stars, Stellar Mass, Stellar Spectra, B Stars, Giant Stars, Main Sequence Stars, O Stars, Astrophysics},
         year = 1980,
        month = jan,
       volume = {18},
        pages = {115-164},
          doi = {10.1146/annurev.aa.18.090180.000555},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980ARA&A..18..115P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harmanec1988,
       author = {{Harmanec}, Petr},
        title = "{Stellar Masses and Radii Based on Modern Binary Data}",
      journal = {Bulletin of the Astronomical Institutes of Czechoslovakia},
     keywords = {Early Stars, Eclipsing Binary Stars, Stellar Mass, Stellar Rotation, B Stars, Light Curve, Main Sequence Stars, Stellar Magnitude, Stellar Spectra, Stellar Temperature, Astrophysics},
         year = 1988,
        month = dec,
       volume = {39},
        pages = {329},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988BAICz..39..329H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andersen1991,
       author = {{Andersen}, J.},
        title = "{Accurate masses and radii of normal stars}",
      journal = {\aapr},
     keywords = {Eclipsing Binary Stars, Stellar Mass, Stellar Spectrophotometry, Stellar Structure, Abundance, Stellar Evolution, Stellar Models, Stellar Physics, Astrophysics, Stars: binaries: general, stars: diameters of, stars: evolution of, stars: luminosities of, stars: mass of, stars: structure of},
         year = 1991,
        month = jan,
       volume = {3},
       number = {2},
        pages = {91-126},
          doi = {10.1007/BF00873538},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991A&ARv...3...91A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{PaiAsnodkar2021,
       author = {{Pai Asnodkar}, Anusha and {Wang}, Ji and {Gaudi}, B. Scott and {Cauley}, P. Wilson and {Eastman}, Jason D. and {Ilyin}, Ilya and {Strassmeier}, Klaus and {Beatty}, Thomas},
        title = "{KELT-9 as an Eclipsing Double-lined Spectroscopic Binary: A Unique and Self-consistent Solution to the System}",
      journal = {\aj},
     keywords = {486, 487, 498, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = feb,
       volume = {163},
       number = {2},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-3881/ac32c7},
archivePrefix = {arXiv},
       eprint = {2110.15275},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....163...40P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Perna2010,
       author = {{Perna}, Rosalba and {Menou}, Kristen and {Rauscher}, Emily},
        title = "{Magnetic Drag on Hot Jupiter Atmospheric Winds}",
      journal = {\apj},
     keywords = {planets and satellites: atmospheres, planets and satellites: individual: HD 209458b, planets and satellites: magnetic fields, Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = aug,
       volume = {719},
       number = {2},
        pages = {1421-1426},
          doi = {10.1088/0004-637X/719/2/1421},
archivePrefix = {arXiv},
       eprint = {1003.3838},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...719.1421P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Savel2021,
       author = {{Savel}, Arjun B. and {Kempton}, Eliza M. -R. and {Malik}, Matej and {Komacek}, Thaddeus D. and {Bean}, Jacob L. and {May}, Erin M. and {Stevenson}, Kevin B. and {Mansfield}, Megan and {Rauscher}, Emily},
        title = "{No umbrella needed: Confronting the hypothesis of iron rain on WASP-76b with post-processed general circulation models}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = aug,
          eid = {arXiv:2109.00163},
        pages = {arXiv:2109.00163},
archivePrefix = {arXiv},
       eprint = {2109.00163},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210900163S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@unpublished{WangInPrep,
author  = "{Wang}, Ji and {Stephan}, Alexander",
title = "Nodal precession of KELT-9 b",
year = {in prep.}
}

@ARTICLE{Flowers2019,
       author = {{Flowers}, Erin and {Brogi}, Matteo and {Rauscher}, Emily and {Kempton}, Eliza M. -R. and {Chiavassa}, Andrea},
        title = "{The High-resolution Transmission Spectrum of HD 189733b Interpreted with Atmospheric Doppler Shifts from Three-dimensional General Circulation Models}",
      journal = {\aj},
     keywords = {hydrodynamics, planets and satellites: atmospheres, planets and satellites: gaseous planets, radiative transfer, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = may,
       volume = {157},
       number = {5},
          eid = {209},
        pages = {209},
          doi = {10.3847/1538-3881/ab164c},
archivePrefix = {arXiv},
       eprint = {1810.06099},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..209F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cauley2021,
       author = {{Cauley}, P. Wilson and {Wang}, Ji and {Shkolnik}, Evgenya L. and {Ilyin}, Ilya and {Strassmeier}, Klaus G. and {Redfield}, Seth and {Jensen}, Adam G.},
        title = "{Time-resolved Rotational Velocities in the Upper Atmosphere of WASP-33 b}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanets, Hot Jupiters, 487, 498, 753, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = mar,
       volume = {161},
       number = {3},
          eid = {152},
        pages = {152},
          doi = {10.3847/1538-3881/abde43},
archivePrefix = {arXiv},
       eprint = {2010.02118},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..152C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek2016,
       author = {{Komacek}, Thaddeus D. and {Showman}, Adam P.},
        title = "{Atmospheric Circulation of Hot Jupiters: Dayside-Nightside Temperature Differences}",
      journal = {\apj},
     keywords = {hydrodynamics, methods: analytical, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = apr,
       volume = {821},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.3847/0004-637X/821/1/16},
archivePrefix = {arXiv},
       eprint = {1601.00069},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...821...16K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rauscher2013,
       author = {{Rauscher}, Emily and {Menou}, Kristen},
        title = "{Three-dimensional Atmospheric Circulation Models of HD 189733b and HD 209458b with Consistent Magnetic Drag and Ohmic Dissipation}",
      journal = {\apj},
     keywords = {hydrodynamics, magnetic fields, methods: numerical, planets and satellites: individual: HD 189733b HD 209458b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2013,
        month = feb,
       volume = {764},
       number = {1},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/764/1/103},
archivePrefix = {arXiv},
       eprint = {1208.2274},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...764..103R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Beltz2021b,
       author = {{Beltz}, Hayley and {Rauscher}, Emily and {Roman}, Michael and {Guilliat}, Abigail},
        title = "{Exploring the Effects of Active Magnetic Drag in a GCM of the Ultra-Hot Jupiter WASP-76b}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.13371},
        pages = {arXiv:2109.13371},
archivePrefix = {arXiv},
       eprint = {2109.13371},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210913371B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lothringer2019,
       author = {{Lothringer}, Joshua D. and {Barman}, Travis},
        title = "{The Influence of Host Star Spectral Type on Ultra-hot Jupiter Atmospheres}",
      journal = {\apj},
     keywords = {methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = may,
       volume = {876},
       number = {1},
          eid = {69},
        pages = {69},
          doi = {10.3847/1538-4357/ab1485},
archivePrefix = {arXiv},
       eprint = {1903.12183},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...876...69L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{TESS2015,
       author = {{Ricker}, George R. and {Winn}, Joshua N. and {Vanderspek}, Roland and {Latham}, David W. and {Bakos}, G{\'a}sp{\'a}r {\'A}. and {Bean}, Jacob L. and {Berta-Thompson}, Zachory K. and {Brown}, Timothy M. and {Buchhave}, Lars and {Butler}, Nathaniel R. and {Butler}, R. Paul and {Chaplin}, William J. and {Charbonneau}, David and {Christensen-Dalsgaard}, J{\o}rgen and {Clampin}, Mark and {Deming}, Drake and {Doty}, John and {De Lee}, Nathan and {Dressing}, Courtney and {Dunham}, Edward W. and {Endl}, Michael and {Fressin}, Francois and {Ge}, Jian and {Henning}, Thomas and {Holman}, Matthew J. and {Howard}, Andrew W. and {Ida}, Shigeru and {Jenkins}, Jon M. and {Jernigan}, Garrett and {Johnson}, John Asher and {Kaltenegger}, Lisa and {Kawai}, Nobuyuki and {Kjeldsen}, Hans and {Laughlin}, Gregory and {Levine}, Alan M. and {Lin}, Douglas and {Lissauer}, Jack J. and {MacQueen}, Phillip and {Marcy}, Geoffrey and {McCullough}, Peter R. and {Morton}, Timothy D. and {Narita}, Norio and {Paegert}, Martin and {Palle}, Enric and {Pepe}, Francesco and {Pepper}, Joshua and {Quirrenbach}, Andreas and {Rinehart}, Stephen A. and {Sasselov}, Dimitar and {Sato}, Bun'ei and {Seager}, Sara and {Sozzetti}, Alessandro and {Stassun}, Keivan G. and {Sullivan}, Peter and {Szentgyorgyi}, Andrew and {Torres}, Guillermo and {Udry}, Stephane and {Villasenor}, Joel},
        title = "{Transiting Exoplanet Survey Satellite (TESS)}",
      journal = {Journal of Astronomical Telescopes, Instruments, and Systems},
         year = 2015,
        month = jan,
       volume = {1},
          eid = {014003},
        pages = {014003},
          doi = {10.1117/1.JATIS.1.1.014003},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015JATIS...1a4003R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Ambikasaran2014,
author = {{Ambikasaran}, S. and {Foreman-Mackey}, D. and
{Greengard}, L. and {Hogg}, D.~W. and {O'Neil}, M.},
title = "{Fast Direct Methods for Gaussian Processes}",
year = 2014,
month = mar,
url = http://arxiv.org/abs/1403.6015
}

@ARTICLE{Charbonneau2005,
       author = {{Charbonneau}, David and {Allen}, Lori E. and {Megeath}, S. Thomas and {Torres}, Guillermo and {Alonso}, Roi and {Brown}, Timothy M. and {Gilliland}, Ronald L. and {Latham}, David W. and {Mandushev}, Georgi and {O'Donovan}, Francis T. and {Sozzetti}, Alessandro},
        title = "{Detection of Thermal Emission from an Extrasolar Planet}",
      journal = {\apj},
     keywords = {Stars: Binaries: Eclipsing, Infrared: Stars, Stars: Planetary Systems, Stars: Individual: Alphanumeric: TrES-1, Techniques: Photometric, Astrophysics},
         year = 2005,
        month = jun,
       volume = {626},
       number = {1},
        pages = {523-529},
          doi = {10.1086/429991},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503457},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...626..523C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hindle2021,
       author = {{Hindle}, A.~W. and {Bushby}, P.~J. and {Rogers}, T.~M.},
        title = "{Observational Consequences of Shallow-water Magnetohydrodynamics on Hot Jupiters}",
      journal = {\apjl},
     keywords = {Magnetohydrodynamics, Astrophysical fluid dynamics, Hot Jupiters, Exoplanet dynamics, Exoplanet atmospheres, Exoplanet atmospheric variability, 1964, 101, 753, 490, 487, 2020, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jul,
       volume = {916},
       number = {1},
          eid = {L8},
        pages = {L8},
          doi = {10.3847/2041-8213/ac0fec},
archivePrefix = {arXiv},
       eprint = {2107.10848},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...916L...8H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fromang2016,
       author = {{Fromang}, S{\'e}bastien and {Leconte}, Jeremy and {Heng}, Kevin},
        title = "{Shear-driven instabilities and shocks in the atmospheres of hot Jupiters}",
      journal = {\aap},
     keywords = {hydrodynamics, instabilities, shock waves, methods: numerical, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = jul,
       volume = {591},
          eid = {A144},
        pages = {A144},
          doi = {10.1051/0004-6361/201527600},
archivePrefix = {arXiv},
       eprint = {1603.02794},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...591A.144F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Menou2020,
       author = {{Menou}, Kristen},
        title = "{Hot Jupiter atmospheric flows at high resolution}",
      journal = {\mnras},
     keywords = {astrochemistry, diffusion, hydrodynamics, radiative transfer, turbulence, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics},
         year = 2020,
        month = apr,
       volume = {493},
       number = {4},
        pages = {5038-5044},
          doi = {10.1093/mnras/staa532},
archivePrefix = {arXiv},
       eprint = {1911.00084},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.5038M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wardenier2021,
       author = {{Wardenier}, Joost P. and {Parmentier}, Vivien and {Lee}, Elspeth K.~H. and {Line}, Michael R. and {Gharib-Nezhad}, Ehsan},
        title = "{Decomposing the iron cross-correlation signal of the ultra-hot Jupiter WASP-76b in transmission using 3D Monte Carlo radiative transfer}",
      journal = {\mnras},
     keywords = {radiative transfer, methods: numerical, planets and satellites: individual: WASP-76b, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
       volume = {506},
       number = {1},
        pages = {1258-1283},
          doi = {10.1093/mnras/stab1797},
archivePrefix = {arXiv},
       eprint = {2105.11034},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.506.1258W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2020,
       author = {{Showman}, Adam P. and {Tan}, Xianyu and {Parmentier}, Vivien},
        title = "{Atmospheric Dynamics of Hot Giant Planets and Brown Dwarfs}",
      journal = {\ssr},
     keywords = {Exoplanets, Giant planets, Hot Jupiters, Jupiter, Saturn, Brown dwarfs, Atmospheric dynamics, Turbulence, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {216},
       number = {8},
          eid = {139},
        pages = {139},
          doi = {10.1007/s11214-020-00758-8},
archivePrefix = {arXiv},
       eprint = {2007.15363},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SSRv..216..139S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993JAnSc..41..439S,
       author = {{Shuster}, Malcolm D.},
        title = "{Survey of attitude representations}",
      journal = {Journal of the Astronautical Sciences},
     keywords = {Attitude Control, Flight Mechanics, Kinematic Equations, Satellite Orientation, Satellite Rotation, Covariance, Errors, Kinematics, Transformations (Mathematics), Astronautics (General)},
         year = 1993,
        month = oct,
       volume = {41},
       number = {4},
        pages = {439-517},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993JAnSc..41..439S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993JGCD...16..393S,
       author = {{Shuster}, Malcolm D.},
        title = "{Attitude determination in higher dimensions}",
      journal = {Journal of Guidance Control Dynamics},
     keywords = {Attitude Control, Matrices (Mathematics), Algorithms, Three Dimensional Models, Space Communications, Spacecraft Communications, Command and Tracking},
         year = 1993,
        month = apr,
       volume = {16},
       number = {2},
        pages = {393-395},
          doi = {10.2514/3.21018},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993JGCD...16..393S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993fmet.symp..259S,
       author = {{Shuster}, Malcolm D.},
        title = "{Attitude analysis in Flatland: The plane truth}",
     keywords = {Attitude (Inclination), Euclidean Geometry, Orbit Calculation, Quaternions, Attitude Indicators, Satellite Attitude Control, Two Dimensional Models, Astrodynamics},
    booktitle = {Flight Mechanics/Estimation Theory Symposium},
         year = 1993,
        month = feb,
        pages = {259-274},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993fmet.symp..259S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley&Ackerman2001,
       author = {{Marley}, M.~S. and {Ackerman}, A.~S.},
        title = "{The Role of Clouds in Brown Dwarf and Extrasolar Giant Planet Atmospheres}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = 2001,
        month = mar,
          eid = {astro-ph/0103269},
        pages = {astro-ph/0103269},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103269},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001astro.ph..3269M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremblin2016,
       author = {{Tremblin}, P. and {Amundsen}, D.~S. and {Chabrier}, G. and {Baraffe}, I. and {Drummond}, B. and {Hinkley}, S. and {Mourier}, P. and {Venot}, O.},
        title = "{Cloudless Atmospheres for L/T Dwarfs and Extrasolar Giant Planets}",
      journal = {\apjl},
     keywords = {brown dwarfs, methods: numerical, methods: observational, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = feb,
       volume = {817},
       number = {2},
          eid = {L19},
        pages = {L19},
          doi = {10.3847/2041-8205/817/2/L19},
archivePrefix = {arXiv},
       eprint = {1601.03652},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817L..19T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burgasser2002,
       author = {{Burgasser}, Adam J. and {Marley}, Mark S. and {Ackerman}, Andrew S. and {Saumon}, Didier and {Lodders}, Katharina and {Dahn}, Conard C. and {Harris}, Hugh C. and {Kirkpatrick}, J. Davy},
        title = "{Evidence of Cloud Disruption in the L/T Dwarf Transition}",
      journal = {\apjl},
     keywords = {Infrared: Stars, Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: SDSS J1254-0122, Stars: Individual: Alphanumeric: 2MASS J0559-1404, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2002,
        month = jun,
       volume = {571},
       number = {2},
        pages = {L151-L154},
          doi = {10.1086/341343},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205051},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...571L.151B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Girardin2013,
       author = {{Girardin}, F. and {Artigau}, {\'E}. and {Doyon}, R.},
        title = "{In Search of Dust Clouds: Photometric Monitoring of a Sample of Late L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: SDSS J105213.51+442255.7 SDSSp J125453.90{\textendash}012247.4, stars: low-mass, stars: variables: general, techniques: photometric},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/767/1/61},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767...61G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Marley2021,
       author = {{Marley}, Mark S. and {Saumon}, Didier and {Visscher}, Channon and {Lupu}, Roxana and {Freedman}, Richard and {Morley}, Caroline and {Fortney}, Jonathan J. and {Seay}, Christopher and {Smith}, Adam J.~R.~W. and {Teal}, D.~J. and {Wang}, Ruoyan},
        title = "{The Sonora Brown Dwarf Atmosphere and Evolution Models. I. Model Description and Application to Cloudless Atmospheres in Rainout Chemical Equilibrium}",
      journal = {\apj},
     keywords = {Brown dwarfs, T dwarfs, L dwarfs, L subdwarfs, T subdwarfs, Y dwarfs, Stellar atmospheres, 185, 1679, 894, 896, 1680, 1827, 1584, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {85},
        pages = {85},
          doi = {10.3847/1538-4357/ac141d},
archivePrefix = {arXiv},
       eprint = {2107.07434},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920...85M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chabrier2000,
       author = {{Chabrier}, G. and {Baraffe}, I. and {Allard}, F. and {Hauschildt}, P.},
        title = "{Evolutionary Models for Very Low-Mass Stars and Brown Dwarfs with Dusty Atmospheres}",
      journal = {\apj},
     keywords = {Hertzsprung-Russell, Stars: Evolution, Stars: Low-Mass, Brown Dwarfs, Stars: Luminosity Function, Mass Function, Astrophysics},
         year = 2000,
        month = oct,
       volume = {542},
       number = {1},
        pages = {464-472},
          doi = {10.1086/309513},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005557},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...542..464C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dupuy2017,
       author = {{Dupuy}, Trent J. and {Liu}, Michael C.},
        title = "{Individual Dynamical Masses of Ultracool Dwarfs}",
      journal = {\apjs},
     keywords = {astrometry, binaries: close, brown dwarfs, fundamental parameters, parallaxes, stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = aug,
       volume = {231},
       number = {2},
          eid = {15},
        pages = {15},
          doi = {10.3847/1538-4365/aa5e4c},
archivePrefix = {arXiv},
       eprint = {1703.05775},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJS..231...15D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows2006,
       author = {{Burrows}, Adam and {Sudarsky}, David and {Hubeny}, Ivan},
        title = "{L and T Dwarf Models and the L to T Transition}",
      journal = {\apj},
     keywords = {Infrared: Stars, Molecular Processes, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = apr,
       volume = {640},
       number = {2},
        pages = {1063-1077},
          doi = {10.1086/500293},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509066},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...640.1063B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kirkpatrick2005,
       author = {{Kirkpatrick}, J. Davy},
        title = "{New Spectral Types L and T}",
      journal = {\araa},
         year = 2005,
        month = sep,
       volume = {43},
       number = {1},
        pages = {195-245},
          doi = {10.1146/annurev.astro.42.053102.134017},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ARA&A..43..195K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cushing2008,
       author = {{Cushing}, Michael C. and {Marley}, Mark S. and {Saumon}, D. and {Kelly}, Brandon C. and {Vacca}, William D. and {Rayner}, John T. and {Freedman}, Richard S. and {Lodders}, Katharina and {Roellig}, Thomas L.},
        title = "{Atmospheric Parameters of Field L and T Dwarfs}",
      journal = {\apj},
     keywords = {infrared: stars, radiative transfer, stars: fundamental parameters, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = may,
       volume = {678},
       number = {2},
        pages = {1372-1395},
          doi = {10.1086/526489},
archivePrefix = {arXiv},
       eprint = {0711.0801},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...678.1372C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Tsuji1996,
       author = {{Tsuji}, T. and {Ohnaka}, K. and {Aoki}, W. and {Nakajima}, T.},
        title = "{Evolution of dusty photospheres through red to brown dwarfs: how dust forms in very low mass objects.}",
      journal = {\aap},
     keywords = {EQUATION OF STATE, MOLECULAR PROCESSES, STARS: ATMOSPHERES, STARS: FUNDAMENTAL PARAMETERS, STARS: LATE-TYPE, STARS: LOW-MASS, BROWN DWARFS},
         year = 1996,
        month = apr,
       volume = {308},
        pages = {L29-L32},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...308L..29T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows2006,
       author = {{Burrows}, Adam and {Sudarsky}, David and {Hubeny}, Ivan},
        title = "{L and T Dwarf Models and the L to T Transition}",
      journal = {\apj},
     keywords = {Infrared: Stars, Molecular Processes, Radiative Transfer, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = apr,
       volume = {640},
       number = {2},
        pages = {1063-1077},
          doi = {10.1086/500293},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509066},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...640.1063B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Reimers2008,
       author = {{Reiners}, A. and {Basri}, G.},
        title = "{Chromospheric Activity, Rotation, and Rotational Braking in M and L Dwarfs}",
      journal = {\apj},
     keywords = {stars: activity, stars: flare, stars: late-type, stars: low-mass, brown dwarfs, stars: rotation, Astrophysics},
         year = 2008,
        month = sep,
       volume = {684},
       number = {2},
        pages = {1390-1403},
          doi = {10.1086/590073},
archivePrefix = {arXiv},
       eprint = {0805.1059},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...684.1390R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Enoch2003,
       author = {{Enoch}, Melissa L. and {Brown}, Michael E. and {Burgasser}, Adam J.},
        title = "{Photometric Variability at the L/T Dwarf Boundary}",
      journal = {\aj},
     keywords = {stars: individual (2MASSW J0030300-145033), stars: individual (SDSSp J015141.69+124429.6), Stars: Low-Mass, Brown Dwarfs, Stars: Variables: Other, Astrophysics},
         year = 2003,
        month = aug,
       volume = {126},
       number = {2},
        pages = {1006-1016},
          doi = {10.1086/376598},
archivePrefix = {arXiv},
       eprint = {astro-ph/0305048},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003AJ....126.1006E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Girardin2013,
       author = {{Girardin}, F. and {Artigau}, {\'E}. and {Doyon}, R.},
        title = "{In Search of Dust Clouds: Photometric Monitoring of a Sample of Late L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: individual: SDSS J105213.51+442255.7 SDSSp J125453.90{\textendash}012247.4, stars: low-mass, stars: variables: general, techniques: photometric},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/767/1/61},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767...61G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Metchev2015,
       author = {{Metchev}, Stanimir A. and {Heinze}, Aren and {Apai}, D{\'a}niel and {Flateau}, Davin and {Radigan}, Jacqueline and {Burgasser}, Adam and {Marley}, Mark S. and {Artigau}, {\'E}tienne and {Plavchan}, Peter and {Goldman}, Bertrand},
        title = "{Weather on Other Worlds. II. Survey Results: Spots are Ubiquitous on L and T Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: low-mass, stars: rotation, starspots, stars: variables: general, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {154},
        pages = {154},
          doi = {10.1088/0004-637X/799/2/154},
archivePrefix = {arXiv},
       eprint = {1411.3051},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..154M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Goncharskii1982,
       author = {{Goncharskii}, A.~V. and {Stepanov}, V.~V. and {Khokhlova}, V.~L. and {Yagola}, A.~G.},
        title = "{Mapping of chemical elements on the surfaces of Ap stars. I. Solution of the inverse problem of finding local profiles of spectral lines}",
      journal = {\sovast},
         year = 1982,
        month = dec,
       volume = {26},
        pages = {690-696},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982SvA....26..690G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goncharskii1977,
       author = {{Goncharskii}, A.~V. and {Stepanov}, V.~V. and {Kokhlova}, V.~L. and {Yagola}, A.~G.},
        title = "{Reconstruction of local line profiles from those observed in an Ap spectrum.}",
      journal = {Pisma v Astronomicheskii Zhurnal},
         year = 1977,
        month = jun,
       volume = {3},
        pages = {278},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977PAZh....3..278G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Deutsch1958,
       author = {{Deutsch}, A.~J.},
        title = "{Harmonic Analysis of the Periodic Spectrum Variables}",
    booktitle = {Electromagnetic Phenomena in Cosmical Physics},
         year = 1958,
       editor = {{Lehnert}, B.},
       volume = {6},
        month = jan,
        pages = {209},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1958IAUS....6..209D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Deutsch1970,
       author = {{Deutsch}, Armin J.},
        title = "{Harmonic Analysis of Rigidly Rotating AP Stars}",
      journal = {\apj},
         year = 1970,
        month = mar,
       volume = {159},
        pages = {985},
          doi = {10.1086/150376},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970ApJ...159..985D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Falk1974,
       author = {{Falk}, Alfred E. and {Wehlau}, William H.},
        title = "{Harmonic Analysis of the Line Profiles of an Oblique Rotator}",
      journal = {\apj},
         year = 1974,
        month = sep,
       volume = {192},
        pages = {409-416},
          doi = {10.1086/153072},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ApJ...192..409F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Khokhlova1976,
       author = {{Khokhlova}, V.~L.},
        title = "{Mapping of ``spots'' on the surface of Ap stars by means of line profiles}",
      journal = {\sovast},
         year = 1976,
        month = apr,
       volume = {19},
        pages = {576},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1976SvA....19..576K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vogt&Penrod1983,
       author = {{Vogt}, S.~S. and {Penrod}, G.~D.},
        title = "{Doppler imaging of spotted stars : application to the RS Canum Venaticorum star HR 1099.}",
      journal = {\pasp},
     keywords = {Binary Stars, Imaging Techniques, Starspots, Coronal Holes, Doppler Effect, Line Spectra, Mapping, Stellar Rotation, Astrophysics},
         year = 1983,
        month = sep,
       volume = {95},
        pages = {565-576},
          doi = {10.1086/131208},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983PASP...95..565V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Piskunov1990,
       author = {{Piskunov}, N.~E. and {Tuominen}, I. and {Vilhu}, O.},
        title = "{Surface imaging of late-type stars.}",
      journal = {\aap},
     keywords = {Imaging Techniques, Late Stars, Stellar Structure, Surface Properties, Giant Stars, Stellar Atmospheres, Stellar Models, Astrophysics},
         year = 1990,
        month = apr,
       volume = {230},
        pages = {363-370},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990A&A...230..363P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Donati1999,
       author = {{Donati}, J. -F.},
        title = "{Magnetic cycles of HR 1099 and LQ Hydrae}",
      journal = {\mnras},
     keywords = {LINE: PROFILES, STARS: ACTIVITY, BINARIES: GENERAL, STARS: IMAGING, STARS: MAGNETIC FIELDS, STARS: ROTATION},
         year = 1999,
        month = jan,
       volume = {302},
       number = {3},
        pages = {457-481},
          doi = {10.1046/j.1365-8711.1999.02096.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999MNRAS.302..457D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier1999a,
       author = {{Strassmeier}, K.~G. and {Lupinek}, S. and {Dempsey}, R.~C. and {Rice}, J.~B.},
        title = "{Doppler imaging of stellar surface structure. X. The FK Comae-type star HD 199178 = V 1794 Cygni}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: IMAGING, STARS: INDIVIDUAL: HD 199178, STARS: LATE-TYPE, STARS: STARSPOTS},
         year = 1999,
        month = jul,
       volume = {347},
        pages = {212-224},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&A...347..212S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strassmeier1999b,
       author = {{Strassmeier}, K.~G.},
        title = "{Doppler imaging of stellar surface structure. XI. The super starspots on the K0 giant HD 12545: larger than the entire Sun}",
      journal = {\aap},
     keywords = {STARS: ACTIVITY, STARS: IMAGING, STARS: INDIVIDUAL: HD 12545, STARS: LATE-TYPE, STARS: STARSPOTS},
         year = 1999,
        month = jul,
       volume = {347},
        pages = {225-234},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&A...347..225S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burgasser1999,
       author = {{Burgasser}, Adam J. and {Kirkpatrick}, J. Davy and {Brown}, Michael E. and {Reid}, I. Neill and {Gizis}, John E. and {Dahn}, Conard C. and {Monet}, David G. and {Beichman}, Charles A. and {Liebert}, James and {Cutri}, Roc M. and {Skrutskie}, Michael F.},
        title = "{Discovery of Four Field Methane (T-Type) Dwarfs with the Two Micron All-Sky Survey}",
      journal = {\apjl},
     keywords = {INFRARED: STARS, STARS: FUNDAMENTAL PARAMETERS, STARS: INDIVIDUAL: ALPHANUMERIC: 2MASSI J1047539+212423, STARS: INDIVIDUAL: ALPHANUMERIC: 2MASSW J1217111-031113, STARS: INDIVIDUAL: ALPHANUMERIC: 2MASSW J1225543-273947, STARS: INDIVIDUAL: ALPHANUMERIC: 2MASSW J1237392+652615, STARS: INDIVIDUAL: ALPHANUMERIC: 2MASSW J1346464-003150, STARS: LOW-MASS, BROWN DWARFS, Infrared: Stars, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: 2MASSI J1047539+212423, Stars: Individual: Alphanumeric: 2MASSW J1217111-031113, Stars: Individual: Alphanumeric: 2MASSW J1225543-273947, Stars: Individual: Alphanumeric: 2MASSW J1237392+652615, Stars: Individual: Alphanumeric: 2MASSW J1346464-003150, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 1999,
        month = sep,
       volume = {522},
       number = {1},
        pages = {L65-L68},
          doi = {10.1086/312221},
archivePrefix = {arXiv},
       eprint = {astro-ph/9907019},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...522L..65B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{CollierCameron&Unruh1994,
       author = {{Collier Cameron}, A. and {Unruh}, Y.~C.},
        title = "{Doppler images of AB Doradus in 1992 January.}",
      journal = {\mnras},
         year = 1994,
        month = aug,
       volume = {269},
        pages = {814-836},
          doi = {10.1093/mnras/269.3.814},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994MNRAS.269..814C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hatzes1995,
       author = {{Hatzes}, Artie P.},
        title = "{Doppler Imaging of the Cool SPOT Distribution on the Weak T Tauri Star V410 Tauri}",
      journal = {\apj},
     keywords = {LINE: PROFILES, STARS: ACTIVITY, STARS: CHROMOSPHERES, STARS: INDIVIDUAL CONSTELLATION NAME: V410 TAURI, STARS: PRE-MAIN-SEQUENCE},
         year = 1995,
        month = oct,
       volume = {451},
        pages = {784},
          doi = {10.1086/176265},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...451..784H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows1997,
       author = {{Burrows}, A. and {Marley}, M. and {Hubbard}, W.~B. and {Lunine}, J.~I. and {Guillot}, T. and {Saumon}, D. and {Freedman}, R. and {Sudarsky}, D. and {Sharp}, C.},
        title = "{A Nongray Theory of Extrasolar Giant Planets and Brown Dwarfs}",
      journal = {\apj},
     keywords = {Stars: Planetary Systems, Stars: Atmospheres, stars: interiors -- stars: low-mass, brown dwarfs, Astrophysics},
         year = 1997,
        month = dec,
       volume = {491},
       number = {2},
        pages = {856-875},
          doi = {10.1086/305002},
archivePrefix = {arXiv},
       eprint = {astro-ph/9705201},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...491..856B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Barnes2017,
       author = {{Barnes}, J.~R. and {Jeffers}, S.~V. and {Haswell}, C.~A. and {Jones}, H.~R.~A. and {Shulyak}, D. and {Pavlenko}, Ya. V. and {Jenkins}, J.~S.},
        title = "{Surprisingly different star-spot distributions on the near equal-mass equal-rotation-rate stars in the M dwarf binary GJ 65 AB}",
      journal = {\mnras},
     keywords = {techniques: imaging spectroscopy, techniques: spectroscopic, stars: atmospheres, stars: imaging, stars: low-mass, starspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = oct,
       volume = {471},
       number = {1},
        pages = {811-823},
          doi = {10.1093/mnras/stx1482},
archivePrefix = {arXiv},
       eprint = {1706.03979},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471..811B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirkpatrick1999,
       author = {{Kirkpatrick}, J. Davy and {Reid}, I. Neill and {Liebert}, James and {Cutri}, Roc M. and {Nelson}, Brant and {Beichman}, Charles A. and {Dahn}, Conard C. and {Monet}, David G. and {Gizis}, John E. and {Skrutskie}, Michael F.},
        title = "{Dwarfs Cooler than ``M``: The Definition of Spectral Type ``L'' Using Discoveries from the 2 Micron All-Sky Survey (2MASS)}",
      journal = {\apj},
     keywords = {INFRARED: STARS, STARS: ATMOSPHERES, STARS: DISTANCES, STARS: FUNDAMENTAL PARAMETERS, STARS: LOW-MASS, BROWN DWARFS, Infrared: Stars, Stars: Atmospheres, Stars: Distances, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs},
         year = 1999,
        month = jul,
       volume = {519},
       number = {2},
        pages = {802-833},
          doi = {10.1086/307414},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...519..802K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Barnes&CollierCameron2001a,
       author = {{Barnes}, J.~R. and {Collier Cameron}, A. and {James}, D.~J. and {Donati}, J. -F.},
        title = "{Doppler images from dual-site observations of southern rapidly rotating stars - II. Starspot patterns and differential rotation on Speedy Mic}",
      journal = {\mnras},
     keywords = {LINE: PROFILES, METHODS: DATA ANALYSIS, TECHNIQUES: MISCELLANEOUS, STARS: ACTIVITY, STARS: INDIVIDUAL: SPEEDY MIC (HD 197890), STARS: LATE-TYPE},
         year = 2001,
        month = jun,
       volume = {324},
       number = {1},
        pages = {231-242},
          doi = {10.1046/j.1365-8711.2001.04309.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.324..231B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon2008,
       author = {{Saumon}, D. and {Marley}, Mark S.},
        title = "{The Evolution of L and T Dwarfs in Color-Magnitude Diagrams}",
      journal = {\apj},
     keywords = {stars: atmospheres, stars: evolution, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = dec,
       volume = {689},
       number = {2},
        pages = {1327-1344},
          doi = {10.1086/592734},
archivePrefix = {arXiv},
       eprint = {0808.2611},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...689.1327S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zaire2021,
       author = {{Zaire}, B. and {Donati}, J. -F. and {Klein}, B.},
        title = "{Magnetic field and activity phenomena of the K2 dwarf V471 Tau}",
      journal = {\mnras},
     keywords = {magnetic fields, techniques: polarimetric, binaries: eclipsing, stars: imaging, stars: individual: V471 Tau, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jun,
       volume = {504},
       number = {2},
        pages = {1969-1988},
          doi = {10.1093/mnras/stab1019},
archivePrefix = {arXiv},
       eprint = {2104.02619},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.504.1969Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Finociety2021,
       author = {{Finociety}, B. and {Donati}, J. -F. and {Klein}, B. and {Zaire}, B. and {Lehmann}, L. and {Moutou}, C. and {Bouvier}, J. and {Alencar}, S.~H.~P. and {Yu}, L. and {Grankin}, K. and {Artigau}, {\'E}. and {Doyon}, R. and {Delfosse}, X. and {Fouqu{\'e}}, P. and {H{\'e}brard}, G. and {Jardine}, M. and {K{\'o}sp{\'a}l}, {\'A}. and {M{\'e}nard}, F. and {M{\'e}nard}, F. and {SLS consortium}},
        title = "{The T Tauri star V410 Tau in the eyes of SPIRou and TESS}",
      journal = {\mnras},
     keywords = {techniques: polarimetric, stars: activity, stars: imaging, stars: individual: V410 Tau, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = dec,
       volume = {508},
       number = {3},
        pages = {3427-3445},
          doi = {10.1093/mnras/stab2778},
archivePrefix = {arXiv},
       eprint = {2109.11755},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.508.3427F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman2016,
       author = {{Showman}, Adam P.},
        title = "{Astrophysics: Illuminating brown dwarfs}",
      journal = {\nat},
         year = 2016,
        month = may,
       volume = {533},
       number = {7603},
        pages = {330-331},
          doi = {10.1038/533330a},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016Natur.533..330S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Barnes&CollierCameron2001b,
       author = {{Barnes}, J.~R. and {Collier Cameron}, A.},
        title = "{Starspot patterns on the M dwarfs HK Aqr and RE 1816 +541}",
      journal = {\mnras},
     keywords = {LINE: PROFILES, METHODS: DATA ANALYSIS, STARS: ACTIVITY, STARS: IMAGING, STARS: LATE-TYPE, STARS: SPOTS},
         year = 2001,
        month = sep,
       volume = {326},
       number = {3},
        pages = {950-958},
          doi = {10.1046/j.1365-8711.2001.04649.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.326..950B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barnes2004,
       author = {{Barnes}, J.~R. and {James}, D.~J. and {Collier Cameron}, A.},
        title = "{Differential rotation and star-spot evolution on HK Aqr in 2001 and 2002}",
      journal = {\mnras},
     keywords = {line: profiles, methods: data analysis, techniques: miscellaneous, stars: activity, stars: individual: HK Aqr (Gl 890), stars: late-type},
         year = 2004,
        month = aug,
       volume = {352},
       number = {2},
        pages = {589-599},
          doi = {10.1111/j.1365-2966.2004.07949.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.352..589B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fegley&Lodders1996,
       author = {{Fegley}, Bruce, Jr. and {Lodders}, Katharina},
        title = "{Atmospheric Chemistry of the Brown Dwarf Gliese 229B: Thermochemical Equilibrium Predictions}",
      journal = {\apjl},
     keywords = {INFRARED: STARS, STARS: ABUNDANCES, STARS: ATMOSPHERES, STARS: LOW-MASS, BROWN DWARFS, STARS: INDIVIDUAL NAME: GLIESE 229B},
         year = 1996,
        month = nov,
       volume = {472},
        pages = {L37},
          doi = {10.1086/310356},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...472L..37F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Noll1997,
       author = {{Noll}, Keith S. and {Geballe}, T.~R. and {Marley}, Mark S.},
        title = "{Detection of Abundant Carbon Monoxide in the Brown Dwarf Gliese 229B}",
      journal = {\apjl},
     keywords = {INFRARED: STARS, STARS: LOW-MASS, BROWN DWARFS, STARS: INDIVIDUAL NAME: GLIESE 229B, Infrared: Stars, Stars: Individual: Name: Gliese 229B, Stars: Low-Mass, Brown Dwarfs},
         year = 1997,
        month = nov,
       volume = {489},
       number = {1},
        pages = {L87-L90},
          doi = {10.1086/310954},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...489L..87N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allard1996,
       author = {{Allard}, France and {Hauschildt}, Peter H. and {Baraffe}, Isabelle and {Chabrier}, Gilles},
        title = "{Synthetic Spectra and Mass Determination of the Brown Dwarf GI 229B}",
      journal = {\apjl},
     keywords = {SUN: ATMOSPHERE, STARS: EVOLUTION, STARS: FUNDAMENTAL PARAMETERS, STARS: LOW-MASS, BROWN DWARFS},
         year = 1996,
        month = jul,
       volume = {465},
        pages = {L123},
          doi = {10.1086/310143},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...465L.123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Griffith&Yelle1999,
       author = {{Griffith}, Caitlin A. and {Yelle}, Roger V.},
        title = "{Disequilibrium Chemistry in a Brown Dwarf's Atmosphere: Carbon Monoxide in Gliese 229B}",
      journal = {\apjl},
     keywords = {CONVECTION, PLANETS AND SATELLITES: GENERAL, STARS: ATMOSPHERES, STARS: INDIVIDUAL: NAME: GLIESE 229B, STARS: LOW-MASS, BROWN DWARFS, Convection, Planets and Satellites: General, Stars: Atmospheres, Stars: Individual: Name: Gliese 229B, Stars: Low-Mass, Brown Dwarfs},
         year = 1999,
        month = jul,
       volume = {519},
       number = {1},
        pages = {L85-L88},
          doi = {10.1086/312103},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...519L..85G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon2000,
       author = {{Saumon}, D. and {Geballe}, T.~R. and {Leggett}, S.~K. and {Marley}, M.~S. and {Freedman}, R.~S. and {Lodders}, K. and {Fegley}, B., Jr. and {Sengupta}, S.~K.},
        title = "{Molecular Abundances in the Atmosphere of the T Dwarf GL 229B}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Individual: Alphanumeric: Gl 229B, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2000,
        month = sep,
       volume = {541},
       number = {1},
        pages = {374-389},
          doi = {10.1086/309410},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003353},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...541..374S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nakajima1995,
       author = {{Nakajima}, T. and {Oppenheimer}, B.~R. and {Kulkarni}, S.~R. and {Golimowski}, D.~A. and {Matthews}, K. and {Durrance}, S.~T.},
        title = "{Discovery of a cool brown dwarf}",
      journal = {\nat},
         year = 1995,
        month = nov,
       volume = {378},
       number = {6556},
        pages = {463-465},
          doi = {10.1038/378463a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995Natur.378..463N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Saumon2006,
       author = {{Saumon}, D. and {Marley}, M.~S. and {Cushing}, M.~C. and {Leggett}, S.~K. and {Roellig}, T.~L. and {Lodders}, K. and {Freedman}, R.~S.},
        title = "{Ammonia as a Tracer of Chemical Equilibrium in the T7.5 Dwarf Gliese 570D}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Individual: Name: Gliese 570D, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2006,
        month = aug,
       volume = {647},
       number = {1},
        pages = {552-557},
          doi = {10.1086/505419},
archivePrefix = {arXiv},
       eprint = {astro-ph/0605563},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...647..552S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon2007,
       author = {{Saumon}, D. and {Marley}, M.~S. and {Leggett}, S.~K. and {Geballe}, T.~R. and {Stephens}, D. and {Golimowski}, D.~A. and {Cushing}, M.~C. and {Fan}, X. and {Rayner}, J.~T. and {Lodders}, K. and {Freedman}, R.~S.},
        title = "{Physical Parameters of Two Very Cool T Dwarfs}",
      journal = {\apj},
     keywords = {stars: individual (2MASS J04151954-0935066), stars: individual (2MASS J12171110-0311131), stars: individual (Gl 570D), Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = feb,
       volume = {656},
       number = {2},
        pages = {1136-1149},
          doi = {10.1086/510557},
archivePrefix = {arXiv},
       eprint = {astro-ph/0611062},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...656.1136S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley1996,
       author = {{Marley}, M.~S. and {Saumon}, D. and {Guillot}, T. and {Freedman}, R.~S. and {Hubbard}, W.~B. and {Burrows}, A. and {Lunine}, J.~I.},
        title = "{Atmospheric, Evolutionary, and Spectral Models of the Brown Dwarf Gliese 229 B}",
      journal = {Science},
     keywords = {Astrophysics},
         year = 1996,
        month = jun,
       volume = {272},
       number = {5270},
        pages = {1919-1921},
          doi = {10.1126/science.272.5270.1919},
archivePrefix = {arXiv},
       eprint = {astro-ph/9606036},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996Sci...272.1919M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hubeny&Burrows2007,
       author = {{Hubeny}, Ivan and {Burrows}, Adam},
        title = "{A Systematic Study of Departures from Chemical Equilibrium in the Atmospheres of Substellar Mass Objects}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Individual: Name: Gliese 570D, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {1248-1261},
          doi = {10.1086/522107},
archivePrefix = {arXiv},
       eprint = {0705.3922},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669.1248H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2007a,
       author = {{Leggett}, S.~K. and {Saumon}, D. and {Marley}, M.~S. and {Geballe}, T.~R. and {Golimowski}, D.~A. and {Stephens}, D. and {Fan}, X.},
        title = "{3.6-7.9 {\ensuremath{\mu}}m Photometry of L and T Dwarfs and the Prevalence of Vertical Mixing in their Atmospheres}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = feb,
       volume = {655},
       number = {2},
        pages = {1079-1094},
          doi = {10.1086/510014},
archivePrefix = {arXiv},
       eprint = {astro-ph/0610214},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...655.1079L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2007b,
       author = {{Leggett}, S.~K. and {Marley}, M.~S. and {Freedman}, R. and {Saumon}, D. and {Liu}, Michael C. and {Geballe}, T.~R. and {Golimowski}, D.~A. and {Stephens}, D.~C.},
        title = "{Physical and Spectral Characteristics of the T8 and Later Type Dwarfs}",
      journal = {\apj},
     keywords = {Infrared: Stars, stars: individual (2MASS J04151954-0935066), stars: individual (2MASS J09393548-2448279), stars: individual (2MASS J11145133-2618235), stars: individual (HD 3651B), stars: individual (Gl 570D), Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2007,
        month = sep,
       volume = {667},
       number = {1},
        pages = {537-548},
          doi = {10.1086/519948},
archivePrefix = {arXiv},
       eprint = {0705.2602},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...667..537L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leggett2008,
       author = {{Leggett}, S.~K. and {Saumon}, D. and {Albert}, Loic and {Cushing}, Michael C. and {Liu}, Michael C. and {Luhman}, K.~L. and {Marley}, M.~S. and {Kirkpatrick}, J. Davy and {Roellig}, Thomas L. and {Allers}, K.~N.},
        title = "{HN Peg B: A Test of Models of the L to T Dwarf Transition}",
      journal = {\apj},
     keywords = {binaries: visual, stars: individual: 2MASS J21442847+1446077 HN Peg HN Peg B, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = aug,
       volume = {682},
       number = {2},
        pages = {1256-1263},
          doi = {10.1086/589146},
archivePrefix = {arXiv},
       eprint = {0804.1386},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...682.1256L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Freytag2010,
       author = {{Freytag}, B. and {Allard}, F. and {Ludwig}, H. -G. and {Homeier}, D. and {Steffen}, M.},
        title = "{The role of convection, overshoot, and gravity waves for the transport of dust in M dwarf and brown dwarf atmospheres}",
      journal = {\aap},
     keywords = {brown dwarfs, hydrodynamics, convection, waves, stars: atmospheres, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = apr,
       volume = {513},
          eid = {A19},
        pages = {A19},
          doi = {10.1051/0004-6361/200913354},
archivePrefix = {arXiv},
       eprint = {1002.3437},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...513A..19F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Stephens2009,
       author = {{Stephens}, D.~C. and {Leggett}, S.~K. and {Cushing}, Michael C. and {Marley}, Mark S. and {Saumon}, D. and {Geballe}, T.~R. and {Golimowski}, David A. and {Fan}, Xiaohui and {Noll}, K.~S.},
        title = "{The 0.8-14.5 {\ensuremath{\mu}}m Spectra of Mid-L to Mid-T Dwarfs: Diagnostics of Effective Temperature, Grain Sedimentation, Gas Transport, and Surface Gravity}",
      journal = {\apj},
     keywords = {stars: individual: 2MASS J00361617+1821104 2MASS J05591914{\textendash}1404488 2MASS J08251968+2115521 2MASS J09083803+5032088 2MASS J15074769{\textendash}1627386 2MASS J22244381{\textendash}0158521 2MASS J22443167+2043433 2MASS J22541892+3123498 DENIS-P J025503.3{\textendash}470049 SDSS J000013.54+255418.6 SDSS J075840.32+324723.3 SDSS J080531.83+481233.1 SDSS J085758.44+570851.4 SDSS J105213.50+442255.6AB SDSS J111009.99+011613.0 SDSS J115553.85+ 055957.5 SDSS J120747.17+024424.8 SDSS J125453.90{\textendash}012247.5 SDSS J133148.88{\textendash}011652.5 SDSS J151643.00+305344.3 SDSS J152039.82+354619.8, stars: low-mass, brown dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = sep,
       volume = {702},
       number = {1},
        pages = {154-170},
          doi = {10.1088/0004-637X/702/1/154},
archivePrefix = {arXiv},
       eprint = {0906.2991},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...702..154S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Adcroft2004,
author = {Adcroft, Alistair and Hill, Chris and Campin, Jean-Michel and Marshall, John and Heimbach, Patrick},
year = {2004},
month = {01},
pages = {},
title = {Overview of the formulation and numerics of the MIT GCM},
journal = {Proceedings of the ECMWF Seminar Series on Numerical Methods, Recent Developments in Numerical Methods for Atmosphere and Ocean Modeling}
}

@ARTICLE{Shepherd1987,
       author = {{Shepherd}, Theodor G.},
        title = "{Rossby waves and two-dimensional turbulence in a large-scale zonal jet}",
      journal = {Journal of Fluid Mechanics},
     keywords = {Rossby Regimes, Turbulent Jets, Two Dimensional Flow, Zonal Flow (Meteorology), Atmospheric Turbulence, Energy Transfer, Flux Quantization, Isotropic Turbulence, Ray Tracing, Vortices, Fluid Mechanics and Heat Transfer},
         year = 1987,
        month = oct,
       volume = {183},
        pages = {467-509},
          doi = {10.1017/S0022112087002738},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987JFM...183..467S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Heng2017,
       author = {{Heng}, Kevin},
        title = "{Exoplanetary Atmospheres: Theoretical Concepts and Foundations}",
         year = 2017,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017eatc.book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Beuzit2008,
       author = {{Beuzit}, Jean-Luc and {Feldt}, Markus and {Dohlen}, Kjetil and {Mouillet}, David and {Puget}, Pascal and {Wildi}, Francois and {Abe}, Lyu and {Antichi}, Jacopo and {Baruffolo}, Andrea and {Baudoz}, Pierre and {Boccaletti}, Anthony and {Carbillet}, Marcel and {Charton}, Julien and {Claudi}, Riccardo and {Downing}, Mark and {Fabron}, Christophe and {Feautrier}, Philippe and {Fedrigo}, Enrico and {Fusco}, Thierry and {Gach}, Jean-Luc and {Gratton}, Raffaele and {Henning}, Thomas and {Hubin}, Norbert and {Joos}, Franco and {Kasper}, Markus and {Langlois}, Maud and {Lenzen}, Rainer and {Moutou}, Claire and {Pavlov}, Alexey and {Petit}, Cyril and {Pragt}, Johan and {Rabou}, Patrick and {Rigal}, Florence and {Roelfsema}, Ronald and {Rousset}, G{\'e}rard and {Saisse}, Michel and {Schmid}, Hans-Martin and {Stadler}, Eric and {Thalmann}, Christian and {Turatto}, Massimo and {Udry}, St{\'e}phane and {Vakili}, Farrokh and {Waters}, Rens},
        title = "{SPHERE: a 'Planet Finder' instrument for the VLT}",
    booktitle = {Ground-based and Airborne Instrumentation for Astronomy II},
         year = 2008,
       editor = {{McLean}, Ian S. and {Casali}, Mark M.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7014},
        month = jul,
          eid = {701418},
        pages = {701418},
          doi = {10.1117/12.790120},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SPIE.7014E..18B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Macintosh2014,
       author = {{Macintosh}, Bruce and {Graham}, James R. and {Ingraham}, Patrick and {Konopacky}, Quinn and {Marois}, Christian and {Perrin}, Marshall and {Poyneer}, Lisa and {Bauman}, Brian and {Barman}, Travis and {Burrows}, Adam S. and {Cardwell}, Andrew and {Chilcote}, Jeffrey and {De Rosa}, Robert J. and {Dillon}, Daren and {Doyon}, Rene and {Dunn}, Jennifer and {Erikson}, Darren and {Fitzgerald}, Michael P. and {Gavel}, Donald and {Goodsell}, Stephen and {Hartung}, Markus and {Hibon}, Pascale and {Kalas}, Paul and {Larkin}, James and {Maire}, Jerome and {Marchis}, Franck and {Marley}, Mark S. and {McBride}, James and {Millar-Blanchaer}, Max and {Morzinski}, Katie and {Norton}, Andrew and {Oppenheimer}, B.~R. and {Palmer}, David and {Patience}, Jennifer and {Pueyo}, Laurent and {Rantakyro}, Fredrik and {Sadakuni}, Naru and {Saddlemyer}, Leslie and {Savransky}, Dmitry and {Serio}, Andrew and {Soummer}, Remi and {Sivaramakrishnan}, Anand and {Song}, Inseok and {Thomas}, Sandrine and {Wallace}, J. Kent and {Wiktorowicz}, Sloane and {Wolff}, Schuyler},
        title = "{First light of the Gemini Planet Imager}",
      journal = {Proceedings of the National Academy of Science},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = sep,
       volume = {111},
       number = {35},
        pages = {12661-12666},
          doi = {10.1073/pnas.1304215111},
archivePrefix = {arXiv},
       eprint = {1403.7520},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PNAS..11112661M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sparks&Ford2002,
       author = {{Sparks}, William B. and {Ford}, Holland C.},
        title = "{Imaging Spectroscopy for Extrasolar Planet Detection}",
      journal = {\apj},
     keywords = {Instrumentation: Miscellaneous, Methods: Analytical, Stars: Planetary Systems, Astrophysics},
         year = 2002,
        month = oct,
       volume = {578},
       number = {1},
        pages = {543-564},
          doi = {10.1086/342401},
archivePrefix = {arXiv},
       eprint = {astro-ph/0209078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...578..543S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Riaud&Schneider2007,
       author = {{Riaud}, P. and {Schneider}, J.},
        title = "{Improving Earth-like planets' detection with an ELT: the differential radial velocity experiment}",
      journal = {\aap},
     keywords = {stars: planetary systems, techniques: spectroscopic, techniques: radial velocities, astrobiology},
         year = 2007,
        month = jul,
       volume = {469},
       number = {1},
        pages = {355-361},
          doi = {10.1051/0004-6361:20077085},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...469..355R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kawahara&Hirano2014,
       author = {{Kawahara}, Hajime and {Hirano}, Teruyuki},
        title = "{Characterizing Earth-like Planets Using a Combination of High-Dispersion Spectroscopy and High-Contrast Instruments: Doppler-shifted Water and Oxygen Lines}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = sep,
          eid = {arXiv:1409.5740},
        pages = {arXiv:1409.5740},
archivePrefix = {arXiv},
       eprint = {1409.5740},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1409.5740K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Snellen2015,
       author = {{Snellen}, I. and {de Kok}, R. and {Birkby}, J.~L. and {Brandl}, B. and {Brogi}, M. and {Keller}, C. and {Kenworthy}, M. and {Schwarz}, H. and {Stuik}, R.},
        title = "{Combining high-dispersion spectroscopy with high contrast imaging: Probing rocky planets around our nearest neighbors}",
      journal = {\aap},
     keywords = {infrared: planetary systems, techniques: imaging spectroscopy, techniques: high angular resolution, methods: data analysis, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = apr,
       volume = {576},
          eid = {A59},
        pages = {A59},
          doi = {10.1051/0004-6361/201425018},
archivePrefix = {arXiv},
       eprint = {1503.01136},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...576A..59S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Snellen2010,
       author = {{Snellen}, Ignas A.~G. and {de Kok}, Remco J. and {de Mooij}, Ernst J.~W. and {Albrecht}, Simon},
        title = "{The orbital motion, absolute mass and high-altitude winds of exoplanet HD209458b}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2010,
        month = jun,
       volume = {465},
       number = {7301},
        pages = {1049-1051},
          doi = {10.1038/nature09111},
archivePrefix = {arXiv},
       eprint = {1006.4364},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Natur.465.1049S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bryan2020b,
       author = {{Bryan}, Marta L. and {Ginzburg}, Sivan and {Chiang}, Eugene and {Morley}, Caroline and {Bowler}, Brendan P. and {Xuan}, Jerry W. and {Knutson}, Heather A.},
        title = "{As the Worlds Turn: Constraining Spin Evolution in the Planetary-mass Regime}",
      journal = {\apj},
     keywords = {High resolution spectroscopy, Exoplanet formation, 2096, 492, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {905},
       number = {1},
          eid = {37},
        pages = {37},
          doi = {10.3847/1538-4357/abc0ef},
archivePrefix = {arXiv},
       eprint = {2010.07315},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...905...37B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Snellen2014,
       author = {{Snellen}, Ignas A.~G. and {Brandl}, Bernhard R. and {de Kok}, Remco J. and {Brogi}, Matteo and {Birkby}, Jayne and {Schwarz}, Henriette},
        title = "{Fast spin of the young extrasolar planet {\ensuremath{\beta}} Pictoris b}",
      journal = {\nat},
         year = 2014,
        month = may,
       volume = {509},
       number = {7498},
        pages = {63-65},
          doi = {10.1038/nature13253},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014Natur.509...63S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chauvin2004,
       author = {{Chauvin}, G. and {Lagrange}, A. -M. and {Dumas}, C. and {Zuckerman}, B. and {Mouillet}, D. and {Song}, I. and {Beuzit}, J. -L. and {Lowrance}, P.},
        title = "{A giant planet candidate near a young brown dwarf. Direct VLT/NACO observations using IR wavefront sensing}",
      journal = {\aap},
     keywords = {2MASSWJ 1207334-393254, brown dwarf, giant planet, adaptive optics imaging and spectroscopy, Astrophysics},
         year = 2004,
        month = oct,
       volume = {425},
        pages = {L29-L32},
          doi = {10.1051/0004-6361:200400056},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409323},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...425L..29C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dupuy&Liu2012,
       author = {{Dupuy}, Trent J. and {Liu}, Michael C.},
        title = "{The Hawaii Infrared Parallax Program. I. Ultracool Binaries and the L/T Transition}",
      journal = {\apjs},
     keywords = {astrometry, brown dwarfs, infrared: stars, parallaxes, proper motions, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2012,
        month = aug,
       volume = {201},
       number = {2},
          eid = {19},
        pages = {19},
          doi = {10.1088/0067-0049/201/2/19},
archivePrefix = {arXiv},
       eprint = {1201.2465},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJS..201...19D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lagrange2009,
       author = {{Lagrange}, A. -M. and {Gratadour}, D. and {Chauvin}, G. and {Fusco}, T. and {Ehrenreich}, D. and {Mouillet}, D. and {Rousset}, G. and {Rouan}, D. and {Allard}, F. and {Gendron}, {\'E}. and {Charton}, J. and {Mugnier}, L. and {Rabou}, P. and {Montri}, J. and {Lacombe}, F.},
        title = "{A probable giant planet imaged in the {\ensuremath{\beta}} Pictoris disk. VLT/NaCo deep L'-band imaging}",
      journal = {\aap},
     keywords = {instrumentation: adaptive optics, stars: early-type, stars: planetary systems, stars: individual: {\ensuremath{\beta}} Pic, Astrophysics},
         year = 2009,
        month = jan,
       volume = {493},
       number = {2},
        pages = {L21-L25},
          doi = {10.1051/0004-6361:200811325},
archivePrefix = {arXiv},
       eprint = {0811.3583},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...493L..21L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allers&Liu2013,
       author = {{Allers}, K.~N. and {Liu}, Michael C.},
        title = "{A Near-infrared Spectroscopic Study of Young Field Ultracool Dwarfs}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, planets and satellites: atmospheres, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = aug,
       volume = {772},
       number = {2},
          eid = {79},
        pages = {79},
          doi = {10.1088/0004-637X/772/2/79},
archivePrefix = {arXiv},
       eprint = {1305.4418},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...772...79A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu2016,
       author = {{Liu}, Michael C. and {Dupuy}, Trent J. and {Allers}, Katelyn N.},
        title = "{The Hawaii Infrared Parallax Program. II. Young Ultracool Field Dwarfs}",
      journal = {\apj},
     keywords = {astrometry, brown dwarfs, parallaxes, planets and satellites: gaseous planets, stars: distances, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = dec,
       volume = {833},
       number = {1},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/833/1/96},
archivePrefix = {arXiv},
       eprint = {1612.02426},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...833...96L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Samland2017,
       author = {{Samland}, M. and {Molli{\`e}re}, P. and {Bonnefoy}, M. and {Maire}, A. -L. and {Cantalloube}, F. and {Cheetham}, A.~C. and {Mesa}, D. and {Gratton}, R. and {Biller}, B.~A. and {Wahhaj}, Z. and {Bouwman}, J. and {Brandner}, W. and {Melnick}, D. and {Carson}, J. and {Janson}, M. and {Henning}, T. and {Homeier}, D. and {Mordasini}, C. and {Langlois}, M. and {Quanz}, S.~P. and {van Boekel}, R. and {Zurlo}, A. and {Schlieder}, J.~E. and {Avenhaus}, H. and {Beuzit}, J. -L. and {Boccaletti}, A. and {Bonavita}, M. and {Chauvin}, G. and {Claudi}, R. and {Cudel}, M. and {Desidera}, S. and {Feldt}, M. and {Fusco}, T. and {Galicher}, R. and {Kopytova}, T.~G. and {Lagrange}, A. -M. and {Le Coroller}, H. and {Martinez}, P. and {Moeller-Nilsson}, O. and {Mouillet}, D. and {Mugnier}, L.~M. and {Perrot}, C. and {Sevin}, A. and {Sissa}, E. and {Vigan}, A. and {Weber}, L.},
        title = "{Spectral and atmospheric characterization of 51 Eridani b using VLT/SPHERE}",
      journal = {\aap},
     keywords = {stars: individual: 51 Eridani, planets and satellites: atmospheres, methods: data analysis, techniques: high angular resolution, techniques: image processing, Astrophysics - Earth and Planetary Astrophysics},
         year = 2017,
        month = jul,
       volume = {603},
          eid = {A57},
        pages = {A57},
          doi = {10.1051/0004-6361/201629767},
archivePrefix = {arXiv},
       eprint = {1704.02987},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...603A..57S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INCOLLECTION{Biller2018book,
       author = {{Biller}, Beth A. and {Bonnefoy}, Micka{\"e}l},
        title = "{Exoplanet Atmosphere Measurements from Direct Imaging}",
     keywords = {Physics, Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {Handbook of Exoplanets},
         year = 2018,
       editor = {{Deeg}, Hans J. and {Belmonte}, Juan Antonio},
          eid = {101},
        pages = {101},
          doi = {10.1007/978-3-319-55333-7\_101},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018haex.bookE.101B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Macintosh2015,
       author = {{Macintosh}, B. and {Graham}, J.~R. and {Barman}, T. and {De Rosa}, R.~J. and {Konopacky}, Q. and {Marley}, M.~S. and {Marois}, C. and {Nielsen}, E.~L. and {Pueyo}, L. and {Rajan}, A. and {Rameau}, J. and {Saumon}, D. and {Wang}, J.~J. and {Patience}, J. and {Ammons}, M. and {Arriaga}, P. and {Artigau}, E. and {Beckwith}, S. and {Brewster}, J. and {Bruzzone}, S. and {Bulger}, J. and {Burningham}, B. and {Burrows}, A.~S. and {Chen}, C. and {Chiang}, E. and {Chilcote}, J.~K. and {Dawson}, R.~I. and {Dong}, R. and {Doyon}, R. and {Draper}, Z.~H. and {Duch{\^e}ne}, G. and {Esposito}, T.~M. and {Fabrycky}, D. and {Fitzgerald}, M.~P. and {Follette}, K.~B. and {Fortney}, J.~J. and {Gerard}, B. and {Goodsell}, S. and {Greenbaum}, A.~Z. and {Hibon}, P. and {Hinkley}, S. and {Cotten}, T.~H. and {Hung}, L. -W. and {Ingraham}, P. and {Johnson-Groh}, M. and {Kalas}, P. and {Lafreniere}, D. and {Larkin}, J.~E. and {Lee}, J. and {Line}, M. and {Long}, D. and {Maire}, J. and {Marchis}, F. and {Matthews}, B.~C. and {Max}, C.~E. and {Metchev}, S. and {Millar-Blanchaer}, M.~A. and {Mittal}, T. and {Morley}, C.~V. and {Morzinski}, K.~M. and {Murray-Clay}, R. and {Oppenheimer}, R. and {Palmer}, D.~W. and {Patel}, R. and {Perrin}, M.~D. and {Poyneer}, L.~A. and {Rafikov}, R.~R. and {Rantakyr{\"o}}, F.~T. and {Rice}, E.~L. and {Rojo}, P. and {Rudy}, A.~R. and {Ruffio}, J. -B. and {Ruiz}, M.~T. and {Sadakuni}, N. and {Saddlemyer}, L. and {Salama}, M. and {Savransky}, D. and {Schneider}, A.~C. and {Sivaramakrishnan}, A. and {Song}, I. and {Soummer}, R. and {Thomas}, S. and {Vasisht}, G. and {Wallace}, J.~K. and {Ward-Duong}, K. and {Wiktorowicz}, S.~J. and {Wolff}, S.~G. and {Zuckerman}, B.},
        title = "{Discovery and spectroscopy of the young jovian planet 51 Eri b with the Gemini Planet Imager}",
      journal = {Science},
     keywords = {ASTRONOMY, PLANET SCI, Astrophysics - Earth and Planetary Astrophysics},
         year = 2015,
        month = oct,
       volume = {350},
       number = {6256},
        pages = {64-67},
          doi = {10.1126/science.aac5891},
archivePrefix = {arXiv},
       eprint = {1508.03084},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015Sci...350...64M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mohanty2007,
       author = {{Mohanty}, Subhanjoy and {Jayawardhana}, Ray and {Hu{\'e}lamo}, Nuria and {Mamajek}, Eric},
        title = "{The Planetary Mass Companion 2MASS 1207-3932B: Temperature, Mass, and Evidence for an Edge-on Disk}",
      journal = {\apj},
     keywords = {Stars: Circumstellar Matter, Stars: Planetary Systems, Stars: Formation, Stars: Low-Mass, Brown Dwarfs, Stars: Pre-Main-Sequence, Techniques: Spectroscopic, Astrophysics},
         year = 2007,
        month = mar,
       volume = {657},
       number = {2},
        pages = {1064-1091},
          doi = {10.1086/510877},
archivePrefix = {arXiv},
       eprint = {astro-ph/0610550},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...657.1064M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Apai2016,
       author = {{Apai}, D{\'a}niel and {Kasper}, Markus and {Skemer}, Andrew and {Hanson}, Jake R. and {Lagrange}, Anne-Marie and {Biller}, Beth A. and {Bonnefoy}, Micka{\"e}l and {Buenzli}, Esther and {Vigan}, Arthur},
        title = "{High-cadence, High-contrast Imaging for Exoplanet Mapping: Observations of the HR 8799 Planets with VLT/SPHERE Satellite-spot-corrected Relative Photometry}",
      journal = {\apj},
     keywords = {methods: observational, planetary systems, planets and satellites: atmospheres, planets and satellites: gaseous planets, planets and satellites: individual: HR 8799, techniques: photometric, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = mar,
       volume = {820},
       number = {1},
          eid = {40},
        pages = {40},
          doi = {10.3847/0004-637X/820/1/40},
archivePrefix = {arXiv},
       eprint = {1602.02856},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...820...40A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Biller2021,
       author = {{Biller}, Beth A. and {Apai}, D{\'a}niel and {Bonnefoy}, Micka{\"e}l and {Desidera}, Silvano and {Gratton}, Raffaele and {Kasper}, Markus and {Kenworthy}, Matthew and {Lagrange}, Anne-Marie and {Lazzoni}, Cecilia and {Mesa}, Dino and {Vigan}, Arthur and {Wagner}, Kevin and {Vos}, Johanna M. and {Zurlo}, Alice},
        title = "{A high-contrast search for variability in HR 8799bc with VLT-SPHERE}",
      journal = {\mnras},
     keywords = {planets and satellites: gaseous planets, infrared: planetary systems, (stars:) brown dwarfs, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = may,
       volume = {503},
       number = {1},
        pages = {743-767},
          doi = {10.1093/mnras/stab202},
archivePrefix = {arXiv},
       eprint = {2101.08514},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503..743B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bowler2020,
       author = {{Bowler}, Brendan P. and {Zhou}, Yifan and {Morley}, Caroline V. and {Kataria}, Tiffany and {Bryan}, Marta L. and {Benneke}, Bj{\"o}rn and {Batygin}, Konstantin},
        title = "{Strong Near-infrared Spectral Variability of the Young Cloudy L Dwarf Companion VHS J1256-1257 b}",
      journal = {\apjl},
     keywords = {185, 2020, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = apr,
       volume = {893},
       number = {2},
          eid = {L30},
        pages = {L30},
          doi = {10.3847/2041-8213/ab8197},
archivePrefix = {arXiv},
       eprint = {2004.05170},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...893L..30B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Currie2022,
       author = {{Currie}, Thayne and {Biller}, Beth and {Lagrange}, Anne-Marie and {Marois}, Christian and {Guyon}, Olivier and {Nielsen}, Eric and {Bonnefoy}, Mickael and {De Rosa}, Robert},
        title = "{Direct Imaging and Spectroscopy of Extrasolar Planets}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = may,
          eid = {arXiv:2205.05696},
        pages = {arXiv:2205.05696},
archivePrefix = {arXiv},
       eprint = {2205.05696},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220505696C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Rich2016,
       author = {{Rich}, Evan A. and {Currie}, Thayne and {Wisniewski}, John P. and {Hashimoto}, Jun and {Brandt}, Timothy D. and {Carson}, Joseph C. and {Kuzuhara}, Masayuki and {Uyama}, Taichi},
        title = "{Thermal Infrared Imaging and Atmospheric Modeling of VHS J125601.92-125723.9 b: Evidence for Moderately Thick Clouds and Equilibrium Carbon Chemistry in a Hierarchical Triple System}",
      journal = {\apj},
     keywords = {binaries: general, brown dwarfs, stars: low-mass, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {830},
       number = {2},
          eid = {114},
        pages = {114},
          doi = {10.3847/0004-637X/830/2/114},
archivePrefix = {arXiv},
       eprint = {1607.06007},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...830..114R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilson2014,
       author = {{Wilson}, P.~A. and {Rajan}, A. and {Patience}, J.},
        title = "{The brown dwarf atmosphere monitoring (BAM) project. I. The largest near-IR monitoring survey of L and T dwarfs}",
      journal = {\aap},
     keywords = {techniques: photometric, brown dwarfs, stars: low-mass, stars: atmospheres, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = jun,
       volume = {566},
          eid = {A111},
        pages = {A111},
          doi = {10.1051/0004-6361/201322995},
archivePrefix = {arXiv},
       eprint = {1404.4633},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...566A.111W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Cushing2006,
       author = {{Cushing}, M.~C. and {Roellig}, T.~L.},
        title = "{Spitzer Space Telescope Observations of M, L, and T Dwarfs}",
    booktitle = {The Spitzer Space Telescope: New Views of the Cosmos},
         year = 2006,
       editor = {{Armus}, L. and {Reach}, W.~T.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {357},
        month = dec,
        pages = {66},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..357...66C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luna&Morley2021,
       author = {{Luna}, Jessica L. and {Morley}, Caroline V.},
        title = "{Empirically Determining Substellar Cloud Compositions in the Era of the James Webb Space Telescope}",
      journal = {\apj},
     keywords = {Brown dwarfs, L dwarfs, Stellar atmospheres, Extrasolar gaseous giant planets, Exoplanet atmospheres, 185, 894, 1584, 509, 487, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {146},
        pages = {146},
          doi = {10.3847/1538-4357/ac1865},
archivePrefix = {arXiv},
       eprint = {2108.03161},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920..146L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia&Ammons2017,
       author = {{Garcia}, E. Victor and {Ammons}, S. Mark and {Salama}, Maissa and {Crossfield}, Ian and {Bendek}, Eduardo and {Chilcote}, Jeffrey and {Garrel}, Vincent and {Graham}, James R. and {Kalas}, Paul and {Konopacky}, Quinn and {Lu}, Jessica R. and {Macintosh}, Bruce and {Marin}, Eduardo and {Marois}, Christian and {Nielsen}, Eric and {Neichel}, Beno{\^\i}t and {Pham}, Don and {De Rosa}, Robert J. and {Ryan}, Dominic M. and {Service}, Maxwell and {Sivo}, Gaetano},
        title = "{Individual, Model-independent Masses of the Closest Known Brown Dwarf Binary to the Sun}",
      journal = {\apj},
     keywords = {astrometry, binaries: visual, brown dwarfs, stars: fundamental parameters, stars: individual: WISE J104915.57{\textendash}531906.1, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = sep,
       volume = {846},
       number = {2},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/aa844f},
archivePrefix = {arXiv},
       eprint = {1708.02714},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...846...97G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saumon1995,
       author = {{Saumon}, D. and {Chabrier}, G. and {van Horn}, H.~M.},
        title = "{An Equation of State for Low-Mass Stars and Giant Planets}",
      journal = {\apjs},
     keywords = {EQUATION OF STATE, STARS: INTERIORS, STARS: LOW-MASS, BROWN DWARFS, STARS: PLANETARY SYSTEMS},
         year = 1995,
        month = aug,
       volume = {99},
        pages = {713},
          doi = {10.1086/192204},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJS...99..713S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allen2005,
       author = {{Allen}, Peter R. and {Koerner}, David W. and {Reid}, I. Neill and {Trilling}, David E.},
        title = "{The Substellar Mass Function: A Bayesian Approach}",
      journal = {\apj},
     keywords = {Stars: Evolution, Stars: Low-Mass, Brown Dwarfs, Stars: Luminosity Function, Mass Function, Astrophysics},
         year = 2005,
        month = may,
       volume = {625},
       number = {1},
        pages = {385-397},
          doi = {10.1086/429548},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502189},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...625..385A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kao2018,
       author = {{Kao}, Melodie M. and {Hallinan}, Gregg and {Pineda}, J. Sebastian and {Stevenson}, David and {Burgasser}, Adam},
        title = "{The Strongest Magnetic Fields on the Coolest Brown Dwarfs}",
      journal = {\apjs},
     keywords = {brown dwarfs, planets and satellites: aurorae, planets and satellites: magnetic fields, radio continuum: stars, stars: individual: 2MASS 10430758+2225236, 2MASS 12373919+6526148, SDSS 04234858-0414035, SIMP J01365662+0933473, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = aug,
       volume = {237},
       number = {2},
          eid = {25},
        pages = {25},
          doi = {10.3847/1538-4365/aac2d5},
archivePrefix = {arXiv},
       eprint = {1808.02485},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..237...25K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tannock2021,
       author = {{Tannock}, Megan E. and {Metchev}, Stanimir and {Heinze}, Aren and {Miles-P{\'a}ez}, Paulo A. and {Gagn{\'e}}, Jonathan and {Burgasser}, Adam and {Marley}, Mark S. and {Apai}, D{\'a}niel and {Su{\'a}rez}, Genaro and {Plavchan}, Peter},
        title = "{Weather on Other Worlds. V. The Three Most Rapidly Rotating Ultra-cool Dwarfs}",
      journal = {\aj},
     keywords = {Brown dwarfs, Stellar rotation, Variable stars, Infrared photometry, Spectroscopy, 185, 1629, 1761, 792, 1558, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = may,
       volume = {161},
       number = {5},
          eid = {224},
        pages = {224},
          doi = {10.3847/1538-3881/abeb67},
archivePrefix = {arXiv},
       eprint = {2103.01990},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161..224T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PROCEEDINGS{Joergens2014,
        title = "{50 Years of Brown Dwarfs: From Prediction to Discovery to Forefront of Research}",
        author = {{Joergens}, V.},
     keywords = {Physics},
    booktitle = {50 Years of Brown Dwarfs},
         year = 2014,
       series = {Astrophysics and Space Science Library},
       volume = {401},
        month = jan,
          doi = {10.1007/978-3-319-01162-2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ASSL..401.....J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Karalidi2021,
       author = {{Karalidi}, Theodora and {Marley}, Mark and {Fortney}, Jonathan J. and {Morley}, Caroline and {Saumon}, Didier and {Lupu}, Roxana and {Visscher}, Channon and {Freedman}, Richard},
        title = "{The Sonora Substellar Atmosphere Models. II. Cholla: A Grid of Cloud-free, Solar Metallicity Models in Chemical Disequilibrium for the JWST Era}",
      journal = {\apj},
     keywords = {185, 498, 2120, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = dec,
       volume = {923},
       number = {2},
          eid = {269},
        pages = {269},
          doi = {10.3847/1538-4357/ac3140},
    archivePrefix = {arXiv},
       eprint = {2110.11824},
     primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923..269K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cushing2011,
       author = {{Cushing}, Michael C. and {Kirkpatrick}, J. Davy and {Gelino}, Christopher R. and {Griffith}, Roger L. and {Skrutskie}, Michael F. and {Mainzer}, A. and {Marsh}, Kenneth A. and {Beichman}, Charles A. and {Burgasser}, Adam J. and {Prato}, Lisa A. and {Simcoe}, Robert A. and {Marley}, Mark S. and {Saumon}, D. and {Freedman}, Richard S. and {Eisenhardt}, Peter R. and {Wright}, Edward L.},
        title = "{The Discovery of Y Dwarfs using Data from the Wide-field Infrared Survey Explorer (WISE)}",
      journal = {\apj},
     keywords = {brown dwarfs, infrared: stars, stars: individual: UGPS J072227.51{\textendash}054031.2 WISEPC J014807.25{\textendash}720258.8 WISEP J041022.71+150248.5 WISEPC J140518.40+553421.5 WISEP J154151.65-225025.2 WISEP J173835.52+273258.9 WISEP J182831.08+265037.8 WISEPC J205628.90+145953.3, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = dec,
       volume = {743},
       number = {1},
          eid = {50},
        pages = {50},
          doi = {10.1088/0004-637X/743/1/50},
archivePrefix = {arXiv},
       eprint = {1108.4678},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...743...50C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirkpatrick2013,
       author = {{Kirkpatrick}, J. Davy and {Cushing}, Michael C. and {Gelino}, Christopher R. and {Beichman}, Charles A. and {Tinney}, C.~G. and {Faherty}, Jacqueline K. and {Schneider}, Adam and {Mace}, Gregory N.},
        title = "{Discovery of the Y1 Dwarf WISE J064723.23-623235.5}",
      journal = {\apj},
     keywords = {brown dwarfs, stars: atmospheres, stars: distances, stars: individual: WISE J064723.23{\textendash}623235.5, stars: low-mass, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {776},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.1088/0004-637X/776/2/128},
archivePrefix = {arXiv},
       eprint = {1308.5372},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...776..128K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirkpatrick2012,
       author = {{Kirkpatrick}, J. Davy and {Gelino}, Christopher R. and {Cushing}, Michael C. and {Mace}, Gregory N. and {Griffith}, Roger L. and {Skrutskie}, Michael F. and {Marsh}, Kenneth A. and {Wright}, Edward L. and {Eisenhardt}, Peter R. and {McLean}, Ian S. and {Mainzer}, Amanda K. and {Burgasser}, Adam J. and {Tinney}, C.~G. and {Parker}, Stephen and {Salter}, Graeme},
        title = "{Further Defining Spectral Type ``Y'' and Exploring the Low-mass End of the Field Brown Dwarf Mass Function}",
      journal = {\apj},
     keywords = {brown dwarfs, solar neighborhood, stars: low-mass, stars: luminosity function, mass function, surveys, techniques: spectroscopic, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jul,
       volume = {753},
       number = {2},
          eid = {156},
        pages = {156},
          doi = {10.1088/0004-637X/753/2/156},
archivePrefix = {arXiv},
       eprint = {1205.2122},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...753..156K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tinney2012,
       author = {{Tinney}, C.~G. and {Faherty}, Jacqueline K. and {Kirkpatrick}, J. Davy and {Wright}, Edward L. and {Gelino}, Christopher R. and {Cushing}, Michael C. and {Griffith}, Roger L. and {Salter}, Graeme},
        title = "{WISE J163940.83-684738.6: A Y Dwarf Identified by Methane Imaging}",
      journal = {\apj},
     keywords = {brown dwarfs, methods: observational, parallaxes, stars: individual: WISE J163940.83{\textendash}684738.6, techniques: photometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = nov,
       volume = {759},
       number = {1},
          eid = {60},
        pages = {60},
          doi = {10.1088/0004-637X/759/1/60},
archivePrefix = {arXiv},
       eprint = {1209.6123},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...759...60T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu2012,
       author = {{Liu}, Michael C. and {Dupuy}, Trent J. and {Bowler}, Brendan P. and {Leggett}, S.~K. and {Best}, William M.~J.},
        title = "{Two Extraordinary Substellar Binaries at the T/Y Transition and the Y-band Fluxes of the Coolest Brown Dwarfs}",
      journal = {\apj},
     keywords = {binaries: close, binaries: general, brown dwarfs, infrared: stars, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = oct,
       volume = {758},
       number = {1},
          eid = {57},
        pages = {57},
          doi = {10.1088/0004-637X/758/1/57},
archivePrefix = {arXiv},
       eprint = {1206.4044},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...758...57L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley2015,
       author = {{Marley}, M.~S. and {Robinson}, T.~D.},
        title = "{On the Cool Side: Modeling the Atmospheres of Brown Dwarfs and Giant Planets}",
      journal = {\araa},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {279-323},
          doi = {10.1146/annurev-astro-082214-122522},
archivePrefix = {arXiv},
       eprint = {1410.6512},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..279M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Prandtl1925,
       author = {{Prandtl}, L.},
        title = "{7. Bericht {\"u}ber Untersuchungen zur ausgebildeten Turbulenz}",
      journal = {Zeitschrift Angewandte Mathematik und Mechanik},
         year = 1925,
        month = jan,
       volume = {5},
       number = {2},
        pages = {136-139},
          doi = {10.1002/zamm.19250050212},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1925ZaMM....5..136P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vitense1953,
       author = {{Vitense}, E.},
        title = "{Die Wasserstoffkonvektionszone der Sonne. Mit 11 Textabbildungen}",
      journal = {\zap},
         year = 1953,
        month = jan,
       volume = {32},
        pages = {135},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1953ZA.....32..135V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BohmVitense1958,
       author = {{B{\"o}hm-Vitense}, E.},
        title = "{{\"U}ber die Wasserstoffkonvektionszone in Sternen verschiedener Effektivtemperaturen und Leuchtkr{\"a}fte. Mit 5 Textabbildungen}",
      journal = {\zap},
         year = 1958,
        month = jan,
       volume = {46},
        pages = {108},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1958ZA.....46..108B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ludwig2006,
       author = {{Ludwig}, H. -G. and {Allard}, F. and {Hauschildt}, P.~H.},
        title = "{Energy transport, overshoot, and mixing in the atmospheres of M-type main- and pre-main-sequence objects}",
      journal = {\aap},
     keywords = {convection, hydrodynamics, radiative transfer, stars: atmospheres, stars: late-type, Astrophysics},
         year = 2006,
        month = nov,
       volume = {459},
       number = {2},
        pages = {599-612},
          doi = {10.1051/0004-6361:20054010},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608264},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...459..599L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Manabe1964,
       author = {{Manabe}, Syukuro and {Strickler}, Robert F.},
        title = "{Thermal Equilibrium of the Atmosphere with a Convective Adjustment.}",
      journal = {Journal of Atmospheric Sciences},
         year = 1964,
        month = jul,
       volume = {21},
       number = {4},
        pages = {361-385},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964JAtS...21..361M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Fermi1936, 
    place={New York}, 
    edition={1}, 
    title={thermodynamics}, publisher={Dover Publications, Inc.}, 
    author={{Fermi}, Enrico}, 
    year={1936}}

@INCOLLECTION{Showman2010,
       author = {{Showman}, A.~P. and {Cho}, J.~Y. -K. and {Menou}, K.},
        title = "{Atmospheric Circulation of Exoplanets}",
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {Exoplanets},
         year = 2010,
       editor = {{Seager}, S.},
        pages = {471-516},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010exop.book..471S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rhines1975,
       author = {{Rhines}, P.~B.},
        title = "{Waves and turbulence on a beta-plane}",
      journal = {Journal of Fluid Mechanics},
         year = 1975,
        month = jan,
       volume = {69},
        pages = {417-443},
          doi = {10.1017/S0022112075001504},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1975JFM....69..417R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fortney2008,
       author = {{Fortney}, J.~J. and {Lodders}, K. and {Marley}, M.~S. and {Freedman}, R.~S.},
        title = "{A Unified Theory for the Atmospheres of the Hot and Very Hot Jupiters: Two Classes of Irradiated Atmospheres}",
      journal = {\apj},
     keywords = {planetary systems, radiative transfer, Astrophysics},
         year = 2008,
        month = may,
       volume = {678},
       number = {2},
        pages = {1419-1435},
          doi = {10.1086/528370},
archivePrefix = {arXiv},
       eprint = {0710.2558},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...678.1419F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Knutson2009,
       author = {{Knutson}, Heather A. and {Charbonneau}, David and {Cowan}, Nicolas B. and {Fortney}, Jonathan J. and {Showman}, Adam P. and {Agol}, Eric and {Henry}, Gregory W. and {Everett}, Mark E. and {Allen}, Lori E.},
        title = "{Multiwavelength Constraints on the Day-Night Circulation Patterns of HD 189733b}",
      journal = {\apj},
     keywords = {binaries: eclipsing, infrared: stars, planetary systems, stars: individual: HD 189733, techniques: photometric, Astrophysics},
         year = 2009,
        month = jan,
       volume = {690},
       number = {1},
        pages = {822-836},
          doi = {10.1088/0004-637X/690/1/822},
archivePrefix = {arXiv},
       eprint = {0802.1705},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...690..822K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marley&McKay1999,
       author = {{Marley}, Mark S. and {McKay}, Christopher P.},
        title = "{Thermal Structure of Uranus' Atmosphere}",
      journal = {\icarus},
     keywords = {Uranus},
         year = 1999,
        month = apr,
       volume = {138},
       number = {2},
        pages = {268-286},
          doi = {10.1006/icar.1998.6071},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999Icar..138..268M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Freedman2008,
       author = {{Freedman}, Richard S. and {Marley}, Mark S. and {Lodders}, Katharina},
        title = "{Line and Mean Opacities for Ultracool Dwarfs and Extrasolar Planets}",
      journal = {\apjs},
     keywords = {line: profiles, molecular data, stars: atmospheres, stars: low-mass, brown dwarfs, Astrophysics},
         year = 2008,
        month = feb,
       volume = {174},
       number = {2},
        pages = {504-513},
          doi = {10.1086/521793},
archivePrefix = {arXiv},
       eprint = {0706.2374},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJS..174..504F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lee2016,
       author = {{Lee}, E. and {Dobbs-Dixon}, I. and {Helling}, Ch. and {Bognar}, K. and {Woitke}, P.},
        title = "{Dynamic mineral clouds on HD 189733b. I. 3D RHD with kinetic, non-equilibrium cloud formation}",
      journal = {\aap},
     keywords = {planets and satellites: atmospheres, planets and satellites: individual: HD 189733b, hydrodynamics, radiative transfer, methods: numerical, Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A48},
        pages = {A48},
          doi = {10.1051/0004-6361/201628606},
archivePrefix = {arXiv},
       eprint = {1603.09098},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..48L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parmentier2016,
       author = {{Parmentier}, Vivien and {Fortney}, Jonathan J. and {Showman}, Adam P. and {Morley}, Caroline and {Marley}, Mark S.},
        title = "{Transitions in the Cloud Composition of Hot Jupiters}",
      journal = {\apj},
     keywords = {planets and satellites: atmospheres, planets and satellites: gaseous planets, radiative transfer, scattering, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = sep,
       volume = {828},
       number = {1},
          eid = {22},
        pages = {22},
          doi = {10.3847/0004-637X/828/1/22},
archivePrefix = {arXiv},
       eprint = {1602.03088},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...828...22P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sing2016,
       author = {{Sing}, David K. and {Fortney}, Jonathan J. and {Nikolov}, Nikolay and {Wakeford}, Hannah R. and {Kataria}, Tiffany and {Evans}, Thomas M. and {Aigrain}, Suzanne and {Ballester}, Gilda E. and {Burrows}, Adam S. and {Deming}, Drake and {D{\'e}sert}, Jean-Michel and {Gibson}, Neale P. and {Henry}, Gregory W. and {Huitson}, Catherine M. and {Knutson}, Heather A. and {Lecavelier Des Etangs}, Alain and {Pont}, Frederic and {Showman}, Adam P. and {Vidal-Madjar}, Alfred and {Williamson}, Michael H. and {Wilson}, Paul A.},
        title = "{A continuum from clear to cloudy hot-Jupiter exoplanets without primordial water depletion}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = jan,
       volume = {529},
       number = {7584},
        pages = {59-62},
          doi = {10.1038/nature16068},
archivePrefix = {arXiv},
       eprint = {1512.04341},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016Natur.529...59S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gao2021,
       author = {{Gao}, Peter and {Powell}, Diana},
        title = "{A Universal Cloud Composition on the Nightsides of Hot Jupiters}",
      journal = {\apjl},
     keywords = {Exoplanet atmospheres, Atmospheric clouds, Planetary atmospheres, Exoplanet atmospheric composition, Hot Jupiters, 487, 2180, 1244, 2021, 753, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
       volume = {918},
       number = {1},
          eid = {L7},
        pages = {L7},
          doi = {10.3847/2041-8213/ac139f},
archivePrefix = {arXiv},
       eprint = {2107.06417},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...918L...7G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Knapp2004,
       author = {{Knapp}, G.~R. and {Leggett}, S.~K. and {Fan}, X. and {Marley}, M.~S. and {Geballe}, T.~R. and {Golimowski}, D.~A. and {Finkbeiner}, D. and {Gunn}, J.~E. and {Hennawi}, J. and {Ivezi{\'c}}, Z. and {Lupton}, R.~H. and {Schlegel}, D.~J. and {Strauss}, M.~A. and {Tsvetanov}, Z.~I. and {Chiu}, K. and {Hoversten}, E.~A. and {Glazebrook}, K. and {Zheng}, W. and {Hendrickson}, M. and {Williams}, C.~C. and {Uomoto}, A. and {Vrba}, F.~J. and {Henden}, A.~A. and {Luginbuhl}, C.~B. and {Guetter}, H.~H. and {Munn}, J.~A. and {Canzian}, B. and {Schneider}, Donald P. and {Brinkmann}, J.},
        title = "{Near-Infrared Photometry and Spectroscopy of L and T Dwarfs: The Effects of Temperature, Clouds, and Gravity}",
      journal = {\aj},
     keywords = {-Stars: Fundamental Parameters, Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs, Astrophysics},
         year = 2004,
        month = jun,
       volume = {127},
       number = {6},
        pages = {3553-3578},
          doi = {10.1086/420707},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402451},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004AJ....127.3553K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Geballe2002,
       author = {{Geballe}, T.~R. and {Knapp}, G.~R. and {Leggett}, S.~K. and {Fan}, X. and {Golimowski}, D.~A. and {Anderson}, S. and {Brinkmann}, J. and {Csabai}, I. and {Gunn}, J.~E. and {Hawley}, S.~L. and {Hennessy}, G. and {Henry}, T.~J. and {Hill}, G.~J. and {Hindsley}, R.~B. and {Ivezi{\'c}}, {\v{Z}}. and {Lupton}, R.~H. and {McDaniel}, A. and {Munn}, J.~A. and {Narayanan}, V.~K. and {Peng}, E. and {Pier}, J.~R. and {Rockosi}, C.~M. and {Schneider}, D.~P. and {Smith}, J. Allyn and {Strauss}, M.~A. and {Tsvetanov}, Z.~I. and {Uomoto}, A. and {York}, D.~G. and {Zheng}, W.},
        title = "{Toward Spectral Classification of L and T Dwarfs: Infrared and Optical Spectroscopy and Analysis}",
      journal = {\apj},
     keywords = {Infrared: Stars, Stars: Low-Mass, Brown Dwarfs, Surveys, Astrophysics},
         year = 2002,
        month = jan,
       volume = {564},
       number = {1},
        pages = {466-481},
          doi = {10.1086/324078},
archivePrefix = {arXiv},
       eprint = {astro-ph/0108443},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...564..466G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mayor&Queloz1995,
       author = {{Mayor}, Michel and {Queloz}, Didier},
        title = "{A Jupiter-mass companion to a solar-type star}",
      journal = {\nat},
         year = 1995,
        month = nov,
       volume = {378},
       number = {6555},
        pages = {355-359},
          doi = {10.1038/378355a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995Natur.378..355M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INCOLLECTION{Parmentier&Crossfield2018,
       author = {{Parmentier}, Vivien and {Crossfield}, Ian J.~M.},
        title = "{Exoplanet Phase Curves: Observations and Theory}",
     keywords = {Physics, Astrophysics - Earth and Planetary Astrophysics},
    booktitle = {Handbook of Exoplanets},
         year = 2018,
       editor = {{Deeg}, Hans J. and {Belmonte}, Juan Antonio},
          eid = {116},
        pages = {116},
          doi = {10.1007/978-3-319-55333-7\_116},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018haex.bookE.116P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guillot1996,
       author = {{Guillot}, T. and {Burrows}, A. and {Hubbard}, W.~B. and {Lunine}, J.~I. and {Saumon}, D.},
        title = "{Giant Planets at Small Orbital Distances}",
      journal = {\apjl},
     keywords = {STARS: PLANETARY SYSTEMS, PLANETS AND SATELLITES: GENERAL, Astrophysics},
         year = 1996,
        month = mar,
       volume = {459},
        pages = {L35},
          doi = {10.1086/309935},
archivePrefix = {arXiv},
       eprint = {astro-ph/9511109},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...459L..35G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman&Polvani2011,
       author = {{Showman}, Adam P. and {Polvani}, Lorenzo M.},
        title = "{Equatorial Superrotation on Tidally Locked Exoplanets}",
      journal = {\apj},
     keywords = {hydrodynamics, methods: analytical, methods: numerical, planets and satellites: atmospheres, planets and satellites: individual: HD 189733b, waves, Astrophysics - Earth and Planetary Astrophysics},
         year = 2011,
        month = sep,
       volume = {738},
       number = {1},
          eid = {71},
        pages = {71},
          doi = {10.1088/0004-637X/738/1/71},
archivePrefix = {arXiv},
       eprint = {1103.3101},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...738...71S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Showman&Guillot2002,
       author = {{Showman}, A.~P. and {Guillot}, T.},
        title = "{Atmospheric circulation and tides of ``51 Pegasus b-like'' planets}",
      journal = {\aap},
     keywords = {PLANETS AND SATELLITES: GENERAL, STARS: PLANETARY SYSTEMS, Astrophysics},
         year = 2002,
        month = apr,
       volume = {385},
        pages = {166-180},
          doi = {10.1051/0004-6361:20020101},
archivePrefix = {arXiv},
       eprint = {astro-ph/0202236},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...385..166S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beltz2021,
       author = {{Beltz}, Hayley and {Rauscher}, Emily and {Brogi}, Matteo and {Kempton}, Eliza M. -R.},
        title = "{A Significant Increase in Detection of High-resolution Emission Spectra Using a Three-dimensional Atmospheric Model of a Hot Jupiter}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, High resolution spectroscopy, Hot Jupiters, Hydrodynamical simulations, Radiative transfer simulations, 487, 2096, 753, 767, 1967, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = jan,
       volume = {161},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.3847/1538-3881/abb67b},
archivePrefix = {arXiv},
       eprint = {2009.09030},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....161....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Parmentier2018,
       author = {{Parmentier}, Vivien and {Line}, Mike R. and {Bean}, Jacob L. and {Mansfield}, Megan and {Kreidberg}, Laura and {Lupu}, Roxana and {Visscher}, Channon and {D{\'e}sert}, Jean-Michel and {Fortney}, Jonathan J. and {Deleuil}, Magalie and {Arcangeli}, Jacob and {Showman}, Adam P. and {Marley}, Mark S.},
        title = "{From thermal dissociation to condensation in the atmospheres of ultra hot Jupiters: WASP-121b in context}",
      journal = {\aap},
     keywords = {radiative transfer, planets and satellites: gaseous planets, planets and satellites: atmospheres, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = sep,
       volume = {617},
          eid = {A110},
        pages = {A110},
          doi = {10.1051/0004-6361/201833059},
archivePrefix = {arXiv},
       eprint = {1805.00096},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...617A.110P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tan&Komacek2019,
       author = {{Tan}, Xianyu and {Komacek}, Thaddeus D.},
        title = "{The Atmospheric Circulation of Ultra-hot Jupiters}",
      journal = {\apj},
     keywords = {Exoplanet atmospheres, Hot Jupiters, Hydrodynamics, 753, 487, 1963, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = nov,
       volume = {886},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/ab4a76},
archivePrefix = {arXiv},
       eprint = {1910.01622},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886...26T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek&Tan2022,
       author = {{Komacek}, Thaddeus D. and {Tan}, Xianyu and {Gao}, Peter and {Lee}, Elspeth K.~H.},
        title = "{Patchy nightside clouds on ultra-hot Jupiters: General Circulation Model simulations with radiatively active cloud tracers}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2022,
        month = may,
          eid = {arXiv:2205.07834},
        pages = {arXiv:2205.07834},
archivePrefix = {arXiv},
       eprint = {2205.07834},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220507834K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{May2021,
       author = {{May}, Erin M. and {Komacek}, Thaddeus D. and {Stevenson}, Kevin B. and {Kempton}, Eliza M. -R. and {Bean}, Jacob L. and {Malik}, Matej and {Ih}, Jegug and {Mansfield}, Megan and {Savel}, Arjun B. and {Deming}, Drake and {Desert}, Jean-Michel and {Feng}, Y. Katherina and {Fortney}, Jonathan J. and {Kataria}, Tiffany and {Lewis}, Nikole and {Morley}, Caroline and {Rauscher}, Emily and {Showman}, Adam},
        title = "{Spitzer Phase-curve Observations and Circulation Models of the Inflated Ultrahot Jupiter WASP-76b}",
      journal = {\aj},
     keywords = {Exoplanet atmospheres, Exoplanet astronomy, Hot Jupiters, 487, 486, 753, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = oct,
       volume = {162},
       number = {4},
          eid = {158},
        pages = {158},
          doi = {10.3847/1538-3881/ac0e30},
archivePrefix = {arXiv},
       eprint = {2107.03349},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021AJ....162..158M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bell&Cowan2018,
       author = {{Bell}, Taylor J. and {Cowan}, Nicolas B.},
        title = "{Increased Heat Transport in Ultra-hot Jupiter Atmospheres through H$_{2}$ Dissociation and Recombination}",
      journal = {\apjl},
     keywords = {methods: analytical, methods: numerical, planets and satellites: atmospheres, planets and satellites: gaseous planets, Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = apr,
       volume = {857},
       number = {2},
          eid = {L20},
        pages = {L20},
          doi = {10.3847/2041-8213/aabcc8},
archivePrefix = {arXiv},
       eprint = {1802.07725},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...857L..20B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PaiAsnodkar2022,
       author = {{Pai Asnodkar}, Anusha and {Wang}, Ji and {Eastman}, Jason D. and {Cauley}, P. Wilson and {Gaudi}, B. Scott and {Ilyin}, Ilya and {Strassmeier}, Klaus},
        title = "{Variable and Supersonic Winds in the Atmosphere of an Ultrahot Giant Planet}",
      journal = {\aj},
     keywords = {Exoplanet astronomy, Exoplanet atmospheres, Exoplanet atmospheric variability, Exoplanets, 486, 487, 2020, 498, Astrophysics - Earth and Planetary Astrophysics},
         year = 2022,
        month = apr,
       volume = {163},
       number = {4},
          eid = {155},
        pages = {155},
          doi = {10.3847/1538-3881/ac51d2},
archivePrefix = {arXiv},
       eprint = {2201.04154},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....163..155P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komacek&Tan2018,
       author = {{Komacek}, Thaddeus D. and {Tan}, Xianyu},
        title = "{Effects of Dissociation/Recombination on the Day-Night Temperature Contrasts of Ultra-hot Jupiters}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2018,
        month = may,
       volume = {2},
       number = {2},
          eid = {36},
        pages = {36},
          doi = {10.3847/2515-5172/aac5e7},
archivePrefix = {arXiv},
       eprint = {1805.07415},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018RNAAS...2...36K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INCOLLECTION{Guillot2004,
       author = {{Guillot}, Tristan and {Stevenson}, David J. and {Hubbard}, William B. and {Saumon}, Didier},
        title = "{The interior of Jupiter}",
     keywords = {Jupiter: Interior},
    booktitle = {Jupiter. The Planet, Satellites and Magnetosphere},
         year = 2004,
       editor = {{Bagenal}, Fran and {Dowling}, Timothy E. and {McKinnon}, William B.},
       volume = {1},
        pages = {35-57},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004jpsm.book...35G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

























































